Stand-In Effects and Pooling Amplification: Lessons from Biological World Models for Testing Action Effects

Action-conditioned world models are often checked by replacing actions and measuring prediction error. In autocorrelated designs, future actions can stand in for hidden history and give a false impression of action effects. A conditional randomization test expressed as an e-value has finite-sample validity under the conditional design, score and resampling assumptions, for any admissibly frozen scorer. When many sites share an action, pooling can amplify a shared score error and destroy power. In a registered reanalysis of optogenetics data the pooled test failed its positive controls. A tempered statistic registered before the new data were obtained rejected on a previously unopened field under a reconstructed assignment law. In two registered simulator studies on released world models, fixed mixtures restored or retained power in the tested settings. A third registered study used recorded robot video and assessed sensitivity under a reconstructed command law and undocumented timing. A fourth registered study repeated an exploratory TD-MPC2 design on new seeds. At one step with partial execution, a bounded-stake mixture rejected in 376 of 576 units and temperature scaling in 248. In exploratory evaluations, the original inverse-dynamics reference exceeded the 317M model in all 30 tasks under uniform actions. Under policy-centred actions a tested reference exceeded it in every task across the original and follow-up evaluations. In four pole tasks, with the tested conditional action law and scorer configurations held fixed, two TD-MPC2 scorers retained 6% to 33% of their policy-centred evidence when steps were uniform with probability one half. A reference critic retained 73% to 80%. On fresh units with frozen scorers, pointwise bootstrap intervals for both models' retention minus the critic's lay below zero in all four pole tasks.

==> macros/P1_macros.tex <==
\newcommand{\PoneDhiCOnecRejections}{180}
\newcommand{\PoneDhiKishRejections}{54}
\newcommand{\PoneDhiMRejections}{178}
\newcommand{\PoneDhiVRejections}{185}
\newcommand{\PoneDhiRRejections}{80}
\newcommand{\PoneDhiRhalfRejections}{176}
\newcommand{\PoneDloCOnecRejections}{15}
\newcommand{\PoneDloKishRejections}{0}
\newcommand{\PoneDloMRejections}{2}
\newcommand{\PoneDloVRejections}{11}
\newcommand{\PoneDloRRejections}{1}
\newcommand{\PoneDloRhalfRejections}{12}
\newcommand{\PoneFixKishFullCells}{12}
\newcommand{\PoneFixMFullCells}{12}
\newcommand{\PoneFixRFullCells}{0}
\newcommand{\PoneFixRMaxCellRejections}{0}
\newcommand{\PoneFixRhalfFullCells}{0}
\newcommand{\PoneFixRhalfMaxCellRejections}{2}
\newcommand{\PoneNullMaxRejectionsNewArms}{1}
\newcommand{\PoneOutcome}{1}
\newcommand{\PoneGateCells}{51}
\newcommand{\PoneGateDecisionCellsIdentical}{51}
\newcommand{\PoneGateFailVoneCells}{4}
\newcommand{\PoneGateFailAmendedCells}{0}
\newcommand{\PoneGateMaxScaledDiffDisp}{\ensuremath{8.6\times10^{-6}}}


==> macros/P2_macros.tex <==
\newcommand{\PtwoCZeroActiveRejectionsTotal}{0}
\newcommand{\PtwoKishActiveRejectionsTotal}{0}
\newcommand{\PtwoContrastActiveRejectionsTotal}{1}
\newcommand{\PtwoVActiveRejectionsTotal}{96}
\newcommand{\PtwoMActiveRejectionsTotal}{96}
\newcommand{\PtwoMThirteenActiveRejectionsTotal}{96}
\newcommand{\PtwoRActiveRejectionsTotal}{96}
\newcommand{\PtwoRhalfActiveRejectionsTotal}{96}
\newcommand{\PtwoNullRejectionsAllStatisticsTotal}{0}
\newcommand{\PtwoCZeroActiveMedianLogEMinDisp}{\ensuremath{-}222{,}582}
\newcommand{\PtwoCZeroActiveMedianLogEMaxDisp}{\ensuremath{-}5408}
\newcommand{\PtwoKishActiveMedianLogEMinDisp}{\ensuremath{-}2698}
\newcommand{\PtwoKishActiveMedianLogEMaxDisp}{\ensuremath{-}383}
\newcommand{\PtwoContrastActiveMedianLogEMinDisp}{\ensuremath{-}4012}
\newcommand{\PtwoContrastActiveMedianLogEMaxDisp}{\ensuremath{-}95.3}
\newcommand{\PtwoMActiveMedianLogEMinDisp}{126}
\newcommand{\PtwoMActiveMedianLogEMaxDisp}{455}
\newcommand{\PtwoMNullMedianLogEMinDisp}{\ensuremath{-}2.79}
\newcommand{\PtwoMNullMedianLogEMaxDisp}{\ensuremath{-}1.35}
\newcommand{\PtwoLambdaKishActiveMin}{0.0181}
\newcommand{\PtwoLambdaKishActiveMax}{0.320}
\newcommand{\PtwoLambdaContrastActiveMin}{0.0241}
\newcommand{\PtwoLambdaContrastActiveMax}{0.0773}
\newcommand{\PtwoLambdaVActiveMin}{0.00195}
\newcommand{\PtwoLambdaVActiveMax}{0.00391}
\newcommand{\PtwoContrastOverVActiveMin}{12.3}
\newcommand{\PtwoContrastOverVActiveMax}{19.8}
\newcommand{\PtwoReplacementEffectsActiveTotal}{96}
\newcommand{\PtwoReplacementEffectsNullTotal}{5}
\newcommand{\PtwoPredictionsMet}{4}
\newcommand{\PtwoPilotNullMaxRejections}{0}
\newcommand{\PtwoPilotMaxQuantDiffDisp}{\ensuremath{2.05\times10^{-7}}}
\newcommand{\PtwoDevTwoUnitsCompleted}{84}
\newcommand{\PtwoDevTwoMaxQuantDiffDisp}{\ensuremath{2.66\times10^{-7}}}
\newcommand{\PtwoRerunUnitsCompared}{84}
\newcommand{\PtwoRerunUnitsIdentical}{84}


==> macros/all_macros.tex <==
\newcommand{\TODOnum}[1]{\textcolor{red}{[TODO:\detokenize{#1}]}}
\input{macros/bio_macros.tex}
\input{macros/demo_macros.tex}
\input{macros/demo_aliases.tex}
\input{macros/demo_display.tex}
\input{macros/bio_display.tex}
\RequirePackage{longtable,array}
\input{macros/P1_macros.tex}
\input{macros/P2_macros.tex}


==> macros/bio_display.tex <==
\newcommand{\MfourLogESlotOneDisp}{\ensuremath{-}9576}
\newcommand{\MfourLogESlotOneTab}{\ensuremath{-}9576.45}
\newcommand{\MfourLogESlotTwoDisp}{\ensuremath{-}2975}
\newcommand{\MfourLogESlotTwoTab}{\ensuremath{-}2974.53}
\newcommand{\MfourLogESlotThreeDisp}{\ensuremath{-}1.68}
\newcommand{\MfourLogESlotThreeTab}{\ensuremath{-}1.68}
\newcommand{\MfourLogESlotFourDisp}{3466}
\newcommand{\MfourLogESlotFourTab}{3466.13}
\newcommand{\MfourLogESlotFiveDisp}{17{,}573}
\newcommand{\MfourLogESlotFiveTab}{17{,}572.64}
\newcommand{\MfourLogEPerModelSummaryErkMinDisp}{\ensuremath{-}17{,}989}
\newcommand{\MfourLogEPerModelSummaryErkMinTab}{\ensuremath{-}17{,}988.75}
\newcommand{\MfourLogEPerModelSummaryErkMaxDisp}{\ensuremath{-}2973}
\newcommand{\MfourLogEPerModelSummaryErkMaxTab}{\ensuremath{-}2973.15}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMinDisp}{2301}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMinTab}{2301.15}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMaxDisp}{3468}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMaxTab}{3467.52}
\newcommand{\MfourLogEPerModelLGErkHtenDisp}{\ensuremath{-}17{,}989}
\newcommand{\MfourLogEPerModelLGErkHtenTab}{\ensuremath{-}17{,}988.75}
\newcommand{\MfourLogEPerModelGRUErkHtenDisp}{\ensuremath{-}14{,}890}
\newcommand{\MfourLogEPerModelGRUErkHtenTab}{\ensuremath{-}14{,}890.29}
\newcommand{\MfourLogEPerModelTFErkHtenDisp}{\ensuremath{-}12{,}972}
\newcommand{\MfourLogEPerModelTFErkHtenTab}{\ensuremath{-}12{,}971.87}
\newcommand{\MfourLogEPerModelGBErkHtenDisp}{\ensuremath{-}9575}
\newcommand{\MfourLogEPerModelGBErkHtenTab}{\ensuremath{-}9575.07}
\newcommand{\MfourLogEPerModelLGErkHthirtyDisp}{\ensuremath{-}3922}
\newcommand{\MfourLogEPerModelLGErkHthirtyTab}{\ensuremath{-}3922.16}
\newcommand{\MfourLogEPerModelGRUErkHthirtyDisp}{\ensuremath{-}2973}
\newcommand{\MfourLogEPerModelGRUErkHthirtyTab}{\ensuremath{-}2973.15}
\newcommand{\MfourLogEPerModelTFErkHthirtyDisp}{\ensuremath{-}4352}
\newcommand{\MfourLogEPerModelTFErkHthirtyTab}{\ensuremath{-}4352.33}
\newcommand{\MfourLogEPerModelGBErkHthirtyDisp}{\ensuremath{-}3198}
\newcommand{\MfourLogEPerModelGBErkHthirtyTab}{\ensuremath{-}3198.00}
\newcommand{\MfourLogEPerModelLGCcasHoneDisp}{\ensuremath{-}0.29}
\newcommand{\MfourLogEPerModelLGCcasHoneTab}{\ensuremath{-}0.29}
\newcommand{\MfourLogEPerModelGRUCcasHoneDisp}{\ensuremath{-}439}
\newcommand{\MfourLogEPerModelGRUCcasHoneTab}{\ensuremath{-}439.43}
\newcommand{\MfourLogEPerModelTFCcasHoneDisp}{\ensuremath{-}11.5}
\newcommand{\MfourLogEPerModelTFCcasHoneTab}{\ensuremath{-}11.54}
\newcommand{\MfourLogEPerModelGBCcasHoneDisp}{\ensuremath{-}85.0}
\newcommand{\MfourLogEPerModelGBCcasHoneTab}{\ensuremath{-}84.98}
\newcommand{\MfourLogEPerModelLGCcasHsixDisp}{2301}
\newcommand{\MfourLogEPerModelLGCcasHsixTab}{2301.15}
\newcommand{\MfourLogEPerModelGRUCcasHsixDisp}{2884}
\newcommand{\MfourLogEPerModelGRUCcasHsixTab}{2884.10}
\newcommand{\MfourLogEPerModelTFCcasHsixDisp}{3468}
\newcommand{\MfourLogEPerModelTFCcasHsixTab}{3467.52}
\newcommand{\MfourLogEPerModelGBCcasHsixDisp}{3289}
\newcommand{\MfourLogEPerModelGBCcasHsixTab}{3289.16}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMinDisp}{617}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMinTab}{617.45}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMaxDisp}{1338}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMaxTab}{1337.55}
\newcommand{\MfourLugagneVerifiedLogEDisp}{16{,}771}
\newcommand{\MfourLugagneVerifiedLogETab}{16{,}770.95}
\newcommand{\MfourLugagneRawNSingletonLogEDisp}{3.02}
\newcommand{\MfourLugagneRawNSingletonLogETab}{3.02}
\newcommand{\XLogEHtenDisp}{349}
\newcommand{\XLogEHtenTab}{349.00}
\newcommand{\XLogEPerModelLGHtenDisp}{294}
\newcommand{\XLogEPerModelLGHtenTab}{294.09}
\newcommand{\XLogEPerModelGRUHtenDisp}{326}
\newcommand{\XLogEPerModelGRUHtenTab}{326.08}
\newcommand{\XLogEPerModelTFHtenDisp}{301}
\newcommand{\XLogEPerModelTFHtenTab}{300.58}
\newcommand{\XLogEPerModelGBHtenDisp}{350}
\newcommand{\XLogEPerModelGBHtenTab}{350.39}
\newcommand{\XExactDesignBoundHtenDisp}{925}
\newcommand{\XExactDesignBoundHtenTab}{924.54}
\newcommand{\XMCDesignBoundHtenDisp}{914}
\newcommand{\XMCDesignBoundHtenTab}{913.62}
\newcommand{\XLogEHthirtyDisp}{218}
\newcommand{\XLogEHthirtyTab}{217.52}
\newcommand{\XLogEPerModelLGHthirtyDisp}{217}
\newcommand{\XLogEPerModelLGHthirtyTab}{217.49}
\newcommand{\XLogEPerModelGRUHthirtyDisp}{215}
\newcommand{\XLogEPerModelGRUHthirtyTab}{215.04}
\newcommand{\XLogEPerModelTFHthirtyDisp}{185}
\newcommand{\XLogEPerModelTFHthirtyTab}{184.90}
\newcommand{\XLogEPerModelGBHthirtyDisp}{219}
\newcommand{\XLogEPerModelGBHthirtyTab}{218.60}
\newcommand{\XExactDesignBoundHthirtyDisp}{925}
\newcommand{\XExactDesignBoundHthirtyTab}{924.54}
\newcommand{\XMCDesignBoundHthirtyDisp}{848}
\newcommand{\XMCDesignBoundHthirtyTab}{848.37}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMinDisp}{185}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMinTab}{184.90}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMaxDisp}{350}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMaxTab}{350.39}
\newcommand{\XSingleFieldExactBoundMinDisp}{52.7}
\newcommand{\XSingleFieldExactBoundMinTab}{52.75}
\newcommand{\XSingleFieldExactBoundMaxDisp}{166}
\newcommand{\XSingleFieldExactBoundMaxTab}{166.02}
\newcommand{\MfiveLogEHtenDisp}{23.1}
\newcommand{\MfiveLogEHtenTab}{23.13}
\newcommand{\MfiveLogEPerModelLGHtenDisp}{23.0}
\newcommand{\MfiveLogEPerModelLGHtenTab}{22.99}
\newcommand{\MfiveLogEPerModelGRUHtenDisp}{23.0}
\newcommand{\MfiveLogEPerModelGRUHtenTab}{22.96}
\newcommand{\MfiveLogEPerModelTFHtenDisp}{22.5}
\newcommand{\MfiveLogEPerModelTFHtenTab}{22.45}
\newcommand{\MfiveLogEPerModelGBHtenDisp}{23.7}
\newcommand{\MfiveLogEPerModelGBHtenTab}{23.70}
\newcommand{\MfiveExactDesignBoundHtenDisp}{51.7}
\newcommand{\MfiveExactDesignBoundHtenTab}{51.70}
\newcommand{\MfiveLogEHthirtyDisp}{19.1}
\newcommand{\MfiveLogEHthirtyTab}{19.09}
\newcommand{\MfiveLogEPerModelLGHthirtyDisp}{19.9}
\newcommand{\MfiveLogEPerModelLGHthirtyTab}{19.88}
\newcommand{\MfiveLogEPerModelGRUHthirtyDisp}{18.7}
\newcommand{\MfiveLogEPerModelGRUHthirtyTab}{18.72}
\newcommand{\MfiveLogEPerModelTFHthirtyDisp}{17.0}
\newcommand{\MfiveLogEPerModelTFHthirtyTab}{17.02}
\newcommand{\MfiveLogEPerModelGBHthirtyDisp}{19.1}
\newcommand{\MfiveLogEPerModelGBHthirtyTab}{19.07}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMinDisp}{17.0}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMinTab}{17.02}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMaxDisp}{19.9}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMaxTab}{19.88}
\newcommand{\MfiveExactDesignBoundHthirtyDisp}{51.7}
\newcommand{\MfiveExactDesignBoundHthirtyTab}{51.70}
\newcommand{\MfourRiskMagnitudePooledSummaryCcasHoneMaxSci}{\ensuremath{2.9\times10^{-4}}}
\newcommand{\MtwoeRehearsalLogEHtenDisp}{136}
\newcommand{\DebugOracleTieBoundHtenDisp}{135}
\newcommand{\FixSelectionPooledPerModelLGCOneHardestCellMedianLogETab}{131.53}
\newcommand{\FixSelectionPooledPerModelLGCTwoHardestCellMedianLogETab}{131.39}
\newcommand{\FixSelectionPooledPerModelLGCThreeHardestCellMedianLogETab}{83.60}


==> macros/bio_macros.tex <==
\newcommand{\MfourLogESlotOne}{\ensuremath{-}9576.45}
\newcommand{\MfourLogESlotTwo}{\ensuremath{-}2974.53}
\newcommand{\MfourLogESlotThree}{\ensuremath{-}1.68}
\newcommand{\MfourLogESlotFour}{3466.13}
\newcommand{\MfourLogESlotFive}{17572.64}
\newcommand{\MfourLogEPerModelSummaryErkMin}{\ensuremath{-}17{,}989}
\newcommand{\MfourLogEPerModelSummaryErkMax}{\ensuremath{-}2973}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMin}{2301}
\newcommand{\MfourLogEPerModelSummaryCcasHsixMax}{3468}
\newcommand{\MfourLogEPerModelLGErkHten}{\ensuremath{-}17988.75}
\newcommand{\MfourLogEPerModelGRUErkHten}{\ensuremath{-}14890.29}
\newcommand{\MfourLogEPerModelTFErkHten}{\ensuremath{-}12971.87}
\newcommand{\MfourLogEPerModelGBErkHten}{\ensuremath{-}9575.07}
\newcommand{\MfourLogEPerModelLGErkHthirty}{\ensuremath{-}3922.16}
\newcommand{\MfourLogEPerModelGRUErkHthirty}{\ensuremath{-}2973.15}
\newcommand{\MfourLogEPerModelTFErkHthirty}{\ensuremath{-}4352.33}
\newcommand{\MfourLogEPerModelGBErkHthirty}{\ensuremath{-}3198.00}
\newcommand{\MfourLogEPerModelLGCcasHone}{\ensuremath{-}0.29}
\newcommand{\MfourLogEPerModelGRUCcasHone}{\ensuremath{-}439.43}
\newcommand{\MfourLogEPerModelTFCcasHone}{\ensuremath{-}11.54}
\newcommand{\MfourLogEPerModelGBCcasHone}{\ensuremath{-}84.98}
\newcommand{\MfourLogEPerModelLGCcasHsix}{2301.15}
\newcommand{\MfourLogEPerModelGRUCcasHsix}{2884.10}
\newcommand{\MfourLogEPerModelTFCcasHsix}{3467.52}
\newcommand{\MfourLogEPerModelGBCcasHsix}{3289.16}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMin}{617}
\newcommand{\MfourOwnLogEPerModelSummaryCcasHsixMax}{1338}
\newcommand{\MfourBatchPPerModelLGErkHten}{0.093750}
\newcommand{\MfourBatchPPerModelGRUErkHten}{0.093750}
\newcommand{\MfourBatchPPerModelTFErkHten}{0.093750}
\newcommand{\MfourBatchPPerModelGBErkHten}{0.093750}
\newcommand{\MfourBatchPPerModelSummaryErkHtenMin}{0.094}
\newcommand{\MfourBatchPPerModelSummaryErkHtenMax}{0.094}
\newcommand{\MfourBatchPPerModelLGErkHthirty}{0.007812}
\newcommand{\MfourBatchPPerModelGRUErkHthirty}{0.015625}
\newcommand{\MfourBatchPPerModelTFErkHthirty}{0.015625}
\newcommand{\MfourBatchPPerModelGBErkHthirty}{0.015625}
\newcommand{\MfourBatchPPerModelSummaryErkHthirtyMin}{0.0078125}
\newcommand{\MfourBatchPPerModelSummaryErkHthirtyMax}{0.0156250}
\newcommand{\MfourBatchPPerModelLGCcasHone}{0.476562}
\newcommand{\MfourBatchPPerModelGRUCcasHone}{0.695312}
\newcommand{\MfourBatchPPerModelTFCcasHone}{0.812500}
\newcommand{\MfourBatchPPerModelGBCcasHone}{0.695312}
\newcommand{\MfourBatchPPerModelLGCcasHsix}{0.007812}
\newcommand{\MfourBatchPPerModelGRUCcasHsix}{0.007812}
\newcommand{\MfourBatchPPerModelTFCcasHsix}{0.007812}
\newcommand{\MfourBatchPPerModelGBCcasHsix}{0.007812}
\newcommand{\MfourBatchPPerModelSummaryCcasHsixMin}{0.0078125}
\newcommand{\MfourBatchPPerModelSummaryCcasHsixMax}{0.0078125}
\newcommand{\MfourLugagneBatchP}{0.0078125}
\newcommand{\MfourLugagneVerifiedLogE}{16770.9}
\newcommand{\MfourLugagneRawNSingletonLogE}{3.02}
\newcommand{\MfourRiskDifferencePooledSummaryErkMin}{14.6\%}
\newcommand{\MfourRiskDifferencePooledSummaryErkMax}{46.3\%}
\newcommand{\MfourRiskMagnitudePooledSummaryCcasHoneMin}{\ensuremath{2.9\times10^{-8}}}
\newcommand{\MfourRiskMagnitudePooledSummaryCcasHoneMax}{\ensuremath{0.00029}}
\newcommand{\MfourTestMemberReads}{72}
\newcommand{\MfourTestUniqueMembers}{33}
\newcommand{\MtwoaZeroRejectionsPerModelLGProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaSwapRejectionsPerModelLGProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaExactTestRejectionsPerModelLGProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaMCTestRejectionsPerModelLGProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaBatchCrtRejectionsPerModelLGProxyTrapMarkovLinearUnitsFiveTwelve}{15/256}
\newcommand{\MtwoaZeroRejectionsPerModelGRUProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaSwapRejectionsPerModelGRUProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaExactTestRejectionsPerModelGRUProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaMCTestRejectionsPerModelGRUProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaBatchCrtRejectionsPerModelGRUProxyTrapMarkovLinearUnitsFiveTwelve}{17/256}
\newcommand{\MtwoaZeroRejectionsPerModelTFProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaSwapRejectionsPerModelTFProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaExactTestRejectionsPerModelTFProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaMCTestRejectionsPerModelTFProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaBatchCrtRejectionsPerModelTFProxyTrapMarkovLinearUnitsFiveTwelve}{11/256}
\newcommand{\MtwoaZeroRejectionsPerModelGBProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaSwapRejectionsPerModelGBProxyTrapMarkovLinearUnitsFiveTwelve}{256/256}
\newcommand{\MtwoaExactTestRejectionsPerModelGBProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaMCTestRejectionsPerModelGBProxyTrapMarkovLinearUnitsFiveTwelve}{0/256}
\newcommand{\MtwoaBatchCrtRejectionsPerModelGBProxyTrapMarkovLinearUnitsFiveTwelve}{13/256}
\newcommand{\MtwobPrimaryCellsPassingPooled}{64/64}
\newcommand{\MtwobFalsePositiveRatePooledPrimaryMax}{0.40\%}
\newcommand{\MtwobProxyTrapRatePerModelGRUZeroCcasHone}{91\%}
\newcommand{\MtwobProxyTrapRatePerModelTFAblCcasHone}{92.8\%}
\newcommand{\MtwoeRehearsalLogEHten}{135.8}
\newcommand{\MtwoeRehearsalLogEHthirty}{69.5}
\newcommand{\MthreeNullRejectionsPooled}{0/3400}
\newcommand{\PartBFieldHtenLGMedianCorrelation}{0.1982}
\newcommand{\PartBFieldHtenLGCorrelationMin}{0.1387}
\newcommand{\PartBFieldHtenLGCorrelationMax}{0.2540}
\newcommand{\PartBFieldHtenLGMedianDesignEffect}{20.6}
\newcommand{\PartBFieldHtenLGDesignEffectMin}{14.7}
\newcommand{\PartBFieldHtenLGDesignEffectMax}{26.1}
\newcommand{\PartBFieldHtenGRUMedianCorrelation}{0.2161}
\newcommand{\PartBFieldHtenGRUCorrelationMin}{0.1313}
\newcommand{\PartBFieldHtenGRUCorrelationMax}{0.2867}
\newcommand{\PartBFieldHtenGRUMedianDesignEffect}{22.4}
\newcommand{\PartBFieldHtenGRUDesignEffectMin}{14.0}
\newcommand{\PartBFieldHtenGRUDesignEffectMax}{29.4}
\newcommand{\PartBFieldHtenTFMedianCorrelation}{0.2434}
\newcommand{\PartBFieldHtenTFCorrelationMin}{0.1497}
\newcommand{\PartBFieldHtenTFCorrelationMax}{0.3132}
\newcommand{\PartBFieldHtenTFMedianDesignEffect}{25.1}
\newcommand{\PartBFieldHtenTFDesignEffectMin}{15.8}
\newcommand{\PartBFieldHtenTFDesignEffectMax}{32.0}
\newcommand{\PartBFieldHtenGBMedianCorrelation}{0.1985}
\newcommand{\PartBFieldHtenGBCorrelationMin}{0.1437}
\newcommand{\PartBFieldHtenGBCorrelationMax}{0.2699}
\newcommand{\PartBFieldHtenGBMedianDesignEffect}{20.6}
\newcommand{\PartBFieldHtenGBDesignEffectMin}{15.2}
\newcommand{\PartBFieldHtenGBDesignEffectMax}{27.7}
\newcommand{\PartBFieldHthirtyLGMedianCorrelation}{0.1111}
\newcommand{\PartBFieldHthirtyLGCorrelationMin}{0.0829}
\newcommand{\PartBFieldHthirtyLGCorrelationMax}{0.2036}
\newcommand{\PartBFieldHthirtyLGMedianDesignEffect}{12.0}
\newcommand{\PartBFieldHthirtyLGDesignEffectMin}{9.2}
\newcommand{\PartBFieldHthirtyLGDesignEffectMax}{21.2}
\newcommand{\PartBFieldHthirtyGRUMedianCorrelation}{0.1040}
\newcommand{\PartBFieldHthirtyGRUCorrelationMin}{0.0582}
\newcommand{\PartBFieldHthirtyGRUCorrelationMax}{0.1414}
\newcommand{\PartBFieldHthirtyGRUMedianDesignEffect}{11.3}
\newcommand{\PartBFieldHthirtyGRUDesignEffectMin}{6.8}
\newcommand{\PartBFieldHthirtyGRUDesignEffectMax}{15.0}
\newcommand{\PartBFieldHthirtyTFMedianCorrelation}{0.1690}
\newcommand{\PartBFieldHthirtyTFCorrelationMin}{0.0729}
\newcommand{\PartBFieldHthirtyTFCorrelationMax}{0.2052}
\newcommand{\PartBFieldHthirtyTFMedianDesignEffect}{17.7}
\newcommand{\PartBFieldHthirtyTFDesignEffectMin}{8.2}
\newcommand{\PartBFieldHthirtyTFDesignEffectMax}{21.3}
\newcommand{\PartBFieldHthirtyGBMedianCorrelation}{0.1072}
\newcommand{\PartBFieldHthirtyGBCorrelationMin}{0.0944}
\newcommand{\PartBFieldHthirtyGBCorrelationMax}{0.1872}
\newcommand{\PartBFieldHthirtyGBMedianDesignEffect}{11.6}
\newcommand{\PartBFieldHthirtyGBDesignEffectMin}{10.3}
\newcommand{\PartBFieldHthirtyGBDesignEffectMax}{19.5}
\newcommand{\PartBFieldCorrelationAcrossModelsHorizonsMin}{0.0582}
\newcommand{\PartBFieldCorrelationAcrossModelsHorizonsMax}{0.3132}
\newcommand{\PartBFieldDesignEffectAcrossModelsHorizonsMin}{6.8}
\newcommand{\PartBFieldDesignEffectAcrossModelsHorizonsMax}{32.0}
\newcommand{\PartCLogEPerModelLGCzeroHtenSignalTenPercentRhoZeroCellsFiveHundred}{\ensuremath{-}317}
\newcommand{\PartCLogEPerModelLGCzeroHtenSignalThirtyPercentRhoZeroCellsFiveHundred}{\ensuremath{-}1680}
\newcommand{\MthreeVendoredMethodcoreFunctions}{59}
\newcommand{\DebugOracleRejectionsPerModelOracleHtenSignalTenPercentRhoZeroCellsFiveHundred}{16/16}
\newcommand{\DebugOracleRejectionsPerModelOracleHtenSignalThirtyPercentRhoZeroCellsFiveHundred}{16/16}
\newcommand{\DebugOracleRejectionsPerModelOracleHthirtySignalTenPercentRhoZeroCellsFiveHundred}{16/16}
\newcommand{\DebugOracleRejectionsPerModelOracleHthirtySignalThirtyPercentRhoZeroCellsFiveHundred}{16/16}
\newcommand{\DebugNullRejectionsPooledErk}{0/64}
\newcommand{\DebugNullMeanFactorEErk}{1.00027}
\newcommand{\DebugNullRejectionsPooledCcas}{0/64}
\newcommand{\DebugNullMeanFactorECcas}{0.99998}
\newcommand{\DebugComponentSwapRejectionsPerModelLGBefore}{8/8}
\newcommand{\DebugComponentSwapRejectionsPerModelLGAfterFieldPooling}{0/8}
\newcommand{\DebugOracleTieBoundHten}{135.44}
\newcommand{\DebugOracleTieBoundHthirty}{70.68}
\newcommand{\FixNonNullCellCountPerModelLGConePooledAcrossGrid}{12}
\newcommand{\FixAlternativeRejectionsPerModelLGConeAcrossNonNullGridMin}{16/16}
\newcommand{\FixAlternativeRejectionsPerModelLGConeAcrossNonNullGridMax}{16/16}
\newcommand{\FixNullRejectionsPerModelLGConeIndependentHten}{0/32}
\newcommand{\FixNullRejectionsPerModelLGConeSharedHten}{0/32}
\newcommand{\FixNonNullCellCountPerModelLGCtwoPooledAcrossGrid}{12}
\newcommand{\FixAlternativeRejectionsPerModelLGCtwoAcrossNonNullGridMin}{16/16}
\newcommand{\FixAlternativeRejectionsPerModelLGCtwoAcrossNonNullGridMax}{16/16}
\newcommand{\FixNullRejectionsPerModelLGCtwoIndependentHten}{0/32}
\newcommand{\FixNullRejectionsPerModelLGCtwoSharedHten}{0/32}
\newcommand{\FixNonNullCellCountPerModelLGCthreePooledAcrossGrid}{12}
\newcommand{\FixAlternativeRejectionsPerModelLGCthreeAcrossNonNullGridMin}{16/16}
\newcommand{\FixAlternativeRejectionsPerModelLGCthreeAcrossNonNullGridMax}{16/16}
\newcommand{\FixNullRejectionsPerModelLGCthreeIndependentHten}{0/32}
\newcommand{\FixNullRejectionsPerModelLGCthreeSharedHten}{0/32}
\newcommand{\FixCzeroMedianLogEPerModelLGMtwoeHtenIndependentCellsFiveHundred}{95}
\newcommand{\FixCzeroMedianLogEPerModelLGMtwoeHtenSharedCellsFiveHundred}{\ensuremath{-}10{,}494}
\newcommand{\FixCzeroMedianLogEPerModelLGMtwoeHthirtyIndependentCellsFiveHundred}{25}
\newcommand{\FixCzeroMedianLogEPerModelLGMtwoeHthirtySharedCellsFiveHundred}{\ensuremath{-}6453}
\newcommand{\RhoHatHtenLG}{0.2265}
\newcommand{\RhoHatDesignEffectFiveHundredHtenLG}{114.0}
\newcommand{\RhoHatHtenGRU}{0.2293}
\newcommand{\RhoHatDesignEffectFiveHundredHtenGRU}{115.4}
\newcommand{\RhoHatHtenTF}{0.2514}
\newcommand{\RhoHatDesignEffectFiveHundredHtenTF}{126.5}
\newcommand{\RhoHatHtenGB}{0.2052}
\newcommand{\RhoHatDesignEffectFiveHundredHtenGB}{103.4}
\newcommand{\RhoHatHthirtyLG}{0.1273}
\newcommand{\RhoHatDesignEffectFiveHundredHthirtyLG}{64.5}
\newcommand{\RhoHatHthirtyGRU}{0.1145}
\newcommand{\RhoHatDesignEffectFiveHundredHthirtyGRU}{58.1}
\newcommand{\RhoHatHthirtyTF}{0.1774}
\newcommand{\RhoHatDesignEffectFiveHundredHthirtyTF}{89.5}
\newcommand{\RhoHatHthirtyGB}{0.1194}
\newcommand{\RhoHatDesignEffectFiveHundredHthirtyGB}{60.6}
\newcommand{\RhoHatDesignEffectFiveHundredAcrossModelsHorizonsMin}{58.1}
\newcommand{\RhoHatDesignEffectFiveHundredAcrossModelsHorizonsMax}{126.5}
\newcommand{\PthreeRejectionsPerModelLGSoneHtenSignalTenPercentIndependentCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHtenSignalTenPercentSharedCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHtenSignalThirtyPercentIndependentCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHtenSignalThirtyPercentSharedCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHthirtySignalTenPercentIndependentCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHthirtySignalTenPercentSharedCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHthirtySignalThirtyPercentIndependentCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGSoneHthirtySignalThirtyPercentSharedCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGMtwoeHtenSignalTenPercentIndependentCellsFiveHundredSingleField}{32/32}
\newcommand{\PthreeRejectionsPerModelLGMtwoeHtenSignalTenPercentSharedCellsFiveHundredSingleField}{27/32}
\newcommand{\PthreeRejectionsPerModelLGMtwoeHthirtySignalTenPercentIndependentCellsFiveHundredSingleField}{31/32}
\newcommand{\PthreeRejectionsPerModelLGMtwoeHthirtySignalTenPercentSharedCellsFiveHundredSingleField}{2/32}
\newcommand{\XLogEHten}{349.000}
\newcommand{\XLogEPerModelLGHten}{294.089}
\newcommand{\XLogEPerModelGRUHten}{326.079}
\newcommand{\XLogEPerModelTFHten}{300.578}
\newcommand{\XLogEPerModelGBHten}{350.387}
\newcommand{\XExactDesignBoundHten}{924.5}
\newcommand{\XMCDesignBoundHten}{913.616}
\newcommand{\XLogRatioToExactBoundPooledHten}{37.7\%}
\newcommand{\XLogRatioToMCBoundPooledHten}{38.2\%}
\newcommand{\XLogEHthirty}{217.521}
\newcommand{\XLogEPerModelLGHthirty}{217.489}
\newcommand{\XLogEPerModelGRUHthirty}{215.036}
\newcommand{\XLogEPerModelTFHthirty}{184.896}
\newcommand{\XLogEPerModelGBHthirty}{218.602}
\newcommand{\XExactDesignBoundHthirty}{924.5}
\newcommand{\XMCDesignBoundHthirty}{848.374}
\newcommand{\XLogRatioToExactBoundPooledHthirty}{23.5\%}
\newcommand{\XLogRatioToMCBoundPooledHthirty}{25.6\%}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMin}{185}
\newcommand{\XLogEPerModelSummaryAcrossHorizonsMax}{350}
\newcommand{\XSingleFieldExactBoundMin}{53}
\newcommand{\XSingleFieldExactBoundMax}{166}
\newcommand{\MfiveLogEHten}{23.129}
\newcommand{\MfiveLogEHtenTwoDecimals}{23.13}
\newcommand{\MfiveEHtenScientific}{\ensuremath{1.1\times10^{10}}}
\newcommand{\MfiveLogEPerModelLGHten}{22.99}
\newcommand{\MfiveLogEPerModelGRUHten}{22.96}
\newcommand{\MfiveLogEPerModelTFHten}{22.45}
\newcommand{\MfiveLogEPerModelGBHten}{23.70}
\newcommand{\MfiveExactDesignBoundHten}{51.70}
\newcommand{\MfiveLogRatioToExactBoundPooledHten}{44.7\%}
\newcommand{\MfiveHtenCells}{500}
\newcommand{\MfiveHtenOrigins}{1581}
\newcommand{\MfiveHtenValidCellOrigins}{560{,}409}
\newcommand{\MfiveHtenExcludedCellOrigins}{230{,}091}
\newcommand{\MfiveHtenNeutralBagFactors}{1083}
\newcommand{\MfiveHtenZeroEntropyFactors}{1083}
\newcommand{\MfiveLogEHthirty}{19.090}
\newcommand{\MfiveLogEPerModelLGHthirty}{19.88}
\newcommand{\MfiveLogEPerModelGRUHthirty}{18.72}
\newcommand{\MfiveLogEPerModelTFHthirty}{17.02}
\newcommand{\MfiveLogEPerModelGBHthirty}{19.07}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMin}{17.0}
\newcommand{\MfiveLogEPerModelSummaryHthirtyMax}{19.9}
\newcommand{\MfiveExactDesignBoundHthirty}{51.70}
\newcommand{\MfiveLogRatioToExactBoundPooledHthirty}{36.9\%}
\newcommand{\MfiveMinimumNonRestMinutes}{31}
\newcommand{\MfiveRestSegmentIndex}{15}
\newcommand{\MfiveGateDiagnosticPOne}{0.27}
\newcommand{\MfiveGateDiagnosticPTwo}{0.37}
\newcommand{\MfiveGateDiagnosticPThree}{0.56}
\newcommand{\ErkDiagRhoHatHtenLG}{0.2265}
\newcommand{\ErkDiagRhoContrastHtenLG}{0.1430}
\newcommand{\ErkDiagRhoRatioHtenLG}{0.631}
\newcommand{\ErkDiagLambdaRatioFiveHundredHtenLG}{1.58}
\newcommand{\ErkDiagRhoHatHtenGRU}{0.2293}
\newcommand{\ErkDiagRhoContrastHtenGRU}{0.1271}
\newcommand{\ErkDiagRhoRatioHtenGRU}{0.554}
\newcommand{\ErkDiagLambdaRatioFiveHundredHtenGRU}{1.79}
\newcommand{\ErkDiagRhoHatHtenTF}{0.2514}
\newcommand{\ErkDiagRhoContrastHtenTF}{0.2028}
\newcommand{\ErkDiagRhoRatioHtenTF}{0.806}
\newcommand{\ErkDiagLambdaRatioFiveHundredHtenTF}{1.24}
\newcommand{\ErkDiagRhoHatHtenGB}{0.2052}
\newcommand{\ErkDiagRhoContrastHtenGB}{0.1678}
\newcommand{\ErkDiagRhoRatioHtenGB}{0.818}
\newcommand{\ErkDiagLambdaRatioFiveHundredHtenGB}{1.22}
\newcommand{\ErkDiagRhoHatHthirtyLG}{0.1273}
\newcommand{\ErkDiagRhoContrastHthirtyLG}{0.0966}
\newcommand{\ErkDiagRhoRatioHthirtyLG}{0.759}
\newcommand{\ErkDiagLambdaRatioFiveHundredHthirtyLG}{1.31}
\newcommand{\ErkDiagRhoHatHthirtyGRU}{0.1145}
\newcommand{\ErkDiagRhoContrastHthirtyGRU}{0.0657}
\newcommand{\ErkDiagRhoRatioHthirtyGRU}{0.574}
\newcommand{\ErkDiagLambdaRatioFiveHundredHthirtyGRU}{1.72}
\newcommand{\ErkDiagRhoHatHthirtyTF}{0.1774}
\newcommand{\ErkDiagRhoContrastHthirtyTF}{0.1233}
\newcommand{\ErkDiagRhoRatioHthirtyTF}{0.695}
\newcommand{\ErkDiagLambdaRatioFiveHundredHthirtyTF}{1.43}
\newcommand{\ErkDiagRhoHatHthirtyGB}{0.1194}
\newcommand{\ErkDiagRhoContrastHthirtyGB}{0.0988}
\newcommand{\ErkDiagRhoRatioHthirtyGB}{0.828}
\newcommand{\ErkDiagLambdaRatioFiveHundredHthirtyGB}{1.20}
\newcommand{\ErkDiagRhoRatioPooledHtenMin}{0.554}
\newcommand{\ErkDiagRhoRatioPooledHtenMax}{0.818}
\newcommand{\ErkDiagRhoRatioPooledHthirtyMin}{0.574}
\newcommand{\ErkDiagRhoRatioPooledHthirtyMax}{0.828}
\newcommand{\ErkDiagRhoRatioSingleFieldMin}{0.41}
\newcommand{\ErkDiagRhoRatioSingleFieldMinField}{min20\_optmean\_rep1}
\newcommand{\ErkDiagRhoRatioSingleFieldMinModel}{Transformer}
\newcommand{\ErkDiagRhoRatioSingleFieldMinHorizon}{10}
\newcommand{\ErkDiagRhoRatioSingleFieldMax}{1.27}
\newcommand{\ErkDiagRhoRatioSingleFieldMaxField}{min10\_optmean\_rep1}
\newcommand{\ErkDiagRhoRatioSingleFieldMaxModel}{Transformer}
\newcommand{\ErkDiagRhoRatioSingleFieldMaxHorizon}{10}
\newcommand{\PosthocNcWrongRateTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRateTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{63/64}
\newcommand{\PosthocNcProperRateTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRateTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRateTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRateTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{64/64}
\newcommand{\PosthocNcProperRateTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRateTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRateTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRateTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PosthocNcWrongRejectionsTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{64/64}
\newcommand{\PosthocNcProperRateTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRateTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsTwoModelAvgAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{63/64}
\newcommand{\PosthocNcProperRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{64/64}
\newcommand{\PosthocNcProperRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRatePerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{63/64}
\newcommand{\PosthocNcWrongRatePerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PosthocNcWrongRejectionsPerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{64/64}
\newcommand{\PosthocNcProperRatePerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelCNNAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{93.8\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{60/64}
\newcommand{\PosthocNcWrongRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{96.9\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{62/64}
\newcommand{\PosthocNcProperRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{0/64}
\newcommand{\PosthocNcWrongRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{92.2\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{59/64}
\newcommand{\PosthocNcWrongRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{63/64}
\newcommand{\PosthocNcProperRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{1.6\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{1/64}
\newcommand{\PosthocNcWrongRatePerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{92.2\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{59/64}
\newcommand{\PosthocNcWrongRatePerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{98.4\%}
\newcommand{\PosthocNcWrongRejectionsPerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{63/64}
\newcommand{\PosthocNcProperRatePerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{0/64}
\newcommand{\PosthocNcProperRatePerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{1.6\%}
\newcommand{\PosthocNcProperRejectionsPerModelLGAcrossNoiseAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{1/64}
\newcommand{\PosthocNcWrongRatePooledPerModelRangeAcrossNoiseTrainingSizesMin}{92.2\%}
\newcommand{\PosthocNcWrongRatePooledPerModelRangeAcrossNoiseTrainingSizesMax}{100\%}
\newcommand{\PosthocNcWrongRejectionsPooledPerModelRangeAcrossNoiseTrainingSizesMin}{59/64}
\newcommand{\PosthocNcWrongRejectionsPooledPerModelRangeAcrossNoiseTrainingSizesMax}{64/64}
\newcommand{\PosthocNcProperRejectionsPerModelLGGainTrainSixteenHfourPixelsTwoFiftySix}{1/64}
\newcommand{\PosthocNcProperRateTwoModelAvgAcrossNoiseTrainingSizesMin}{0\%}
\newcommand{\PosthocNcProperRateTwoModelAvgAcrossNoiseTrainingSizesMax}{0\%}
\newcommand{\PosthocNcWrongExceedsCorrectComparisonsPooled}{18/18}
\newcommand{\PosthocSealedFilesUnchanged}{8153}
\newcommand{\PxcheckTrapDiagRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{92.2\%}
\newcommand{\PxcheckTrapDiagRatePerModelCNNNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckTrapDiagRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{64.1\%}
\newcommand{\PxcheckTrapDiagRatePerModelLGNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckTrapDiagRatePooledNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{64.1\%}
\newcommand{\PxcheckTrapDiagRatePooledNoneAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckTrapDiagRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{90.6\%}
\newcommand{\PxcheckTrapDiagRatePerModelCNNGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckTrapDiagRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{76.6\%}
\newcommand{\PxcheckTrapDiagRatePerModelLGGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckTrapDiagRatePooledGainAcrossTrainingSizesHfourPixelsTwoFiftySixMin}{76.6\%}
\newcommand{\PxcheckTrapDiagRatePooledGainAcrossTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckNcWrongRatePooledPerModelRangeAcrossNoiseTrainingSizesHfourPixelsTwoFiftySixMin}{92.2\%}
\newcommand{\PxcheckNcWrongRatePooledPerModelRangeAcrossNoiseTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\PxcheckNcWrongRateTwoModelAvgAcrossNoiseTrainingSizesHfourPixelsTwoFiftySixMin}{98.4\%}
\newcommand{\PxcheckNcWrongRateTwoModelAvgAcrossNoiseTrainingSizesHfourPixelsTwoFiftySixMax}{100\%}
\newcommand{\MtwoaBatchRatePerModelLGTrapMarkovLinearUnitsFiveTwelve}{5.9\%}
\newcommand{\MtwoaBatchTailPPerModelLGTrapMarkovLinearUnitsFiveTwelve}{0.22357331}
\newcommand{\MtwoaBatchRejectionsPerModelLGTrapMarkovLinearUnitsFiveTwelve}{15/256}
\newcommand{\MtwoaBatchRatePerModelGRUTrapMarkovLinearUnitsFiveTwelve}{6.6\%}
\newcommand{\MtwoaBatchTailPPerModelGRUTrapMarkovLinearUnitsFiveTwelve}{0.09607954}
\newcommand{\MtwoaBatchRejectionsPerModelGRUTrapMarkovLinearUnitsFiveTwelve}{17/256}
\newcommand{\MtwoaBatchRatePerModelTFTrapMarkovLinearUnitsFiveTwelve}{4.3\%}
\newcommand{\MtwoaBatchTailPPerModelTFTrapMarkovLinearUnitsFiveTwelve}{0.65782387}
\newcommand{\MtwoaBatchRejectionsPerModelTFTrapMarkovLinearUnitsFiveTwelve}{11/256}
\newcommand{\MtwoaBatchRatePerModelGBTrapMarkovLinearUnitsFiveTwelve}{5.1\%}
\newcommand{\MtwoaBatchTailPPerModelGBTrapMarkovLinearUnitsFiveTwelve}{0.42401278}
\newcommand{\MtwoaBatchRejectionsPerModelGBTrapMarkovLinearUnitsFiveTwelve}{13/256}
\newcommand{\MtwoaBatchAlpha}{0.05}
\newcommand{\MtwoaBatchB}{127}
\newcommand{\MtwoaBatchNominalRatePooledReference}{4.7\%}
\newcommand{\MtwoaBatchRejectionsPooledAcrossModels}{56/1024}
\newcommand{\MtwoaBatchRatePooledAcrossModels}{5.5\%}
\newcommand{\FixSelectionPooledPerModelLGCOneMinNonNullRejectionRate}{100\%}
\newcommand{\FixSelectionPooledPerModelLGCOneNullRhoZeroHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCOneNullRhoSharedHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCOneHardestCellMedianLogE}{131.529}
\newcommand{\FixSelectionPooledPerModelLGCTwoMinNonNullRejectionRate}{100\%}
\newcommand{\FixSelectionPooledPerModelLGCTwoNullRhoZeroHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCTwoNullRhoSharedHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCTwoHardestCellMedianLogE}{131.395}
\newcommand{\FixSelectionPooledPerModelLGCThreeMinNonNullRejectionRate}{100\%}
\newcommand{\FixSelectionPooledPerModelLGCThreeNullRhoZeroHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCThreeNullRhoSharedHtenRejections}{0/32}
\newcommand{\FixSelectionPooledPerModelLGCThreeHardestCellMedianLogE}{83.598}
\newcommand{\ErkDiagPooledPerModelLGHtenRhoMean}{0.197}
\newcommand{\ErkDiagPooledPerModelLGHtenRhoContrast}{0.143}
\newcommand{\ErkDiagPooledPerModelLGHtenRhoMed}{0.227}
\newcommand{\ErkDiagPooledPerModelLGHtenRhoContrastOverRhoMean}{0.725}
\newcommand{\ErkDiagPooledPerModelLGHtenRhoContrastOverRhoMed}{0.631}
\newcommand{\ErkDiagPooledPerModelLGHtenNfMean}{91.239}
\newcommand{\ErkDiagPooledPerModelLGHtenNfMin}{64}
\newcommand{\ErkDiagPooledPerModelLGHtenNfMax}{100}
\newcommand{\ErkDiagPooledPerModelGRUHtenRhoMean}{0.213}
\newcommand{\ErkDiagPooledPerModelGRUHtenRhoContrast}{0.127}
\newcommand{\ErkDiagPooledPerModelGRUHtenRhoMed}{0.229}
\newcommand{\ErkDiagPooledPerModelGRUHtenRhoContrastOverRhoMean}{0.598}
\newcommand{\ErkDiagPooledPerModelGRUHtenRhoContrastOverRhoMed}{0.554}
\newcommand{\ErkDiagPooledPerModelGRUHtenNfMean}{91.239}
\newcommand{\ErkDiagPooledPerModelGRUHtenNfMin}{64}
\newcommand{\ErkDiagPooledPerModelGRUHtenNfMax}{100}
\newcommand{\ErkDiagPooledPerModelTFHtenRhoMean}{0.237}
\newcommand{\ErkDiagPooledPerModelTFHtenRhoContrast}{0.203}
\newcommand{\ErkDiagPooledPerModelTFHtenRhoMed}{0.251}
\newcommand{\ErkDiagPooledPerModelTFHtenRhoContrastOverRhoMean}{0.854}
\newcommand{\ErkDiagPooledPerModelTFHtenRhoContrastOverRhoMed}{0.806}
\newcommand{\ErkDiagPooledPerModelTFHtenNfMean}{91.239}
\newcommand{\ErkDiagPooledPerModelTFHtenNfMin}{64}
\newcommand{\ErkDiagPooledPerModelTFHtenNfMax}{100}
\newcommand{\ErkDiagPooledPerModelGBHtenRhoMean}{0.203}
\newcommand{\ErkDiagPooledPerModelGBHtenRhoContrast}{0.168}
\newcommand{\ErkDiagPooledPerModelGBHtenRhoMed}{0.205}
\newcommand{\ErkDiagPooledPerModelGBHtenRhoContrastOverRhoMean}{0.828}
\newcommand{\ErkDiagPooledPerModelGBHtenRhoContrastOverRhoMed}{0.818}
\newcommand{\ErkDiagPooledPerModelGBHtenNfMean}{91.239}
\newcommand{\ErkDiagPooledPerModelGBHtenNfMin}{64}
\newcommand{\ErkDiagPooledPerModelGBHtenNfMax}{100}
\newcommand{\ErkDiagPooledPerModelLGHthirtyRhoMean}{0.127}
\newcommand{\ErkDiagPooledPerModelLGHthirtyRhoContrast}{0.097}
\newcommand{\ErkDiagPooledPerModelLGHthirtyRhoMed}{0.127}
\newcommand{\ErkDiagPooledPerModelLGHthirtyRhoContrastOverRhoMean}{0.760}
\newcommand{\ErkDiagPooledPerModelLGHthirtyRhoContrastOverRhoMed}{0.759}
\newcommand{\ErkDiagPooledPerModelLGHthirtyNfMean}{90.930}
\newcommand{\ErkDiagPooledPerModelLGHthirtyNfMin}{63}
\newcommand{\ErkDiagPooledPerModelLGHthirtyNfMax}{100}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyRhoMean}{0.102}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyRhoContrast}{0.066}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyRhoMed}{0.115}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyRhoContrastOverRhoMean}{0.645}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyRhoContrastOverRhoMed}{0.574}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyNfMean}{90.930}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyNfMin}{63}
\newcommand{\ErkDiagPooledPerModelGRUHthirtyNfMax}{100}
\newcommand{\ErkDiagPooledPerModelTFHthirtyRhoMean}{0.154}
\newcommand{\ErkDiagPooledPerModelTFHthirtyRhoContrast}{0.123}
\newcommand{\ErkDiagPooledPerModelTFHthirtyRhoMed}{0.177}
\newcommand{\ErkDiagPooledPerModelTFHthirtyRhoContrastOverRhoMean}{0.801}
\newcommand{\ErkDiagPooledPerModelTFHthirtyRhoContrastOverRhoMed}{0.695}
\newcommand{\ErkDiagPooledPerModelTFHthirtyNfMean}{90.930}
\newcommand{\ErkDiagPooledPerModelTFHthirtyNfMin}{63}
\newcommand{\ErkDiagPooledPerModelTFHthirtyNfMax}{100}
\newcommand{\ErkDiagPooledPerModelGBHthirtyRhoMean}{0.124}
\newcommand{\ErkDiagPooledPerModelGBHthirtyRhoContrast}{0.099}
\newcommand{\ErkDiagPooledPerModelGBHthirtyRhoMed}{0.119}
\newcommand{\ErkDiagPooledPerModelGBHthirtyRhoContrastOverRhoMean}{0.797}
\newcommand{\ErkDiagPooledPerModelGBHthirtyRhoContrastOverRhoMed}{0.828}
\newcommand{\ErkDiagPooledPerModelGBHthirtyNfMean}{90.930}
\newcommand{\ErkDiagPooledPerModelGBHthirtyNfMin}{63}
\newcommand{\ErkDiagPooledPerModelGBHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenRhoMean}{0.172}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenRhoContrast}{0.137}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenRhoMed}{0.180}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMean}{0.795}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMed}{0.762}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenNfMean}{82.422}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenNfMin}{64}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenRhoMean}{0.176}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenRhoContrast}{0.124}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenRhoMed}{0.175}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMean}{0.703}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMed}{0.707}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenNfMean}{82.422}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenNfMin}{64}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenRhoMean}{0.249}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenRhoContrast}{0.319}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenRhoMed}{0.250}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMean}{1.278}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMed}{1.274}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenNfMean}{82.422}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenNfMin}{64}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenRhoMean}{0.196}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenRhoContrast}{0.211}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenRhoMed}{0.194}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMean}{1.079}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMed}{1.090}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenNfMean}{82.422}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenNfMin}{64}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenRhoMean}{0.224}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenRhoContrast}{0.147}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenRhoMed}{0.253}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMean}{0.658}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMed}{0.582}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenNfMean}{99.748}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenRhoMean}{0.256}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenRhoContrast}{0.150}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenRhoMed}{0.279}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMean}{0.587}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMed}{0.538}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenNfMean}{99.748}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenRhoMean}{0.237}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenRhoContrast}{0.171}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenRhoMed}{0.253}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMean}{0.721}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMed}{0.677}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenNfMean}{99.748}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenRhoMean}{0.201}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenRhoContrast}{0.143}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenRhoMed}{0.216}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMean}{0.713}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMed}{0.662}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenNfMean}{99.748}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenRhoMean}{0.254}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenRhoContrast}{0.197}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenRhoMed}{0.371}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMean}{0.775}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMed}{0.530}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenNfMean}{100.000}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenNfMin}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenRhoMean}{0.287}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenRhoContrast}{0.186}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenRhoMed}{0.410}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMean}{0.647}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMed}{0.452}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenNfMean}{100.000}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenNfMin}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenRhoMean}{0.313}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenRhoContrast}{0.188}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenRhoMed}{0.463}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMean}{0.600}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMed}{0.406}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenNfMean}{100.000}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenNfMin}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenRhoMean}{0.270}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenRhoContrast}{0.203}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenRhoMed}{0.397}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMean}{0.752}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMed}{0.512}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenNfMean}{100.000}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenNfMin}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHtenNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenRhoMean}{0.139}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenRhoContrast}{0.111}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenRhoMed}{0.200}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMean}{0.800}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenRhoContrastOverRhoMed}{0.556}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenNfMean}{82.787}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHtenNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenRhoMean}{0.131}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenRhoContrast}{0.080}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenRhoMed}{0.179}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMean}{0.608}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenRhoContrastOverRhoMed}{0.445}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenNfMean}{82.787}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHtenNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenRhoMean}{0.150}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenRhoContrast}{0.110}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenRhoMed}{0.203}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMean}{0.734}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenRhoContrastOverRhoMed}{0.540}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenNfMean}{82.787}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHtenNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenRhoMean}{0.144}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenRhoContrast}{0.118}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenRhoMed}{0.190}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMean}{0.822}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenRhoContrastOverRhoMed}{0.622}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenNfMean}{82.787}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHtenNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyRhoMean}{0.089}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyRhoContrast}{0.091}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyRhoMed}{0.089}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMean}{1.024}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMed}{1.020}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyNfMean}{81.553}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyNfMin}{63}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelLGHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyRhoMean}{0.082}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyRhoContrast}{0.074}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyRhoMed}{0.085}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMean}{0.902}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMed}{0.871}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyNfMean}{81.553}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyNfMin}{63}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGRUHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyRhoMean}{0.140}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyRhoContrast}{0.174}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyRhoMed}{0.144}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMean}{1.250}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMed}{1.207}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyNfMean}{81.553}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyNfMin}{63}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelTFHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyRhoMean}{0.099}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyRhoContrast}{0.098}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyRhoMed}{0.098}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMean}{0.986}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMed}{0.998}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyNfMean}{81.553}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyNfMin}{63}
\newcommand{\ErkDiagPerFieldMinTenOptmeanRepOnePerModelGBHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyRhoMean}{0.134}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyRhoContrast}{0.087}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyRhoMed}{0.142}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMean}{0.654}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMed}{0.614}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyNfMean}{99.665}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelLGHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyRhoMean}{0.141}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyRhoContrast}{0.107}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyRhoMed}{0.144}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMean}{0.756}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMed}{0.742}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyNfMean}{99.665}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGRUHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyRhoMean}{0.198}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyRhoContrast}{0.189}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyRhoMed}{0.210}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMean}{0.953}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMed}{0.898}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyNfMean}{99.665}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelTFHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyRhoMean}{0.115}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyRhoContrast}{0.078}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyRhoMed}{0.120}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMean}{0.675}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMed}{0.650}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyNfMean}{99.665}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyNfMin}{93}
\newcommand{\ErkDiagPerFieldMinFifteenOptmeanRepOnePerModelGBHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyRhoMean}{0.204}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyRhoContrast}{0.137}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyRhoMed}{0.279}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMean}{0.670}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMed}{0.490}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyNfMean}{99.996}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyNfMin}{98}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelLGHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyRhoMean}{0.126}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyRhoContrast}{0.062}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyRhoMed}{0.152}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMean}{0.494}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMed}{0.409}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyNfMean}{99.996}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyNfMin}{98}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGRUHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyRhoMean}{0.205}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyRhoContrast}{0.109}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyRhoMed}{0.257}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMean}{0.530}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMed}{0.424}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyNfMean}{99.996}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyNfMin}{98}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelTFHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyRhoMean}{0.187}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyRhoContrast}{0.130}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyRhoMed}{0.256}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMean}{0.693}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMed}{0.507}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyNfMean}{99.996}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyNfMin}{98}
\newcommand{\ErkDiagPerFieldMinTwentyOptmeanRepOnePerModelGBHthirtyNfMax}{100}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyRhoMean}{0.083}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyRhoContrast}{0.084}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyRhoMed}{0.112}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMean}{1.017}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyRhoContrastOverRhoMed}{0.751}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyNfMean}{82.507}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelLGHthirtyNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyRhoMean}{0.058}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyRhoContrast}{0.036}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyRhoMed}{0.079}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMean}{0.621}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyRhoContrastOverRhoMed}{0.456}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyNfMean}{82.507}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGRUHthirtyNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyRhoMean}{0.073}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyRhoContrast}{0.053}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyRhoMed}{0.099}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMean}{0.721}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyRhoContrastOverRhoMed}{0.532}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyNfMean}{82.507}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelTFHthirtyNfMax}{91}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyRhoMean}{0.094}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyRhoContrast}{0.095}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyRhoMed}{0.119}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMean}{1.009}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyRhoContrastOverRhoMed}{0.800}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyNfMean}{82.507}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyNfMin}{71}
\newcommand{\ErkDiagPerFieldMinTwentyFiveOptmeanRepOnePerModelGBHthirtyNfMax}{91}
\newcommand{\FixCellwisePooledPerModelLGCOneMedianWinCells}{9}
\newcommand{\FixCellwisePooledPerModelLGCTwoMedianWinCells}{2}
\newcommand{\FixCellwisePooledPerModelLGCThreeMedianWinCells}{1}
\newcommand{\FixCellwisePooledPerModelLGCOneMinusCTwoMin}{\ensuremath{-}0.04}
\newcommand{\FixCellwisePooledPerModelLGCOneMinusCTwoMedian}{0.14}
\newcommand{\FixCellwisePooledPerModelLGCOneMinusCTwoMax}{0.96}
\newcommand{\FixCellwisePooledPerModelLGCOneMinusCTwoHardestCell}{0.13}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{5/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBablRejectionsMin}{39/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBablRejectionsMax}{57/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{163/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{203/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBswapRejectionsMin}{141/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBswapRejectionsMax}{180/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBmargRejectionsMin}{213/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBmargRejectionsMax}{254/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBruleRejectionsMin}{174/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeBruleRejectionsMax}{179/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{26/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{36/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{2/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{15/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{79/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{194/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{205/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{179/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{199/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{220/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{254/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{184/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{195/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{31/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{42/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{2/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBablRejectionsMin}{17/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBablRejectionsMax}{73/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{171/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{212/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{177/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{204/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{225/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{170/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{179/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{39/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{44/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{12/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{19/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBablRejectionsMin}{44/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBablRejectionsMax}{206/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{244/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{244/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBswapRejectionsMin}{238/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBswapRejectionsMax}{249/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBruleRejectionsMin}{236/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeBruleRejectionsMax}{240/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{5/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{27/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{12/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{37/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{236/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{238/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{242/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{239/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{246/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{224/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{227/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{6/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{24/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{16/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBablRejectionsMin}{37/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBablRejectionsMax}{222/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{230/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{246/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{236/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{248/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{230/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{235/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{3/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{33/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{3/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{101/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{197/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{228/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{232/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{225/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{230/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{255/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{162/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{163/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{3/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{232/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{231/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{236/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{234/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{235/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{254/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{149/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{150/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{8/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{5/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{224/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{232/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{236/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{227/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{230/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{255/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{155/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{155/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{5/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{2/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBablRejectionsMin}{40/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBablRejectionsMax}{72/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{193/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{224/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBswapRejectionsMin}{183/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBswapRejectionsMax}{204/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBmargRejectionsMin}{224/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBmargRejectionsMax}{255/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBruleRejectionsMin}{171/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeBruleRejectionsMax}{174/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{33/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{38/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{2/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{17/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{86/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{206/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{213/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{185/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{209/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{228/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{253/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{180/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{187/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{38/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{48/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{2/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBablRejectionsMin}{9/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBablRejectionsMax}{84/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{173/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{210/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{185/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{207/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{235/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{250/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{177/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{182/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{29/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{39/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBablRejectionsMin}{25/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBablRejectionsMax}{154/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{62/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{92/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{9/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{130/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{42/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{15/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{59/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{19/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{148/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{40/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{85/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{7/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{247/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{8/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{46/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{8/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{183/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{17/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{144/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{23/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{68/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{5/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{126/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{35/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{13/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{42/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{14/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{25/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBswapRejectionsMin}{18/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBswapRejectionsMax}{19/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBmargRejectionsMin}{21/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBmargRejectionsMax}{59/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBruleRejectionsMin}{28/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeBruleRejectionsMax}{30/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{35/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{37/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{5/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{9/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{10/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{31/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{13/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{18/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{50/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{25/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{29/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{33/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{36/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{26/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{14/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{35/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{69/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{34/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{38/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBablRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{23/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{48/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBswapRejectionsMin}{21/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBswapRejectionsMax}{23/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBmargRejectionsMin}{25/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBmargRejectionsMax}{41/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBruleRejectionsMin}{39/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeBruleRejectionsMax}{45/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{21/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{32/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{7/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{28/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{70/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{16/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{22/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{28/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{41/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{56/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{60/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{20/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{29/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{6/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{11/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{33/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{36/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{55/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{50/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{58/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{21/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharpSpilloverShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{24/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{16/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{31/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{81/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{22/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{5/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{18/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{30/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{32/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{67/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{20/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{10/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{23/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{24/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{38/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{86/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{19/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{11/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{8/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{10/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{17/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{25/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBswapRejectionsMin}{14/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBswapRejectionsMax}{19/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBmargRejectionsMin}{31/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBmargRejectionsMax}{50/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBruleRejectionsMin}{42/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeBruleRejectionsMax}{44/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{33/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{13/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{18/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{17/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{39/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{16/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{50/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{27/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{29/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{20/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{31/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{10/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{23/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{15/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{21/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{53/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{31/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{32/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{22/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBablRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{107/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{8/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{13/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{118/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{119/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBmargRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBmargRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeBruleRejectionsMax}{9/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{19/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{6/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{10/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{126/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{131/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{11/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{13/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{6/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBablRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{112/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{125/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBablRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{126/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{126/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBmargRejectionsMin}{5/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBmargRejectionsMax}{16/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBruleRejectionsMin}{5/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeBruleRejectionsMax}{35/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{25/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{8/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{123/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{128/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{31/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{14/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{44/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{10/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBablRejectionsMax}{10/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{111/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{123/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{9/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{50/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{16/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{8/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{100/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{102/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{5/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{7/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{11/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{7/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{11/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{103/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{106/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{36/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{8/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{116/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{118/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{11/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{16/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{134/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{135/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBmargRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBmargRejectionsMax}{17/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeBruleRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{13/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{13/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{121/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{127/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{29/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{19/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{25/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{11/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{14/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBablRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{120/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{128/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{3/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{18/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{2/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{10/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{15/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{132/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{193/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{44/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{105/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{139/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{140/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{1/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{49/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{27/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{104/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{187/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{45/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoiseClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{3/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{3/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{4/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{16/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBablRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{47/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{71/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBswapRejectionsMin}{7/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBswapRejectionsMax}{12/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBmargRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBmargRejectionsMax}{31/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBruleRejectionsMin}{43/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeBruleRejectionsMax}{49/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{3/256}
\newcommand{\MtwoaDevMaskedXorRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{3/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{4/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{25/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{68/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{5/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{26/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{31/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{38/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{13/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{4/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{19/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{62/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{13/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{32/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{34/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{37/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{13/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBablRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBablRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{54/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{82/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBswapRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBswapRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBmargRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBmargRejectionsMax}{24/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBruleRejectionsMin}{66/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeBruleRejectionsMax}{77/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{13/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{8/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{32/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{74/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{6/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{24/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{52/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{63/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{13/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{7/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBablRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{29/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{82/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{13/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{35/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{61/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{76/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{20/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{21/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{34/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{64/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{27/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{14/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{5/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{6/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{14/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{16/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{47/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{16/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{9/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{30/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{12/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{10/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{9/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{13/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{27/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{54/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{8/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{37/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{15/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{51/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{77/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBswapRejectionsMin}{5/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBswapRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBmargRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBmargRejectionsMax}{22/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBruleRejectionsMin}{27/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeBruleRejectionsMax}{33/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{17/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{17/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{25/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{66/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{7/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{12/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{22/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{39/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{44/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{3/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{3/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{14/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBablRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBablRejectionsMax}{5/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{28/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{63/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{21/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{29/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{45/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{50/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{3/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBablRejectionsMin}{130/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBablRejectionsMax}{130/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{152/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{177/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{123/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{127/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{69/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{130/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{87/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{93/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{131/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{131/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{92/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{183/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{126/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{126/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{29/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{129/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{89/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{90/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{128/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{86/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{192/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{124/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{125/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{103/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{87/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{88/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{66/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{84/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{67/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{81/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{66/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{67/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBablRejectionsMin}{21/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBablRejectionsMax}{21/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{96/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{111/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBswapRejectionsMin}{87/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBswapRejectionsMax}{100/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBmargRejectionsMin}{21/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBmargRejectionsMax}{114/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBruleRejectionsMin}{81/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeBruleRejectionsMax}{85/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{34/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{41/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{66/256}
\newcommand{\MtwoaDevMaskedSharedRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{84/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{49/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{63/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{55/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{64/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{54/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{68/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{24/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{27/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{72/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{106/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{85/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{92/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{28/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{103/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{82/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{91/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{41/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{47/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{49/256}
\newcommand{\MtwoaDevMaskedSharedRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{63/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{16/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{15/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{17/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{19/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBablRejectionsMin}{7/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBablRejectionsMax}{16/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{76/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{104/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{89/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{101/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{114/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{80/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{83/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{25/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{28/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedSharedRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{16/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{5/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{34/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBablRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBablRejectionsMax}{44/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{96/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBswapRejectionsMin}{66/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBswapRejectionsMax}{91/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBmargRejectionsMin}{41/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBmargRejectionsMax}{102/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBruleRejectionsMin}{94/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeBruleRejectionsMax}{105/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{32/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{19/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{15/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{42/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{49/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{98/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{65/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{83/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{40/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{90/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{99/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{102/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{17/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{19/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedSharedShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{41/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{62/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{39/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{59/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{74/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{87/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBablRejectionsMin}{31/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBablRejectionsMax}{37/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{67/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{117/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{81/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{93/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{39/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{120/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{101/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{107/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{54/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{59/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{41/256}
\newcommand{\MtwoaDevMaskedSharedShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{62/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{5/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{24/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{29/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{115/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{117/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{108/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{110/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{29/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{117/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{79/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{81/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{1/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{2/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{3/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{5/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{11/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{13/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{33/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{124/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{134/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{122/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{127/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{33/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{142/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{87/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{89/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{18/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{3/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{6/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{12/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{15/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{11/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{13/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{22/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{32/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{122/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{124/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{125/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{32/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{132/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{88/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{89/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{9/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{12/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedSharedBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{27/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{19/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{30/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{47/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{54/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBablRejectionsMin}{20/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBablRejectionsMax}{27/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{89/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{111/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBswapRejectionsMin}{72/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBswapRejectionsMax}{89/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBmargRejectionsMin}{26/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBmargRejectionsMax}{113/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBruleRejectionsMin}{77/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeBruleRejectionsMax}{80/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{35/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{38/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{14/256}
\newcommand{\MtwoaDevMaskedSharedMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{27/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{31/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{32/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{52/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{58/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{23/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{30/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{63/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{95/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{71/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{89/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{32/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{95/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{82/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{90/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{39/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{48/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{31/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{62/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{97/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{63/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{86/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{59/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{62/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBablRejectionsMin}{19/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBablRejectionsMax}{29/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{78/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{113/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{96/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{108/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{30/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{121/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{95/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{98/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{39/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{43/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{62/256}
\newcommand{\MtwoaDevMaskedSharedMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{97/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBablRejectionsMin}{126/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBablRejectionsMax}{126/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{149/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{192/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{123/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{132/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{73/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{126/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{89/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{99/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{128/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{82/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{176/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{116/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{121/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{32/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{128/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{89/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{94/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{134/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{134/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{93/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{186/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{129/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{130/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{113/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{134/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{102/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{107/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBablRejectionsMin}{48/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBablRejectionsMax}{62/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBzeroRejectionsMin}{178/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBzeroRejectionsMax}{212/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBswapRejectionsMin}{156/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBswapRejectionsMax}{184/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBmargRejectionsMin}{214/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBmargRejectionsMax}{252/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBruleRejectionsMin}{163/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeBruleRejectionsMax}{169/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBablRejectionsMin}{16/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBablRejectionsMax}{75/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBzeroRejectionsMin}{190/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBzeroRejectionsMax}{203/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBswapRejectionsMin}{173/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBswapRejectionsMax}{192/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBmargRejectionsMin}{227/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBmargRejectionsMax}{255/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBruleRejectionsMin}{169/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeBruleRejectionsMax}{179/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBablRejectionsMin}{11/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBablRejectionsMax}{75/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBzeroRejectionsMin}{169/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBzeroRejectionsMax}{204/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBswapRejectionsMin}{158/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBswapRejectionsMax}{178/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBmargRejectionsMin}{229/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBmargRejectionsMax}{252/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBruleRejectionsMin}{173/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeBruleRejectionsMax}{182/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyRenewalDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBablRejectionsMin}{56/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBablRejectionsMax}{206/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBzeroRejectionsMin}{248/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBzeroRejectionsMax}{248/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBswapRejectionsMin}{239/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBswapRejectionsMax}{247/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBruleRejectionsMin}{218/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeBruleRejectionsMax}{225/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBablRejectionsMin}{46/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBablRejectionsMax}{246/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBzeroRejectionsMin}{247/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBzeroRejectionsMax}{249/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBswapRejectionsMin}{242/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBswapRejectionsMax}{251/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBruleRejectionsMin}{227/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeBruleRejectionsMax}{237/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBablRejectionsMin}{30/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBablRejectionsMax}{220/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBzeroRejectionsMin}{234/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBzeroRejectionsMax}{242/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBswapRejectionsMin}{243/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBswapRejectionsMax}{254/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBruleRejectionsMin}{230/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeBruleRejectionsMax}{235/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyShuffleDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBablRejectionsMin}{103/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBablRejectionsMax}{208/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMin}{242/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBzeroRejectionsMax}{247/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBswapRejectionsMin}{227/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBswapRejectionsMax}{234/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBruleRejectionsMin}{143/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeBruleRejectionsMax}{143/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBablRejectionsMax}{238/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMin}{238/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBzeroRejectionsMax}{239/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMin}{236/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBswapRejectionsMax}{236/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMin}{159/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeBruleRejectionsMax}{160/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBablRejectionsMax}{226/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMin}{239/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBzeroRejectionsMax}{243/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMin}{222/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBswapRejectionsMax}{223/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMin}{255/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMin}{145/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeBruleRejectionsMax}{145/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyBoundedWalkDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBablRejectionsMin}{41/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBablRejectionsMax}{68/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBzeroRejectionsMin}{181/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBzeroRejectionsMax}{208/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBswapRejectionsMin}{168/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBswapRejectionsMax}{193/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBmargRejectionsMin}{224/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBmargRejectionsMax}{254/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBruleRejectionsMin}{165/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeBruleRejectionsMax}{174/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBablRejectionsMin}{21/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBablRejectionsMax}{96/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBzeroRejectionsMin}{194/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBzeroRejectionsMax}{207/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBswapRejectionsMin}{179/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBswapRejectionsMax}{202/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBmargRejectionsMin}{226/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBmargRejectionsMax}{254/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBruleRejectionsMin}{187/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeBruleRejectionsMax}{189/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBablRejectionsMin}{9/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBablRejectionsMax}{75/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBzeroRejectionsMin}{178/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBzeroRejectionsMax}{212/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBswapRejectionsMin}{189/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBswapRejectionsMax}{206/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBmargRejectionsMin}{234/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBmargRejectionsMax}{252/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBruleRejectionsMin}{188/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeBruleRejectionsMax}{198/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyMarkovDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBablRejectionsMin}{23/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBablRejectionsMax}{159/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBzeroRejectionsMin}{38/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBzeroRejectionsMax}{78/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBswapRejectionsMin}{14/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBswapRejectionsMax}{130/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBmargRejectionsMin}{5/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBmargRejectionsMax}{40/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBruleRejectionsMin}{20/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeBruleRejectionsMax}{67/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedLinearPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBablRejectionsMin}{21/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBablRejectionsMax}{158/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMin}{36/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBzeroRejectionsMax}{93/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBswapRejectionsMin}{10/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBswapRejectionsMax}{244/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBmargRejectionsMin}{10/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBmargRejectionsMax}{52/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBruleRejectionsMin}{18/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeBruleRejectionsMax}{179/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedSaturatingPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBablRejectionsMin}{18/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBablRejectionsMax}{157/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBzeroRejectionsMin}{26/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBzeroRejectionsMax}{82/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBswapRejectionsMin}{5/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBswapRejectionsMax}{140/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBmargRejectionsMin}{7/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBmargRejectionsMax}{41/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBruleRejectionsMin}{10/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeBruleRejectionsMax}{47/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyClockLockedDelayedPooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{19/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{236/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{23/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{246/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{5/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{249/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{4/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{8/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{240/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{48/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{2/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{3/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{18/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{12/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{30/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{60/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{37/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharpSpilloverPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{6/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{5/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{4/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{20/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{105/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{100/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{193/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{28/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{49/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{50/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{25/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevSharedNoisePooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{5/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{97/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{86/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{87/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{134/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{49/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{192/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{65/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{132/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{18/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{142/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{77/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{107/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{59/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedSharedPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{97/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{9/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{20/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{131/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{16/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{192/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{4/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{127/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{2/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{130/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{10/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{93/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{21/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevMaskedXorPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{9/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBatchCRTRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBablRejectionsMin}{3/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBablRejectionsMax}{246/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMin}{26/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBzeroRejectionsMax}{249/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBswapRejectionsMin}{5/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBswapRejectionsMax}{254/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBmargRejectionsMin}{5/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBruleRejectionsMin}{10/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsBruleRejectionsMax}{237/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsHRTnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevZeroEntropyPooledPerModelAcrossDesignsDynamicsProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeTestExactRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeTestExactRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeTestMCRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeTestMCRejectionsMax}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBatchCRTRejectionsMin}{11/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBatchCRTRejectionsMax}{17/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBablRejectionsMin}{159/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBablRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBzeroRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBzeroRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBswapRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBswapRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBmargRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBmargRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBruleRejectionsMin}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeBruleRejectionsMax}{256/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeHRTnaiveRejectionsMin}{31/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeHRTnaiveRejectionsMax}{37/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeProdnaiveRejectionsMin}{0/256}
\newcommand{\MtwoaDevProxyTrapMarkovLinearUnitsFiveTwelvePooledPerModelRangeProdnaiveRejectionsMax}{0/256}
\newcommand{\MtwobPrimaryAllDatasetsPooledPerModelCellsTotal}{64}
\newcommand{\MtwobPrimaryAllDatasetsPooledPerModelCellsPassingCPNinetyFive}{64}
\newcommand{\MtwobPrimaryAllDatasetsPooledPerModelCellsPointFalsePositiveRateMax}{0.40\%}
\newcommand{\MtwobPrimaryAllDatasetsPooledPerModelCellsCPNinetyFiveUpperMax}{1.3\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsTestRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsTestRateMax}{0.40\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBablRateMin}{0.20\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBablRateMax}{92.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBzeroRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBzeroRateMax}{91\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBswapRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBswapRateMax}{14.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBmargRateMin}{0.40\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBmargRateMax}{54.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBruleRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsBruleRateMax}{34.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsHRTnaiveRateMin}{2.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsHRTnaiveRateMax}{7.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsProdnaiveRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryAllDatasetsPooledPerModelAcrossHorizonsProdnaiveRateMax}{0.40\%}
\newcommand{\MtwobPrimaryERKPooledPerModelCellsTotal}{32}
\newcommand{\MtwobPrimaryERKPooledPerModelCellsPassingCPNinetyFive}{32}
\newcommand{\MtwobPrimaryERKPooledPerModelCellsPointFalsePositiveRateMax}{0\%}
\newcommand{\MtwobPrimaryERKPooledPerModelCellsCPNinetyFiveUpperMax}{0.60\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsTestRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsTestRateMax}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBablRateMin}{0.20\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBablRateMax}{33.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBzeroRateMin}{0.80\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBzeroRateMax}{13.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBswapRateMin}{5.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBswapRateMax}{9\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBmargRateMin}{3.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBmargRateMax}{6.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBruleRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsBruleRateMax}{20.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsHRTnaiveRateMin}{2.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsHRTnaiveRateMax}{6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsProdnaiveRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryERKPooledPerModelAcrossHorizonsProdnaiveRateMax}{0\%}
\newcommand{\MtwobPrimaryCcaSPooledPerModelCellsTotal}{32}
\newcommand{\MtwobPrimaryCcaSPooledPerModelCellsPassingCPNinetyFive}{32}
\newcommand{\MtwobPrimaryCcaSPooledPerModelCellsPointFalsePositiveRateMax}{0.40\%}
\newcommand{\MtwobPrimaryCcaSPooledPerModelCellsCPNinetyFiveUpperMax}{1.3\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsTestRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsTestRateMax}{0.40\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBablRateMin}{2.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBablRateMax}{92.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBzeroRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBzeroRateMax}{91\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBswapRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBswapRateMax}{14.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBmargRateMin}{0.40\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBmargRateMax}{54.8\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBruleRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsBruleRateMax}{34.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsHRTnaiveRateMin}{2.6\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsHRTnaiveRateMax}{7.2\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsProdnaiveRateMin}{0\%}
\newcommand{\MtwobProxyTrapSTwoPrimaryCcaSPooledPerModelAcrossHorizonsProdnaiveRateMax}{0.40\%}
\newcommand{\MtwocSizeFullGridPooledFourModelAvgThresholdTwentyCellsTotal}{16}
\newcommand{\MtwocSizeFullGridPooledFourModelAvgThresholdTwentyCellsPassingCPNinetyFive}{16}
\newcommand{\MtwocSizeFullGridPooledFourModelAvgThresholdTwentyCPNinetyFiveUpperMax}{3.1\%}
\newcommand{\MtwocPowerPooledFourModelAvgSignalTenPercentThresholdHundredAcrossCellsMin}{100\%}
\newcommand{\MtwocPowerPooledFourModelAvgSignalThirtyPercentThresholdHundredAcrossCellsMin}{100\%}
\newcommand{\MtwocPowerErkHthirtyPooledFourModelAvgSignalTwoPercentThresholdHundredAcrossFamiliesMin}{4.5\%}
\newcommand{\MtwocPowerErkHthirtyPooledFourModelAvgSignalTwoPercentThresholdHundredAcrossFamiliesMax}{71\%}
\newcommand{\MtwocPowerErkHthirtyPooledFourModelAvgSignalTwoPercentThresholdTwentyAcrossFamiliesMin}{13\%}
\newcommand{\MtwocPowerErkHthirtyPooledFourModelAvgSignalTwoPercentThresholdTwentyAcrossFamiliesMax}{89\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroOneRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroOneRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroOneCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroTwoRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroTwoRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroTwoCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroThreeRejections}{0/400}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroThreeRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroThreeCPNinetyFiveUpper}{0.75\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFourRejections}{0/400}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFourRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFourCPNinetyFiveUpper}{0.75\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFiveRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFiveRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroFiveCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSixRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSixRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSixCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSevenRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSevenRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroSevenCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroEightRejections}{0/800}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroEightRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroEightCPNinetyFiveUpper}{0.37\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroNineRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroNineRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFZeroNineCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneZeroRejections}{0/400}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneZeroRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneZeroCPNinetyFiveUpper}{0.75\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneOneRejections}{0/200}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneOneRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledFOneOneCPNinetyFiveUpper}{1.5\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledAllFamiliesRejections}{0/3400}
\newcommand{\MthreeSizeRegisteredStatisticPooledAllFamiliesRate}{0\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledAllFamiliesCPNinetyFiveUpper}{0.088\%}
\newcommand{\MthreeSizeRegisteredStatisticPooledAcrossFamiliesCPNinetyFiveUpperMax}{1.5\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroOneCellcZeroZeroOneHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroOneCellcZeroZeroOneHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroOneCellcZeroZeroOneHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroOneCellcZeroZeroOneHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroTwoCellcZeroZeroThreeHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroTwoCellcZeroZeroThreeHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroTwoCellcZeroZeroThreeHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroTwoCellcZeroZeroThreeHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroFiveHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroFiveHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroFiveHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroFiveHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroSevenHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroSevenHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroSevenHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroThreeCellcZeroZeroSevenHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroZeroNineHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroZeroNineHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroZeroNineHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroZeroNineHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroOneOneHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroOneOneHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroOneOneHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFourCellcZeroOneOneHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFiveCellcZeroOneThreeHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFiveCellcZeroOneThreeHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFiveCellcZeroOneThreeHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroFiveCellcZeroOneThreeHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSixCellcZeroOneFiveHOneThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSixCellcZeroOneFiveHOneThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSixCellcZeroOneFiveHOneThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSixCellcZeroOneFiveHOneThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSevenCellcZeroOneSevenHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSevenCellcZeroOneSevenHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSevenCellcZeroOneSevenHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroSevenCellcZeroOneSevenHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoZeroHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoZeroHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoZeroHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoZeroHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoThreeHThreeExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoThreeHThreeExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoThreeHThreeExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroEightCellcZeroTwoThreeHThreeExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroNineCellcZeroTwoFiveHOneExactCeilingEligibleRate}{12\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroNineCellcZeroTwoFiveHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroNineCellcZeroTwoFiveHOneExactCeilingEligibleRejections}{24/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFZeroNineCellcZeroTwoFiveHOneExactCeilingEligibleMeetsEightyPercent}{0}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeOneHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeOneHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeOneHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeOneHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeThreeHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeThreeHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeThreeHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeThreeHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeFiveHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeFiveHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeFiveHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeFiveHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeSevenHOneExactCeilingEligibleRate}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeSevenHOneExactCeilingEligibleCeiling}{100\%}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeSevenHOneExactCeilingEligibleRejections}{200/200}
\newcommand{\MthreePowerRegisteredStatisticPooledFOneOneCellcZeroThreeSevenHOneExactCeilingEligibleMeetsEightyPercent}{1}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroOneCOneGatedRateMin}{3.5\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroOneCOneGatedRateMax}{99\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroOneCOneGatedRateMin}{3.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroOneCOneGatedRateMax}{100\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroOneCOneGatedRateMin}{20.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroOneCOneGatedRateMax}{98\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroOneCOneGatedRateMin}{2.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroOneCOneGatedRateMax}{93\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroOneCOneGatedRateMin}{3.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroOneCOneGatedRateMax}{89.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroOneCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroOneCOneGatedRateMax}{6.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroOneCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroOneCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroTwoCOneGatedRateMin}{0.50\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroTwoCOneGatedRateMax}{92\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroTwoCOneGatedRateMin}{1\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroTwoCOneGatedRateMax}{56.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroTwoCOneGatedRateMin}{13\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroTwoCOneGatedRateMax}{41\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroTwoCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroTwoCOneGatedRateMax}{31.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroTwoCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroTwoCOneGatedRateMax}{91\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroTwoCOneGatedRateMin}{1.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroTwoCOneGatedRateMax}{4.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroTwoCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroTwoCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroThreeCOneGatedRateMin}{2\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroThreeCOneGatedRateMax}{45.2\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroThreeCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroThreeCOneGatedRateMax}{94.2\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroThreeCOneGatedRateMin}{11.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroThreeCOneGatedRateMax}{72.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroThreeCOneGatedRateMin}{5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroThreeCOneGatedRateMax}{40.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroThreeCOneGatedRateMin}{5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroThreeCOneGatedRateMax}{28.2\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroThreeCOneGatedRateMin}{4\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroThreeCOneGatedRateMax}{5.8\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroThreeCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroThreeCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroFourCOneGatedRateMin}{17.2\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroFourCOneGatedRateMax}{58\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroFourCOneGatedRateMin}{50\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroFourCOneGatedRateMax}{84.8\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroFourCOneGatedRateMin}{32.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroFourCOneGatedRateMax}{65\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroFourCOneGatedRateMin}{21.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroFourCOneGatedRateMax}{45.8\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroFourCOneGatedRateMin}{22.8\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroFourCOneGatedRateMax}{76.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroFourCOneGatedRateMin}{4.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroFourCOneGatedRateMax}{9\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroFourCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroFourCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroFiveCOneGatedRateMin}{0.50\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroFiveCOneGatedRateMax}{11\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroFiveCOneGatedRateMin}{4\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroFiveCOneGatedRateMax}{92\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroFiveCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroFiveCOneGatedRateMax}{41\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroFiveCOneGatedRateMin}{5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroFiveCOneGatedRateMax}{57.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroFiveCOneGatedRateMin}{1.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroFiveCOneGatedRateMax}{48.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroFiveCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroFiveCOneGatedRateMax}{15.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroFiveCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroFiveCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroSixCOneGatedRateMin}{0.50\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroSixCOneGatedRateMax}{28.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroSixCOneGatedRateMin}{5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroSixCOneGatedRateMax}{7.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroSixCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroSixCOneGatedRateMax}{34.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroSixCOneGatedRateMin}{6.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroSixCOneGatedRateMax}{10\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroSixCOneGatedRateMin}{1.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroSixCOneGatedRateMax}{33\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroSixCOneGatedRateMin}{5.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroSixCOneGatedRateMax}{7.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroSixCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroSixCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroSevenCOneGatedRateMin}{4\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroSevenCOneGatedRateMax}{39\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroSevenCOneGatedRateMin}{2.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroSevenCOneGatedRateMax}{7.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroSevenCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroSevenCOneGatedRateMax}{86.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroSevenCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroSevenCOneGatedRateMax}{50\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroSevenCOneGatedRateMin}{23\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroSevenCOneGatedRateMax}{59\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroSevenCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroSevenCOneGatedRateMax}{9\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroSevenCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroSevenCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroEightCOneGatedRateMin}{5.5\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroEightCOneGatedRateMax}{22.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroEightCOneGatedRateMin}{5.2\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroEightCOneGatedRateMax}{7.8\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroEightCOneGatedRateMin}{1.2\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroEightCOneGatedRateMax}{17.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroEightCOneGatedRateMin}{1\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroEightCOneGatedRateMax}{9.2\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroEightCOneGatedRateMin}{13\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroEightCOneGatedRateMax}{31.2\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroEightCOneGatedRateMin}{5.8\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroEightCOneGatedRateMax}{7.4\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroEightCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroEightCOneGatedRateMax}{0.25\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroNineCOneGatedRateMin}{2\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFZeroNineCOneGatedRateMax}{55.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroNineCOneGatedRateMin}{2\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFZeroNineCOneGatedRateMax}{4.5\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroNineCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFZeroNineCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroNineCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFZeroNineCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroNineCOneGatedRateMin}{9.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFZeroNineCOneGatedRateMax}{49\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroNineCOneGatedRateMin}{2.5\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFZeroNineCOneGatedRateMax}{3.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroNineCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFZeroNineCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFOneZeroCOneGatedRateMin}{3.5\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFOneZeroCOneGatedRateMax}{91\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFOneZeroCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFOneZeroCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFOneZeroCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFOneZeroCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFOneZeroCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFOneZeroCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFOneZeroCOneGatedRateMin}{2.8\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFOneZeroCOneGatedRateMax}{35.2\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFOneZeroCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFOneZeroCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFOneZeroCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFOneZeroCOneGatedRateMax}{0\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFOneOneCOneGatedRateMin}{2\%}
\newcommand{\MthreeBaselineBablPooledPerModelRangeFOneOneCOneGatedRateMax}{31.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFOneOneCOneGatedRateMin}{1.5\%}
\newcommand{\MthreeBaselineBmargPooledPerModelRangeFOneOneCOneGatedRateMax}{6\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFOneOneCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineBrulePooledPerModelRangeFOneOneCOneGatedRateMax}{20.5\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFOneOneCOneGatedRateMin}{4\%}
\newcommand{\MthreeBaselineBswapPooledPerModelRangeFOneOneCOneGatedRateMax}{6.5\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFOneOneCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineBzeroPooledPerModelRangeFOneOneCOneGatedRateMax}{6\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFOneOneCOneGatedRateMin}{3\%}
\newcommand{\MthreeBaselineHRTnaivePooledPerModelRangeFOneOneCOneGatedRateMax}{6.5\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFOneOneCOneGatedRateMin}{0\%}
\newcommand{\MthreeBaselineProdnaivePooledPerModelRangeFOneOneCOneGatedRateMax}{0\%}
\newcommand{\MthreeZeroEntropyPooledRegisteredStatisticCellcZeroTwoSixHOneAllEAndEExactlyOne}{1}
\newcommand{\MthreeZeroEntropyPooledRegisteredStatisticCellcZeroTwoSevenHOneAllEAndEExactlyOne}{1}
\newcommand{\MthreeZeroEntropyPooledRegisteredStatisticCellcZeroTwoEightHOneThreeAllEAndEExactlyOne}{1}
\newcommand{\MthreeZeroEntropyPooledRegisteredStatisticCellcZeroTwoNineHOneThreeAllEAndEExactlyOne}{1}
\newcommand{\MtwoaBatchRatePerModelMinPercent}{4.3\%}
\newcommand{\MtwoaBatchRatePerModelMaxPercent}{6.6\%}
\newcommand{\MtwoaBatchTailPMinAcrossModels}{0.096}
\newcommand{\MtwoaHeadlineExactTestRejectionsMaxAcrossModels}{0/256}
\newcommand{\MthreeFamilyCount}{11}
\newcommand{\MthreeZeroEntropyMaxAbsLogE}{0.0}
\newcommand{\MthreePowerEligibleCellsTotal}{16}
\newcommand{\MthreePowerEligibleCellsMeetingEighty}{15}
\newcommand{\PxCzeroRejectRateTwoModelAvgDHiMaxPixelsGeTwoFiftySix}{0\%}
\newcommand{\PxRhoHatMaxNoneGain}{0.000629}
\newcommand{\PxRhoHatOffsetMin}{0.159}
\newcommand{\PxRhoHatOffsetMax}{0.182}
\newcommand{\PxCfourRejectRateTwoModelAvgDHiMin}{0\%}
\newcommand{\PxCfourRejectRateTwoModelAvgDHiMax}{75\%}
\newcommand{\PxConeCRejectRateTwoModelAvgDHiMin}{81.2\%}
\newcommand{\PxConeCRejectRateTwoModelAvgDHiMax}{100\%}
\newcommand{\PxConeCMedianLogETwoModelAvgDHiMin}{7.06}
\newcommand{\PxConeCMedianLogETwoModelAvgDHiMax}{10.3}
\newcommand{\PxConeCRejectRateTwoModelAvgDLoMax}{25\%}
\newcommand{\PxDeffContrastExceedsKishRowsNoneGain}{48/48}
\newcommand{\PxDeffContrastExceedsKishRowsNoneGainAllTFour}{62/90}
\newcommand{\PxDeffContrastBelowKishRowsOffset}{24/24}
\newcommand{\PxDeffContrastBelowKishRowsOffsetAllTFour}{36/36}
\newcommand{\PxTrapConeTwoModelAvgRejectRateMaxGTwo}{0\%}
\newcommand{\PxTrapDiagRateCNNTrainSixteenMin}{90.6\%}
\newcommand{\PxTrapNcFrozenConeRejectionsMaxGTwo}{0/64}
\newcommand{\BiowmEvalForecastGainPooledErkHthirty}{49.6\%}
\newcommand{\BiowmEvalForecastGainPooledCcasHthirty}{0.91\%}
\newcommand{\BiowmEvalPracticalGainThresholdPooled}{2\%}
\newcommand{\DesignLawErkPermutationCount}{10{,}000}
\newcommand{\DesignLawErkPermutationSeed}{20{,}261{,}005}
\newcommand{\DesignLawErkBonferroniThreshold}{0.000256410}
\newcommand{\DesignLawErkMinTenOptmeanRepOneSpearmanStatistic}{0.1219}
\newcommand{\DesignLawErkMinTenOptmeanRepOneSpearmanP}{0.2802}
\newcommand{\DesignLawErkMinTenOptmeanRepOneRunsStatistic}{59}
\newcommand{\DesignLawErkMinTenOptmeanRepOneRunsP}{0.1704}
\newcommand{\DesignLawErkMinTenOptmeanRepOneLagOneStatistic}{0.0005}
\newcommand{\DesignLawErkMinTenOptmeanRepOneLagOneP}{0.9043}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoSpearmanStatistic}{0.1712}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoSpearmanP}{0.1362}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoRunsStatistic}{52}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoRunsP}{0.4239}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoLagOneStatistic}{\ensuremath{-}0.1506}
\newcommand{\DesignLawErkMinTenOptmeanRepTwoLagOneP}{0.2210}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneSpearmanStatistic}{0.0257}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneSpearmanP}{0.8529}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneRunsStatistic}{44}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneRunsP}{0.1330}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneLagOneStatistic}{0.0059}
\newcommand{\DesignLawErkMinFifteenOptmeanRepOneLagOneP}{0.8622}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoSpearmanStatistic}{\ensuremath{-}0.1152}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoSpearmanP}{0.4091}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoRunsStatistic}{34}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoRunsP}{0.8731}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoLagOneStatistic}{0.0839}
\newcommand{\DesignLawErkMinFifteenOptmeanRepTwoLagOneP}{0.4375}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneSpearmanStatistic}{0.0170}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneSpearmanP}{0.9071}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneRunsStatistic}{28}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneRunsP}{0.4879}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneLagOneStatistic}{0.0422}
\newcommand{\DesignLawErkMinTwentyOptmeanRepOneLagOneP}{0.6522}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoSpearmanStatistic}{0.3176}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoSpearmanP}{0.0331}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoRunsStatistic}{36}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoRunsP}{0.0566}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoLagOneStatistic}{\ensuremath{-}0.2539}
\newcommand{\DesignLawErkMinTwentyOptmeanRepTwoLagOneP}{0.1074}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneSpearmanStatistic}{\ensuremath{-}0.1391}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneSpearmanP}{0.4359}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneRunsStatistic}{20}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneRunsP}{0.4121}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneLagOneStatistic}{0.3225}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepOneLagOneP}{0.0288}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoSpearmanStatistic}{\ensuremath{-}0.1980}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoSpearmanP}{0.2634}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoRunsStatistic}{24}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoRunsP}{0.5365}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoLagOneStatistic}{0.1707}
\newcommand{\DesignLawErkMinTwentyFiveOptmeanRepTwoLagOneP}{0.2240}
\newcommand{\DesignLawErkMinThreeMeanTwentySpearmanStatistic}{\ensuremath{-}0.0797}
\newcommand{\DesignLawErkMinThreeMeanTwentySpearmanP}{0.5578}
\newcommand{\DesignLawErkMinThreeMeanTwentyRunsStatistic}{36}
\newcommand{\DesignLawErkMinThreeMeanTwentyRunsP}{0.6390}
\newcommand{\DesignLawErkMinThreeMeanTwentyLagOneStatistic}{\ensuremath{-}0.0284}
\newcommand{\DesignLawErkMinThreeMeanTwentyLagOneP}{0.9400}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveSpearmanStatistic}{\ensuremath{-}0.1236}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveSpearmanP}{0.3387}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveRunsStatistic}{36}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveRunsP}{0.2930}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveLagOneStatistic}{\ensuremath{-}0.0217}
\newcommand{\DesignLawErkMinThreeMeanTwentyFiveLagOneP}{0.9688}
\newcommand{\DesignLawErkMinThreeMeanThirtySpearmanStatistic}{\ensuremath{-}0.2283}
\newcommand{\DesignLawErkMinThreeMeanThirtySpearmanP}{0.1577}
\newcommand{\DesignLawErkMinThreeMeanThirtyRunsStatistic}{28}
\newcommand{\DesignLawErkMinThreeMeanThirtyRunsP}{0.4462}
\newcommand{\DesignLawErkMinThreeMeanThirtyLagOneStatistic}{\ensuremath{-}0.0629}
\newcommand{\DesignLawErkMinThreeMeanThirtyLagOneP}{0.8389}
\newcommand{\DesignLawErkMinThreeMeanFortySpearmanStatistic}{\ensuremath{-}0.0143}
\newcommand{\DesignLawErkMinThreeMeanFortySpearmanP}{0.9441}
\newcommand{\DesignLawErkMinThreeMeanFortyRunsStatistic}{19}
\newcommand{\DesignLawErkMinThreeMeanFortyRunsP}{1.0000}
\newcommand{\DesignLawErkMinThreeMeanFortyLagOneStatistic}{\ensuremath{-}0.0091}
\newcommand{\DesignLawErkMinThreeMeanFortyLagOneP}{0.8791}
\newcommand{\DesignLawErkMinThreeMeanFiftySpearmanStatistic}{\ensuremath{-}0.2105}
\newcommand{\DesignLawErkMinThreeMeanFiftySpearmanP}{0.3162}
\newcommand{\DesignLawErkMinThreeMeanFiftyRunsStatistic}{15}
\newcommand{\DesignLawErkMinThreeMeanFiftyRunsP}{0.8175}
\newcommand{\DesignLawErkMinThreeMeanFiftyLagOneStatistic}{\ensuremath{-}0.0243}
\newcommand{\DesignLawErkMinThreeMeanFiftyLagOneP}{0.9379}
\newcommand{\DesignLawErkFisherCombinedSpearmanP}{0.2921}
\newcommand{\DesignLawErkFisherCombinedRunsP}{0.5117}
\newcommand{\DesignLawErkFisherCombinedLagOneP}{0.7157}
\newcommand{\DesignLawErkRestIntervalMinutes}{241}
\newcommand{\DesignLawCcasAprilOneThreeFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilOneThreeEligibleRandomRows}{3056}
\newcommand{\DesignLawCcasAprilOneThreeRawRows}{3456}
\newcommand{\DesignLawCcasAprilOneThreeTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilOneThreeOnRunTV}{0.01485}
\newcommand{\DesignLawCcasDOneAprilOneThreeOffRunTV}{0.01422}
\newcommand{\DesignLawCcasDOneAprilOneThreeMaxLagError}{0.00199}
\newcommand{\DesignLawCcasAprilOneFiveFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilOneFiveEligibleRandomRows}{3733}
\newcommand{\DesignLawCcasAprilOneFiveRawRows}{4133}
\newcommand{\DesignLawCcasAprilOneFiveTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilOneFiveOnRunTV}{0.00729}
\newcommand{\DesignLawCcasDOneAprilOneFiveOffRunTV}{0.00900}
\newcommand{\DesignLawCcasDOneAprilOneFiveMaxLagError}{0.00115}
\newcommand{\DesignLawCcasAprilOneNineFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilOneNineEligibleRandomRows}{3741}
\newcommand{\DesignLawCcasAprilOneNineRawRows}{4141}
\newcommand{\DesignLawCcasAprilOneNineTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilOneNineOnRunTV}{0.01140}
\newcommand{\DesignLawCcasDOneAprilOneNineOffRunTV}{0.01019}
\newcommand{\DesignLawCcasDOneAprilOneNineMaxLagError}{0.00425}
\newcommand{\DesignLawCcasAprilTwoOneFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilTwoOneEligibleRandomRows}{5127}
\newcommand{\DesignLawCcasAprilTwoOneRawRows}{5527}
\newcommand{\DesignLawCcasAprilTwoOneTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilTwoOneOnRunTV}{0.01025}
\newcommand{\DesignLawCcasDOneAprilTwoOneOffRunTV}{0.00652}
\newcommand{\DesignLawCcasDOneAprilTwoOneMaxLagError}{0.00272}
\newcommand{\DesignLawCcasAprilTwoTwoFixedTemplateRows}{335}
\newcommand{\DesignLawCcasAprilTwoTwoEligibleRandomRows}{3823}
\newcommand{\DesignLawCcasAprilTwoTwoRawRows}{4158}
\newcommand{\DesignLawCcasAprilTwoTwoTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilTwoTwoOnRunTV}{0.01120}
\newcommand{\DesignLawCcasDOneAprilTwoTwoOffRunTV}{0.00982}
\newcommand{\DesignLawCcasDOneAprilTwoTwoMaxLagError}{0.00483}
\newcommand{\DesignLawCcasAprilTwoThreeFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilTwoThreeEligibleRandomRows}{3751}
\newcommand{\DesignLawCcasAprilTwoThreeRawRows}{4151}
\newcommand{\DesignLawCcasAprilTwoThreeTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilTwoThreeOnRunTV}{0.00900}
\newcommand{\DesignLawCcasDOneAprilTwoThreeOffRunTV}{0.00892}
\newcommand{\DesignLawCcasDOneAprilTwoThreeMaxLagError}{0.00873}
\newcommand{\DesignLawCcasAprilTwoFourFixedTemplateRows}{400}
\newcommand{\DesignLawCcasAprilTwoFourEligibleRandomRows}{3743}
\newcommand{\DesignLawCcasAprilTwoFourRawRows}{4143}
\newcommand{\DesignLawCcasAprilTwoFourTemplateCount}{2}
\newcommand{\DesignLawCcasDOneAprilTwoFourOnRunTV}{0.01022}
\newcommand{\DesignLawCcasDOneAprilTwoFourOffRunTV}{0.00832}
\newcommand{\DesignLawCcasDOneAprilTwoFourMaxLagError}{0.00826}
\newcommand{\DesignLawCcasFixedTemplateRowsPooled}{2735}
\newcommand{\DesignLawCcasTemplateGroupsPooled}{14}
\newcommand{\DesignLawCcasEvaluationEligibleRows}{12{,}611}
\newcommand{\DesignLawCcasDOneDelaySteps}{1}
\newcommand{\DesignLawCcasSourceActiveComponents}{6}
\newcommand{\DesignLawCcasMOneAprilOneThreeZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilOneThreeOnRunTV}{0.0213}
\newcommand{\DesignLawCcasMOneAprilOneThreeOffRunTV}{0.0412}
\newcommand{\DesignLawCcasMOneAprilOneThreeMaxLagError}{0.0257}
\newcommand{\DesignLawCcasMOneAprilOneFiveZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilOneFiveOnRunTV}{0.0196}
\newcommand{\DesignLawCcasMOneAprilOneFiveOffRunTV}{0.0252}
\newcommand{\DesignLawCcasMOneAprilOneFiveMaxLagError}{0.0232}
\newcommand{\DesignLawCcasMOneAprilOneNineZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilOneNineOnRunTV}{0.0182}
\newcommand{\DesignLawCcasMOneAprilOneNineOffRunTV}{0.0362}
\newcommand{\DesignLawCcasMOneAprilOneNineMaxLagError}{0.0261}
\newcommand{\DesignLawCcasMOneAprilTwoOneZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilTwoOneOnRunTV}{0.0165}
\newcommand{\DesignLawCcasMOneAprilTwoOneOffRunTV}{0.0327}
\newcommand{\DesignLawCcasMOneAprilTwoOneMaxLagError}{0.0247}
\newcommand{\DesignLawCcasMOneAprilTwoTwoZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilTwoTwoOnRunTV}{0.0181}
\newcommand{\DesignLawCcasMOneAprilTwoTwoOffRunTV}{0.0324}
\newcommand{\DesignLawCcasMOneAprilTwoTwoMaxLagError}{0.0215}
\newcommand{\DesignLawCcasMOneAprilTwoThreeZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilTwoThreeOnRunTV}{0.0170}
\newcommand{\DesignLawCcasMOneAprilTwoThreeOffRunTV}{0.0298}
\newcommand{\DesignLawCcasMOneAprilTwoThreeMaxLagError}{0.0237}
\newcommand{\DesignLawCcasMOneAprilTwoFourZeroLikelihoodRows}{0}
\newcommand{\DesignLawCcasMOneAprilTwoFourOnRunTV}{0.0176}
\newcommand{\DesignLawCcasMOneAprilTwoFourOffRunTV}{0.0371}
\newcommand{\DesignLawCcasMOneAprilTwoFourMaxLagError}{0.0243}
\newcommand{\DesignLawCcasMOneAprilOneThreeOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneThreeOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneThreeMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneThreeSwitchDistributionP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneThreeLoglikKSP}{0.10448}
\newcommand{\DesignLawCcasMOneAprilOneFiveOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneFiveOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneFiveMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneFiveSwitchDistributionP}{0.01990}
\newcommand{\DesignLawCcasMOneAprilOneFiveLoglikKSP}{0.06468}
\newcommand{\DesignLawCcasMOneAprilOneNineOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneNineOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneNineMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneNineSwitchDistributionP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilOneNineLoglikKSP}{0.30846}
\newcommand{\DesignLawCcasMOneAprilTwoOneOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoOneOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoOneMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoOneSwitchDistributionP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoOneLoglikKSP}{0.02488}
\newcommand{\DesignLawCcasMOneAprilTwoTwoOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoTwoOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoTwoMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoTwoSwitchDistributionP}{0.02985}
\newcommand{\DesignLawCcasMOneAprilTwoTwoLoglikKSP}{0.27861}
\newcommand{\DesignLawCcasMOneAprilTwoThreeOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoThreeOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoThreeMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoThreeSwitchDistributionP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoThreeLoglikKSP}{0.05473}
\newcommand{\DesignLawCcasMOneAprilTwoFourOnRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoFourOffRunsP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoFourMinLagP}{0.00498}
\newcommand{\DesignLawCcasMOneAprilTwoFourSwitchDistributionP}{0.00995}
\newcommand{\DesignLawCcasMOneAprilTwoFourLoglikKSP}{0.18905}
\newcommand{\DesignLawCcasKFourAprilOneThreeOrder}{8}
\newcommand{\DesignLawCcasKFourAprilOneFiveOrder}{10}
\newcommand{\DesignLawCcasKFourAprilOneNineOrder}{10}
\newcommand{\DesignLawCcasKFourAprilTwoOneOrder}{10}
\newcommand{\DesignLawCcasKFourAprilTwoTwoOrder}{10}
\newcommand{\DesignLawCcasKFourAprilTwoThreeOrder}{10}
\newcommand{\DesignLawCcasKFourAprilTwoFourOrder}{8}
\newcommand{\DesignLawCcasKFourSmoothing}{0.5}
\newcommand{\DesignLawCcasKFourCVFolds}{3}
\newcommand{\DesignLawCcasKFourOrderMin}{1}
\newcommand{\DesignLawCcasKFourOrderMax}{12}
\newcommand{\BiowmEvalEarlierErkGainExpOne}{56.2\%}
\newcommand{\BiowmEvalEarlierErkGainExpTwo}{57.6\%}
\newcommand{\DesignLawGofRunTVThreshold}{0.02}
\newcommand{\DesignLawErkMinPerFieldP}{0.0288}
\newcommand{\MtwoaCRTNullCells}{240}
\newcommand{\MtwoaCRTNullCellsPerFamily}{60}
\newcommand{\MtwoaCRTCellsGeThirteen}{26}
\newcommand{\MtwoaCRTCellsGeSeventeen}{7}
\newcommand{\MtwoaCRTCellsGeTwenty}{1}
\newcommand{\MtwoaCRTMaxCount}{20}
\newcommand{\MfourBatchPPerModelLGErkHtenFrac}{12/128}
\newcommand{\MfourBatchPPerModelGRUErkHtenFrac}{12/128}
\newcommand{\MfourBatchPPerModelTFErkHtenFrac}{12/128}
\newcommand{\MfourBatchPPerModelGBErkHtenFrac}{12/128}
\newcommand{\MfourBatchPPerModelSummaryErkHtenMinFrac}{12/128}
\newcommand{\MfourBatchPPerModelSummaryErkHtenMaxFrac}{12/128}
\newcommand{\MfourBatchPPerModelLGErkHthirtyFrac}{1/128}
\newcommand{\MfourBatchPPerModelGRUErkHthirtyFrac}{2/128}
\newcommand{\MfourBatchPPerModelTFErkHthirtyFrac}{2/128}
\newcommand{\MfourBatchPPerModelGBErkHthirtyFrac}{2/128}
\newcommand{\MfourBatchPPerModelSummaryErkHthirtyMinFrac}{1/128}
\newcommand{\MfourBatchPPerModelSummaryErkHthirtyMaxFrac}{2/128}
\newcommand{\MfourBatchPPerModelLGCcasHoneFrac}{61/128}
\newcommand{\MfourBatchPPerModelGRUCcasHoneFrac}{89/128}
\newcommand{\MfourBatchPPerModelTFCcasHoneFrac}{104/128}
\newcommand{\MfourBatchPPerModelGBCcasHoneFrac}{89/128}
\newcommand{\MfourBatchPPerModelLGCcasHsixFrac}{1/128}
\newcommand{\MfourBatchPPerModelGRUCcasHsixFrac}{1/128}
\newcommand{\MfourBatchPPerModelTFCcasHsixFrac}{1/128}
\newcommand{\MfourBatchPPerModelGBCcasHsixFrac}{1/128}
\newcommand{\MfourBatchPPerModelSummaryCcasHsixMinFrac}{1/128}
\newcommand{\MfourBatchPPerModelSummaryCcasHsixMaxFrac}{1/128}
\newcommand{\MfourLugagneBatchPFrac}{1/128}


==> macros/demo_aliases.tex <==
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowARejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowAK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowACpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowACpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowAMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowASeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowARCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowBRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowBK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowBCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowBCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowBMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowBSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowBRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowDRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowDK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowDCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowDCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowDMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowDSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowDRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowERejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowEK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowECpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowECpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowEMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowESeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowERCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowFRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowFK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowFCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowFCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowFMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowFSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowFRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowGRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowGK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowGCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowGCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowGMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowGSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowHRejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowHK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowHCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowHCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowHMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowHSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowHRCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowIRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowIK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowICpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowICpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowIMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowISeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowIRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowJRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowJK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowJCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowJCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowJMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowJSeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowJRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowKRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowKK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowKCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowKCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowKMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowKSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowKRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowLRejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowLK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowLCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowLCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowLMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowLSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowLRCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowMRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowMK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowMCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowMCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowMMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowMSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowMRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowNRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowNK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowNCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowNCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowNMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowNSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowORejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowOK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowOCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowOCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowOMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowOSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowORCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowPRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowPK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowPCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowPCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowPMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowPSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowPRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowQRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowQK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowQCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowQCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowQMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowQSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowQRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowRRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowRK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowRCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowRCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowRMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowRSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowRRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowSRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowSK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowSCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowSCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowSMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowSSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowSRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowTRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowTK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowTCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowTCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowTMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowTSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowTRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowURejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowUK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowUCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowUCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowUMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowUSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowURCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowVRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowVK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowVCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowVCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowVMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowVSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowVRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowWRejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowWK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowWCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowWCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowWMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowWSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowWRCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowXRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowXK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowXCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowXCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowXMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowXSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowXRCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowYRejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowYK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowYCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowYCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowYMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowYSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowZRejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowZK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowZCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowZCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowZMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowZSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowZRCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAARejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAAK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAACpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAACpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAAMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAASeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAARCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowABRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowABK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowABCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowABCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowABMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowABSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowABRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowACRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowACK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowACCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowACCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowACMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowACSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowACRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowADRejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowADK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowADCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowADCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowADMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowADSeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowADRCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAERejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAEK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAECpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAECpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAEMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAESeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAERCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAFRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAFK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAFCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAFCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAFMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAFSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAGRejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAGK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAGCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAGCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAGMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAGSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAGRCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAHRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAHK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAHCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAHCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAHMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAHSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAHRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAIRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAIK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAICpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAICpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAIMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAISeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAIRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAJRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAJK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAJCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAJCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAJMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAJSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAJRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAKRejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAKK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAKCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAKCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAKMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAKSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAKRCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowALRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowALK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowALCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowALCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowALMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowALSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowALRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAMRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAMK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAMCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAMCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAMMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAMSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowANRejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowANK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowANCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowANCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowANMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowANSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowANRCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAORejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAOK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAOCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAOCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAOMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAOSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAORCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAPRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAPK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAPCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAPCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAPMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAPSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAPRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAQRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAQK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAQCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAQCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAQMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAQSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAQRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowARRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowARK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowARCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowARCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowARMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowARSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowARRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowASRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowASK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowASCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowASCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowASMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowASSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowASRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowATRejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowATK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowATCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowATCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowATMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowATSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowATRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAURejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAUK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAUCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAUCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAUMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAUSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAURCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAVRejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAVK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAVCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAVCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAVMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAVSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAVRCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAWRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAWK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAWCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAWCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAWMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAWSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowAWRCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowAXRejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowAXK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowAXCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowAXCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowAXMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowAXSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowAYRejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowAYK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowAYCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowAYCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowAYMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowAYSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowAYRCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowAZRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowAZK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowAZCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowAZCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowAZMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowAZSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowAZRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBARejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBAK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBACpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBACpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBAMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBASeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBARCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBBRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBBK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBBCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBBCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBBMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBBSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBBRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBCRejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBCK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBCCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBCCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBCMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBCSeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBCRCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBDRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBDK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBDCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBDCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBDMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBDSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBDRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBERejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBEK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBECpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBECpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBEMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBESeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBFRejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBFK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBFCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBFCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBFMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBFSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBFRCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBGRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBGK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBGCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBGCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBGMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBGSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBGRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBHRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBHK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBHCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBHCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBHMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBHSeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBHRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBIRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBIK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBICpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBICpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBIMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBISeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBIRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBJRejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBJK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBJCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBJCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBJMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBJSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBJRCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBKRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBKK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBKCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBKCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBKMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBKSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBKRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBLRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBLK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBLCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBLCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBLMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBLSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBMRejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBMK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBMCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBMCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBMMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBMSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBMRCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBNRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBNK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBNCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBNCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBNMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBNSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBNRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBORejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBOK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBOCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBOCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBOMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBOSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBORCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBPRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBPK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBPCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBPCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBPMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBPSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBPRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBQRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBQK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBQCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBQCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBQMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBQSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBQRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBRRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBRK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBRCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBRCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBRMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBRSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBRRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBSRejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBSK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBSCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBSCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBSMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBSSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBSRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBTRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBTK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBTCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBTCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBTMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBTSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBTRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBURejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBUK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBUCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBUCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBUMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBUSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBURCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBVRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBVK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBVCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBVCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBVMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBVSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowBVRCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowBWRejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowBWK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowBWCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowBWCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowBWMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowBWSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowBXRejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowBXK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowBXCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowBXCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowBXMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowBXSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowBXRCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowBYRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowBYK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowBYCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowBYCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowBYMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowBYSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowBYRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowBZRejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowBZK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowBZCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowBZCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowBZMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowBZSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowBZRCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCARejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCAK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCACpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCACpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCAMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCASeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCARCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCBRejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCBK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCBCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCBCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCBMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCBSeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCBRCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCCRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCCK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCCCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCCCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCCMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCCSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCCRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCDRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCDK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCDCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCDCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCDMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCDSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCERejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCEK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCECpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCECpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCEMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCESeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCERCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCFRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCFK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCFCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCFCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCFMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCFSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCFRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCGRejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCGK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCGCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCGCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCGMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCGSeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCGRCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCHRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCHK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCHCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCHCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCHMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCHSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCHRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCIRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCIK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCICpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCICpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCIMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCISeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCIRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCJRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCJK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCJCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCJCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCJMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCJSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCJRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCKRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCKK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCKCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCKCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCKMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCKSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCLRejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCLK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCLCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCLCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCLMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCLSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCLRCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCMRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCMK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCMCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCMCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCMMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCMSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCMRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCNRejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCNK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCNCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCNCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCNMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCNSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCNRCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCORejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCOK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCOCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCOCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCOMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCOSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCORCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCPRejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCPK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCPCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCPCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCPMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCPSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCPRCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCQRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCQK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCQCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCQCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCQMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCQSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCQRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCRRejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCRK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCRCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCRCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCRMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCRSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCRRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCSRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCSK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCSCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCSCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCSMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCSSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCSRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCTRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCTK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCTCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCTCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCTMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCTSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCTRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCURejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCUK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCUCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCUCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCUMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCUSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCount}{\DemoTOneRowCURCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCount}{\DemoTOneRowCVRejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTOneRowCVK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILower}{\DemoTOneRowCVCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpper}{\DemoTOneRowCVCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanE}{\DemoTOneRowCVMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorE}{\DemoTOneRowCVSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowCWRejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowCWK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowCWCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowCWCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowCWMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowCWSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowCWRCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowCXRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowCXK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowCXCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowCXCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowCXMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowCXSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowCXRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowCYRejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowCYK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowCYCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowCYCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowCYMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowCYSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowCYRCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowCZRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowCZK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowCZCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowCZCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowCZMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowCZSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowCZRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDARejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDAK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDACpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDACpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDAMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDASeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDARCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDBRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDBK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDBCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDBCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDBMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDBSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDBRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDCRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDCK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDCCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDCCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDCMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDCSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDDRejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDDK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDDCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDDCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDDMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDDSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDDRCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDERejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDEK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDECpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDECpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDEMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDESeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDERCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDFRejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDFK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDFCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDFCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDFMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDFSeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDFRCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDGRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDGK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDGCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDGCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDGMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDGSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDGRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDHRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDHK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDHCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDHCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDHMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDHSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDHRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDIRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDIK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDICpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDICpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDIMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDISeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDIRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDJRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDJK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDJCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDJCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDJMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDJSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDKRejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDKK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDKCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDKCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDKMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDKSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDKRCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDLRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDLK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDLCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDLCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDLMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDLSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDLRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDMRejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDMK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDMCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDMCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDMMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDMSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDMRCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDNRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDNK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDNCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDNCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDNMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDNSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDNRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDORejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDOK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDOCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDOCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDOMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDOSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDORCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDPRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDPK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDPCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDPCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDPMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDPSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDPRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDQRejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDQK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDQCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDQCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDQMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDQSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDQRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDRRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDRK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDRCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDRCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDRMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDRSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDRRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDSRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDSK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDSCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDSCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDSMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDSSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDSRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDTRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDTK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDTCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDTCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDTMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDTSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCount}{\DemoTOneRowDTRCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCount}{\DemoTOneRowDURejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTOneRowDUK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILower}{\DemoTOneRowDUCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpper}{\DemoTOneRowDUCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanE}{\DemoTOneRowDUMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorE}{\DemoTOneRowDUSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowDVRejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowDVK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowDVCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowDVCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowDVMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowDVSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowDVRCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowDWRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowDWK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowDWCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowDWCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowDWMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowDWSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowDWRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowDXRejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowDXK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowDXCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowDXCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowDXMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowDXSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowDXRCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowDYRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowDYK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowDYCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowDYCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowDYMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowDYSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowDYRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowDZRejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowDZK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowDZCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowDZCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowDZMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowDZSeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowDZRCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEARejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEAK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEACpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEACpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEAMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEASeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEARCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEBRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEBK}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEBCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEBCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEBMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEBSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowECRejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowECK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowECCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowECCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowECMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowECSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowECRCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEDRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEDK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEDCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEDCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEDMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEDSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEDRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEERejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEEK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEECpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEECpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEEMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEESeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEERCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEFRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEFK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEFCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEFCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEFMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEFSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEFRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEGRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEGK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEGCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEGCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEGMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEGSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEGRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEHRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEHK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEHCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEHCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEHMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEHSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEHRCrit}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEIRejections}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEIK}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEICpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEICpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEIMeanE}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEISeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEJRejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEJK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEJCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEJCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEJMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEJSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEJRCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEKRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEKK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEKCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEKCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEKMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEKSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEKRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowELRejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowELK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowELCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowELCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowELMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowELSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowELRCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEMRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEMK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEMCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEMCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEMMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEMSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEMRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowENRejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowENK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowENCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowENCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowENMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowENSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowENRCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEORejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEOK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEOCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEOCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEOMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEOSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEORCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEPRejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEPK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEPCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEPCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEPMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEPSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEPRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowEQRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowEQK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowEQCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowEQCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowEQMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowEQSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowEQRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowERRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowERK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowERCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowERCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowERMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowERSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowERRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowESRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowESK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowESCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowESCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowESMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowESSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCount}{\DemoTOneRowESRCrit}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCount}{\DemoTOneRowETRejections}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTOneRowETK}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILower}{\DemoTOneRowETCpNineFiveLower}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpper}{\DemoTOneRowETCpNineFiveUpper}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanE}{\DemoTOneRowETMeanE}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorE}{\DemoTOneRowETSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEURejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEUK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEUCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEUCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEUMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEUSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEURCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEVRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEVK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEVCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEVCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEVMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEVSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEVRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEWRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEWK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEWCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEWCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEWMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEWSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEWRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEXRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEXK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEXCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEXCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEXMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEXSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEXRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEYRejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEYK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEYCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEYCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEYMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEYSeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEYRCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowEZRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowEZK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowEZCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowEZCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowEZMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowEZSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowEZRCrit}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFARejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFAK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFACpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFACpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFAMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFASeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFARCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFBRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFBK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFBCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFBCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFBMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFBSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFBRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFCRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFCK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFCCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFCCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFCMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFCSeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFCRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFDRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFDK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFDCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFDCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFDMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFDSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFDRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFERejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFEK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFECpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFECpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFEMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFESeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFERCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFFRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFFK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFFCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFFCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFFMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFFSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFFRCrit}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFGRejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFGK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFGCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFGCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFGMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFGSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFGRCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFHRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFHK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFHCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFHCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFHMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFHSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFHRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFIRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFIK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFICpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFICpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFIMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFISeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFIRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFJRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFJK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFJCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFJCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFJMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFJSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFJRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFKRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFKK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFKCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFKCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFKMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFKSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFKRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFLRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFLK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFLCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFLCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFLMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFLSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFLRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFMRejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFMK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFMCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFMCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFMMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFMSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFMRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFNRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFNK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFNCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFNCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFNMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFNSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFNRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFORejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFOK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFOCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFOCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFOMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFOSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFORCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFPRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFPK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFPCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFPCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFPMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFPSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFPRCrit}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFQRejections}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFQK}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFQCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFQCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFQMeanE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFQSeE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFQRCrit}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFRRejections}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFRK}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFRCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFRCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFRMeanE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFRSeE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFRRCrit}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFSRejections}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFSK}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFSCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFSCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFSMeanE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFSSeE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFSRCrit}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFTRejections}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFTK}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFTCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFTCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFTMeanE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFTSeE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFTRCrit}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFURejections}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFUK}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFUCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFUCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFUMeanE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFUSeE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFURCrit}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFVRejections}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFVK}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFVCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFVCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFVMeanE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFVSeE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFVRCrit}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFWRejections}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFWK}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFWCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFWCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFWMeanE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFWSeE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFWRCrit}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFXRejections}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFXK}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFXCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFXCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFXMeanE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFXSeE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFXRCrit}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFYRejections}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFYK}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFYCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFYCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFYMeanE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFYSeE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFYRCrit}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowFZRejections}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowFZK}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowFZCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowFZCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowFZMeanE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowFZSeE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowFZRCrit}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGARejections}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGAK}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGACpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGACpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGAMeanE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGASeE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGARCrit}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGBRejections}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGBK}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGBCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGBCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGBMeanE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGBSeE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGBRCrit}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGCRejections}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGCK}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGCCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGCCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGCMeanE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGCSeE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGCRCrit}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGDRejections}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGDK}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGDCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGDCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGDMeanE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGDSeE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGDRCrit}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGERejections}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGEK}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGECpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGECpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGEMeanE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGESeE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGERCrit}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGFRejections}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGFK}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGFCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGFCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGFMeanE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGFSeE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGFRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGGRejections}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGGK}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGGCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGGCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGGMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGGSeE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGGRCrit}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGHRejections}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGHK}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGHCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGHCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGHMeanE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGHSeE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGHRCrit}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGIRejections}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGIK}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGICpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGICpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGIMeanE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGISeE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGIRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGJRejections}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGJK}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGJCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGJCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGJMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGJSeE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGJRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGKRejections}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGKK}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGKCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGKCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGKMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGKSeE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGKRCrit}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGLRejections}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGLK}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGLCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGLCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGLMeanE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGLSeE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGLRCrit}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGMRejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGMK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGMCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGMCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGMMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGMSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGMRCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGNRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGNK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGNCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGNCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGNMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGNSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGNRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGORejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGOK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGOCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGOCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGOMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGOSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGORCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGPRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGPK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGPCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGPCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGPMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGPSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGPRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGQRejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGQK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGQCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGQCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGQMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGQSeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGQRCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGRRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGRK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGRCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGRCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGRMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGRSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGRRCrit}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGSRejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGSK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGSCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGSCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGSMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGSSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGSRCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGTRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGTK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGTCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGTCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGTMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGTSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGTRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGURejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGUK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGUCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGUCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGUMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGUSeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGURCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGVRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGVK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGVCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGVCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGVMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGVSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGVRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGWRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGWK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGWCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGWCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGWMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGWSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGWRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGXRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGXK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGXCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGXCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGXMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGXSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGXRCrit}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGYRejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGYK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGYCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGYCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGYMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGYSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGYRCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowGZRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowGZK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowGZCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowGZCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowGZMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowGZSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowGZRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHARejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHAK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHACpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHACpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHAMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHASeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHARCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHBRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHBK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHBCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHBCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHBMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHBSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHBRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHCRejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHCK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHCCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHCCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHCMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHCSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHCRCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHDRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHDK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHDCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHDCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHDMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHDSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHDRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHERejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHEK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHECpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHECpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHEMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHESeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHERCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHFRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHFK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHFCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHFCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHFMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHFSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHFRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHGRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHGK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHGCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHGCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHGMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHGSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHGRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHHRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHHK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHHCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHHCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHHMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHHSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHHRCrit}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHIRejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHIK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHICpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHICpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHIMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHISeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHIRCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHJRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHJK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHJCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHJCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHJMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHJSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHJRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHKRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHKK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHKCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHKCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHKMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHKSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHKRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHLRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHLK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHLCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHLCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHLMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHLSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHLRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHMRejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHMK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHMCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHMCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHMMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHMSeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHMRCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHNRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHNK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHNCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHNCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHNMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHNSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHNRCrit}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHORejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHOK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHOCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHOCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHOMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHOSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHORCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHPRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHPK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHPCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHPCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHPMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHPSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHPRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHQRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHQK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHQCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHQCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHQMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHQSeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHQRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHRRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHRK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHRCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHRCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHRMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHRSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHRRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHSRejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHSK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHSCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHSCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHSMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHSSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHSRCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHTRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHTK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHTCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHTCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHTMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHTSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHTRCrit}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHURejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHUK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHUCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHUCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHUMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHUSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHURCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHVRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHVK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHVCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHVCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHVMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHVSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHVRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHWRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHWK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHWCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHWCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHWMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHWSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHWRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHXRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHXK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHXCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHXCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHXMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHXSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHXRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHYRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHYK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHYCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHYCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHYMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHYSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHYRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowHZRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowHZK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowHZCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowHZCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowHZMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowHZSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowHZRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIARejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIAK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIACpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIACpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIAMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIASeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIARCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIBRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIBK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIBCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIBCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIBMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIBSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIBRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowICRejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowICK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowICCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowICCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowICMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowICSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowICRCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIDRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIDK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIDCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIDCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIDMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIDSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIDRCrit}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIERejections}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIEK}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIECpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIECpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIEMeanE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIESeE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIERCrit}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIFRejections}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIFK}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIFCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIFCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIFMeanE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIFSeE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIFRCrit}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIGRejections}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIGK}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIGCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIGCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIGMeanE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIGSeE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIGRCrit}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIHRejections}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIHK}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIHCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIHCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIHMeanE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIHSeE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIHRCrit}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIIRejections}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIIK}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIICpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIICpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIIMeanE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIISeE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIIRCrit}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIJRejections}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIJK}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIJCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIJCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIJMeanE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIJSeE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIJRCrit}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIKRejections}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIKK}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIKCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIKCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIKMeanE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIKSeE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIKRCrit}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowILRejections}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowILK}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowILCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowILCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowILMeanE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowILSeE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowILRCrit}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIMRejections}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIMK}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIMCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIMCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIMMeanE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIMSeE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIMRCrit}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowINRejections}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowINK}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowINCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowINCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowINMeanE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowINSeE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowINRCrit}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIORejections}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIOK}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIOCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIOCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIOMeanE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIOSeE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIORCrit}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIPRejections}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIPK}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIPCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIPCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIPMeanE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIPSeE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIPRCrit}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIQRejections}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIQK}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIQCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIQCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIQMeanE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIQSeE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIQRCrit}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIRRejections}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIRK}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIRCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIRCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIRMeanE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIRSeE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIRRCrit}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowISRejections}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowISK}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowISCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowISCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowISMeanE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowISSeE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowISRCrit}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowITRejections}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowITK}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowITCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowITCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowITMeanE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowITSeE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowITRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIURejections}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIUK}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIUCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIUCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIUMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIUSeE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIURCrit}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIVRejections}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIVK}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIVCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIVCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIVMeanE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIVSeE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIVRCrit}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIWRejections}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIWK}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIWCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIWCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIWMeanE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIWSeE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIWRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIXRejections}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIXK}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIXCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIXCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIXMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIXSeE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIXRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIYRejections}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIYK}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIYCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIYCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIYMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIYSeE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIYRCrit}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowIZRejections}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowIZK}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowIZCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowIZCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowIZMeanE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowIZSeE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowIZRCrit}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJARejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJAK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJACpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJACpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJAMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJASeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJARCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJBRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJBK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJBCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJBCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJBMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJBSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJBRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJCRejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJCK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJCCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJCCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJCMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJCSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJCRCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJDRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJDK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJDCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJDCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJDMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJDSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJDRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJERejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJEK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJECpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJECpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJEMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJESeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJERCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJFRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJFK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJFCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJFCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJFMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJFSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJFRCrit}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJGRejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJGK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJGCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJGCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJGMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJGSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJGRCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJHRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJHK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJHCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJHCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJHMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJHSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJHRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJIRejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJIK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJICpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJICpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJIMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJISeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJIRCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJJRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJJK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJJCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJJCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJJMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJJSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJJRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJKRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJKK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJKCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJKCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJKMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJKSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJKRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJLRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJLK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJLCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJLCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJLMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJLSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJLRCrit}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJMRejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJMK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJMCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJMCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJMMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJMSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJMRCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJNRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJNK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJNCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJNCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJNMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJNSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJNRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJORejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJOK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJOCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJOCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJOMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJOSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJORCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJPRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJPK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJPCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJPCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJPMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJPSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJPRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJQRejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJQK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJQCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJQCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJQMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJQSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJQRCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJRRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJRK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJRCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJRCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJRMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJRSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJRRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJSRejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJSK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJSCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJSCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJSMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJSSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJSRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJTRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJTK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJTCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJTCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJTMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJTSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJTRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJURejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJUK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJUCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJUCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJUMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJUSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJURCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJVRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJVK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJVCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJVCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJVMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJVSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJVRCrit}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJWRejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJWK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJWCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJWCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJWMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJWSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJWRCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJXRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJXK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJXCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJXCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJXMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJXSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJXRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJYRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJYK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJYCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJYCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJYMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJYSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJYRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowJZRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowJZK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowJZCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowJZCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowJZMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowJZSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowJZRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKARejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKAK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKACpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKACpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKAMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKASeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKARCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKBRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKBK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKBCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKBCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKBMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKBSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKBRCrit}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKCRejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKCK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKCCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKCCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKCMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKCSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKCRCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKDRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKDK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKDCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKDCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKDMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKDSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKDRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKERejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKEK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKECpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKECpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKEMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKESeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKERCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKFRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKFK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKFCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKFCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKFMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKFSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKFRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKGRejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKGK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKGCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKGCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKGMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKGSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKGRCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKHRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKHK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKHCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKHCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKHMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKHSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKHRCrit}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKIRejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKIK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKICpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKICpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKIMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKISeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKIRCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKJRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKJK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKJCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKJCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKJMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKJSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKJRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKKRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKKK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKKCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKKCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKKMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKKSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKKRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKLRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKLK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKLCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKLCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKLMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKLSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKLRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKMRejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKMK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKMCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKMCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKMMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKMSeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKMRCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKNRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKNK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKNCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKNCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKNMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKNSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKNRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKORejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKOK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKOCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKOCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKOMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKOSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKORCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKPRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKPK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKPCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKPCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKPMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKPSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKPRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKQRejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKQK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKQCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKQCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKQMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKQSeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKQRCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKRRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKRK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKRCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKRCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKRMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKRSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKRRCrit}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKSRejections}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKSK}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKSCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKSCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKSMeanE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKSSeE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKSRCrit}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKTRejections}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKTK}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKTCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKTCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKTMeanE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKTSeE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKTRCrit}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKURejections}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKUK}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKUCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKUCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKUMeanE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKUSeE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKURCrit}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKVRejections}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKVK}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKVCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKVCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKVMeanE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKVSeE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKVRCrit}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKWRejections}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKWK}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKWCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKWCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKWMeanE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKWSeE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKWRCrit}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKXRejections}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKXK}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKXCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKXCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKXMeanE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKXSeE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKXRCrit}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKYRejections}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKYK}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKYCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKYCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKYMeanE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKYSeE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKYRCrit}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowKZRejections}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowKZK}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowKZCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowKZCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowKZMeanE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowKZSeE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowKZRCrit}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLARejections}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLAK}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLACpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLACpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLAMeanE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLASeE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLARCrit}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLBRejections}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLBK}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLBCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLBCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLBMeanE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLBSeE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLBRCrit}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLCRejections}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLCK}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLCCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLCCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLCMeanE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLCSeE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLCRCrit}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLDRejections}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLDK}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLDCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLDCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLDMeanE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLDSeE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLDRCrit}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLERejections}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLEK}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLECpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLECpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLEMeanE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLESeE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLERCrit}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLFRejections}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLFK}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLFCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLFCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLFMeanE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLFSeE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLFRCrit}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLGRejections}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLGK}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLGCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLGCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLGMeanE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLGSeE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLGRCrit}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLHRejections}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLHK}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLHCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLHCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLHMeanE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLHSeE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLHRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLIRejections}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLIK}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLICpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLICpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLIMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLISeE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLIRCrit}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLJRejections}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLJK}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLJCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLJCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLJMeanE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLJSeE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLJRCrit}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLKRejections}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLKK}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLKCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLKCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLKMeanE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLKSeE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLKRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLLRejections}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLLK}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLLCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLLCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLLMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLLSeE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLLRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLMRejections}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLMK}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLMCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLMCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLMMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLMSeE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLMRCrit}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLNRejections}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLNK}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLNCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLNCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLNMeanE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLNSeE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLNRCrit}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLORejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLOK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLOCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLOCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLOMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLOSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLORCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLPRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLPK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLPCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLPCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLPMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLPSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLPRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLQRejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLQK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLQCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLQCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLQMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLQSeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLQRCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLRRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLRK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLRCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLRCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLRMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLRSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLRRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLSRejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLSK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLSCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLSCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLSMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLSSeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLSRCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLTRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLTK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLTCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLTCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLTMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLTSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLTRCrit}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLURejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLUK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLUCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLUCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLUMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLUSeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLURCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLVRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLVK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLVCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLVCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLVMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLVSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLVRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLWRejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLWK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLWCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLWCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLWMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLWSeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLWRCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLXRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLXK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLXCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLXCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLXMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLXSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLXRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLYRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLYK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLYCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLYCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLYMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLYSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLYRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowLZRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowLZK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowLZCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowLZCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowLZMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowLZSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowLZRCrit}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMARejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMAK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMACpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMACpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMAMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMASeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMARCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMBRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMBK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMBCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMBCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMBMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMBSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMBRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMCRejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMCK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMCCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMCCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMCMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMCSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMCRCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMDRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMDK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMDCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMDCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMDMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMDSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMDRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMERejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMEK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMECpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMECpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMEMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMESeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMERCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMFRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMFK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMFCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMFCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMFMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMFSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMFRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMGRejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMGK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMGCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMGCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMGMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMGSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMGRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMHRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMHK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMHCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMHCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMHMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMHSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMHRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMIRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMIK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMICpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMICpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMIMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMISeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMIRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMJRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMJK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMJCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMJCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMJMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMJSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMJRCrit}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMKRejections}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMKK}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMKCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMKCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMKMeanE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMKSeE}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMKRCrit}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMLRejections}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMLK}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMLCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMLCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMLMeanE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMLSeE}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMLRCrit}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMMRejections}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMMK}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMMCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMMCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMMMeanE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMMSeE}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMMRCrit}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMNRejections}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMNK}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMNCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMNCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMNMeanE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMNSeE}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMNRCrit}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMORejections}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMOK}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMOCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMOCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMOMeanE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMOSeE}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMORCrit}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMPRejections}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMPK}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMPCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMPCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMPMeanE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMPSeE}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMPRCrit}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMQRejections}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMQK}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMQCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMQCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMQMeanE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMQSeE}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMQRCrit}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMRRejections}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMRK}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMRCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMRCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMRMeanE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMRSeE}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMRRCrit}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMSRejections}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMSK}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMSCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMSCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMSMeanE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMSSeE}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMSRCrit}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMTRejections}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMTK}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMTCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMTCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMTMeanE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMTSeE}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMTRCrit}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMURejections}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMUK}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMUCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMUCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMUMeanE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMUSeE}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMURCrit}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMVRejections}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMVK}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMVCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMVCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMVMeanE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMVSeE}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMVRCrit}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMWRejections}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMWK}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMWCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMWCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMWMeanE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMWSeE}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMWRCrit}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMXRejections}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMXK}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMXCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMXCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMXMeanE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMXSeE}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMXRCrit}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMYRejections}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMYK}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMYCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMYCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMYMeanE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMYSeE}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMYRCrit}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowMZRejections}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowMZK}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowMZCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowMZCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowMZMeanE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowMZSeE}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowMZRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNARejections}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNAK}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNACpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNACpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNAMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNASeE}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNARCrit}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNBRejections}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNBK}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNBCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNBCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNBMeanE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNBSeE}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNBRCrit}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNCRejections}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNCK}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNCCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNCCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNCMeanE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNCSeE}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNCRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNDRejections}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNDK}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNDCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNDCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNDMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNDSeE}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNDRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNERejections}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNEK}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNECpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNECpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNEMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNESeE}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNERCrit}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNFRejections}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNFK}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNFCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNFCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNFMeanE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNFSeE}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNFRCrit}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNGRejections}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNGK}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNGCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNGCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNGMeanE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNGSeE}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNGRCrit}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNHRejections}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNHK}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNHCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNHCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNHMeanE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNHSeE}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNHRCrit}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNIRejections}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNIK}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNICpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNICpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNIMeanE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNISeE}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNIRCrit}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNJRejections}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNJK}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNJCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNJCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNJMeanE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNJSeE}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNJRCrit}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNKRejections}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNKK}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNKCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNKCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNKMeanE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNKSeE}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNKRCrit}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNLRejections}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNLK}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNLCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNLCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNLMeanE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNLSeE}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNLRCrit}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNMRejections}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNMK}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNMCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNMCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNMMeanE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNMSeE}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNMRCrit}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNNRejections}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNNK}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNNCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNNCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNNMeanE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNNSeE}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNNRCrit}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNORejections}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNOK}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNOCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNOCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNOMeanE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNOSeE}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNORCrit}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNPRejections}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNPK}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNPCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNPCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNPMeanE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNPSeE}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNPRCrit}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNQRejections}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNQK}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNQCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNQCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNQMeanE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNQSeE}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNQRCrit}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNRRejections}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNRK}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNRCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNRCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNRMeanE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNRSeE}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNRRCrit}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNSRejections}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNSK}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNSCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNSCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNSMeanE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNSSeE}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNSRCrit}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNTRejections}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNTK}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNTCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNTCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNTMeanE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNTSeE}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNTRCrit}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNURejections}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNUK}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNUCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNUCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNUMeanE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNUSeE}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNURCrit}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNVRejections}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNVK}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNVCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNVCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNVMeanE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNVSeE}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNVRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNWRejections}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNWK}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNWCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNWCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNWMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNWSeE}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNWRCrit}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNXRejections}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNXK}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNXCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNXCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNXMeanE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNXSeE}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNXRCrit}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNYRejections}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNYK}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNYCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNYCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNYMeanE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNYSeE}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNYRCrit}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowNZRejections}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowNZK}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowNZCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowNZCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowNZMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowNZSeE}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowNZRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOARejections}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOAK}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOACpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOACpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOAMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOASeE}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOARCrit}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOBRejections}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOBK}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOBCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOBCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOBMeanE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOBSeE}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOBRCrit}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOCRejections}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOCK}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOCCpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOCCpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOCMeanE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOCSeE}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOCRCrit}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowODRejections}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowODK}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowODCpNineFiveLower}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowODCpNineFiveUpper}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowODMeanE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowODSeE}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowODRCrit}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOERejections}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOEK}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOECpNineFiveLower}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOECpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOEMeanE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOESeE}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOERCrit}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOFRejections}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOFK}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOFCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOFCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOFMeanE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOFSeE}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOFRCrit}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOGRejections}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOGK}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOGCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOGCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOGMeanE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOGSeE}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOGRCrit}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOHRejections}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOHK}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOHCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOHCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOHMeanE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOHSeE}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOHRCrit}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOIRejections}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOIK}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOICpNineFiveLower}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOICpNineFiveUpper}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOIMeanE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOISeE}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOIRCrit}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOJRejections}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOJK}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOJCpNineFiveLower}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOJCpNineFiveUpper}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOJMeanE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOJSeE}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOJRCrit}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOKRejections}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOKK}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOKCpNineFiveLower}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOKCpNineFiveUpper}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOKMeanE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOKSeE}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOKRCrit}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOLRejections}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOLK}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOLCpNineFiveLower}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOLCpNineFiveUpper}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOLMeanE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOLSeE}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOLRCrit}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOMRejections}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOMK}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOMCpNineFiveLower}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOMCpNineFiveUpper}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOMMeanE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOMSeE}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOMRCrit}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowONRejections}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowONK}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowONCpNineFiveLower}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowONCpNineFiveUpper}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowONMeanE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowONSeE}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowONRCrit}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOORejections}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOOK}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOOCpNineFiveLower}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOOCpNineFiveUpper}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOOMeanE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOOSeE}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOORCrit}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOPRejections}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOPK}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOPCpNineFiveLower}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOPCpNineFiveUpper}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOPMeanE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOPSeE}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOPRCrit}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOQRejections}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOQK}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOQCpNineFiveLower}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOQCpNineFiveUpper}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOQMeanE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOQSeE}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOQRCrit}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowORRejections}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowORK}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowORCpNineFiveLower}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowORCpNineFiveUpper}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowORMeanE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowORSeE}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowORRCrit}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOSRejections}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOSK}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOSCpNineFiveLower}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOSCpNineFiveUpper}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOSMeanE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOSSeE}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOSRCrit}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOTRejections}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOTK}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOTCpNineFiveLower}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOTCpNineFiveUpper}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOTMeanE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOTSeE}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOTRCrit}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOURejections}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOUK}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOUCpNineFiveLower}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOUCpNineFiveUpper}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOUMeanE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOUSeE}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOURCrit}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOVRejections}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOVK}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOVCpNineFiveLower}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOVCpNineFiveUpper}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOVMeanE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOVSeE}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOVRCrit}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOWRejections}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOWK}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOWCpNineFiveLower}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOWCpNineFiveUpper}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOWMeanE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOWSeE}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOWRCrit}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCount}{\DemoTOneRowOXRejections}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTOneRowOXK}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTOneRowOXCpNineFiveLower}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTOneRowOXCpNineFiveUpper}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanE}{\DemoTOneRowOXMeanE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorE}{\DemoTOneRowOXSeE}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCount}{\DemoTOneRowOXRCrit}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowARate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowACpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowACpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBRate}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowERate}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowECpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowECpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHRate}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowICpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowICpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKRate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMRate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNRate}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowORate}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPRate}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowUMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowUQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowUQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowURate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowUCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowUCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowVMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowVQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowVQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowVRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowVCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowVCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowWMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowWRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowWCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowXMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowXQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowXQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowXRate}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowXCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowXCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowYMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowYQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowYQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowYRate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowYCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowYCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowZMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowZRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowZCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAAMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAAQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAAQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAARate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAACpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAACpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowABMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowABQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowABQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowABRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowABCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowABCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowABMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowACMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowACQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowACQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowACRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowACCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowACCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowACMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowADMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowADQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowADQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowADRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowADCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowADCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowADMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAEMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAEQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAEQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAERate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAECpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAECpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAFMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAFRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAFCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAGMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAGQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAGQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAGRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAGCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAGCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAHMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAHQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAHQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAHRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAHCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAHCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAHMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAIMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAIQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAIQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAIRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAICpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAICpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAIMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAJMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAJQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAJQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAJRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAJCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAJCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAJMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAKMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAKQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAKQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAKRate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAKCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAKCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAKMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowALMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowALQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowALQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowALRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowALCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowALCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowALMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAMMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAMRate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAMCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowANMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowANQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowANQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowANRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowANCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowANCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowANMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAOMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAOQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAOQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAORate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAOCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAOCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAPMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAPRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAPCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAQMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAQQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAQQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAQRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAQCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAQCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowARMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowARQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowARQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowARRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowARCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowARCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowARMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowASMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowASQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowASQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowASRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowASCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowASCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowASMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowATMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowATQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowATQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowATRate}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowATCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowATCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowATMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAUMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAUQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAUQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAURate}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAUCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAUCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAVMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAVRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAVCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAWMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAWQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAWQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAWRate}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAWCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAWCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAXMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAXQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAXQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAXRate}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAXCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAXCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAYMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAYQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAYQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAYRate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAYCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAYCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAYMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowAZMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowAZQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowAZQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowAZRate}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowAZCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowAZCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowAZMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBAMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBAQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBAQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBARate}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBACpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBACpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBBMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBBQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBBQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBBRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBBCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBBCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBCMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBCQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBCQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBCRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBCCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBCCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBDMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBDQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBDQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBDRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBDCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBDCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBDMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBEMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBEQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBEQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBERate}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBECpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBECpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBEMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBFMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBFQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBFQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBFRate}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBFCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBFCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBFMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBGMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBGQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBGQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBGRate}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBGCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBGCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBGMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBHMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBHQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBHQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBHRate}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBHCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBHCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBIMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBIQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBIQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBIRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBICpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBICpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBIMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBJMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBJQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBJQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBJRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBJCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBJCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBJMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBKMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBKQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBKQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBKRate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBKCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBKCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBLMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBLQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBLQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBLRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBLCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBLCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBMMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBMQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBMQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBMRate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBMCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBMCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBNMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBNQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBNQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBNRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBNCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBNCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBOMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBOQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBOQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBORate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBOCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBOCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBOMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBPMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBPQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBPQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBPRate}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBPCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBPCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBPMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBQMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBQQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBQQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBQRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBQCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBQCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBRMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBRQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBRQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBRRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBRCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBRCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBSMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBSQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBSQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBSRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBSCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBSCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBTMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBTQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBTQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBTRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBTCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBTCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBUMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBUQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBUQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBURate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBUCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBUCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBUMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBVMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBVQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBVQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBVRate}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBVCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBVCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBVMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBWMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBWQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBWQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBWRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBWCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBWCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBXMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBXQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBXQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBXRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBXCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBXCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBYMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBYQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBYQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBYRate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBYCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBYCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowBZMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowBZQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowBZQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowBZRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowBZCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowBZCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowBZMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCAMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCAQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCAQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCARate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCACpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCACpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCAMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCBMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCBQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCBQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCBRate}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCBCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCBCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCBMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCCMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCCQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCCQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCCRate}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCCCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCCCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCCMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCDMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCDQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCDQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCDRate}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCDCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCDCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCEMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCEQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCEQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCERate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCECpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCECpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCEMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCFMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCFQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCFQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCFRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCFCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCFCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCFMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCGMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCGQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCGQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCGRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCGCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCGCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCHMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCHQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCHQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCHRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCHCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCHCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCIMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCIQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCIQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCIRate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCICpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCICpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCJMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCJQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCJQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCJRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCJCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCJCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCKMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCKQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCKQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCKRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCKCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCKCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCKMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCLMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCLQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCLQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCLRate}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCLCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCLCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCLMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCMMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCMQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCMQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCMRate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCMCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCMCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCNMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCNQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCNQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCNRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCNCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCNCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCOMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCOQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCOQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCORate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCOCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCOCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCPMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCPQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCPQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCPRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCPCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCPCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCQMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCQRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCQCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCRMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCRQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCRQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCRRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCRCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCRCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCSMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCSQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCSQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCSRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCSCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCSCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCTMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCTRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCTCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCUMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCUQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCUQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCURate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCUCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCUCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCVMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCVQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCVQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCVRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCVCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCVCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCVMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCWMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCWQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCWQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCWRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCWCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCWCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCWMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCXMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCXQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCXQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCXRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCXCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCXCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCXMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCYMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCYQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCYQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCYRate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCYCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCYCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCYMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowCZMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowCZQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowCZQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowCZRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowCZCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowCZCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowCZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDAMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDARate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDACpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDACpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDBMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDBQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDBQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDBRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDBCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDBCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDCMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDCQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDCQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDCRate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDCCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDCCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDDMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDDQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDDQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDDRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDDCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDDCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDEMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDEQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDEQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDERate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDECpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDECpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDFMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDFQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDFQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDFRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDFCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDFCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDGMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDGRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDGCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDHMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDHQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDHQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDHRate}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDHCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDHCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDIMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDIQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDIQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDIRate}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDICpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDICpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDJMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDJRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDJCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDKMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDKQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDKQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDKRate}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDKCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDKCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDLMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDLQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDLQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDLRate}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDLCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDLCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDMMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDMRate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDMCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDNMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDNQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDNQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDNRate}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDNCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDNCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDNMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDOMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDOQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDOQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDORate}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDOCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDOCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDPMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDPRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDPCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDQMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDQQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDQQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDQRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDQCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDQCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDRMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDRQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDRQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDRRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDRCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDRCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDRMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDSMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDSQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDSQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDSRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDSCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDSCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDSMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDTMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDTQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDTQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDTRate}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDTCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDTCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDTMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDUMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDUQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDUQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDURate}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDUCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDUCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDUMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDVMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDVQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDVQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDVRate}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDVCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDVCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDWMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDWRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDWCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDXMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDXQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDXQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDXRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDXCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDXCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDYMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDYQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDYQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDYRate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDYCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDYCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowDZMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowDZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowDZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowDZRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowDZCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowDZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowDZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEAMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEAQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEAQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEARate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEACpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEACpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEBMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEBQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEBQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEBRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEBCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEBCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowECMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowECQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowECQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowECRate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowECCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowECCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowECMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEDMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEDQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEDQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEDRate}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEDCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEDCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEDMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEEMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEEQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEEQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEERate}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEECpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEECpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEFMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEFRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEFCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEGMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEGQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEGQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEGRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEGCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEGCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEHMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEHQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEHQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEHRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEHCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEHCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEIMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEIQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEIQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEIRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEICpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEICpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEIMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEJMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEJQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEJQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEJRate}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEJCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEJCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEJMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEKMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEKQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEKQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEKRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEKCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEKCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowELMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowELQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowELQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowELRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowELCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowELCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowELMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEMMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEMQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEMQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEMRate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEMCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEMCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowENMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowENQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowENQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowENRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowENCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowENCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowENMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEOMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEOQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEOQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEORate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEOCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEOCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEOMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEPMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEPQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEPQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEPRate}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEPCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEPCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEPMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEQMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEQQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEQQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEQRate}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEQCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEQCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEQMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowERMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowERQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowERQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowERRate}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowERCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowERCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowERMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowESMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowESQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowESQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowESRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowESCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowESCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowESMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowETMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowETQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowETQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowETRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowETCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowETCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowETMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEUMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEUQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEUQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEURate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEUCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEUCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEVMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEVRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEVCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEWMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEWQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEWQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEWRate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEWCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEWCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEXMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEXQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEXQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEXRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEXCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEXCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEYMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEYQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEYQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEYRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEYCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEYCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEYMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowEZMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowEZQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowEZQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowEZRate}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowEZCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowEZCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowEZMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFAMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFAQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFAQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFARate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFACpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFACpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFBMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFBQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFBQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFBRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFBCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFBCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFCMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFCQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFCQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFCRate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFCCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFCCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFDMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFDQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFDQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFDRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFDCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFDCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFEMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFEQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFEQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFERate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFECpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFECpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFEMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFFMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFFQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFFQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFFRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFFCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFFCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFFMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFGMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFGQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFGQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFGRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFGCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFGCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFHMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFHQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFHQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFHRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFHCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFHCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFIMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFIQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFIQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFIRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFICpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFICpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFJMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFJQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFJQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFJRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFJCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFJCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFJMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFKMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFKQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFKQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFKRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFKCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFKCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFKMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFLMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFLQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFLQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFLRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFLCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFLCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFLMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFMMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFMQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFMQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFMRate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFMCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFMCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFMMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFNMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFNQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFNQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFNRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFNCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFNCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFOMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFOQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFOQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFORate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFOCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFOCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFOMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFPMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFPQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFPQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFPRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFPCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFPCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFPMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFQMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFQQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFQQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFQRate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFQCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFQCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFRMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFRQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFRQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFRRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFRCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFRCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFSMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFSQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFSQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFSRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFSCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFSCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFTMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFTQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFTQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFTRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFTCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFTCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFUMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFUQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFUQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFURate}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFUCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFUCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFUMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFVMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFVQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFVQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFVRate}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFVCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFVCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFVMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFWMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFWQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFWQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFWRate}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFWCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFWCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFXMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFXQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFXQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFXRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFXCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFXCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFYMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFYQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFYQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFYRate}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFYCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFYCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowFZMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowFZQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowFZQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowFZRate}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowFZCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowFZCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowFZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGAMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGARate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGACpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGACpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGBMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGBQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGBQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGBRate}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGBCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGBCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGCMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGCQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGCQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGCRate}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGCCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGCCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGDMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGDQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGDQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGDRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGDCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGDCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGEMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGEQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGEQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGERate}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGECpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGECpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGFMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGFQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGFQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGFRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGFCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGFCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGFMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGGMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGGQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGGQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGGRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGGCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGGCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGGMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGHMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGHQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGHQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGHRate}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGHCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGHCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGHMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGIMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGIQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGIQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGIRate}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGICpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGICpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGIMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGJMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGJQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGJQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGJRate}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGJCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGJCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGKMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGKQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGKQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGKRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGKCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGKCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGKMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGLMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGLQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGLQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGLRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGLCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGLCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGLMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGMMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGMQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGMQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGMRate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGMCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGMCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGNMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGNQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGNQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGNRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGNCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGNCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGOMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGOQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGOQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGORate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGOCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGOCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGPMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGPQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGPQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGPRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGPCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGPCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGQMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGQRate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGQCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGRMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGRQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGRQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGRRate}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGRCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGRCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGSMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGSQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGSQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGSRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGSCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGSCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGTMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGTRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGTCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGUMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGUQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGUQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGURate}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGUCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGUCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGVMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGVQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGVQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGVRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGVCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGVCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGWMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGWRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGWCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGXMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGXQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGXQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGXRate}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGXCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGXCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGYMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGYQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGYQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGYRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGYCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGYCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowGZMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowGZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowGZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowGZRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowGZCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowGZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowGZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHAMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHAQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHAQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHARate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHACpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHACpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHBMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHBQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHBQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHBRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHBCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHBCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHBMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHCMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHCQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHCQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHCRate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHCCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHCCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHCMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHDMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHDQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHDQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHDRate}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHDCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHDCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHDMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHEMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHEQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHEQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHERate}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHECpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHECpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHEMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHFMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHFQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHFQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHFRate}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHFCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHFCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHGMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHGRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHGCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHHMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHHQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHHQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHHRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHHCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHHCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHIMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHIQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHIQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHIRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHICpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHICpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHJMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHJRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHJCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHKMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHKQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHKQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHKRate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHKCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHKCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHLMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHLQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHLQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHLRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHLCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHLCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHMMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHMRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHMCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHNMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHNQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHNQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHNRate}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHNCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHNCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHNMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHOMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHOQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHOQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHORate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHOCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHOCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHPMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHPRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHPCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHQMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHQQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHQQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHQRate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHQCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHQCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHRMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHRQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHRQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHRRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHRCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHRCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHSMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHSQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHSQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHSRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHSCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHSCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHSMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHTMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHTQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHTQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHTRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHTCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHTCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHTMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHUMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHUQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHUQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHURate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHUCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHUCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHVMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHVRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHVCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHWMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHWQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHWQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHWRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHWCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHWCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHXMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHXQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHXQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHXRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHXCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHXCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHXMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHYMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHYQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHYQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHYRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHYCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHYCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHYMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowHZMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowHZQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowHZQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowHZRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowHZCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowHZCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowHZMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIAMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIAQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIAQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIARate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIACpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIACpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIAMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIBMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIBQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIBQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIBRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIBCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIBCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowICMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowICQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowICQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowICRate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowICCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowICCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowICMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIDMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIDQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIDQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIDRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIDCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIDCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIDMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIEMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIEQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIEQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIERate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIECpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIECpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIFMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIFRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIFCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIGMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIGQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIGQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIGRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIGCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIGCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIHMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIHQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIHQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIHRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIHCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIHCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIIMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIIQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIIQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIIRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIICpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIICpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIIMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIJMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIJQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIJQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIJRate}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIJCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIJCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIJMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIKMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIKQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIKQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIKRate}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIKCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIKCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowILMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowILQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowILQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowILRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowILCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowILCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowILMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIMMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIMQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIMQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIMRate}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIMCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIMCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowINMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowINQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowINQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowINRate}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowINCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowINCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowINMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIOMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIOQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIOQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIORate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIOCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIOCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIOMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIPMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIPQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIPQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIPRate}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIPCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIPCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIPMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIQMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIQQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIQQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIQRate}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIQCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIQCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIRMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIRQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIRQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIRRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIRCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIRCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowISMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowISQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowISQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowISRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowISCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowISCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowISMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowITMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowITQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowITQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowITRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowITCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowITCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowITMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIUMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIUQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIUQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIURate}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIUCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIUCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIUMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIVMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIVQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIVQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIVRate}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIVCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIVCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIVMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIWMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIWQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIWQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIWRate}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIWCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIWCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIWMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIXMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIXQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIXQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIXRate}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIXCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIXCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIYMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIYQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIYQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIYRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIYCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIYCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIYMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowIZMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowIZQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowIZQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowIZRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowIZCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowIZCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowIZMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJAMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJAQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJAQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJARate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJACpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJACpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJBMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJBQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJBQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJBRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJBCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJBCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJCMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJCQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJCQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJCRate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJCCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJCCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJDMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJDQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJDQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJDRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJDCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJDCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJEMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJEQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJEQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJERate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJECpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJECpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJEMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJFMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJFQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJFQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJFRate}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJFCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJFCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJFMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJGMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJGQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJGQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJGRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJGCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJGCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJHMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJHQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJHQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJHRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJHCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJHCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJIMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJIQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJIQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJIRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJICpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJICpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJJMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJJQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJJQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJJRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJJCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJJCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJKMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJKQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJKQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJKRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJKCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJKCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJKMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJLMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJLQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJLQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJLRate}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJLCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJLCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJLMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJMMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJMQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJMQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJMRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJMCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJMCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJNMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJNQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJNQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJNRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJNCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJNCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJOMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJOQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJOQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJORate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJOCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJOCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJPMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJPQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJPQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJPRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJPCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJPCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJPMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJQMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJQQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJQQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJQRate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJQCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJQCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJQMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJRMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJRQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJRQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJRRate}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJRCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJRCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJRMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJSMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJSQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJSQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJSRate}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJSCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJSCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJSMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJTMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJTQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJTQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJTRate}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJTCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJTCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJUMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJUQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJUQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJURate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJUCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJUCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJUMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJVMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJVQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJVQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJVRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJVCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJVCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJVMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJWMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJWQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJWQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJWRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJWCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJWCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJXMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJXQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJXQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJXRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJXCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJXCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJYMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJYQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJYQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJYRate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJYCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJYCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowJZMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowJZQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowJZQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowJZRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowJZCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowJZCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowJZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKAMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKARate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKACpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKACpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKBMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKBQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKBQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKBRate}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKBCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKBCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKCMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKCQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKCQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKCRate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKCCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKCCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKDMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKDQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKDQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKDRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKDCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKDCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKEMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKEQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKEQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKERate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKECpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKECpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKFMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKFQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKFQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKFRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKFCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKFCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKGMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKGRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKGCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKHMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKHQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKHQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKHRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKHCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKHCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKIMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKIQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKIQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKIRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKICpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKICpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKJMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKJRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKJCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKKMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKKQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKKQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKKRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKKCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKKCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKLMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKLQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKLQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKLRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKLCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKLCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKLMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKMMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKMQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKMQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKMRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKMCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKMCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKMMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKNMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKNQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKNQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKNRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKNCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKNCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKNMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKOMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKOQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKOQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKORate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKOCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKOCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKOMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKPMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKPQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKPQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKPRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKPCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKPCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKQMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKQRate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKQCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKRMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKRQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKRQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKRRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKRCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKRCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKSMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKSQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKSQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKSRate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKSCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKSCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKTMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKTRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKTCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKUMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKUQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKUQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKURate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKUCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKUCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKVMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKVQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKVQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKVRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKVCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKVCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKWMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKWRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKWCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKXMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKXQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKXQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKXRate}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKXCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKXCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKYMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKYQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKYQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKYRate}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKYCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKYCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowKZMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowKZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowKZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowKZRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowKZCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowKZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowKZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLAMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLAQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLAQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLARate}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLACpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLACpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLBMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLBQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLBQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLBRate}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLBCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLBCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLCMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLCQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLCQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLCRate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLCCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLCCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLCMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLDMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLDQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLDQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLDRate}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLDCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLDCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLDMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLEMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLEQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLEQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLERate}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLECpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLECpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLFMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLFRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLFCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLGMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLGQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLGQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLGRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLGCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLGCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLHMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLHQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLHQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLHRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLHCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLHCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLHMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLIMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLIQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLIQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLIRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLICpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLICpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLIMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLJMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLJQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLJQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLJRate}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLJCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLJCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLJMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLKMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLKQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLKQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLKRate}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLKCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLKCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLKMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLLMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLLQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLLQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLLRate}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLLCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLLCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLMMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLMRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLMCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLNMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLNQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLNQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLNRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLNCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLNCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLNMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLOMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLOQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLOQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLORate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLOCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLOCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLPMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLPRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLPCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLQMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLQQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLQQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLQRate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLQCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLQCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLRMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLRQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLRQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLRRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLRCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLRCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLSMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLSQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLSQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLSRate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLSCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLSCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLSMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLTMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLTQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLTQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLTRate}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLTCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLTCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLTMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLUMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLUQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLUQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLURate}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLUCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLUCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLVMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLVRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLVCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLWMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLWQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLWQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLWRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLWCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLWCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLXMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLXQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLXQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLXRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLXCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLXCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLYMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLYQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLYQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLYRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLYCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLYCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLYMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowLZMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowLZQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowLZQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowLZRate}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowLZCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowLZCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowLZMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMAMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMAQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMAQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMARate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMACpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMACpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMBMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMBQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMBQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMBRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMBCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMBCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMCMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMCQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMCQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMCRate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMCCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMCCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMDMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMDQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMDQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMDRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMDCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMDCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMDMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMEMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMEQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMEQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMERate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMECpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMECpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMEMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMFMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMFQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMFQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMFRate}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMFCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMFCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMFMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMGMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMGQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMGQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMGRate}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMGCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMGCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMGMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMHMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMHQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMHQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMHRate}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMHCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMHCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMIMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMIQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMIQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMIRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMICpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMICpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMIMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMJMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMJQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMJQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMJRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMJCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMJCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMJMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMKMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMKQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMKQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMKRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMKCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMKCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMLMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMLQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMLQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMLRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMLCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMLCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMMMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMMQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMMQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMMRate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMMCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMMCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMNMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMNQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMNQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMNRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMNCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMNCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMOMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMOQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMOQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMORate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMOCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMOCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMOMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMPMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMPQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMPQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMPRate}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMPCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMPCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMPMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMQMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMQQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMQQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMQRate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMQCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMQCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMRMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMRQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMRQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMRRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMRCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMRCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMSMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMSQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMSQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMSRate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMSCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMSCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMTMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMTQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMTQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMTRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMTCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMTCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMUMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMUQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMUQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMURate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMUCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMUCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMUMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMVMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMVQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMVQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMVRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMVCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMVCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMVMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMWMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMWQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMWQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMWRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMWCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMWCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMXMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMXQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMXQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMXRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMXCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMXCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMYMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMYQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMYQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMYRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMYCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMYCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowMZMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowMZQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowMZQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowMZRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowMZCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowMZCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowMZMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNAMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNAQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNAQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNARate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNACpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNACpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNAMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNBMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNBQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNBQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNBRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNBCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNBCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNBMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNCMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNCQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNCQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNCRate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNCCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNCCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNCMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNDMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNDQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNDQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNDRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNDCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNDCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNEMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNEQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNEQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNERate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNECpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNECpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNEMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNFMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNFQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNFQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNFRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNFCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNFCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNFMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNGMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNGQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNGQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNGRate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNGCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNGCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNHMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNHQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNHQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNHRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNHCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNHCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNIMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNIQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNIQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNIRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNICpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNICpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNJMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNJQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNJQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNJRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNJCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNJCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNKMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNKQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNKQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNKRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNKCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNKCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNKMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNLMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNLQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNLQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNLRate}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNLCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNLCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNLMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNMMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNMQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNMQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNMRate}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNMCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNMCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNNMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNNQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNNQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNNRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNNCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNNCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNOMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNOQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNOQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNORate}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNOCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNOCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNPMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNPQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNPQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNPRate}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNPCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNPCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNQMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNQRate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNQCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNRMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNRQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNRQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNRRate}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNRCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNRCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNSMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNSQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNSQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNSRate}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNSCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNSCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNTMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNTRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNTCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNUMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNUQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNUQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNURate}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNUCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNUCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNVMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNVQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNVQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNVRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNVCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNVCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNVMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNWMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNWQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNWQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNWRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNWCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNWCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNWMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNXMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNXQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNXQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNXRate}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNXCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNXCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNXMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNYMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNYQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNYQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNYRate}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNYCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNYCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNYMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowNZMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowNZQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowNZQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowNZRate}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowNZCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowNZCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowNZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOAMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOARate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOACpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOACpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOBMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOBQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOBQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOBRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOBCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOBCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOCMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOCQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOCQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOCRate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOCCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOCCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowODMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowODQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowODQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowODRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowODCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowODCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowODMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOEMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOEQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOEQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOERate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOECpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOECpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOFMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOFQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOFQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOFRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOFCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOFCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOGMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOGRate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOGCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOHMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOHQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOHQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOHRate}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOHCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOHCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOIMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOIQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOIQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOIRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOICpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOICpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOJMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOJRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOJCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOKMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOKQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOKQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOKRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOKCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOKCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOLMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOLQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOLQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOLRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOLCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOLCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOMMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOMRate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOMCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowONMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowONQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowONQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowONRate}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowONCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowONCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowONMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOOMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOOQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOOQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOORate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOOCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOOCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOPMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOPRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOPCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOQMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOQQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOQQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOQRate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOQCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOQCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowORMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowORQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowORQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowORRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowORCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowORCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowORMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOSMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOSQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOSQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOSRate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOSCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOSCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOSMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOTMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOTQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOTQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOTRate}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOTCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOTCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOTMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOUMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOUQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOUQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOURate}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOUCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOUCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOUMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOVMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOVQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOVQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOVRate}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOVCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOVCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOWMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOWRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOWCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOXMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOXQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOXQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOXRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOXCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOXCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOYMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOYQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOYQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOYRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOYCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOYCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowOZMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowOZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowOZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowOZRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowOZCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowOZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowOZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPAMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPAQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPAQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPARate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPACpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPACpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPBMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPBQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPBQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPBRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPBCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPBCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPCMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPCQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPCQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPCRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPCCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPCCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPCMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPDMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPDQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPDQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPDRate}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPDCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPDCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPDMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPEMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPEQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPEQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPERate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPECpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPECpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPFMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPFRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPFCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPGMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPGQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPGQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPGRate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPGCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPGCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPHMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPHQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPHQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPHRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPHCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPHCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPIMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPIQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPIQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPIRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPICpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPICpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPIMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPJMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPJQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPJQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPJRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPJCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPJCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPJMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPKMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPKQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPKQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPKRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPKCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPKCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPLMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPLQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPLQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPLRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPLCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPLCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPMMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPMQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPMQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPMRate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPMCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPMCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPNMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPNQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPNQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPNRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPNCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPNCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPNMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPOMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPOQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPOQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPORate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPOCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPOCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPOMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPPMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPPQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPPQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPPRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPPCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPPCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPPMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPQMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPQQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPQQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPQRate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPQCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPQCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPQMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPRMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPRQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPRQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPRRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPRCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPRCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPSMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPSQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPSQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPSRate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPSCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPSCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPSMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPTMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPTQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPTQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPTRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPTCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPTCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPTMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPUMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPUQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPUQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPURate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPUCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPUCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPVMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPVRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPVCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPWMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPWQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPWQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPWRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPWCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPWCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPXMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPXQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPXQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPXRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPXCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPXCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPYMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPYQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPYQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPYRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPYCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPYCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPYMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowPZMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowPZQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowPZQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowPZRate}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowPZCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowPZCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowPZMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQAMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQAQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQAQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQARate}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQACpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQACpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQBMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQBQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQBQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQBRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQBCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQBCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQCMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQCQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQCQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQCRate}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQCCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQCCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQDMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQDQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQDQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQDRate}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQDCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQDCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQEMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQEQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQEQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQERate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQECpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQECpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQEMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQFMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQFQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQFQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQFRate}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQFCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQFCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQFMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQGMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQGQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQGQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQGRate}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQGCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQGCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQHMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQHQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQHQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQHRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQHCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQHCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQHMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQIMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQIQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQIQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQIRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQICpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQICpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQJMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQJQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQJQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQJRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQJCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQJCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQJMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQKMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQKQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQKQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQKRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQKCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQKCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQKMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQLMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQLQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQLQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQLRate}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQLCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQLCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQLMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQMMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQMQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQMQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQMRate}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQMCpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQMCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQMMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQNMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQNQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQNQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQNRate}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQNCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQNCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQOMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQOQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQOQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQORate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQOCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQOCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQOMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQPMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQPQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQPQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQPRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQPCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQPCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQPMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQQMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQQQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQQQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQQRate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQQCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQQCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQRMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQRQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQRQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQRRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQRCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQRCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQSMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQSQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQSQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQSRate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQSCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQSCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQTMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQTQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQTQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQTRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQTCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQTCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQUMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQUQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQUQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQURate}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQUCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQUCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQUMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQVMedianLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQVQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQVQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQVRate}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQVCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQVCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQVMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQWMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQWQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQWQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQWRate}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQWCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQWCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQXMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQXQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQXQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQXRate}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQXCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQXCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQXMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQYMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQYQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQYQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQYRate}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQYCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQYCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowQZMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowQZQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowQZQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowQZRate}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowQZCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowQZCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowQZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRAMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRAQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRAQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRARate}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRACpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRACpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRAMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRBMedianLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRBQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRBQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRBRate}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRBCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRBCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRBMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRCMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRCQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRCQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRCRate}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRCCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRCCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRCMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRDMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRDQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRDQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRDRate}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRDCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRDCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRDMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowREMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowREQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowREQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRERate}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRECpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRECpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowREMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRFMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRFQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRFQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRFRate}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRFCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRFCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRFMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRGMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRGQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRGQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRGRate}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRGCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRGCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRGMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRHMedianLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRHQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRHQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRHRate}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRHCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRHCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRHMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRIMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRIQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRIQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRIRate}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRICpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRICpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRIMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRJMedianLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRJQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRJQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRJRate}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRJCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRJCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRKMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRKQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRKQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRKRate}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRKCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRKCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRKMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRLMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRLQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRLQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRLRate}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRLCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRLCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRLMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRMMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRMQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRMQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRMRate}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRMCpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRMCpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRMMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRNMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRNQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRNQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRNRate}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRNCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRNCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRNMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowROMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowROQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowROQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRORate}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowROCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowROCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowROMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRPMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRPQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRPQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRPRate}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRPCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRPCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRQMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRQQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRQQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRQRate}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRQCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRQCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRQMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRRMedianLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRRQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRRQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRRRate}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRRCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRRCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRRMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRSMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRSQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRSQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRSRate}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRSCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRSCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRSMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRTMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRTQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRTQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRTRate}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRTCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRTCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRTMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRUMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRUQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRUQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRURate}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRUCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRUCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRVMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRVQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRVQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRVRate}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRVCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRVCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRWMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRWQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRWQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRWRate}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRWCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRWCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRWMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRXMedianLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRXQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRXQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRXRate}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRXCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRXCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRXMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRYMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRYQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRYQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRYRate}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRYCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRYCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRYMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowRZMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowRZQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowRZQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowRZRate}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowRZCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowRZCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowRZMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSAMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSAQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSAQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSARate}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSACpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSACpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSAMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSBMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSBQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSBQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSBRate}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSBCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSBCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSBMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSCMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSCQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSCQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSCRate}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSCCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSCCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSCMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSDMedianLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSDQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSDQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSDRate}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSDCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSDCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSDMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSEMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSEQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSEQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSERate}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSECpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSECpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSEMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSFMedianLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSFQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSFQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSFRate}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSFCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSFCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSGMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSGQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSGQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSGRate}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSGCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSGCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSGMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSHMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSHQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSHQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSHRate}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSHCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSHCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSHMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSIMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSIQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSIQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSIRate}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSICpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSICpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSIMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSJMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSJQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSJQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSJRate}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSJCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSJCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSJMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSKMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSKQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSKQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSKRate}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSKCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSKCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSKMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSLMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSLQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSLQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSLRate}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSLCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSLCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSLMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSMMedianLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSMQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSMQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSMRate}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSMCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSMCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSMMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSNMedianLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSNQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSNQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSNRate}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSNCpNineFiveLower}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSNCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSNMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSOMedianLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSOQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSOQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSORate}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSOCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSOCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSOMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSPMedianLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSPQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSPQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSPRate}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSPCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSPCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSPMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSQMedianLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSQQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSQQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSQRate}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSQCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSQCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSQMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSRMedianLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSRQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSRQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSRRate}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSRCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSRCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSRMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSSMedianLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSSQTwoFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSSQSevenFiveLogE}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSSRate}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSSCpNineFiveLower}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSSCpNineFiveUpper}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSSMedianLogRatioToExactBound}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSTMedianLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSTQTwoFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSTQSevenFiveLogE}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSTRate}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSTCpNineFiveLower}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSTCpNineFiveUpper}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSTMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSUMedianLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSUQTwoFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSUQSevenFiveLogE}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSURate}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSUCpNineFiveLower}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSUCpNineFiveUpper}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSUMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSVMedianLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSVQTwoFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSVQSevenFiveLogE}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSVRate}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSVCpNineFiveLower}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSVCpNineFiveUpper}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSVMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSWMedianLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSWQTwoFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSWQSevenFiveLogE}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSWRate}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSWCpNineFiveLower}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSWCpNineFiveUpper}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSWMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSXMedianLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSXQTwoFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSXQSevenFiveLogE}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSXRate}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSXCpNineFiveLower}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSXCpNineFiveUpper}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSXMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSYMedianLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSYQTwoFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSYQSevenFiveLogE}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSYRate}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSYCpNineFiveLower}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSYCpNineFiveUpper}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSYMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowSZMedianLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowSZQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowSZQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowSZRate}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowSZCpNineFiveLower}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowSZCpNineFiveUpper}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowSZMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTAMedianLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTAQTwoFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTAQSevenFiveLogE}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTARate}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTACpNineFiveLower}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTACpNineFiveUpper}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTAMedianLogRatioToExactBound}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTBMedianLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTBQTwoFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTBQSevenFiveLogE}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTBRate}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTBCpNineFiveLower}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTBCpNineFiveUpper}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTBMedianLogRatioToExactBound}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTCMedianLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTCQTwoFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTCQSevenFiveLogE}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTCRate}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTCCpNineFiveLower}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTCCpNineFiveUpper}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTCMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTDMedianLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTDQTwoFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTDQSevenFiveLogE}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTDRate}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTDCpNineFiveLower}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTDCpNineFiveUpper}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTDMedianLogRatioToExactBound}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTEMedianLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTEQTwoFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTEQSevenFiveLogE}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTERate}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTECpNineFiveLower}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTECpNineFiveUpper}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTEMedianLogRatioToExactBound}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTFMedianLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTFQTwoFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTFQSevenFiveLogE}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTFRate}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTFCpNineFiveLower}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTFCpNineFiveUpper}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTFMedianLogRatioToExactBound}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTGMedianLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTGQTwoFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTGQSevenFiveLogE}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTGRate}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTGCpNineFiveLower}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTGCpNineFiveUpper}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTGMedianLogRatioToExactBound}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogE}{\DemoTTwoRowTHMedianLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLower}{\DemoTTwoRowTHQTwoFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpper}{\DemoTTwoRowTHQSevenFiveLogE}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRate}{\DemoTTwoRowTHRate}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILower}{\DemoTTwoRowTHCpNineFiveLower}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpper}{\DemoTTwoRowTHCpNineFiveUpper}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBound}{\DemoTTwoRowTHMedianLogRatioToExactBound}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowAEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowAK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowARate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowACpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowACpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowBEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowBK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowBRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowBCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowBCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowCEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowCK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowCRate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowCCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowCCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowDEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowDK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowDRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowDCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowDCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowEEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowEK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowERate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowECpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowECpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowFEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowFK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowFRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowFCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowFCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowGEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowGK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowGRate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowGCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowGCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowHEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowHK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowHRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowHCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowHCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowIEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowIK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowIRate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowICpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowICpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowJEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowJK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowJRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowJCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowJCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowKEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowKK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowKRate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowKCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowKCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowLEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowLK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowLRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowLCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowLCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowMEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowMK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowMRate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowMCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowMCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowNEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowNK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowNRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowNCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowNCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowOEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowOK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowORate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowOCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowOCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowPEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowPK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowPRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowPCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowPCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowQEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowQK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowQRate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowQCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowQCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowREffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowRK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowRRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowRCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowRCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowSEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowSK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowSRate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowSCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowSCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowTEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowTK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowTRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowTCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowTCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowUEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowUK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowURate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowUCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowUCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowVEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowVK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowVRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowVCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowVCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowWEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowWK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowWRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowWCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowWCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCount}{\DemoTThreeRowXEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCount}{\DemoTThreeRowXK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRate}{\DemoTThreeRowXRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILower}{\DemoTThreeRowXCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowXCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowYEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowYK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowYRate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowYCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowYCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowZEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowZK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowZRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowZCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowZCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowAAEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowAAK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowAARate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowAACpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAACpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowABEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowABK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowABRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowABCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowABCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowACEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowACK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowACRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowACCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowACCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCount}{\DemoTThreeRowADEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCount}{\DemoTThreeRowADK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRate}{\DemoTThreeRowADRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILower}{\DemoTThreeRowADCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowADCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAEEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAEK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAERate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAECpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAECpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAFEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAFK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAFRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAFCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAFCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAGEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAGK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAGRate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAGCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAGCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAHEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAHK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAHRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAHCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAHCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAIEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAIK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAIRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAICpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAICpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCount}{\DemoTThreeRowAJEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCount}{\DemoTThreeRowAJK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRate}{\DemoTThreeRowAJRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILower}{\DemoTThreeRowAJCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpper}{\DemoTThreeRowAJCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAKEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAKK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAKRate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAKCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAKCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowALEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowALK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowALRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowALCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowALCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAMEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAMK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAMRate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAMCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAMCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowANEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowANK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowANRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowANCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowANCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAOEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAOK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAORate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAOCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAOCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAPEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAPK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAPRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAPCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAPCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAQEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAQK}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAQRate}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAQCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAQCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAREffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowARK}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowARRate}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowARCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowARCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowASEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowASK}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowASRate}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowASCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowASCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowATEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowATK}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowATRate}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowATCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowATCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAUEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAUK}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAURate}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAUCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAUCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAVEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAVK}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAVRate}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAVCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAVCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAWEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAWK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAWRate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAWCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAWCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAXEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAXK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAXRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAXCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAXCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAYEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAYK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAYRate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAYCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAYCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowAZEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowAZK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowAZRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowAZCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowAZCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBAEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBAK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBARate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBACpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBACpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBBEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBBK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBBRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBBCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBBCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBCEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBCK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBCRate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBCCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBCCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBDEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBDK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBDRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBDCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBDCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBEEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBEK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBERate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBECpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBECpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBFEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBFK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBFRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBFCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBFCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBGEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBGK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBGRate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBGCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBGCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBHEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBHK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBHRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBHCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBHCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBIEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBIK}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBIRate}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBICpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBICpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBJEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBJK}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBJRate}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBJCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBJCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBKEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBKK}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBKRate}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBKCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBKCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBLEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBLK}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBLRate}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBLCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBLCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBMEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBMK}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBMRate}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBMCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBMCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBNEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBNK}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBNRate}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBNCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBNCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBOEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBOK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBORate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBOCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBOCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBPEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBPK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBPRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBPCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBPCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBQEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBQK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBQRate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBQCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBQCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBREffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBRK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBRRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBRCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBRCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBSEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBSK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBSRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBSCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBSCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBTEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBTK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBTRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBTCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBTCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBUEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBUK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBURate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBUCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBUCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBVEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBVK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBVRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBVCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBVCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBWEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBWK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBWRate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBWCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBWCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBXEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBXK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBXRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBXCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBXCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBYEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBYK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBYRate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBYCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBYCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowBZEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowBZK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowBZRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowBZCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowBZCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCAEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCAK}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCARate}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCACpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCACpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCBEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCBK}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCBRate}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCBCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCBCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCCEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCCK}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCCRate}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCCCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCCCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCDEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCDK}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCDRate}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCDCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCDCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCEEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCEK}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCERate}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCECpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCECpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCFEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCFK}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCFRate}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCFCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCFCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCGEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCGK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCGRate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCGCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCGCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCHEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCHK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCHRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCHCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCHCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCIEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCIK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCIRate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCICpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCICpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCJEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCJK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCJRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCJCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCJCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCKEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCKK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCKRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCKCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCKCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCLEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCLK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCLRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCLCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCLCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCMEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCMK}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCMRate}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCMCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCMCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCNEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCNK}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCNRate}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCNCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCNCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCOEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCOK}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCORate}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCOCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCOCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCPEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCPK}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCPRate}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCPCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCPCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCQEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCQK}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCQRate}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCQCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCQCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCREffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCRK}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCRRate}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCRCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCRCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCSEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCSK}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCSRate}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCSCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCSCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCTEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCTK}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCTRate}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCTCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCTCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCUEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCUK}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCURate}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCUCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCUCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCVEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCVK}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCVRate}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCVCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCVCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCWEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCWK}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCWRate}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCWCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCWCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCXEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCXK}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCXRate}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCXCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCXCpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCYEffectReports}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCYK}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCYRate}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCYCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCYCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowCZEffectReports}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowCZK}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowCZRate}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowCZCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowCZCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowDAEffectReports}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowDAK}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowDARate}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowDACpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowDACpNineFiveUpper}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowDBEffectReports}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowDBK}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowDBRate}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowDBCpNineFiveLower}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowDBCpNineFiveUpper}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowDCEffectReports}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowDCK}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowDCRate}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowDCCpNineFiveLower}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowDCCpNineFiveUpper}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCount}{\DemoTThreeRowDDEffectReports}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCount}{\DemoTThreeRowDDK}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRate}{\DemoTThreeRowDDRate}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILower}{\DemoTThreeRowDDCpNineFiveLower}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpper}{\DemoTThreeRowDDCpNineFiveUpper}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowARhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowALambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowALambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowADeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowADeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowBRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowBLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowBLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowBDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowBDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowCRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowCLambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowCLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowCDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowCDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowDRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowDLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowDLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowDDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowDDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowERhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowELambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowELambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowEDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowEDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowFRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowFLambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowFLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowFDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowFDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowGRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowGLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowGLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowGDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowGDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowHRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowHLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowHLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowHDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowHDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowIRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowILambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowILambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowIDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowIDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowJRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowJLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowJLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowJDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowJDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowKRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowKLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowKLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowKDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowKDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHat}{\DemoTFourRowLRhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambda}{\DemoTFourRowLLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaC}{\DemoTFourRowLLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKish}{\DemoTFourRowLDeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrast}{\DemoTFourRowLDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowMRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowMLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowMLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowMDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowMDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowNRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowNLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowNLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowNDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowNDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHat}{\DemoTFourRowORhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambda}{\DemoTFourRowOLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaC}{\DemoTFourRowOLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKish}{\DemoTFourRowODeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrast}{\DemoTFourRowODeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowPRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowPLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowPLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowPDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowPDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowQRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowQLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowQLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowQDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowQDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHat}{\DemoTFourRowRRhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambda}{\DemoTFourRowRLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaC}{\DemoTFourRowRLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKish}{\DemoTFourRowRDeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrast}{\DemoTFourRowRDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowSRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowSLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowSLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowSDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowSDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowTRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowTLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowTLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowTDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowTDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowURhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowULambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowULambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowUDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowUDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowVRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowVLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowVLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowVDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowVDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowWRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowWLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowWLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowWDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowWDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowXRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowXLambda}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowXLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowXDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowXDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowYRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowYLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowYLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowYDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowYDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowZRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowZLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowZLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowZDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowZDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAARhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAALambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAALambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAADeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAADeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowABRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowABLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowABLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowABDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowABDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowACRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowACLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowACLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowACDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowACDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowADRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowADLambda}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowADLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowADDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowADDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAERhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAELambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAELambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAEDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAEDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAFRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAFLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAFLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAFDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAFDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAGRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAGLambda}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAGLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAGDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAGDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAHRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAHLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAHLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAHDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAHDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAIRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAILambda}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAILambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAIDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAIDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAJRhoHat}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAJLambda}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAJLambdaC}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAJDeffKish}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAJDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAKRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAKLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAKLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAKDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAKDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowALRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowALLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowALLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowALDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowALDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAMRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAMLambda}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAMLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAMDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAMDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowANRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowANLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowANLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowANDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowANDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAORhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAOLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAOLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAODeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAODeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAPRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAPLambda}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAPLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAPDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAPDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAQRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowAQLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAQLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAQDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAQDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowARRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowARLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowARLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowARDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowARDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowASRhoHat}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowASLambda}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowASLambdaC}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowASDeffKish}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowASDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowATRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowATLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowATLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowATDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowATDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAURhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAULambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAULambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAUDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAUDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAVRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAVLambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAVLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAVDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAVDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAWRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAWLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAWLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAWDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAWDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAXRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAXLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAXLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAXDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAXDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAYRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAYLambda}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAYLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAYDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAYDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowAZRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowAZLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowAZLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowAZDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowAZDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBARhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBALambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBALambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBADeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBADeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBBRhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBBLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBBLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBBDeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBBDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBCRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBCLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBCLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBCDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBCDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBDRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBDLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBDLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBDDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBDDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBERhoHat}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBELambda}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBELambdaC}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBEDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBEDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBFRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBFLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBFLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBFDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBFDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBGRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBGLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBGLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBGDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBGDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBHRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBHLambda}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBHLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBHDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBHDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBIRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBILambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBILambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBIDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBIDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBJRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBJLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBJLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBJDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBJDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBKRhoHat}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBKLambda}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBKLambdaC}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBKDeffKish}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBKDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBLRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBLLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBLLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBLDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBLDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBMRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBMLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBMLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBMDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBMDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBNRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBNLambda}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBNLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBNDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBNDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBORhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBOLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBOLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBODeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBODeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBPRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBPLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBPLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBPDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBPDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBQRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBQLambda}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBQLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBQDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBQDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBRRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBRLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBRLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBRDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBRDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBSRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBSLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBSLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBSDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBSDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBTRhoHat}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowBTLambda}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBTLambdaC}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBTDeffKish}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBTDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBURhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBULambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBULambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBUDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBUDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBVRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBVLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBVLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBVDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBVDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBWRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBWLambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBWLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBWDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBWDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBXRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBXLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBXLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBXDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBXDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBYRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBYLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBYLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBYDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBYDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowBZRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowBZLambda}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowBZLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowBZDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowBZDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCARhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCALambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCALambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCADeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCADeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCBRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCBLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCBLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCBDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCBDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCCRhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCCLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCCLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCCDeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCCDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCDRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCDLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCDLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCDDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCDDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCERhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCELambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCELambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCEDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCEDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCFRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCFLambda}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCFLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCFDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCFDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCGRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCGLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCGLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCGDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCGDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCHRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCHLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCHLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCHDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCHDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCIRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCILambda}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCILambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCIDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCIDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCJRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCJLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCJLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCJDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCJDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCKRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCKLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCKLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCKDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCKDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCLRhoHat}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCLLambda}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCLLambdaC}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCLDeffKish}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCLDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCMRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCMLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCMLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCMDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCMDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCNRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCNLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCNLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCNDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCNDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCORhoHat}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCOLambda}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCOLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCODeffKish}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCODeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCPRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCPLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCPLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCPDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCPDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCQRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCQLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCQLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCQDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCQDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCRRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCRLambda}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCRLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCRDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCRDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCSRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCSLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCSLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCSDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCSDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCTRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCTLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCTLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCTDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCTDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCURhoHat}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambda}{\DemoTFourRowCULambda}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCULambdaC}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCUDeffKish}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCUDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCVRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowCVLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCVLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCVDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCVDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCWRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowCWLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCWLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCWDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCWDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCXRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowCXLambda}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCXLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCXDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCXDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCYRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowCYLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCYLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCYDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCYDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowCZRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowCZLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowCZLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowCZDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowCZDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDARhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDALambda}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDALambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDADeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDADeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDBRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDBLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDBLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDBDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDBDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDCRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDCLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDCLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDCDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDCDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDDRhoHat}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDDLambda}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDDLambdaC}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDDDeffKish}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDDDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDERhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDELambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDELambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDEDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDEDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDFRhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDFLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDFLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDFDeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDFDeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDGRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDGLambda}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDGLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDGDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDGDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDHRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDHLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDHLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDHDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDHDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDIRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDILambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDILambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDIDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDIDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDJRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDJLambda}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDJLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDJDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDJDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDKRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDKLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDKLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDKDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDKDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDLRhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDLLambda}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDLLambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDLDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDLDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDMRhoHat}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDMLambda}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDMLambdaC}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDMDeffKish}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDMDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDNRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDNLambda}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDNLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDNDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDNDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDORhoHat}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDOLambda}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDOLambdaC}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDODeffKish}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDODeffContrast}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDPRhoHat}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDPLambda}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDPLambdaC}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDPDeffKish}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDPDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDQRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDQLambda}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDQLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDQDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDQDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDRRhoHat}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDRLambda}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDRLambdaC}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDRDeffKish}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDRDeffContrast}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDSRhoHat}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDSLambda}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDSLambdaC}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDSDeffKish}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDSDeffContrast}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDTRhoHat}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDTLambda}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDTLambdaC}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDTDeffKish}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDTDeffContrast}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDURhoHat}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDULambda}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDULambdaC}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDUDeffKish}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDUDeffContrast}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHat}{\DemoTFourRowDVRhoHat}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambda}{\DemoTFourRowDVLambda}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaC}{\DemoTFourRowDVLambdaC}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKish}{\DemoTFourRowDVDeffKish}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrast}{\DemoTFourRowDVDeffContrast}


==> macros/demo_display.tex <==
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{2.799911127e-59}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{2.619746661e-59}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{2.799911127e-59}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{2.619746661e-59}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.6730612027}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.3568285769}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.00169231}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.02035531033}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.979965536}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.01238077017}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.0001120837709}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{9.213933887e-05}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.871127774e-45}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{1.47066863e-45}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{4.219408926e-91}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{4.219408926e-91}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{4.219408926e-91}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{4.219408926e-91}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.2221858117}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.1043061338}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{2}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0.38\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{10.8\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.755666539}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.6623309218}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.9647322824}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.01753816038}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{2.81710164e-05}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{2.186199689e-05}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{3.943057553e-72}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{3.943057483e-72}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.399955563e-59}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{1.309873331e-59}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.399955563e-59}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{1.309873331e-59}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.4476235072}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.2134246208}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.378679424}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.3301133388}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.9723489092}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.01406256308}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{7.012739367e-05}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{4.787391541e-05}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{9.355638871e-46}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{7.353343151e-46}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.472376441e-49}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{5.427216956e-49}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.472376441e-49}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{5.427216956e-49}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.6792882992}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.2758712704}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9808483748}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01751174875}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9724186691}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01228885969}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.01095009305}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01065011902}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.292333384e-29}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.292333384e-29}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.08735949e-89}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{5.062976655e-89}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.08735949e-89}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{5.062976655e-89}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.471661001}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.2259470242}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.5171017849}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.1363679798}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9579788112}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01748989046}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.0006606717149}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.000513363955}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.269763085e-62}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{5.269761922e-62}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{2.73618822e-49}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{2.713608478e-49}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{2.73618822e-49}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{2.713608478e-49}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.5754746501}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.2042964372}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.7489750798}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.07060756549}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9651987402}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01392690584}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.005805382382}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.005327832749}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{6.461666921e-30}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{6.46166692e-30}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{9.969884227e-45}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{9.969883451e-45}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{9.969884227e-45}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{9.969883451e-45}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.5899240712}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1682636567}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.999660132}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.007823833992}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.994394307}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01110882135}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.003690914692}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.002957964428}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{2.748758244e-26}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{2.738071344e-26}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.850418753e-73}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.850418753e-73}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.850418753e-73}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.850418753e-73}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.256028912}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.08686531627}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9853313921}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1343507552}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9940622107}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01321777031}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{6.696189717e-05}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.992084343e-05}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.807993617e-53}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.807993617e-53}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{4.984942113e-45}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{4.984941725e-45}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{4.984942113e-45}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{4.984941725e-45}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.4229764916}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1013003478}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9924957621}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.06780299901}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9942282588}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01124824321}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.001878938294}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.001479650597}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1.374379122e-26}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{1.369035672e-26}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{7.721530739e-51}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{7.721530426e-51}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{7.721530739e-51}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{7.721530426e-51}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{1}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0.040\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{8.4\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.7936396953}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.4090665239}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.9175642852}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.06383034864}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.012281563}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.01398115732}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.0004989213191}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.00027308817}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.680432056e-41}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{1.6804182e-41}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{6.533063862e-106}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{6.533063861e-106}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{6.533063862e-106}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{6.533063861e-106}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.8002308491}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.3896306844}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.3270825859}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.1957775377}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.021780618}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.02141533272}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{6.059172701e-05}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{3.576959505e-05}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{6.461962178e-76}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{6.461962178e-76}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{3.86076537e-51}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{3.860765213e-51}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{3.86076537e-51}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{3.860765213e-51}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.7969352722}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.2937561857}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.6223234355}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.1017828638}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{1.017031091}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.01631420986}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{0.000279756523}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{0.0001369155259}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoMeanEDisp}{8.402160281e-42}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoStandardErrorEDisp}{8.402090998e-42}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{2.031050368e-50}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.721596715e-50}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{2.031050368e-50}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.721596715e-50}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.4938654236}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.1177086279}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.013890567}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.03075393966}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9972453603}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01210135697}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.0004100002866}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.0002876534346}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{3.157341213e-37}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{3.085380668e-37}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.037041439e-81}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.026402709e-81}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.037041439e-81}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.026402709e-81}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.3333344245}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.1093898557}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.7863913874}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.2549090855}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.009571623}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01643633026}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.0002360295788}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.0001790208713}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{5.120706514e-63}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{4.879926123e-63}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.015525184e-50}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{8.607983573e-51}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.015525184e-50}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{8.607983573e-51}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.4135999241}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.1021943159}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.9001409774}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.1278913341}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.003408492}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.01355387644}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{0.0003230149327}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{0.0001682074321}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoMeanEDisp}{1.578670606e-37}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoStandardErrorEDisp}{1.542690334e-37}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1.633899222e-36}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{1.633899222e-36}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1.633899222e-36}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{1.633899222e-36}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.7532806854}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.2808532745}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9931429068}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01565554996}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.998788987}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01199574616}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.0005258724425}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.000328790883}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1.060904941e-23}
\newcommand{\PxTOneNcWrongMarginalConePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{1.060904941e-23}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.50011211e-79}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.499986503e-79}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.50011211e-79}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.499986503e-79}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.2972984692}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1081888871}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.5667956403}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1113903063}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9960266016}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.0147979042}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.0001811364422}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.0001064293238}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{3.987199255e-63}
\newcommand{\PxTOneNcWrongMarginalConePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{3.922212436e-63}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{8.169496109e-37}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{8.169496109e-37}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{8.169496109e-37}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{8.169496109e-37}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.5252895773}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.1874551084}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.7799692735}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.05863697082}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.9974077943}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.01245985943}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{0.0003535044423}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{0.0001754552561}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoCriticalRejectCountDisp}{11}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectCountDisp}{0}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRejectRateCIUpperDisp}{5.6\%}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoMeanEDisp}{5.304524703e-24}
\newcommand{\PxTOneNcWrongMarginalConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoStandardErrorEDisp}{5.304524703e-24}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.190320729}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.5022168643}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.190320729}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.5022168643}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.241249798}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.3718498576}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.000873793}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.01531075387}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9966043789}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.005083051928}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.142588235}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2450061926}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.1084652171}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.07092233801}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.1084652171}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.07092233801}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.088885324}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.4398876373}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.092256464}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.08878292145}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9960638894}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.007203361078}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.8439371593}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.3295405258}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6493929732}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2505659223}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6493929732}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2505659223}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.165067561}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2768654085}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.046565128}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.04549117136}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9963341341}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.004888437785}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9932626971}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2040963809}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6619961625}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.4432998048}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.014692764}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02587237678}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.036183128}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.163306468}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.997838716}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.01760419704}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.003683746}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.004529438728}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.042644773}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2452526328}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{2.186003135e-05}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{1.909590493e-05}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.857079623}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.04721516521}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.7453627526}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.07117630763}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9003322745}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.04842427387}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.973960668}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.01013862455}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.1083732066}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02794176147}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.3310090113}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2216495815}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9358861936}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02911702552}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.8907729405}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0948288033}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9490854952}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02678630725}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.988822207}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.005761711753}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.5755089899}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1304663009}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.3639373051}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.08288910886}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.3639373051}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.08288910886}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.7206577227}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1004909872}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9957874448}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02505429891}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.000755733}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.003992269094}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9690182895}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.10136803}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.1354868951}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0941231449}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.1354868951}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0941231449}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6594020437}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1311903979}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.8849216134}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.103444627}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.000696456}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.004735229777}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6554158063}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1123611099}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.2497121001}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.06586701851}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.2497121001}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.06586701851}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.6900298832}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.09500002359}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.9403545291}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.05538711417}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{1.000726094}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.003772143063}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneMeanEDisp}{0.8122170479}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.08320106157}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.002961854416}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.002808408022}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.002961854416}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.002808408022}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.4192923523}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.2188884708}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.023358409}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.02464139607}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.9972183844}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.002425832207}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.2139667081}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.08885473068}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{3.507714892e-31}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.498877386e-31}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{3.507714892e-31}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.498877386e-31}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.9772754832}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.3156367125}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{2.527794229}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.349678716}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.002464618}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.009385160487}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.0004417415903}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.0002713173045}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.001480927208}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.001404204011}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.001480927208}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.001404204011}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.6982839177}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1880700573}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.775576319}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.6727553215}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.9998415013}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.005364037705}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.1072042248}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.04441918843}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{8.241953991e-11}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{6.928675398e-11}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.014646895}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.02485790233}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.057325881}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1830587328}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.012798693}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.02182711542}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.00271156}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.004334902009}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.396844335}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.368086617}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.194232793e-75}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{8.385930076e-76}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.086326626}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.06571320629}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.106756565}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1256150074}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.089293454}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.07023583467}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.018649852}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.01064009733}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{4.768765337e-05}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.537638926e-05}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{4.120976995e-11}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.464337699e-11}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.050486761}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.03926578907}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.082041223}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1291001782}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.051046074}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.04243984704}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.010680706}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.00646444166}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.6984460115}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.6840425295}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.0006120671662}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.000458670381}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.0006120671662}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.000458670381}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.66273057}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.148752149}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.030500912}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.05816775063}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.9999533888}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.004083297542}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.5633232942}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.3560849528}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.605327795e-19}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.545232289e-19}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{2.504991416e-17}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.367566183e-17}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.208119975}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.3769141327}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.2638002604}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.06855814558}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.007428737}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.00637777747}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.004887738789}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.00377565195}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.0003060335831}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.0002293351905}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.0003060335831}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.0002293351905}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.435425272}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.6243277129}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.647150586}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.04096807815}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{1.003691063}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.004465984069}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneMeanEDisp}{0.2841055165}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1779650769}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{3.143685884e-42}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.20291207e-42}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{3.143685884e-42}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.20291207e-42}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.4394108718}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2557168407}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9635577338}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02627738669}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9991683904}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.002673788596}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.0006129419188}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0005860613931}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{2.989955538e-97}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.917722963e-97}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{2.989955538e-97}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.917722963e-97}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.6684403369}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1058553513}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.08983709413}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02309037268}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9958035907}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.003279655518}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.583059406e-08}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{1.035702554e-08}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.571842942e-42}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{1.101456035e-42}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.571842942e-42}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{1.101456035e-42}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.5539256043}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1332758067}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.526697414}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.01612992819}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9974859905}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.002360640868}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.0003064788747}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0002930304375}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{4.231287359e-162}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{4.231287279e-162}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.055685234}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02645827365}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.090566845}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1148692952}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.060623662}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02277738054}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.011047215}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.004545280135}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{7.421473772e-08}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{6.744323291e-08}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.049604157}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1191934085}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.042920314}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.167973376}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.087082757}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1121803079}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.004675745}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.02015989039}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.326750878e-11}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{8.188098382e-12}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{2.115643679e-162}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.11564364e-162}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.052644695}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0657862185}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.06674358}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.1167587124}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.073853209}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.06112118773}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.00786148}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.01119962633}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{3.711400261e-08}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{3.372138915e-08}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{4.732932821e-18}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{4.732932821e-18}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{4.732932821e-18}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{4.732932821e-18}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.178841135}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.6115925952}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.8246110727}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.06741238833}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.00069149}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.001776765794}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.003587156029}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.00176701198}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{8.011861319e-167}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{8.011861319e-167}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{8.011861319e-167}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{8.011861319e-167}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9613898922}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.2039976043}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{4.537606966e-05}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{4.27376468e-05}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.9996250481}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.004843378058}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.35047215e-09}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{8.864259886e-10}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{2.36646641e-18}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.36646641e-18}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{2.36646641e-18}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{2.36646641e-18}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.070115514}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.3249543247}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.4123282244}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.03371039413}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{1.000158269}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.002634606231}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneMeanEDisp}{0.00179357869}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneStandardErrorEDisp}{0.0008835059465}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{5.59432259e-184}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{5.59432259e-184}
\newcommand{\PxTOneCzeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{5.59432259e-184}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{5.59432259e-184}
\newcommand{\PxTOneConePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.1923351507}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1135384145}
\newcommand{\PxTOneConeCPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.015006032}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.03475480611}
\newcommand{\PxTOneCtwoPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.001284712}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.002320920003}
\newcommand{\PxTOneCthreePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{8.062790274e-06}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{5.701357506e-06}
\newcommand{\PxTOneCfourPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneConePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.897411009}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1914762971}
\newcommand{\PxTOneConeCPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{3.612691245}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.466629162}
\newcommand{\PxTOneCtwoPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.002447383}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.002936937439}
\newcommand{\PxTOneCthreePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.177056595e-09}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.047621897e-09}
\newcommand{\PxTOneCfourPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{2.797161295e-184}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.797161295e-184}
\newcommand{\PxTOneCzeroTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{2.797161295e-184}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.797161295e-184}
\newcommand{\PxTOneConeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.5448730798}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1075405928}
\newcommand{\PxTOneConeCTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{2.313848639}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.731762827}
\newcommand{\PxTOneCtwoTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.001866048}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.001986709976}
\newcommand{\PxTOneCthreeTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{4.031983665e-06}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.850652293e-06}
\newcommand{\PxTOneCfourTwoModelAvgNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.9987294223}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.02518192334}
\newcommand{\PxTOneConePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.9791809431}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.2075230607}
\newcommand{\PxTOneConeCPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.019983392}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.02096710344}
\newcommand{\PxTOneCtwoPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.000000462}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.004125989384}
\newcommand{\PxTOneCthreePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.130991404e-11}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{7.045511134e-12}
\newcommand{\PxTOneCfourPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.131194261}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1274263961}
\newcommand{\PxTOneConePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.206213593}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.2511398464}
\newcommand{\PxTOneConeCPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.088015665}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.1028842843}
\newcommand{\PxTOneCtwoPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.016198693}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.0181865149}
\newcommand{\PxTOneCthreePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{2.034447436e-11}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.299036492e-11}
\newcommand{\PxTOneCfourPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.064961842}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.06709127713}
\newcommand{\PxTOneConeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.092697268}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.163824993}
\newcommand{\PxTOneConeCTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.053999529}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.0517150246}
\newcommand{\PxTOneCtwoTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.008099578}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.009685138815}
\newcommand{\PxTOneCthreeTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.58271942e-11}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{7.180098555e-12}
\newcommand{\PxTOneCfourTwoModelAvgOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{3.178482516e-287}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.178482516e-287}
\newcommand{\PxTOneCzeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{3.178482516e-287}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.178482516e-287}
\newcommand{\PxTOneConePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.4499275932}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.2542386644}
\newcommand{\PxTOneConeCPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.1711596835}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.06892859288}
\newcommand{\PxTOneCtwoPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.002668857}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.00235344911}
\newcommand{\PxTOneCthreePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{9.81465793e-08}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{9.774544589e-08}
\newcommand{\PxTOneCfourPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneCzeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{5.698905071e-225}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{4.098191229e-225}
\newcommand{\PxTOneConePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{1}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.079\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{16.2\%}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.782312878}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.029840335}
\newcommand{\PxTOneConeCPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{6.018396611e-07}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{3.297034099e-07}
\newcommand{\PxTOneCtwoPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.004710772}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.005914528767}
\newcommand{\PxTOneCthreePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{4.255297715e-12}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.426376321e-12}
\newcommand{\PxTOneCfourPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleCzeroOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleConeCOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0}
\newcommand{\PxTOneOracleJointOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.589241258e-287}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{1.589241258e-287}
\newcommand{\PxTOneCzeroTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{2.849452535e-225}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{2.049095614e-225}
\newcommand{\PxTOneConeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.116120236}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.5278703444}
\newcommand{\PxTOneConeCTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{0.08558014268}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.03446428319}
\newcommand{\PxTOneCtwoTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{1.003689815}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{0.003327415331}
\newcommand{\PxTOneCthreeTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectCountDisp}{0}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{10.9\%}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneMeanEDisp}{4.90754173e-08}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneStandardErrorEDisp}{4.8872691e-08}
\newcommand{\PxTOneCfourTwoModelAvgGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneCriticalRejectCountDisp}{7}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}5.51}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.52}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1.97}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}5.51}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.52}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1.97}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.21}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.56}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.42}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.21}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.81}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}10.7}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.7}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.59}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}10.7}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.7}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.59}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.58}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.45}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.27}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.52}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.70}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.04}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.25}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.04}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.8}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{13.0}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{17.6}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.8}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{13.0}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{17.6}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.8}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{13.0}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{17.6}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.8}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{13.0}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{17.6}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.11}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.88}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.66}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.11}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.88}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.66}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.53}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.15}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.51}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.36}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.05}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.05}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.13}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.49}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.77}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.62}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}4.45}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}9.00}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.49}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.41}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.78}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.91}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.31}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.46}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.80}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.49}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{18.8\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{4.0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{45.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}31.2}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}40.1}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}24.5}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.10}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.25}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.58}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.13}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.47}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.87}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.38}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3.97}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}5.96}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.76}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{13.6}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{10.5}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{14.6}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.04}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.44}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.33}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.54}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{13.6}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{10.5}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{14.6}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.04}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.4}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{11.0}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{16.1}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}5.15}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}9.70}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.69}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.47}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.34}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.70}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.36}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.36}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.92}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.07}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.16}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.32}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.42}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.18}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}4.18}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}5.66}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1.64}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}4.18}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}5.66}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1.64}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.56}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.16}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.55}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.20}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.07}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.41}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.61}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.65}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}9.51}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.73}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.65}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}9.51}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.73}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.15}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.58}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.22}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.63}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.14}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.44}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.65}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.16}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{13.5}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{12.3}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{15.2}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.04}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{12.0}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{11.3}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{13.5}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.04}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{13.5}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{12.3}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{15.2}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.04}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{14.6}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{12.5}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{16.7}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.05}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}4.66}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}6.06}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.03}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}4.66}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}6.06}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.03}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.11}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.05}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.64}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.29}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.13}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.06}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.32}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.57}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.47}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}16.6}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}21.5}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}11.3}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}16.6}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}21.5}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}11.3}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{8.03}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{7.04}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.43}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.78}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.68}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.83}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.57}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.38}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{7.24}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}38.9}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}51.6}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}33.6}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}38.9}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}51.6}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}33.6}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{10.7}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{9.51}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{13.0}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.29}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.58}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.45}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.29}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.53}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.12}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.17}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{6.65}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{68.8\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{41.3\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{89.0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{79.0}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{76.7}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.0}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{79.0}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{76.7}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.0}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{79.0}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{76.7}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.0}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{79.0}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{76.7}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.0}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}17.3}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}22.2}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}12.0}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}17.3}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}22.2}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}12.0}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{10.2}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{9.02}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{12.4}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.29}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.13}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.04}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.23}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{5.61}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.40}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.04}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}10.5}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}22.4}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5.30}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{3.77}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.88}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.91}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{68.8\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{41.3\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{89.0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{7.86}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.08}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.83}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.70}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.59}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.74}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{5.55}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.04}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}48.3}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}67.3}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}38.3}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.15}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{5.93}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.40}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{6.47}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{10.3}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.72}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.4}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.23}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.35}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.10}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.04}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.26}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.05}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.72}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{4.31}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{37.5\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{15.2\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{64.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{80.0}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{75.7}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.1}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{18.5}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{17.7}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{19.2}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.06}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{80.0}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{75.7}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{82.1}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.25}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{82.1}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{77.0}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{84.7}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}11.2}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.1}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5.99}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{5.29}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.91}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{5.88}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{10.3}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{8.04}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.8}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.21}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.94}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.86}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.03}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.87}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.75}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{7.31}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}12.1}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}14.9}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.72}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}12.1}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}14.9}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.72}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{8.28}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.65}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.71}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.04}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.14}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.09}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.78}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.68}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.83}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{6.14}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.56}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.21}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}33.3}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}42.4}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.3}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}33.3}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}42.4}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.3}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{8.55}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.98}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{13.8}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.45}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.77}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.04}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.99}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.29}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.29}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.37}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.5}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{56.2\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{29.9\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{80.2\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{82.0}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{77.2}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{85.3}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{80.8}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{76.4}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{84.3}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{82.0}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{77.2}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{85.3}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{82.9}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{78.1}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{86.5}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}12.8}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}15.6}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3.41}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}12.8}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}15.6}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3.41}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{8.86}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.75}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{13.1}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.19}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.28}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.91}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.82}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.09}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogEDisp}{6.29}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.20}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.8}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsSixtyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}82.3}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}100}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}66.4}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}82.3}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}100}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}66.4}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.34}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.35}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.71}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{18.8\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{4.0\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{45.6\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.06}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.02}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.24}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}12.8}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5.04}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}177}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}206}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}154}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.56}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}177}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}206}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}154}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.56}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.52}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.45}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.98}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1.14}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.66}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.37}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}13.4}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}15.2}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}12.2}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{37.9}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{35.4}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{41.6}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{37.6}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{35.3}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{41.0}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{37.9}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{35.4}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{41.4}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{37.9}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{35.4}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{41.6}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}83.0}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}101}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}67.0}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}83.0}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}101}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}67.0}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.59}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.87}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.82}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.41}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.61}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.37}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}11.7}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.62}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}106}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}127}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}88.6}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.34}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.42}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.30}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.79}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.92}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.16}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.66}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{25\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{7.3\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{52.4\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.06}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.06}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8.70}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.0}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}332}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}344}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}301}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.05}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.40}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.61}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.34}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.74}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.87}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.15}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.02}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}19.0}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}21.3}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}16.8}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.06}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{36.4}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{32.3}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{39.1}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{1.44}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.39}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.50}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{36.4}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{32.3}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{39.1}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{38.1}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{33.5}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{40.7}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}107}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}128}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}89.3}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.34}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.47}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.28}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.63}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.78}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.43}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.98}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.13}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.05}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.10}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.06}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.39}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.6}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.69}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}100}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}107}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}75.2}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}100}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}107}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}75.2}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.12}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.67}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.77}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.44}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.01}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.38}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}11.2}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5.85}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}122}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}140}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}113}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.39}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}122}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}140}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}113}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.39}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.09}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.78}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.76}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2.65}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3.81}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.95}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}11.3}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.2}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}8.60}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{38.1}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{34.8}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{40.4}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{30.6}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{28.7}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{32.8}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.10}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{38.1}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{34.8}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{40.4}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{38.7}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{36.3}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{42.4}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.12}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}101}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}108}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}75.9}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}101}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}108}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}75.9}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.13}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.46}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.65}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.64}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.08}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.29}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.09}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.80}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}11.4}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.51}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}271}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}308}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}195}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.86}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}271}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}308}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}195}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.86}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{7.47}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.33}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.89}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.13}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.69}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.56}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.77}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}10.1}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}15.8}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.13}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}400}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}472}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}350}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.27}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}400}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}472}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}350}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.27}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{10.5}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.60}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.2}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3.03}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3.77}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2.03}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{1.11}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.90}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.16}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}11.0}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}14.8}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.02}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{138}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{134}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{138}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{134}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{138}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{138}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}271}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}309}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}196}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.86}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}271}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}309}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}196}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.86}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{10.2}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{7.86}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.3}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.57}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.67}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.34}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.95}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.72}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8.72}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.3}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.50}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}228}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}265}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}197}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.72}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{3.84}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.11}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{4.57}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{7.93}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.79}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{12.2}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.74}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.62}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.87}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.58}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}12.1}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.81}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}468}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}493}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}414}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.48}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{5.22}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.09}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{5.93}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{8.54}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.21}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.8}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.12}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.46}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.23}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{1.02}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.91}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.18}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}12.6}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}14.9}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}8.48}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{138}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.44}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{19.6}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{18.9}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{20.4}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.06}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{138}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.44}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{140}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{134}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{141}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.44}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}228}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}266}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}198}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.72}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{4.74}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.86}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{5.49}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{9.75}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.48}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{13.3}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.24}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.88}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.77}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.05}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.39}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}11.6}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.76}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}285}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}311}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}219}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.90}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}285}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}311}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}219}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.90}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{6.37}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.77}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.25}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.15}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.61}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.57}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.69}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.02}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}13.5}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.12}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}420}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}475}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}327}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.33}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}420}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}475}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}327}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.33}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{7.21}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.14}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.60}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.64}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8.25}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3.67}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.94}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.89}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.04}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}11.8}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}16.8}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}8.60}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{131}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{130}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{135}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{121}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{120}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{125}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.38}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{128}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{127}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{132}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.41}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{133}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{130}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{136}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}285}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}312}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}219}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.91}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}285}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}312}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}219}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.91}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{7.16}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.96}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.96}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.64}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.73}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.53}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{0.79}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.77}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.85}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8.93}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}12.8}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6.81}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}656}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}705}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}587}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}2.08}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}656}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}705}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}587}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}2.08}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.00}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.18}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.90}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.09}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.4}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}22.8}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.4}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}955}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1106}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}899}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}3.03}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}955}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1106}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}899}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}3.03}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.20}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.66}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.78}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3.81}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}6.04}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3.65}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}23.3}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}25.5}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}20.2}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{86.0}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{83.0}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{89.1}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{85.9}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{83.0}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{89.0}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{85.6}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{82.6}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{88.6}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{86.0}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{83.0}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{89.1}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}657}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}706}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}588}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}2.08}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}657}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}706}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}588}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}2.08}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.76}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.80}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.16}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.68}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.84}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.60}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.13}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.2}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.4}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.9}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}608}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}702}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}579}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.93}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.32}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.13}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.65}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.01}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.20}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.9}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.6}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}19.5}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2013}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2105}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1897}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}6.39}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.08}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.27}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.44}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.45}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.89}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.40}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.52}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.02}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.8}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.8}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}23.6}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{81.4}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{79.8}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{84.0}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{1.48}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.45}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.56}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{81.4}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{79.8}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{84.0}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{84.2}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{82.1}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{86.3}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}609}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}703}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}579}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.93}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.33}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.47}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.63}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.63}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.17}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.28}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.10}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.01}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.09}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.8}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}19.7}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}619}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}681}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}475}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.96}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}619}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}681}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}475}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.96}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2.80}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.78}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{12.5\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{1.6\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{38.3\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.24}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.76}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.30}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.01}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}22.4}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}24.7}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.1}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}996}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1146}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}862}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}3.16}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}596}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}693}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}509}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.89}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.47}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2.23}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.39}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.28}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}10.6}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.23}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.01}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}23.0}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.4}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.2}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{83.0}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{79.6}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{86.8}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{46.2}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{44.8}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{47.0}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.15}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{82.4}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{79.3}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{85.9}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.26}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{84.3}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{80.1}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{88.6}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.27}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}620}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}682}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}475}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.97}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}596}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}660}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}467}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}1.89}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.21}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2.55}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.82}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.77}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.30}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.39}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}22.9}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.6}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.9}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1430}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1545}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1355}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.54}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1430}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1545}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1355}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.54}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{6.82}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.51}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{7.77}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.04}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.11}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.06}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.58}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.51}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.63}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}24.4}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}26.9}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.4}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2023}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2327}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1879}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}6.42}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2023}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2327}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1879}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}6.42}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.25}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.24}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.84}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{56.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{29.9\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{80.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}9.11}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}10.1}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.00}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.80}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.64}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.95}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}22.9}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.0}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.7}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{149}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{156}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.48}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{149}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{156}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.48}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{149}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{156}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.48}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{149}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{156}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.48}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1430}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1546}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1356}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.54}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1430}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1546}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1356}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.54}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{7.15}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.52}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.04}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.73}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.80}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.64}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.71}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.63}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.77}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.6}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}24.0}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}17.7}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1554}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1628}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1344}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.93}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{3.07}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.83}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.84}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{56.2\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{29.9\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{80.2\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{7.79}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.92}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.98}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.10}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.05}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.64}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.54}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.73}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}23.7}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}25.0}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2723}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2810}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2484}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.64}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.40}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.88}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{4.87}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{6.68}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.29}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{7.92}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.32}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.83}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.77}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}24.6}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}26.2}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.0}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{154}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{152}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{155}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{19.2}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{18.3}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{19.6}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.06}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{154}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{152}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{155}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{154}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{157}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1555}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1629}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1345}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.93}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{4.03}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.60}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{4.47}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{7.90}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.12}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{9.01}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.23}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.76}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.69}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.83}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}22.0}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}24.1}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}17.7}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1581}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1714}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1454}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}5.02}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1581}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1714}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1454}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}5.02}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{8.36}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.73}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.6}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.15}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.71}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.76}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.65}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.86}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.2}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.9}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}17.3}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2174}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2313}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1835}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}6.90}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2174}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2313}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1835}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}6.90}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{7.06}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.61}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{12.1}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}31.6}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}40.5}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}28.1}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.10}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.97}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.76}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.11}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}24.2}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.1}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.3}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{155}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{147}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{145}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{149}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.47}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{151}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{155}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{155}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{152}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1542}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1655}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1455}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.89}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1542}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1655}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1455}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}4.89}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{9.25}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.25}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{12.2}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.84}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.40}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.66}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{0.86}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.71}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.03}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.3}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}23.8}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}17.9}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2677}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3047}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2447}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.49}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2677}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3047}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2447}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.49}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.76}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.41}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.83}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.17}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.11}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}27.1}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.6}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.0}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3419}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3843}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3127}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}10.8}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3419}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3843}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3127}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}10.8}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.30}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1.56}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.30}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{31.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{11.0\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{58.7\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}11.0}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}17.7}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7.13}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.02}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.14}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}27.0}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}29.5}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.6}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{133}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{139}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2677}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3047}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2448}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.50}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2677}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3047}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2448}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.50}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.31}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{2.83}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{25\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{7.3\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{52.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.71}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.86}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.59}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.06}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.12}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}26.0}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.6}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.0}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3235}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3480}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2887}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}10.3}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.26}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.14}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.51}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.66}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.43}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.10}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.21}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.10}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}26.3}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}29.7}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}26.0}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}7636}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8063}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6780}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}24.2}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.56}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.47}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.14}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.98}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.62}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.54}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.23}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.03}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.07}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}29.1}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}30.5}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}26.6}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{133}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{129}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{137}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{1.55}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{1.50}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.61}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{133}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{129}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{137}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{135}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{141}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.43}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}3236}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3481}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2887}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}10.3}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.15}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.07}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.45}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.45}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.03}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.10}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.01}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.20}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.03}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}26.6}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.4}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.4}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2468}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2661}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2236}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}7.83}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2468}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2661}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2236}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}7.83}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.02}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.95}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.43}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.52}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.96}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.57}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.02}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}28.4}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}29.1}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.5}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2806}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}3034}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2730}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}8.90}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1245}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1354}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1208}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}3.95}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.35}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.14}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.52}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}93.8}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}105}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}82.9}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.30}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.08}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}26.4}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}30.1}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}25.6}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{132}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{129}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{137}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{52.6}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{51.3}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{53.6}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.17}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{126}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{124}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{131}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.40}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{134}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{131}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{137}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.42}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}2469}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}2662}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}2237}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}7.83}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}1245}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}1355}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}1209}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}3.95}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.62}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.18}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.20}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{6.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0.16\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{30.2\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}7.22}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8.65}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5.27}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.05}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.04}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.07}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}26.3}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.3}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}23.8}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6831}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7662}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5908}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6831}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7662}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5908}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{6.73}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.22}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{11.6}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoConeCPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.14}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.35}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.70}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.63}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.89}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.2}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.6}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}20.7}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8061}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8879}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7551}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}25.6}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8061}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8879}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}7551}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}25.6}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{8.07}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.91}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.0}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{81.2\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{54.4\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{96.0\%}
\newcommand{\PxTTwoConeCPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}14.6}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}19.7}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}8.54}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.05}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.94}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.80}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{1.01}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.2}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.7}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.2}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{153}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6832}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7663}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5740}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6832}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7663}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5740}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.7}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{9.23}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.37}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{12.0}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{87.5\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{61.7\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{98.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.67}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.84}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}0.34}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.84}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.74}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.95}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}23.4}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}26.9}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.8}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}5995}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}6428}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5718}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}19.0}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{3.04}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.54}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.25}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{50\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{24.7\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{75.3\%}
\newcommand{\PxTTwoConePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{7.33}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.43}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.07}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{93.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{69.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{99.8\%}
\newcommand{\PxTTwoConeCPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.06}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.05}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.58}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.48}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.64}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.0}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.6}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}20.8}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}8833}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}9243}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}8712}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}28.0}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{2.58}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.32}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.11}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{31.2\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{11.0\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{58.7\%}
\newcommand{\PxTTwoConePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{4.60}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{3.49}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{5.97}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoConeCPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.09}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.26}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.17}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.54}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.46}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.61}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.8}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}28.9}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}23.9}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{155}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{19.0}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{18.5}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{19.5}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.06}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{155}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{155}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{158}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}5996}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}6429}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}5719}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}19.0}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{2.89}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{2.42}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{3.32}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{43.8\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{19.8\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{70.1\%}
\newcommand{\PxTTwoConeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.01}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{7.06}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.54}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{7.65}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}0.16}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.09}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.57}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.46}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.65}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}23.6}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}26.4}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}20.9}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6755}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7287}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6241}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.4}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6755}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7287}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6241}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}21.4}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{8.67}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{5.44}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.6}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.22}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7.77}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}3.44}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.77}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.70}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.85}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}21.2}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}24.7}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}19.0}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}7295}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8251}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6684}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}23.1}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}7295}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8251}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6684}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}23.1}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{6.97}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{4.67}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{8.52}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{75\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{47.6\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{92.7\%}
\newcommand{\PxTTwoConeCPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.02}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}159}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}171}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}150}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.50}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.71}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.70}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.76}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreePerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}25.4}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}27.6}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}21.5}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.08}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{160}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleCzeroOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{153}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{151}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{156}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.49}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{157}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{159}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleConeCOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{158}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{154}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{160}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoOracleJointOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.50}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6567}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7288}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6242}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCzeroTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}20.8}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6567}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}7288}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}6242}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoConeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}20.8}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{9.06}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{6.55}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{10.4}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{79.4\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{100\%}
\newcommand{\PxTTwoConeCTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.03}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}6.91}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}8.46}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}4.14}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCtwoTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.02}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{0.75}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{0.71}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{0.81}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCthreeTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{0.00}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogEDisp}{\ensuremath{-}20.7}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileLowerDisp}{\ensuremath{-}22.2}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLogEQuartileUpperDisp}{\ensuremath{-}18.1}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCILowerDisp}{0\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRejectRateCIUpperDisp}{20.6\%}
\newcommand{\PxTTwoCfourTwoModelAvgGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneMedianLogRatioToExactBoundDisp}{\ensuremath{-}0.07}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{41}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{64.1\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{51.1\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{75.7\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{42}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{65.6\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{52.7\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{77.1\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{59}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{92.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{82.7\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{97.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{63}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{98.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{91.6\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{58}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{90.6\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{80.7\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{96.5\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{60}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{93.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{84.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{98.3\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{63}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{98.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{91.6\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{59}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{92.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{82.7\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{97.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{63}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{98.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{91.6\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{56}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{87.5\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{76.8\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{94.4\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{56}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{87.5\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{76.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{63}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{98.4\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{91.6\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100.0\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{51}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{79.7\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{67.8\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{88.7\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{51}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{79.7\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{67.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{88.7\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{58}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{90.6\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{80.7\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{96.5\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{49}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{76.6\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{64.3\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{86.2\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{52}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{81.2\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{69.5\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{89.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{63}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{98.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{91.6\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{58}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{90.6\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{80.7\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{96.5\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{58}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{90.6\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{80.7\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{96.5\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{60}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{93.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{84.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{98.3\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{60}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{93.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{84.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{98.3\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoReplicationCountDisp}{64}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCILowerDisp}{94.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{5}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{15.6\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{5.3\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{32.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{7}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{21.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{9.3\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{40.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{89.1\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{89.1\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{11}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{34.4\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{18.6\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{53.2\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{7}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{21.9\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{9.3\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{40.0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{4}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{12.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{3.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{29.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{5}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{15.6\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{5.3\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{32.8\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{4}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{12.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{3.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{29.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{31}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{96.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{83.8\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{99.9\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportCountDisp}{5}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateDisp}{15.6\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{5.3\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{32.8\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{12}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{37.5\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{21.1\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{56.3\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{6}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{18.8\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{7.2\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{36.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{4}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{12.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{3.5\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{29.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{89.1\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportCountDisp}{4}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateDisp}{12.5\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{3.5\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{29.0\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdDropPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdZeroPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{5}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{15.6\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{5.3\%}
\newcommand{\PxTThreeCdShufflePerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{32.8\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{31}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{96.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{83.8\%}
\newcommand{\PxTThreeCdZeroPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{99.9\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{1}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{3.1\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.079\%}
\newcommand{\PxTThreeCdShufflePerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{16.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{7}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{21.9\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{9.3\%}
\newcommand{\PxTThreeCdZeroPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{40.0\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdDropPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{0}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0\%}
\newcommand{\PxTThreeCdZeroPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{10.9\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{3}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{9.4\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{2.0\%}
\newcommand{\PxTThreeCdShufflePerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{25.0\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{10}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{31.2\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{16.1\%}
\newcommand{\PxTThreeCdDropPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{50.0\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{100\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{89.1\%}
\newcommand{\PxTThreeCdZeroPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{100\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportCountDisp}{2}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneReplicationCountDisp}{32}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateDisp}{6.2\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCILowerDisp}{0.77\%}
\newcommand{\PxTThreeCdShufflePerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneEffectReportRateCIUpperDisp}{20.8\%}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{0.0693}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{14.4}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{0.109}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{9.20}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0.000409}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{0.906}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{1.10}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{0.0633}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{15.8}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{0.0805}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{12.4}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{0.0718}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{13.9}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{0.0798}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{12.5}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{0.0629}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{15.9}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{0.101}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{9.93}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoRhoHatDisp}{0.00403}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaDisp}{0.493}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffKishDisp}{2.03}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixteenGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{0.0721}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{13.9}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{0.0841}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{11.9}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoRhoHatDisp}{0.00392}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaDisp}{0.500}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffKishDisp}{2.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{0.0729}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{13.7}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{0.0770}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{13.0}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoRhoHatDisp}{0.00363}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaDisp}{0.519}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffKishDisp}{1.93}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainTwoFiftySixGridGTwoDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.403}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.48}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.688}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.45}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.175}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0834}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.141}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{12.0}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{7.09}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.176}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0827}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.353}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{12.1}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.84}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.208}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0710}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{14.1}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.509}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.97}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.701}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.43}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00495}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.762}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.31}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.352}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.84}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.410}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.44}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.170}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0853}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.188}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{11.7}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{5.31}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.167}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0870}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.349}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{11.5}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.86}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.196}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0750}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{13.3}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.358}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.80}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.390}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.56}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00452}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.778}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.29}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.287}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{3.48}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.310}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{3.22}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.159}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0906}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.283}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{11.0}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{3.54}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.160}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0905}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.335}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{11.0}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.98}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.192}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.0763}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{13.1}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.300}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{3.33}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{0.297}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{3.37}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00170}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaDisp}{0.903}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffKishDisp}{1.11}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsSixtyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.154}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{6.49}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.450}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{2.22}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.000115}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.972}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.03}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.175}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0219}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0380}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{45.7}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{26.3}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.177}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0216}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.132}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{46.2}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{7.57}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.202}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0190}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{52.5}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.000230}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.945}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.167}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.06}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{5.97}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.396}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{2.53}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.00388}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.503}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.99}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.116}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{8.65}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.127}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{7.87}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.000332}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.922}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.973}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.08}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.03}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.182}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0211}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0500}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{47.4}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{20.0}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.181}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0212}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0947}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{47.1}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.6}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.208}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0185}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{54.1}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.112}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{8.91}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.125}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{7.99}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.00286}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.579}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.73}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0935}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.7}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0922}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.8}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.000261}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.938}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.996}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.07}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.166}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0231}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0828}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{43.3}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{12.1}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.164}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0233}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0956}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{42.9}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.5}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.204}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.0188}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{53.1}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0991}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.1}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.0917}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{10.9}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneRhoHatDisp}{0.00417}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaDisp}{0.484}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneLambdaCDisp}{0.715}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffKishDisp}{2.06}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTwoFiftySixTrainSixtyFourGridGOneDeffContrastDisp}{1.40}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0572}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{17.5}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.177}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{5.67}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.179}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00544}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.00712}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{184}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{140}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.179}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00542}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0225}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{185}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{44.4}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.203}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00478}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{209}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0405}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{24.7}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.228}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{4.39}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00386}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.202}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{4.95}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0266}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{37.6}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0330}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{30.3}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00000787}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.992}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.946}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.01}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.06}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.171}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00570}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0101}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{176}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{98.8}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.165}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00587}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0256}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{170}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{39.0}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.200}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00486}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{206}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.000504}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.660}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0283}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.52}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{35.4}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0381}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{26.3}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00374}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.207}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.941}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{4.83}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.06}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0263}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{38.1}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0245}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{40.8}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.0000242}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.976}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.985}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.02}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.02}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.173}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00561}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0205}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{178}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{48.9}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.175}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00557}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0257}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{180}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{39.0}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.209}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.00465}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{215}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0246}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{40.6}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.0233}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{43.0}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneRhoHatDisp}{0.00380}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaDisp}{0.205}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneLambdaCDisp}{0.346}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffKishDisp}{4.89}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsTenTwentyFourTrainSixtyFourGridGOneDeffContrastDisp}{2.89}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.0160}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{62.5}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.0749}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{13.4}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.176}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00139}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00222}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{721}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{451}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.173}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00141}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00824}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{709}
\newcommand{\PxTFourTemperingPerModelLGOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{121}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.199}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00123}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{814}
\newcommand{\PxTFourTemperingOracleOffsetDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.000629}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.280}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.0109}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{3.57}
\newcommand{\PxTFourTemperingPerModelCNNGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{92.0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.0397}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{25.2}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.00383}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.0600}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{16.7}
\newcommand{\PxTFourTemperingOracleGainDZeroPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00813}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{123}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00900}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{111}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.000000722}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.997}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.970}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingOracleNoneDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.03}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.172}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00142}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00247}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{705}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{404}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.171}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00143}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00650}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{700}
\newcommand{\PxTFourTemperingPerModelLGOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{154}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.198}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00123}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{813}
\newcommand{\PxTFourTemperingOracleOffsetDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.000262}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.483}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00907}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{2.07}
\newcommand{\PxTFourTemperingPerModelCNNGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{110}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.0102}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{98.2}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.00383}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.0600}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.617}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{16.7}
\newcommand{\PxTFourTemperingOracleGainDLoPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.62}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00707}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{141}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00638}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{157}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.0000135}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.948}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.971}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.06}
\newcommand{\PxTFourTemperingOracleNoneDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.03}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.175}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00140}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00514}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{716}
\newcommand{\PxTFourTemperingPerModelCNNOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{194}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.174}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00140}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00617}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{713}
\newcommand{\PxTFourTemperingPerModelLGOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{162}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.211}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.00116}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{1.00}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{864}
\newcommand{\PxTFourTemperingOracleOffsetDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00732}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelCNNGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{137}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.00631}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{1.00}
\newcommand{\PxTFourTemperingPerModelLGGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{158}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneRhoHatDisp}{0.00387}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaDisp}{0.0594}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneLambdaCDisp}{0.102}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffKishDisp}{16.8}
\newcommand{\PxTFourTemperingOracleGainDHiPixelsFortyNinetySixTrainSixtyFourGridGOneDeffContrastDisp}{9.81}


==> macros/demo_macros.tex <==
\newcommand{\DemoTOneRowARejections}{0} %
\newcommand{\DemoTOneRowAK}{64} %
\newcommand{\DemoTOneRowACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAMeanE}{2.799911127e-59} %
\newcommand{\DemoTOneRowASeE}{2.619746661e-59} %
\newcommand{\DemoTOneRowARCrit}{11} %
\newcommand{\DemoTOneRowBRejections}{0} %
\newcommand{\DemoTOneRowBK}{64} %
\newcommand{\DemoTOneRowBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBMeanE}{2.799911127e-59} %
\newcommand{\DemoTOneRowBSeE}{2.619746661e-59} %
\newcommand{\DemoTOneRowBRCrit}{11} %
\newcommand{\DemoTOneRowCRejections}{0} %
\newcommand{\DemoTOneRowCK}{64} %
\newcommand{\DemoTOneRowCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCMeanE}{0.6730612027} %
\newcommand{\DemoTOneRowCSeE}{0.3568285769} %
\newcommand{\DemoTOneRowCRCrit}{11} %
\newcommand{\DemoTOneRowDRejections}{0} %
\newcommand{\DemoTOneRowDK}{64} %
\newcommand{\DemoTOneRowDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDMeanE}{1.00169231} %
\newcommand{\DemoTOneRowDSeE}{0.02035531033} %
\newcommand{\DemoTOneRowDRCrit}{11} %
\newcommand{\DemoTOneRowERejections}{0} %
\newcommand{\DemoTOneRowEK}{64} %
\newcommand{\DemoTOneRowECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEMeanE}{0.979965536} %
\newcommand{\DemoTOneRowESeE}{0.01238077017} %
\newcommand{\DemoTOneRowERCrit}{11} %
\newcommand{\DemoTOneRowFRejections}{0} %
\newcommand{\DemoTOneRowFK}{64} %
\newcommand{\DemoTOneRowFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowFMeanE}{0.0001120837709} %
\newcommand{\DemoTOneRowFSeE}{9.213933887e-05} %
\newcommand{\DemoTOneRowFRCrit}{11} %
\newcommand{\DemoTOneRowGRejections}{0} %
\newcommand{\DemoTOneRowGK}{64} %
\newcommand{\DemoTOneRowGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowGMeanE}{1.871127774e-45} %
\newcommand{\DemoTOneRowGSeE}{1.47066863e-45} %
\newcommand{\DemoTOneRowHRejections}{0} %
\newcommand{\DemoTOneRowHK}{64} %
\newcommand{\DemoTOneRowHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowHMeanE}{4.219408926e-91} %
\newcommand{\DemoTOneRowHSeE}{4.219408926e-91} %
\newcommand{\DemoTOneRowHRCrit}{11} %
\newcommand{\DemoTOneRowIRejections}{0} %
\newcommand{\DemoTOneRowIK}{64} %
\newcommand{\DemoTOneRowICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowIMeanE}{4.219408926e-91} %
\newcommand{\DemoTOneRowISeE}{4.219408926e-91} %
\newcommand{\DemoTOneRowIRCrit}{11} %
\newcommand{\DemoTOneRowJRejections}{0} %
\newcommand{\DemoTOneRowJK}{64} %
\newcommand{\DemoTOneRowJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowJMeanE}{0.2221858117} %
\newcommand{\DemoTOneRowJSeE}{0.1043061338} %
\newcommand{\DemoTOneRowJRCrit}{11} %
\newcommand{\DemoTOneRowKRejections}{2} %
\newcommand{\DemoTOneRowKK}{64} %
\newcommand{\DemoTOneRowKCpNineFiveLower}{0.003807181382} %
\newcommand{\DemoTOneRowKCpNineFiveUpper}{0.1083705222} %
\newcommand{\DemoTOneRowKMeanE}{1.755666539} %
\newcommand{\DemoTOneRowKSeE}{0.6623309218} %
\newcommand{\DemoTOneRowKRCrit}{11} %
\newcommand{\DemoTOneRowLRejections}{0} %
\newcommand{\DemoTOneRowLK}{64} %
\newcommand{\DemoTOneRowLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowLMeanE}{0.9647322824} %
\newcommand{\DemoTOneRowLSeE}{0.01753816038} %
\newcommand{\DemoTOneRowLRCrit}{11} %
\newcommand{\DemoTOneRowMRejections}{0} %
\newcommand{\DemoTOneRowMK}{64} %
\newcommand{\DemoTOneRowMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowMMeanE}{2.81710164e-05} %
\newcommand{\DemoTOneRowMSeE}{2.186199689e-05} %
\newcommand{\DemoTOneRowMRCrit}{11} %
\newcommand{\DemoTOneRowNRejections}{0} %
\newcommand{\DemoTOneRowNK}{64} %
\newcommand{\DemoTOneRowNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowNMeanE}{3.943057553e-72} %
\newcommand{\DemoTOneRowNSeE}{3.943057483e-72} %
\newcommand{\DemoTOneRowORejections}{0} %
\newcommand{\DemoTOneRowOK}{64} %
\newcommand{\DemoTOneRowOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowOMeanE}{1} %
\newcommand{\DemoTOneRowOSeE}{0} %
\newcommand{\DemoTOneRowORCrit}{11} %
\newcommand{\DemoTOneRowPRejections}{0} %
\newcommand{\DemoTOneRowPK}{64} %
\newcommand{\DemoTOneRowPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowPMeanE}{1} %
\newcommand{\DemoTOneRowPSeE}{0} %
\newcommand{\DemoTOneRowPRCrit}{11} %
\newcommand{\DemoTOneRowQRejections}{0} %
\newcommand{\DemoTOneRowQK}{64} %
\newcommand{\DemoTOneRowQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowQMeanE}{1} %
\newcommand{\DemoTOneRowQSeE}{0} %
\newcommand{\DemoTOneRowQRCrit}{11} %
\newcommand{\DemoTOneRowRRejections}{0} %
\newcommand{\DemoTOneRowRK}{64} %
\newcommand{\DemoTOneRowRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowRCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowRMeanE}{1} %
\newcommand{\DemoTOneRowRSeE}{0} %
\newcommand{\DemoTOneRowRRCrit}{11} %
\newcommand{\DemoTOneRowSRejections}{0} %
\newcommand{\DemoTOneRowSK}{64} %
\newcommand{\DemoTOneRowSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowSCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowSMeanE}{1.399955563e-59} %
\newcommand{\DemoTOneRowSSeE}{1.309873331e-59} %
\newcommand{\DemoTOneRowSRCrit}{11} %
\newcommand{\DemoTOneRowTRejections}{0} %
\newcommand{\DemoTOneRowTK}{64} %
\newcommand{\DemoTOneRowTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowTCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowTMeanE}{1.399955563e-59} %
\newcommand{\DemoTOneRowTSeE}{1.309873331e-59} %
\newcommand{\DemoTOneRowTRCrit}{11} %
\newcommand{\DemoTOneRowURejections}{0} %
\newcommand{\DemoTOneRowUK}{64} %
\newcommand{\DemoTOneRowUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowUCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowUMeanE}{0.4476235072} %
\newcommand{\DemoTOneRowUSeE}{0.2134246208} %
\newcommand{\DemoTOneRowURCrit}{11} %
\newcommand{\DemoTOneRowVRejections}{0} %
\newcommand{\DemoTOneRowVK}{64} %
\newcommand{\DemoTOneRowVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowVCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowVMeanE}{1.378679424} %
\newcommand{\DemoTOneRowVSeE}{0.3301133388} %
\newcommand{\DemoTOneRowVRCrit}{11} %
\newcommand{\DemoTOneRowWRejections}{0} %
\newcommand{\DemoTOneRowWK}{64} %
\newcommand{\DemoTOneRowWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowWCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowWMeanE}{0.9723489092} %
\newcommand{\DemoTOneRowWSeE}{0.01406256308} %
\newcommand{\DemoTOneRowWRCrit}{11} %
\newcommand{\DemoTOneRowXRejections}{0} %
\newcommand{\DemoTOneRowXK}{64} %
\newcommand{\DemoTOneRowXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowXCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowXMeanE}{7.012739367e-05} %
\newcommand{\DemoTOneRowXSeE}{4.787391541e-05} %
\newcommand{\DemoTOneRowXRCrit}{11} %
\newcommand{\DemoTOneRowYRejections}{0} %
\newcommand{\DemoTOneRowYK}{64} %
\newcommand{\DemoTOneRowYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowYCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowYMeanE}{9.355638871e-46} %
\newcommand{\DemoTOneRowYSeE}{7.353343151e-46} %
\newcommand{\DemoTOneRowZRejections}{0} %
\newcommand{\DemoTOneRowZK}{64} %
\newcommand{\DemoTOneRowZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowZCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowZMeanE}{5.472376441e-49} %
\newcommand{\DemoTOneRowZSeE}{5.427216956e-49} %
\newcommand{\DemoTOneRowZRCrit}{11} %
\newcommand{\DemoTOneRowAARejections}{0} %
\newcommand{\DemoTOneRowAAK}{64} %
\newcommand{\DemoTOneRowAACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAAMeanE}{5.472376441e-49} %
\newcommand{\DemoTOneRowAASeE}{5.427216956e-49} %
\newcommand{\DemoTOneRowAARCrit}{11} %
\newcommand{\DemoTOneRowABRejections}{0} %
\newcommand{\DemoTOneRowABK}{64} %
\newcommand{\DemoTOneRowABCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowABCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowABMeanE}{0.6792882992} %
\newcommand{\DemoTOneRowABSeE}{0.2758712704} %
\newcommand{\DemoTOneRowABRCrit}{11} %
\newcommand{\DemoTOneRowACRejections}{0} %
\newcommand{\DemoTOneRowACK}{64} %
\newcommand{\DemoTOneRowACCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowACCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowACMeanE}{0.9808483748} %
\newcommand{\DemoTOneRowACSeE}{0.01751174875} %
\newcommand{\DemoTOneRowACRCrit}{11} %
\newcommand{\DemoTOneRowADRejections}{0} %
\newcommand{\DemoTOneRowADK}{64} %
\newcommand{\DemoTOneRowADCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowADCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowADMeanE}{0.9724186691} %
\newcommand{\DemoTOneRowADSeE}{0.01228885969} %
\newcommand{\DemoTOneRowADRCrit}{11} %
\newcommand{\DemoTOneRowAERejections}{0} %
\newcommand{\DemoTOneRowAEK}{64} %
\newcommand{\DemoTOneRowAECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAEMeanE}{0.01095009305} %
\newcommand{\DemoTOneRowAESeE}{0.01065011902} %
\newcommand{\DemoTOneRowAERCrit}{11} %
\newcommand{\DemoTOneRowAFRejections}{0} %
\newcommand{\DemoTOneRowAFK}{64} %
\newcommand{\DemoTOneRowAFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAFMeanE}{1.292333384e-29} %
\newcommand{\DemoTOneRowAFSeE}{1.292333384e-29} %
\newcommand{\DemoTOneRowAGRejections}{0} %
\newcommand{\DemoTOneRowAGK}{64} %
\newcommand{\DemoTOneRowAGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAGMeanE}{5.08735949e-89} %
\newcommand{\DemoTOneRowAGSeE}{5.062976655e-89} %
\newcommand{\DemoTOneRowAGRCrit}{11} %
\newcommand{\DemoTOneRowAHRejections}{0} %
\newcommand{\DemoTOneRowAHK}{64} %
\newcommand{\DemoTOneRowAHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAHMeanE}{5.08735949e-89} %
\newcommand{\DemoTOneRowAHSeE}{5.062976655e-89} %
\newcommand{\DemoTOneRowAHRCrit}{11} %
\newcommand{\DemoTOneRowAIRejections}{0} %
\newcommand{\DemoTOneRowAIK}{64} %
\newcommand{\DemoTOneRowAICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAIMeanE}{0.471661001} %
\newcommand{\DemoTOneRowAISeE}{0.2259470242} %
\newcommand{\DemoTOneRowAIRCrit}{11} %
\newcommand{\DemoTOneRowAJRejections}{0} %
\newcommand{\DemoTOneRowAJK}{64} %
\newcommand{\DemoTOneRowAJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAJMeanE}{0.5171017849} %
\newcommand{\DemoTOneRowAJSeE}{0.1363679798} %
\newcommand{\DemoTOneRowAJRCrit}{11} %
\newcommand{\DemoTOneRowAKRejections}{0} %
\newcommand{\DemoTOneRowAKK}{64} %
\newcommand{\DemoTOneRowAKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAKCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAKMeanE}{0.9579788112} %
\newcommand{\DemoTOneRowAKSeE}{0.01748989046} %
\newcommand{\DemoTOneRowAKRCrit}{11} %
\newcommand{\DemoTOneRowALRejections}{0} %
\newcommand{\DemoTOneRowALK}{64} %
\newcommand{\DemoTOneRowALCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowALCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowALMeanE}{0.0006606717149} %
\newcommand{\DemoTOneRowALSeE}{0.000513363955} %
\newcommand{\DemoTOneRowALRCrit}{11} %
\newcommand{\DemoTOneRowAMRejections}{0} %
\newcommand{\DemoTOneRowAMK}{64} %
\newcommand{\DemoTOneRowAMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAMMeanE}{5.269763085e-62} %
\newcommand{\DemoTOneRowAMSeE}{5.269761922e-62} %
\newcommand{\DemoTOneRowANRejections}{0} %
\newcommand{\DemoTOneRowANK}{64} %
\newcommand{\DemoTOneRowANCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowANCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowANMeanE}{1} %
\newcommand{\DemoTOneRowANSeE}{0} %
\newcommand{\DemoTOneRowANRCrit}{11} %
\newcommand{\DemoTOneRowAORejections}{0} %
\newcommand{\DemoTOneRowAOK}{64} %
\newcommand{\DemoTOneRowAOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAOMeanE}{1} %
\newcommand{\DemoTOneRowAOSeE}{0} %
\newcommand{\DemoTOneRowAORCrit}{11} %
\newcommand{\DemoTOneRowAPRejections}{0} %
\newcommand{\DemoTOneRowAPK}{64} %
\newcommand{\DemoTOneRowAPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAPMeanE}{1} %
\newcommand{\DemoTOneRowAPSeE}{0} %
\newcommand{\DemoTOneRowAPRCrit}{11} %
\newcommand{\DemoTOneRowAQRejections}{0} %
\newcommand{\DemoTOneRowAQK}{64} %
\newcommand{\DemoTOneRowAQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAQMeanE}{1} %
\newcommand{\DemoTOneRowAQSeE}{0} %
\newcommand{\DemoTOneRowAQRCrit}{11} %
\newcommand{\DemoTOneRowARRejections}{0} %
\newcommand{\DemoTOneRowARK}{64} %
\newcommand{\DemoTOneRowARCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowARCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowARMeanE}{2.73618822e-49} %
\newcommand{\DemoTOneRowARSeE}{2.713608478e-49} %
\newcommand{\DemoTOneRowARRCrit}{11} %
\newcommand{\DemoTOneRowASRejections}{0} %
\newcommand{\DemoTOneRowASK}{64} %
\newcommand{\DemoTOneRowASCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowASCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowASMeanE}{2.73618822e-49} %
\newcommand{\DemoTOneRowASSeE}{2.713608478e-49} %
\newcommand{\DemoTOneRowASRCrit}{11} %
\newcommand{\DemoTOneRowATRejections}{0} %
\newcommand{\DemoTOneRowATK}{64} %
\newcommand{\DemoTOneRowATCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowATCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowATMeanE}{0.5754746501} %
\newcommand{\DemoTOneRowATSeE}{0.2042964372} %
\newcommand{\DemoTOneRowATRCrit}{11} %
\newcommand{\DemoTOneRowAURejections}{0} %
\newcommand{\DemoTOneRowAUK}{64} %
\newcommand{\DemoTOneRowAUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAUCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAUMeanE}{0.7489750798} %
\newcommand{\DemoTOneRowAUSeE}{0.07060756549} %
\newcommand{\DemoTOneRowAURCrit}{11} %
\newcommand{\DemoTOneRowAVRejections}{0} %
\newcommand{\DemoTOneRowAVK}{64} %
\newcommand{\DemoTOneRowAVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAVCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAVMeanE}{0.9651987402} %
\newcommand{\DemoTOneRowAVSeE}{0.01392690584} %
\newcommand{\DemoTOneRowAVRCrit}{11} %
\newcommand{\DemoTOneRowAWRejections}{0} %
\newcommand{\DemoTOneRowAWK}{64} %
\newcommand{\DemoTOneRowAWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAWCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAWMeanE}{0.005805382382} %
\newcommand{\DemoTOneRowAWSeE}{0.005327832749} %
\newcommand{\DemoTOneRowAWRCrit}{11} %
\newcommand{\DemoTOneRowAXRejections}{0} %
\newcommand{\DemoTOneRowAXK}{64} %
\newcommand{\DemoTOneRowAXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAXCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAXMeanE}{6.461666921e-30} %
\newcommand{\DemoTOneRowAXSeE}{6.46166692e-30} %
\newcommand{\DemoTOneRowAYRejections}{0} %
\newcommand{\DemoTOneRowAYK}{64} %
\newcommand{\DemoTOneRowAYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAYCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAYMeanE}{9.969884227e-45} %
\newcommand{\DemoTOneRowAYSeE}{9.969883451e-45} %
\newcommand{\DemoTOneRowAYRCrit}{11} %
\newcommand{\DemoTOneRowAZRejections}{0} %
\newcommand{\DemoTOneRowAZK}{64} %
\newcommand{\DemoTOneRowAZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowAZCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowAZMeanE}{9.969884227e-45} %
\newcommand{\DemoTOneRowAZSeE}{9.969883451e-45} %
\newcommand{\DemoTOneRowAZRCrit}{11} %
\newcommand{\DemoTOneRowBARejections}{0} %
\newcommand{\DemoTOneRowBAK}{64} %
\newcommand{\DemoTOneRowBACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBAMeanE}{0.5899240712} %
\newcommand{\DemoTOneRowBASeE}{0.1682636567} %
\newcommand{\DemoTOneRowBARCrit}{11} %
\newcommand{\DemoTOneRowBBRejections}{0} %
\newcommand{\DemoTOneRowBBK}{64} %
\newcommand{\DemoTOneRowBBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBBCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBBMeanE}{0.999660132} %
\newcommand{\DemoTOneRowBBSeE}{0.007823833992} %
\newcommand{\DemoTOneRowBBRCrit}{11} %
\newcommand{\DemoTOneRowBCRejections}{0} %
\newcommand{\DemoTOneRowBCK}{64} %
\newcommand{\DemoTOneRowBCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBCCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBCMeanE}{0.994394307} %
\newcommand{\DemoTOneRowBCSeE}{0.01110882135} %
\newcommand{\DemoTOneRowBCRCrit}{11} %
\newcommand{\DemoTOneRowBDRejections}{0} %
\newcommand{\DemoTOneRowBDK}{64} %
\newcommand{\DemoTOneRowBDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBDCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBDMeanE}{0.003690914692} %
\newcommand{\DemoTOneRowBDSeE}{0.002957964428} %
\newcommand{\DemoTOneRowBDRCrit}{11} %
\newcommand{\DemoTOneRowBERejections}{0} %
\newcommand{\DemoTOneRowBEK}{64} %
\newcommand{\DemoTOneRowBECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBEMeanE}{2.748758244e-26} %
\newcommand{\DemoTOneRowBESeE}{2.738071344e-26} %
\newcommand{\DemoTOneRowBFRejections}{0} %
\newcommand{\DemoTOneRowBFK}{64} %
\newcommand{\DemoTOneRowBFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBFMeanE}{3.850418753e-73} %
\newcommand{\DemoTOneRowBFSeE}{3.850418753e-73} %
\newcommand{\DemoTOneRowBFRCrit}{11} %
\newcommand{\DemoTOneRowBGRejections}{0} %
\newcommand{\DemoTOneRowBGK}{64} %
\newcommand{\DemoTOneRowBGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBGMeanE}{3.850418753e-73} %
\newcommand{\DemoTOneRowBGSeE}{3.850418753e-73} %
\newcommand{\DemoTOneRowBGRCrit}{11} %
\newcommand{\DemoTOneRowBHRejections}{0} %
\newcommand{\DemoTOneRowBHK}{64} %
\newcommand{\DemoTOneRowBHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBHMeanE}{0.256028912} %
\newcommand{\DemoTOneRowBHSeE}{0.08686531627} %
\newcommand{\DemoTOneRowBHRCrit}{11} %
\newcommand{\DemoTOneRowBIRejections}{0} %
\newcommand{\DemoTOneRowBIK}{64} %
\newcommand{\DemoTOneRowBICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBIMeanE}{0.9853313921} %
\newcommand{\DemoTOneRowBISeE}{0.1343507552} %
\newcommand{\DemoTOneRowBIRCrit}{11} %
\newcommand{\DemoTOneRowBJRejections}{0} %
\newcommand{\DemoTOneRowBJK}{64} %
\newcommand{\DemoTOneRowBJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBJMeanE}{0.9940622107} %
\newcommand{\DemoTOneRowBJSeE}{0.01321777031} %
\newcommand{\DemoTOneRowBJRCrit}{11} %
\newcommand{\DemoTOneRowBKRejections}{0} %
\newcommand{\DemoTOneRowBKK}{64} %
\newcommand{\DemoTOneRowBKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBKCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBKMeanE}{6.696189717e-05} %
\newcommand{\DemoTOneRowBKSeE}{3.992084343e-05} %
\newcommand{\DemoTOneRowBKRCrit}{11} %
\newcommand{\DemoTOneRowBLRejections}{0} %
\newcommand{\DemoTOneRowBLK}{64} %
\newcommand{\DemoTOneRowBLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBLCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBLMeanE}{3.807993617e-53} %
\newcommand{\DemoTOneRowBLSeE}{3.807993617e-53} %
\newcommand{\DemoTOneRowBMRejections}{0} %
\newcommand{\DemoTOneRowBMK}{64} %
\newcommand{\DemoTOneRowBMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBMMeanE}{1} %
\newcommand{\DemoTOneRowBMSeE}{0} %
\newcommand{\DemoTOneRowBMRCrit}{11} %
\newcommand{\DemoTOneRowBNRejections}{0} %
\newcommand{\DemoTOneRowBNK}{64} %
\newcommand{\DemoTOneRowBNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBNCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBNMeanE}{1} %
\newcommand{\DemoTOneRowBNSeE}{0} %
\newcommand{\DemoTOneRowBNRCrit}{11} %
\newcommand{\DemoTOneRowBORejections}{0} %
\newcommand{\DemoTOneRowBOK}{64} %
\newcommand{\DemoTOneRowBOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBOMeanE}{1} %
\newcommand{\DemoTOneRowBOSeE}{0} %
\newcommand{\DemoTOneRowBORCrit}{11} %
\newcommand{\DemoTOneRowBPRejections}{0} %
\newcommand{\DemoTOneRowBPK}{64} %
\newcommand{\DemoTOneRowBPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBPMeanE}{1} %
\newcommand{\DemoTOneRowBPSeE}{0} %
\newcommand{\DemoTOneRowBPRCrit}{11} %
\newcommand{\DemoTOneRowBQRejections}{0} %
\newcommand{\DemoTOneRowBQK}{64} %
\newcommand{\DemoTOneRowBQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBQMeanE}{4.984942113e-45} %
\newcommand{\DemoTOneRowBQSeE}{4.984941725e-45} %
\newcommand{\DemoTOneRowBQRCrit}{11} %
\newcommand{\DemoTOneRowBRRejections}{0} %
\newcommand{\DemoTOneRowBRK}{64} %
\newcommand{\DemoTOneRowBRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBRCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBRMeanE}{4.984942113e-45} %
\newcommand{\DemoTOneRowBRSeE}{4.984941725e-45} %
\newcommand{\DemoTOneRowBRRCrit}{11} %
\newcommand{\DemoTOneRowBSRejections}{0} %
\newcommand{\DemoTOneRowBSK}{64} %
\newcommand{\DemoTOneRowBSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBSCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBSMeanE}{0.4229764916} %
\newcommand{\DemoTOneRowBSSeE}{0.1013003478} %
\newcommand{\DemoTOneRowBSRCrit}{11} %
\newcommand{\DemoTOneRowBTRejections}{0} %
\newcommand{\DemoTOneRowBTK}{64} %
\newcommand{\DemoTOneRowBTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBTCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBTMeanE}{0.9924957621} %
\newcommand{\DemoTOneRowBTSeE}{0.06780299901} %
\newcommand{\DemoTOneRowBTRCrit}{11} %
\newcommand{\DemoTOneRowBURejections}{0} %
\newcommand{\DemoTOneRowBUK}{64} %
\newcommand{\DemoTOneRowBUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBUCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBUMeanE}{0.9942282588} %
\newcommand{\DemoTOneRowBUSeE}{0.01124824321} %
\newcommand{\DemoTOneRowBURCrit}{11} %
\newcommand{\DemoTOneRowBVRejections}{0} %
\newcommand{\DemoTOneRowBVK}{64} %
\newcommand{\DemoTOneRowBVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBVCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBVMeanE}{0.001878938294} %
\newcommand{\DemoTOneRowBVSeE}{0.001479650597} %
\newcommand{\DemoTOneRowBVRCrit}{11} %
\newcommand{\DemoTOneRowBWRejections}{0} %
\newcommand{\DemoTOneRowBWK}{64} %
\newcommand{\DemoTOneRowBWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBWCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBWMeanE}{1.374379122e-26} %
\newcommand{\DemoTOneRowBWSeE}{1.369035672e-26} %
\newcommand{\DemoTOneRowBXRejections}{0} %
\newcommand{\DemoTOneRowBXK}{64} %
\newcommand{\DemoTOneRowBXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBXCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBXMeanE}{7.721530739e-51} %
\newcommand{\DemoTOneRowBXSeE}{7.721530426e-51} %
\newcommand{\DemoTOneRowBXRCrit}{11} %
\newcommand{\DemoTOneRowBYRejections}{0} %
\newcommand{\DemoTOneRowBYK}{64} %
\newcommand{\DemoTOneRowBYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowBYCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowBYMeanE}{7.721530739e-51} %
\newcommand{\DemoTOneRowBYSeE}{7.721530426e-51} %
\newcommand{\DemoTOneRowBYRCrit}{11} %
\newcommand{\DemoTOneRowBZRejections}{1} %
\newcommand{\DemoTOneRowBZK}{64} %
\newcommand{\DemoTOneRowBZCpNineFiveLower}{0.0003955125141} %
\newcommand{\DemoTOneRowBZCpNineFiveUpper}{0.08401032643} %
\newcommand{\DemoTOneRowBZMeanE}{0.7936396953} %
\newcommand{\DemoTOneRowBZSeE}{0.4090665239} %
\newcommand{\DemoTOneRowBZRCrit}{11} %
\newcommand{\DemoTOneRowCARejections}{0} %
\newcommand{\DemoTOneRowCAK}{64} %
\newcommand{\DemoTOneRowCACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCAMeanE}{0.9175642852} %
\newcommand{\DemoTOneRowCASeE}{0.06383034864} %
\newcommand{\DemoTOneRowCARCrit}{11} %
\newcommand{\DemoTOneRowCBRejections}{0} %
\newcommand{\DemoTOneRowCBK}{64} %
\newcommand{\DemoTOneRowCBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCBCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCBMeanE}{1.012281563} %
\newcommand{\DemoTOneRowCBSeE}{0.01398115732} %
\newcommand{\DemoTOneRowCBRCrit}{11} %
\newcommand{\DemoTOneRowCCRejections}{0} %
\newcommand{\DemoTOneRowCCK}{64} %
\newcommand{\DemoTOneRowCCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCCCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCCMeanE}{0.0004989213191} %
\newcommand{\DemoTOneRowCCSeE}{0.00027308817} %
\newcommand{\DemoTOneRowCCRCrit}{11} %
\newcommand{\DemoTOneRowCDRejections}{0} %
\newcommand{\DemoTOneRowCDK}{64} %
\newcommand{\DemoTOneRowCDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCDCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCDMeanE}{1.680432056e-41} %
\newcommand{\DemoTOneRowCDSeE}{1.6804182e-41} %
\newcommand{\DemoTOneRowCERejections}{0} %
\newcommand{\DemoTOneRowCEK}{64} %
\newcommand{\DemoTOneRowCECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCEMeanE}{6.533063862e-106} %
\newcommand{\DemoTOneRowCESeE}{6.533063861e-106} %
\newcommand{\DemoTOneRowCERCrit}{11} %
\newcommand{\DemoTOneRowCFRejections}{0} %
\newcommand{\DemoTOneRowCFK}{64} %
\newcommand{\DemoTOneRowCFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCFMeanE}{6.533063862e-106} %
\newcommand{\DemoTOneRowCFSeE}{6.533063861e-106} %
\newcommand{\DemoTOneRowCFRCrit}{11} %
\newcommand{\DemoTOneRowCGRejections}{0} %
\newcommand{\DemoTOneRowCGK}{64} %
\newcommand{\DemoTOneRowCGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCGMeanE}{0.8002308491} %
\newcommand{\DemoTOneRowCGSeE}{0.3896306844} %
\newcommand{\DemoTOneRowCGRCrit}{11} %
\newcommand{\DemoTOneRowCHRejections}{0} %
\newcommand{\DemoTOneRowCHK}{64} %
\newcommand{\DemoTOneRowCHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCHMeanE}{0.3270825859} %
\newcommand{\DemoTOneRowCHSeE}{0.1957775377} %
\newcommand{\DemoTOneRowCHRCrit}{11} %
\newcommand{\DemoTOneRowCIRejections}{0} %
\newcommand{\DemoTOneRowCIK}{64} %
\newcommand{\DemoTOneRowCICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCIMeanE}{1.021780618} %
\newcommand{\DemoTOneRowCISeE}{0.02141533272} %
\newcommand{\DemoTOneRowCIRCrit}{11} %
\newcommand{\DemoTOneRowCJRejections}{0} %
\newcommand{\DemoTOneRowCJK}{64} %
\newcommand{\DemoTOneRowCJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCJMeanE}{6.059172701e-05} %
\newcommand{\DemoTOneRowCJSeE}{3.576959505e-05} %
\newcommand{\DemoTOneRowCJRCrit}{11} %
\newcommand{\DemoTOneRowCKRejections}{0} %
\newcommand{\DemoTOneRowCKK}{64} %
\newcommand{\DemoTOneRowCKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCKCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCKMeanE}{6.461962178e-76} %
\newcommand{\DemoTOneRowCKSeE}{6.461962178e-76} %
\newcommand{\DemoTOneRowCLRejections}{0} %
\newcommand{\DemoTOneRowCLK}{64} %
\newcommand{\DemoTOneRowCLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCLCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCLMeanE}{1} %
\newcommand{\DemoTOneRowCLSeE}{0} %
\newcommand{\DemoTOneRowCLRCrit}{11} %
\newcommand{\DemoTOneRowCMRejections}{0} %
\newcommand{\DemoTOneRowCMK}{64} %
\newcommand{\DemoTOneRowCMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCMMeanE}{1} %
\newcommand{\DemoTOneRowCMSeE}{0} %
\newcommand{\DemoTOneRowCMRCrit}{11} %
\newcommand{\DemoTOneRowCNRejections}{0} %
\newcommand{\DemoTOneRowCNK}{64} %
\newcommand{\DemoTOneRowCNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCNCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCNMeanE}{1} %
\newcommand{\DemoTOneRowCNSeE}{0} %
\newcommand{\DemoTOneRowCNRCrit}{11} %
\newcommand{\DemoTOneRowCORejections}{0} %
\newcommand{\DemoTOneRowCOK}{64} %
\newcommand{\DemoTOneRowCOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCOMeanE}{1} %
\newcommand{\DemoTOneRowCOSeE}{0} %
\newcommand{\DemoTOneRowCORCrit}{11} %
\newcommand{\DemoTOneRowCPRejections}{0} %
\newcommand{\DemoTOneRowCPK}{64} %
\newcommand{\DemoTOneRowCPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCPMeanE}{3.86076537e-51} %
\newcommand{\DemoTOneRowCPSeE}{3.860765213e-51} %
\newcommand{\DemoTOneRowCPRCrit}{11} %
\newcommand{\DemoTOneRowCQRejections}{0} %
\newcommand{\DemoTOneRowCQK}{64} %
\newcommand{\DemoTOneRowCQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCQMeanE}{3.86076537e-51} %
\newcommand{\DemoTOneRowCQSeE}{3.860765213e-51} %
\newcommand{\DemoTOneRowCQRCrit}{11} %
\newcommand{\DemoTOneRowCRRejections}{0} %
\newcommand{\DemoTOneRowCRK}{64} %
\newcommand{\DemoTOneRowCRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCRCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCRMeanE}{0.7969352722} %
\newcommand{\DemoTOneRowCRSeE}{0.2937561857} %
\newcommand{\DemoTOneRowCRRCrit}{11} %
\newcommand{\DemoTOneRowCSRejections}{0} %
\newcommand{\DemoTOneRowCSK}{64} %
\newcommand{\DemoTOneRowCSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCSCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCSMeanE}{0.6223234355} %
\newcommand{\DemoTOneRowCSSeE}{0.1017828638} %
\newcommand{\DemoTOneRowCSRCrit}{11} %
\newcommand{\DemoTOneRowCTRejections}{0} %
\newcommand{\DemoTOneRowCTK}{64} %
\newcommand{\DemoTOneRowCTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCTCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCTMeanE}{1.017031091} %
\newcommand{\DemoTOneRowCTSeE}{0.01631420986} %
\newcommand{\DemoTOneRowCTRCrit}{11} %
\newcommand{\DemoTOneRowCURejections}{0} %
\newcommand{\DemoTOneRowCUK}{64} %
\newcommand{\DemoTOneRowCUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCUCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCUMeanE}{0.000279756523} %
\newcommand{\DemoTOneRowCUSeE}{0.0001369155259} %
\newcommand{\DemoTOneRowCURCrit}{11} %
\newcommand{\DemoTOneRowCVRejections}{0} %
\newcommand{\DemoTOneRowCVK}{64} %
\newcommand{\DemoTOneRowCVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCVCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCVMeanE}{8.402160281e-42} %
\newcommand{\DemoTOneRowCVSeE}{8.402090998e-42} %
\newcommand{\DemoTOneRowCWRejections}{0} %
\newcommand{\DemoTOneRowCWK}{64} %
\newcommand{\DemoTOneRowCWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCWCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCWMeanE}{2.031050368e-50} %
\newcommand{\DemoTOneRowCWSeE}{1.721596715e-50} %
\newcommand{\DemoTOneRowCWRCrit}{11} %
\newcommand{\DemoTOneRowCXRejections}{0} %
\newcommand{\DemoTOneRowCXK}{64} %
\newcommand{\DemoTOneRowCXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCXCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCXMeanE}{2.031050368e-50} %
\newcommand{\DemoTOneRowCXSeE}{1.721596715e-50} %
\newcommand{\DemoTOneRowCXRCrit}{11} %
\newcommand{\DemoTOneRowCYRejections}{0} %
\newcommand{\DemoTOneRowCYK}{64} %
\newcommand{\DemoTOneRowCYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCYCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCYMeanE}{0.4938654236} %
\newcommand{\DemoTOneRowCYSeE}{0.1177086279} %
\newcommand{\DemoTOneRowCYRCrit}{11} %
\newcommand{\DemoTOneRowCZRejections}{0} %
\newcommand{\DemoTOneRowCZK}{64} %
\newcommand{\DemoTOneRowCZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowCZCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowCZMeanE}{1.013890567} %
\newcommand{\DemoTOneRowCZSeE}{0.03075393966} %
\newcommand{\DemoTOneRowCZRCrit}{11} %
\newcommand{\DemoTOneRowDARejections}{0} %
\newcommand{\DemoTOneRowDAK}{64} %
\newcommand{\DemoTOneRowDACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDAMeanE}{0.9972453603} %
\newcommand{\DemoTOneRowDASeE}{0.01210135697} %
\newcommand{\DemoTOneRowDARCrit}{11} %
\newcommand{\DemoTOneRowDBRejections}{0} %
\newcommand{\DemoTOneRowDBK}{64} %
\newcommand{\DemoTOneRowDBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDBCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDBMeanE}{0.0004100002866} %
\newcommand{\DemoTOneRowDBSeE}{0.0002876534346} %
\newcommand{\DemoTOneRowDBRCrit}{11} %
\newcommand{\DemoTOneRowDCRejections}{0} %
\newcommand{\DemoTOneRowDCK}{64} %
\newcommand{\DemoTOneRowDCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDCCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDCMeanE}{3.157341213e-37} %
\newcommand{\DemoTOneRowDCSeE}{3.085380668e-37} %
\newcommand{\DemoTOneRowDDRejections}{0} %
\newcommand{\DemoTOneRowDDK}{64} %
\newcommand{\DemoTOneRowDDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDDCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDDMeanE}{1.037041439e-81} %
\newcommand{\DemoTOneRowDDSeE}{1.026402709e-81} %
\newcommand{\DemoTOneRowDDRCrit}{11} %
\newcommand{\DemoTOneRowDERejections}{0} %
\newcommand{\DemoTOneRowDEK}{64} %
\newcommand{\DemoTOneRowDECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDEMeanE}{1.037041439e-81} %
\newcommand{\DemoTOneRowDESeE}{1.026402709e-81} %
\newcommand{\DemoTOneRowDERCrit}{11} %
\newcommand{\DemoTOneRowDFRejections}{0} %
\newcommand{\DemoTOneRowDFK}{64} %
\newcommand{\DemoTOneRowDFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDFMeanE}{0.3333344245} %
\newcommand{\DemoTOneRowDFSeE}{0.1093898557} %
\newcommand{\DemoTOneRowDFRCrit}{11} %
\newcommand{\DemoTOneRowDGRejections}{0} %
\newcommand{\DemoTOneRowDGK}{64} %
\newcommand{\DemoTOneRowDGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDGMeanE}{0.7863913874} %
\newcommand{\DemoTOneRowDGSeE}{0.2549090855} %
\newcommand{\DemoTOneRowDGRCrit}{11} %
\newcommand{\DemoTOneRowDHRejections}{0} %
\newcommand{\DemoTOneRowDHK}{64} %
\newcommand{\DemoTOneRowDHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDHMeanE}{1.009571623} %
\newcommand{\DemoTOneRowDHSeE}{0.01643633026} %
\newcommand{\DemoTOneRowDHRCrit}{11} %
\newcommand{\DemoTOneRowDIRejections}{0} %
\newcommand{\DemoTOneRowDIK}{64} %
\newcommand{\DemoTOneRowDICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDIMeanE}{0.0002360295788} %
\newcommand{\DemoTOneRowDISeE}{0.0001790208713} %
\newcommand{\DemoTOneRowDIRCrit}{11} %
\newcommand{\DemoTOneRowDJRejections}{0} %
\newcommand{\DemoTOneRowDJK}{64} %
\newcommand{\DemoTOneRowDJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDJMeanE}{5.120706514e-63} %
\newcommand{\DemoTOneRowDJSeE}{4.879926123e-63} %
\newcommand{\DemoTOneRowDKRejections}{0} %
\newcommand{\DemoTOneRowDKK}{64} %
\newcommand{\DemoTOneRowDKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDKCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDKMeanE}{1} %
\newcommand{\DemoTOneRowDKSeE}{0} %
\newcommand{\DemoTOneRowDKRCrit}{11} %
\newcommand{\DemoTOneRowDLRejections}{0} %
\newcommand{\DemoTOneRowDLK}{64} %
\newcommand{\DemoTOneRowDLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDLCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDLMeanE}{1} %
\newcommand{\DemoTOneRowDLSeE}{0} %
\newcommand{\DemoTOneRowDLRCrit}{11} %
\newcommand{\DemoTOneRowDMRejections}{0} %
\newcommand{\DemoTOneRowDMK}{64} %
\newcommand{\DemoTOneRowDMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDMMeanE}{1} %
\newcommand{\DemoTOneRowDMSeE}{0} %
\newcommand{\DemoTOneRowDMRCrit}{11} %
\newcommand{\DemoTOneRowDNRejections}{0} %
\newcommand{\DemoTOneRowDNK}{64} %
\newcommand{\DemoTOneRowDNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDNCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDNMeanE}{1} %
\newcommand{\DemoTOneRowDNSeE}{0} %
\newcommand{\DemoTOneRowDNRCrit}{11} %
\newcommand{\DemoTOneRowDORejections}{0} %
\newcommand{\DemoTOneRowDOK}{64} %
\newcommand{\DemoTOneRowDOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDOMeanE}{1.015525184e-50} %
\newcommand{\DemoTOneRowDOSeE}{8.607983573e-51} %
\newcommand{\DemoTOneRowDORCrit}{11} %
\newcommand{\DemoTOneRowDPRejections}{0} %
\newcommand{\DemoTOneRowDPK}{64} %
\newcommand{\DemoTOneRowDPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDPMeanE}{1.015525184e-50} %
\newcommand{\DemoTOneRowDPSeE}{8.607983573e-51} %
\newcommand{\DemoTOneRowDPRCrit}{11} %
\newcommand{\DemoTOneRowDQRejections}{0} %
\newcommand{\DemoTOneRowDQK}{64} %
\newcommand{\DemoTOneRowDQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDQMeanE}{0.4135999241} %
\newcommand{\DemoTOneRowDQSeE}{0.1021943159} %
\newcommand{\DemoTOneRowDQRCrit}{11} %
\newcommand{\DemoTOneRowDRRejections}{0} %
\newcommand{\DemoTOneRowDRK}{64} %
\newcommand{\DemoTOneRowDRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDRCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDRMeanE}{0.9001409774} %
\newcommand{\DemoTOneRowDRSeE}{0.1278913341} %
\newcommand{\DemoTOneRowDRRCrit}{11} %
\newcommand{\DemoTOneRowDSRejections}{0} %
\newcommand{\DemoTOneRowDSK}{64} %
\newcommand{\DemoTOneRowDSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDSCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDSMeanE}{1.003408492} %
\newcommand{\DemoTOneRowDSSeE}{0.01355387644} %
\newcommand{\DemoTOneRowDSRCrit}{11} %
\newcommand{\DemoTOneRowDTRejections}{0} %
\newcommand{\DemoTOneRowDTK}{64} %
\newcommand{\DemoTOneRowDTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDTCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDTMeanE}{0.0003230149327} %
\newcommand{\DemoTOneRowDTSeE}{0.0001682074321} %
\newcommand{\DemoTOneRowDTRCrit}{11} %
\newcommand{\DemoTOneRowDURejections}{0} %
\newcommand{\DemoTOneRowDUK}{64} %
\newcommand{\DemoTOneRowDUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDUCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDUMeanE}{1.578670606e-37} %
\newcommand{\DemoTOneRowDUSeE}{1.542690334e-37} %
\newcommand{\DemoTOneRowDVRejections}{0} %
\newcommand{\DemoTOneRowDVK}{64} %
\newcommand{\DemoTOneRowDVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDVCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDVMeanE}{1.633899222e-36} %
\newcommand{\DemoTOneRowDVSeE}{1.633899222e-36} %
\newcommand{\DemoTOneRowDVRCrit}{11} %
\newcommand{\DemoTOneRowDWRejections}{0} %
\newcommand{\DemoTOneRowDWK}{64} %
\newcommand{\DemoTOneRowDWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDWCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDWMeanE}{1.633899222e-36} %
\newcommand{\DemoTOneRowDWSeE}{1.633899222e-36} %
\newcommand{\DemoTOneRowDWRCrit}{11} %
\newcommand{\DemoTOneRowDXRejections}{0} %
\newcommand{\DemoTOneRowDXK}{64} %
\newcommand{\DemoTOneRowDXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDXCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDXMeanE}{0.7532806854} %
\newcommand{\DemoTOneRowDXSeE}{0.2808532745} %
\newcommand{\DemoTOneRowDXRCrit}{11} %
\newcommand{\DemoTOneRowDYRejections}{0} %
\newcommand{\DemoTOneRowDYK}{64} %
\newcommand{\DemoTOneRowDYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDYCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDYMeanE}{0.9931429068} %
\newcommand{\DemoTOneRowDYSeE}{0.01565554996} %
\newcommand{\DemoTOneRowDYRCrit}{11} %
\newcommand{\DemoTOneRowDZRejections}{0} %
\newcommand{\DemoTOneRowDZK}{64} %
\newcommand{\DemoTOneRowDZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowDZCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowDZMeanE}{0.998788987} %
\newcommand{\DemoTOneRowDZSeE}{0.01199574616} %
\newcommand{\DemoTOneRowDZRCrit}{11} %
\newcommand{\DemoTOneRowEARejections}{0} %
\newcommand{\DemoTOneRowEAK}{64} %
\newcommand{\DemoTOneRowEACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEACpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEAMeanE}{0.0005258724425} %
\newcommand{\DemoTOneRowEASeE}{0.000328790883} %
\newcommand{\DemoTOneRowEARCrit}{11} %
\newcommand{\DemoTOneRowEBRejections}{0} %
\newcommand{\DemoTOneRowEBK}{64} %
\newcommand{\DemoTOneRowEBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEBCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEBMeanE}{1.060904941e-23} %
\newcommand{\DemoTOneRowEBSeE}{1.060904941e-23} %
\newcommand{\DemoTOneRowECRejections}{0} %
\newcommand{\DemoTOneRowECK}{64} %
\newcommand{\DemoTOneRowECCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowECCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowECMeanE}{3.50011211e-79} %
\newcommand{\DemoTOneRowECSeE}{3.499986503e-79} %
\newcommand{\DemoTOneRowECRCrit}{11} %
\newcommand{\DemoTOneRowEDRejections}{0} %
\newcommand{\DemoTOneRowEDK}{64} %
\newcommand{\DemoTOneRowEDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEDCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEDMeanE}{3.50011211e-79} %
\newcommand{\DemoTOneRowEDSeE}{3.499986503e-79} %
\newcommand{\DemoTOneRowEDRCrit}{11} %
\newcommand{\DemoTOneRowEERejections}{0} %
\newcommand{\DemoTOneRowEEK}{64} %
\newcommand{\DemoTOneRowEECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEECpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEEMeanE}{0.2972984692} %
\newcommand{\DemoTOneRowEESeE}{0.1081888871} %
\newcommand{\DemoTOneRowEERCrit}{11} %
\newcommand{\DemoTOneRowEFRejections}{0} %
\newcommand{\DemoTOneRowEFK}{64} %
\newcommand{\DemoTOneRowEFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEFCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEFMeanE}{0.5667956403} %
\newcommand{\DemoTOneRowEFSeE}{0.1113903063} %
\newcommand{\DemoTOneRowEFRCrit}{11} %
\newcommand{\DemoTOneRowEGRejections}{0} %
\newcommand{\DemoTOneRowEGK}{64} %
\newcommand{\DemoTOneRowEGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEGCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEGMeanE}{0.9960266016} %
\newcommand{\DemoTOneRowEGSeE}{0.0147979042} %
\newcommand{\DemoTOneRowEGRCrit}{11} %
\newcommand{\DemoTOneRowEHRejections}{0} %
\newcommand{\DemoTOneRowEHK}{64} %
\newcommand{\DemoTOneRowEHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEHCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEHMeanE}{0.0001811364422} %
\newcommand{\DemoTOneRowEHSeE}{0.0001064293238} %
\newcommand{\DemoTOneRowEHRCrit}{11} %
\newcommand{\DemoTOneRowEIRejections}{0} %
\newcommand{\DemoTOneRowEIK}{64} %
\newcommand{\DemoTOneRowEICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEICpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEIMeanE}{3.987199255e-63} %
\newcommand{\DemoTOneRowEISeE}{3.922212436e-63} %
\newcommand{\DemoTOneRowEJRejections}{0} %
\newcommand{\DemoTOneRowEJK}{64} %
\newcommand{\DemoTOneRowEJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEJCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEJMeanE}{1} %
\newcommand{\DemoTOneRowEJSeE}{0} %
\newcommand{\DemoTOneRowEJRCrit}{11} %
\newcommand{\DemoTOneRowEKRejections}{0} %
\newcommand{\DemoTOneRowEKK}{64} %
\newcommand{\DemoTOneRowEKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEKCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEKMeanE}{1} %
\newcommand{\DemoTOneRowEKSeE}{0} %
\newcommand{\DemoTOneRowEKRCrit}{11} %
\newcommand{\DemoTOneRowELRejections}{0} %
\newcommand{\DemoTOneRowELK}{64} %
\newcommand{\DemoTOneRowELCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowELCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowELMeanE}{1} %
\newcommand{\DemoTOneRowELSeE}{0} %
\newcommand{\DemoTOneRowELRCrit}{11} %
\newcommand{\DemoTOneRowEMRejections}{0} %
\newcommand{\DemoTOneRowEMK}{64} %
\newcommand{\DemoTOneRowEMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEMCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEMMeanE}{1} %
\newcommand{\DemoTOneRowEMSeE}{0} %
\newcommand{\DemoTOneRowEMRCrit}{11} %
\newcommand{\DemoTOneRowENRejections}{0} %
\newcommand{\DemoTOneRowENK}{64} %
\newcommand{\DemoTOneRowENCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowENCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowENMeanE}{8.169496109e-37} %
\newcommand{\DemoTOneRowENSeE}{8.169496109e-37} %
\newcommand{\DemoTOneRowENRCrit}{11} %
\newcommand{\DemoTOneRowEORejections}{0} %
\newcommand{\DemoTOneRowEOK}{64} %
\newcommand{\DemoTOneRowEOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEOCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEOMeanE}{8.169496109e-37} %
\newcommand{\DemoTOneRowEOSeE}{8.169496109e-37} %
\newcommand{\DemoTOneRowEORCrit}{11} %
\newcommand{\DemoTOneRowEPRejections}{0} %
\newcommand{\DemoTOneRowEPK}{64} %
\newcommand{\DemoTOneRowEPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEPCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEPMeanE}{0.5252895773} %
\newcommand{\DemoTOneRowEPSeE}{0.1874551084} %
\newcommand{\DemoTOneRowEPRCrit}{11} %
\newcommand{\DemoTOneRowEQRejections}{0} %
\newcommand{\DemoTOneRowEQK}{64} %
\newcommand{\DemoTOneRowEQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEQCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowEQMeanE}{0.7799692735} %
\newcommand{\DemoTOneRowEQSeE}{0.05863697082} %
\newcommand{\DemoTOneRowEQRCrit}{11} %
\newcommand{\DemoTOneRowERRejections}{0} %
\newcommand{\DemoTOneRowERK}{64} %
\newcommand{\DemoTOneRowERCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowERCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowERMeanE}{0.9974077943} %
\newcommand{\DemoTOneRowERSeE}{0.01245985943} %
\newcommand{\DemoTOneRowERRCrit}{11} %
\newcommand{\DemoTOneRowESRejections}{0} %
\newcommand{\DemoTOneRowESK}{64} %
\newcommand{\DemoTOneRowESCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowESCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowESMeanE}{0.0003535044423} %
\newcommand{\DemoTOneRowESSeE}{0.0001754552561} %
\newcommand{\DemoTOneRowESRCrit}{11} %
\newcommand{\DemoTOneRowETRejections}{0} %
\newcommand{\DemoTOneRowETK}{64} %
\newcommand{\DemoTOneRowETCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowETCpNineFiveUpper}{0.05600908939} %
\newcommand{\DemoTOneRowETMeanE}{5.304524703e-24} %
\newcommand{\DemoTOneRowETSeE}{5.304524703e-24} %
\newcommand{\DemoTOneRowEURejections}{0} %
\newcommand{\DemoTOneRowEUK}{32} %
\newcommand{\DemoTOneRowEUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEUMeanE}{1.190320729} %
\newcommand{\DemoTOneRowEUSeE}{0.5022168643} %
\newcommand{\DemoTOneRowEURCrit}{7} %
\newcommand{\DemoTOneRowEVRejections}{0} %
\newcommand{\DemoTOneRowEVK}{32} %
\newcommand{\DemoTOneRowEVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEVMeanE}{1.190320729} %
\newcommand{\DemoTOneRowEVSeE}{0.5022168643} %
\newcommand{\DemoTOneRowEVRCrit}{7} %
\newcommand{\DemoTOneRowEWRejections}{0} %
\newcommand{\DemoTOneRowEWK}{32} %
\newcommand{\DemoTOneRowEWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEWMeanE}{1.241249798} %
\newcommand{\DemoTOneRowEWSeE}{0.3718498576} %
\newcommand{\DemoTOneRowEWRCrit}{7} %
\newcommand{\DemoTOneRowEXRejections}{0} %
\newcommand{\DemoTOneRowEXK}{32} %
\newcommand{\DemoTOneRowEXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEXMeanE}{1.000873793} %
\newcommand{\DemoTOneRowEXSeE}{0.01531075387} %
\newcommand{\DemoTOneRowEXRCrit}{7} %
\newcommand{\DemoTOneRowEYRejections}{0} %
\newcommand{\DemoTOneRowEYK}{32} %
\newcommand{\DemoTOneRowEYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEYMeanE}{0.9966043789} %
\newcommand{\DemoTOneRowEYSeE}{0.005083051928} %
\newcommand{\DemoTOneRowEYRCrit}{7} %
\newcommand{\DemoTOneRowEZRejections}{0} %
\newcommand{\DemoTOneRowEZK}{32} %
\newcommand{\DemoTOneRowEZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowEZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowEZMeanE}{1.142588235} %
\newcommand{\DemoTOneRowEZSeE}{0.2450061926} %
\newcommand{\DemoTOneRowEZRCrit}{7} %
\newcommand{\DemoTOneRowFARejections}{0} %
\newcommand{\DemoTOneRowFAK}{32} %
\newcommand{\DemoTOneRowFACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFAMeanE}{0.1084652171} %
\newcommand{\DemoTOneRowFASeE}{0.07092233801} %
\newcommand{\DemoTOneRowFARCrit}{7} %
\newcommand{\DemoTOneRowFBRejections}{0} %
\newcommand{\DemoTOneRowFBK}{32} %
\newcommand{\DemoTOneRowFBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFBMeanE}{0.1084652171} %
\newcommand{\DemoTOneRowFBSeE}{0.07092233801} %
\newcommand{\DemoTOneRowFBRCrit}{7} %
\newcommand{\DemoTOneRowFCRejections}{0} %
\newcommand{\DemoTOneRowFCK}{32} %
\newcommand{\DemoTOneRowFCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFCMeanE}{1.088885324} %
\newcommand{\DemoTOneRowFCSeE}{0.4398876373} %
\newcommand{\DemoTOneRowFCRCrit}{7} %
\newcommand{\DemoTOneRowFDRejections}{0} %
\newcommand{\DemoTOneRowFDK}{32} %
\newcommand{\DemoTOneRowFDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFDMeanE}{1.092256464} %
\newcommand{\DemoTOneRowFDSeE}{0.08878292145} %
\newcommand{\DemoTOneRowFDRCrit}{7} %
\newcommand{\DemoTOneRowFERejections}{0} %
\newcommand{\DemoTOneRowFEK}{32} %
\newcommand{\DemoTOneRowFECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFEMeanE}{0.9960638894} %
\newcommand{\DemoTOneRowFESeE}{0.007203361078} %
\newcommand{\DemoTOneRowFERCrit}{7} %
\newcommand{\DemoTOneRowFFRejections}{0} %
\newcommand{\DemoTOneRowFFK}{32} %
\newcommand{\DemoTOneRowFFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFFMeanE}{0.8439371593} %
\newcommand{\DemoTOneRowFFSeE}{0.3295405258} %
\newcommand{\DemoTOneRowFFRCrit}{7} %
\newcommand{\DemoTOneRowFGRejections}{0} %
\newcommand{\DemoTOneRowFGK}{32} %
\newcommand{\DemoTOneRowFGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFGMeanE}{1} %
\newcommand{\DemoTOneRowFGSeE}{0} %
\newcommand{\DemoTOneRowFGRCrit}{7} %
\newcommand{\DemoTOneRowFHRejections}{0} %
\newcommand{\DemoTOneRowFHK}{32} %
\newcommand{\DemoTOneRowFHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFHMeanE}{1} %
\newcommand{\DemoTOneRowFHSeE}{0} %
\newcommand{\DemoTOneRowFHRCrit}{7} %
\newcommand{\DemoTOneRowFIRejections}{0} %
\newcommand{\DemoTOneRowFIK}{32} %
\newcommand{\DemoTOneRowFICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFIMeanE}{1} %
\newcommand{\DemoTOneRowFISeE}{0} %
\newcommand{\DemoTOneRowFIRCrit}{7} %
\newcommand{\DemoTOneRowFJRejections}{0} %
\newcommand{\DemoTOneRowFJK}{32} %
\newcommand{\DemoTOneRowFJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFJMeanE}{1} %
\newcommand{\DemoTOneRowFJSeE}{0} %
\newcommand{\DemoTOneRowFJRCrit}{7} %
\newcommand{\DemoTOneRowFKRejections}{0} %
\newcommand{\DemoTOneRowFKK}{32} %
\newcommand{\DemoTOneRowFKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFKMeanE}{0.6493929732} %
\newcommand{\DemoTOneRowFKSeE}{0.2505659223} %
\newcommand{\DemoTOneRowFKRCrit}{7} %
\newcommand{\DemoTOneRowFLRejections}{0} %
\newcommand{\DemoTOneRowFLK}{32} %
\newcommand{\DemoTOneRowFLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFLMeanE}{0.6493929732} %
\newcommand{\DemoTOneRowFLSeE}{0.2505659223} %
\newcommand{\DemoTOneRowFLRCrit}{7} %
\newcommand{\DemoTOneRowFMRejections}{0} %
\newcommand{\DemoTOneRowFMK}{32} %
\newcommand{\DemoTOneRowFMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFMMeanE}{1.165067561} %
\newcommand{\DemoTOneRowFMSeE}{0.2768654085} %
\newcommand{\DemoTOneRowFMRCrit}{7} %
\newcommand{\DemoTOneRowFNRejections}{0} %
\newcommand{\DemoTOneRowFNK}{32} %
\newcommand{\DemoTOneRowFNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFNMeanE}{1.046565128} %
\newcommand{\DemoTOneRowFNSeE}{0.04549117136} %
\newcommand{\DemoTOneRowFNRCrit}{7} %
\newcommand{\DemoTOneRowFORejections}{0} %
\newcommand{\DemoTOneRowFOK}{32} %
\newcommand{\DemoTOneRowFOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFOMeanE}{0.9963341341} %
\newcommand{\DemoTOneRowFOSeE}{0.004888437785} %
\newcommand{\DemoTOneRowFORCrit}{7} %
\newcommand{\DemoTOneRowFPRejections}{0} %
\newcommand{\DemoTOneRowFPK}{32} %
\newcommand{\DemoTOneRowFPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFPMeanE}{0.9932626971} %
\newcommand{\DemoTOneRowFPSeE}{0.2040963809} %
\newcommand{\DemoTOneRowFPRCrit}{7} %
\newcommand{\DemoTOneRowFQRejections}{0} %
\newcommand{\DemoTOneRowFQK}{32} %
\newcommand{\DemoTOneRowFQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFQMeanE}{0.6619961625} %
\newcommand{\DemoTOneRowFQSeE}{0.4432998048} %
\newcommand{\DemoTOneRowFQRCrit}{7} %
\newcommand{\DemoTOneRowFRRejections}{0} %
\newcommand{\DemoTOneRowFRK}{32} %
\newcommand{\DemoTOneRowFRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFRMeanE}{1.014692764} %
\newcommand{\DemoTOneRowFRSeE}{0.02587237678} %
\newcommand{\DemoTOneRowFRRCrit}{7} %
\newcommand{\DemoTOneRowFSRejections}{0} %
\newcommand{\DemoTOneRowFSK}{32} %
\newcommand{\DemoTOneRowFSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFSMeanE}{1.036183128} %
\newcommand{\DemoTOneRowFSSeE}{0.163306468} %
\newcommand{\DemoTOneRowFSRCrit}{7} %
\newcommand{\DemoTOneRowFTRejections}{0} %
\newcommand{\DemoTOneRowFTK}{32} %
\newcommand{\DemoTOneRowFTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFTMeanE}{0.997838716} %
\newcommand{\DemoTOneRowFTSeE}{0.01760419704} %
\newcommand{\DemoTOneRowFTRCrit}{7} %
\newcommand{\DemoTOneRowFURejections}{0} %
\newcommand{\DemoTOneRowFUK}{32} %
\newcommand{\DemoTOneRowFUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFUMeanE}{1.003683746} %
\newcommand{\DemoTOneRowFUSeE}{0.004529438728} %
\newcommand{\DemoTOneRowFURCrit}{7} %
\newcommand{\DemoTOneRowFVRejections}{0} %
\newcommand{\DemoTOneRowFVK}{32} %
\newcommand{\DemoTOneRowFVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFVMeanE}{1.042644773} %
\newcommand{\DemoTOneRowFVSeE}{0.2452526328} %
\newcommand{\DemoTOneRowFVRCrit}{7} %
\newcommand{\DemoTOneRowFWRejections}{0} %
\newcommand{\DemoTOneRowFWK}{32} %
\newcommand{\DemoTOneRowFWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFWMeanE}{2.186003135e-05} %
\newcommand{\DemoTOneRowFWSeE}{1.909590493e-05} %
\newcommand{\DemoTOneRowFWRCrit}{7} %
\newcommand{\DemoTOneRowFXRejections}{0} %
\newcommand{\DemoTOneRowFXK}{32} %
\newcommand{\DemoTOneRowFXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFXMeanE}{0.857079623} %
\newcommand{\DemoTOneRowFXSeE}{0.04721516521} %
\newcommand{\DemoTOneRowFXRCrit}{7} %
\newcommand{\DemoTOneRowFYRejections}{0} %
\newcommand{\DemoTOneRowFYK}{32} %
\newcommand{\DemoTOneRowFYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFYMeanE}{0.7453627526} %
\newcommand{\DemoTOneRowFYSeE}{0.07117630763} %
\newcommand{\DemoTOneRowFYRCrit}{7} %
\newcommand{\DemoTOneRowFZRejections}{0} %
\newcommand{\DemoTOneRowFZK}{32} %
\newcommand{\DemoTOneRowFZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowFZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowFZMeanE}{0.9003322745} %
\newcommand{\DemoTOneRowFZSeE}{0.04842427387} %
\newcommand{\DemoTOneRowFZRCrit}{7} %
\newcommand{\DemoTOneRowGARejections}{0} %
\newcommand{\DemoTOneRowGAK}{32} %
\newcommand{\DemoTOneRowGACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGAMeanE}{0.973960668} %
\newcommand{\DemoTOneRowGASeE}{0.01013862455} %
\newcommand{\DemoTOneRowGARCrit}{7} %
\newcommand{\DemoTOneRowGBRejections}{0} %
\newcommand{\DemoTOneRowGBK}{32} %
\newcommand{\DemoTOneRowGBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGBMeanE}{0.1083732066} %
\newcommand{\DemoTOneRowGBSeE}{0.02794176147} %
\newcommand{\DemoTOneRowGBRCrit}{7} %
\newcommand{\DemoTOneRowGCRejections}{0} %
\newcommand{\DemoTOneRowGCK}{32} %
\newcommand{\DemoTOneRowGCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGCMeanE}{1} %
\newcommand{\DemoTOneRowGCSeE}{0} %
\newcommand{\DemoTOneRowGCRCrit}{7} %
\newcommand{\DemoTOneRowGDRejections}{0} %
\newcommand{\DemoTOneRowGDK}{32} %
\newcommand{\DemoTOneRowGDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGDMeanE}{1} %
\newcommand{\DemoTOneRowGDSeE}{0} %
\newcommand{\DemoTOneRowGDRCrit}{7} %
\newcommand{\DemoTOneRowGERejections}{0} %
\newcommand{\DemoTOneRowGEK}{32} %
\newcommand{\DemoTOneRowGECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGEMeanE}{1} %
\newcommand{\DemoTOneRowGESeE}{0} %
\newcommand{\DemoTOneRowGERCrit}{7} %
\newcommand{\DemoTOneRowGFRejections}{0} %
\newcommand{\DemoTOneRowGFK}{32} %
\newcommand{\DemoTOneRowGFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGFMeanE}{1} %
\newcommand{\DemoTOneRowGFSeE}{0} %
\newcommand{\DemoTOneRowGFRCrit}{7} %
\newcommand{\DemoTOneRowGGRejections}{0} %
\newcommand{\DemoTOneRowGGK}{32} %
\newcommand{\DemoTOneRowGGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGGMeanE}{0.3310090113} %
\newcommand{\DemoTOneRowGGSeE}{0.2216495815} %
\newcommand{\DemoTOneRowGGRCrit}{7} %
\newcommand{\DemoTOneRowGHRejections}{0} %
\newcommand{\DemoTOneRowGHK}{32} %
\newcommand{\DemoTOneRowGHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGHMeanE}{0.9358861936} %
\newcommand{\DemoTOneRowGHSeE}{0.02911702552} %
\newcommand{\DemoTOneRowGHRCrit}{7} %
\newcommand{\DemoTOneRowGIRejections}{0} %
\newcommand{\DemoTOneRowGIK}{32} %
\newcommand{\DemoTOneRowGICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGIMeanE}{0.8907729405} %
\newcommand{\DemoTOneRowGISeE}{0.0948288033} %
\newcommand{\DemoTOneRowGIRCrit}{7} %
\newcommand{\DemoTOneRowGJRejections}{0} %
\newcommand{\DemoTOneRowGJK}{32} %
\newcommand{\DemoTOneRowGJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGJMeanE}{0.9490854952} %
\newcommand{\DemoTOneRowGJSeE}{0.02678630725} %
\newcommand{\DemoTOneRowGJRCrit}{7} %
\newcommand{\DemoTOneRowGKRejections}{0} %
\newcommand{\DemoTOneRowGKK}{32} %
\newcommand{\DemoTOneRowGKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGKMeanE}{0.988822207} %
\newcommand{\DemoTOneRowGKSeE}{0.005761711753} %
\newcommand{\DemoTOneRowGKRCrit}{7} %
\newcommand{\DemoTOneRowGLRejections}{0} %
\newcommand{\DemoTOneRowGLK}{32} %
\newcommand{\DemoTOneRowGLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGLMeanE}{0.5755089899} %
\newcommand{\DemoTOneRowGLSeE}{0.1304663009} %
\newcommand{\DemoTOneRowGLRCrit}{7} %
\newcommand{\DemoTOneRowGMRejections}{0} %
\newcommand{\DemoTOneRowGMK}{32} %
\newcommand{\DemoTOneRowGMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGMMeanE}{0.3639373051} %
\newcommand{\DemoTOneRowGMSeE}{0.08288910886} %
\newcommand{\DemoTOneRowGMRCrit}{7} %
\newcommand{\DemoTOneRowGNRejections}{0} %
\newcommand{\DemoTOneRowGNK}{32} %
\newcommand{\DemoTOneRowGNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGNMeanE}{0.3639373051} %
\newcommand{\DemoTOneRowGNSeE}{0.08288910886} %
\newcommand{\DemoTOneRowGNRCrit}{7} %
\newcommand{\DemoTOneRowGORejections}{0} %
\newcommand{\DemoTOneRowGOK}{32} %
\newcommand{\DemoTOneRowGOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGOMeanE}{0.7206577227} %
\newcommand{\DemoTOneRowGOSeE}{0.1004909872} %
\newcommand{\DemoTOneRowGORCrit}{7} %
\newcommand{\DemoTOneRowGPRejections}{0} %
\newcommand{\DemoTOneRowGPK}{32} %
\newcommand{\DemoTOneRowGPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGPMeanE}{0.9957874448} %
\newcommand{\DemoTOneRowGPSeE}{0.02505429891} %
\newcommand{\DemoTOneRowGPRCrit}{7} %
\newcommand{\DemoTOneRowGQRejections}{0} %
\newcommand{\DemoTOneRowGQK}{32} %
\newcommand{\DemoTOneRowGQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGQMeanE}{1.000755733} %
\newcommand{\DemoTOneRowGQSeE}{0.003992269094} %
\newcommand{\DemoTOneRowGQRCrit}{7} %
\newcommand{\DemoTOneRowGRRejections}{0} %
\newcommand{\DemoTOneRowGRK}{32} %
\newcommand{\DemoTOneRowGRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGRMeanE}{0.9690182895} %
\newcommand{\DemoTOneRowGRSeE}{0.10136803} %
\newcommand{\DemoTOneRowGRRCrit}{7} %
\newcommand{\DemoTOneRowGSRejections}{0} %
\newcommand{\DemoTOneRowGSK}{32} %
\newcommand{\DemoTOneRowGSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGSMeanE}{0.1354868951} %
\newcommand{\DemoTOneRowGSSeE}{0.0941231449} %
\newcommand{\DemoTOneRowGSRCrit}{7} %
\newcommand{\DemoTOneRowGTRejections}{0} %
\newcommand{\DemoTOneRowGTK}{32} %
\newcommand{\DemoTOneRowGTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGTMeanE}{0.1354868951} %
\newcommand{\DemoTOneRowGTSeE}{0.0941231449} %
\newcommand{\DemoTOneRowGTRCrit}{7} %
\newcommand{\DemoTOneRowGURejections}{0} %
\newcommand{\DemoTOneRowGUK}{32} %
\newcommand{\DemoTOneRowGUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGUMeanE}{0.6594020437} %
\newcommand{\DemoTOneRowGUSeE}{0.1311903979} %
\newcommand{\DemoTOneRowGURCrit}{7} %
\newcommand{\DemoTOneRowGVRejections}{0} %
\newcommand{\DemoTOneRowGVK}{32} %
\newcommand{\DemoTOneRowGVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGVMeanE}{0.8849216134} %
\newcommand{\DemoTOneRowGVSeE}{0.103444627} %
\newcommand{\DemoTOneRowGVRCrit}{7} %
\newcommand{\DemoTOneRowGWRejections}{0} %
\newcommand{\DemoTOneRowGWK}{32} %
\newcommand{\DemoTOneRowGWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGWMeanE}{1.000696456} %
\newcommand{\DemoTOneRowGWSeE}{0.004735229777} %
\newcommand{\DemoTOneRowGWRCrit}{7} %
\newcommand{\DemoTOneRowGXRejections}{0} %
\newcommand{\DemoTOneRowGXK}{32} %
\newcommand{\DemoTOneRowGXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGXMeanE}{0.6554158063} %
\newcommand{\DemoTOneRowGXSeE}{0.1123611099} %
\newcommand{\DemoTOneRowGXRCrit}{7} %
\newcommand{\DemoTOneRowGYRejections}{0} %
\newcommand{\DemoTOneRowGYK}{32} %
\newcommand{\DemoTOneRowGYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGYMeanE}{1} %
\newcommand{\DemoTOneRowGYSeE}{0} %
\newcommand{\DemoTOneRowGYRCrit}{7} %
\newcommand{\DemoTOneRowGZRejections}{0} %
\newcommand{\DemoTOneRowGZK}{32} %
\newcommand{\DemoTOneRowGZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowGZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowGZMeanE}{1} %
\newcommand{\DemoTOneRowGZSeE}{0} %
\newcommand{\DemoTOneRowGZRCrit}{7} %
\newcommand{\DemoTOneRowHARejections}{0} %
\newcommand{\DemoTOneRowHAK}{32} %
\newcommand{\DemoTOneRowHACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHAMeanE}{1} %
\newcommand{\DemoTOneRowHASeE}{0} %
\newcommand{\DemoTOneRowHARCrit}{7} %
\newcommand{\DemoTOneRowHBRejections}{0} %
\newcommand{\DemoTOneRowHBK}{32} %
\newcommand{\DemoTOneRowHBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHBMeanE}{1} %
\newcommand{\DemoTOneRowHBSeE}{0} %
\newcommand{\DemoTOneRowHBRCrit}{7} %
\newcommand{\DemoTOneRowHCRejections}{0} %
\newcommand{\DemoTOneRowHCK}{32} %
\newcommand{\DemoTOneRowHCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHCMeanE}{0.2497121001} %
\newcommand{\DemoTOneRowHCSeE}{0.06586701851} %
\newcommand{\DemoTOneRowHCRCrit}{7} %
\newcommand{\DemoTOneRowHDRejections}{0} %
\newcommand{\DemoTOneRowHDK}{32} %
\newcommand{\DemoTOneRowHDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHDMeanE}{0.2497121001} %
\newcommand{\DemoTOneRowHDSeE}{0.06586701851} %
\newcommand{\DemoTOneRowHDRCrit}{7} %
\newcommand{\DemoTOneRowHERejections}{0} %
\newcommand{\DemoTOneRowHEK}{32} %
\newcommand{\DemoTOneRowHECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHEMeanE}{0.6900298832} %
\newcommand{\DemoTOneRowHESeE}{0.09500002359} %
\newcommand{\DemoTOneRowHERCrit}{7} %
\newcommand{\DemoTOneRowHFRejections}{0} %
\newcommand{\DemoTOneRowHFK}{32} %
\newcommand{\DemoTOneRowHFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHFMeanE}{0.9403545291} %
\newcommand{\DemoTOneRowHFSeE}{0.05538711417} %
\newcommand{\DemoTOneRowHFRCrit}{7} %
\newcommand{\DemoTOneRowHGRejections}{0} %
\newcommand{\DemoTOneRowHGK}{32} %
\newcommand{\DemoTOneRowHGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHGMeanE}{1.000726094} %
\newcommand{\DemoTOneRowHGSeE}{0.003772143063} %
\newcommand{\DemoTOneRowHGRCrit}{7} %
\newcommand{\DemoTOneRowHHRejections}{0} %
\newcommand{\DemoTOneRowHHK}{32} %
\newcommand{\DemoTOneRowHHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHHMeanE}{0.8122170479} %
\newcommand{\DemoTOneRowHHSeE}{0.08320106157} %
\newcommand{\DemoTOneRowHHRCrit}{7} %
\newcommand{\DemoTOneRowHIRejections}{0} %
\newcommand{\DemoTOneRowHIK}{32} %
\newcommand{\DemoTOneRowHICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHIMeanE}{0.002961854416} %
\newcommand{\DemoTOneRowHISeE}{0.002808408022} %
\newcommand{\DemoTOneRowHIRCrit}{7} %
\newcommand{\DemoTOneRowHJRejections}{0} %
\newcommand{\DemoTOneRowHJK}{32} %
\newcommand{\DemoTOneRowHJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHJMeanE}{0.002961854416} %
\newcommand{\DemoTOneRowHJSeE}{0.002808408022} %
\newcommand{\DemoTOneRowHJRCrit}{7} %
\newcommand{\DemoTOneRowHKRejections}{0} %
\newcommand{\DemoTOneRowHKK}{32} %
\newcommand{\DemoTOneRowHKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHKMeanE}{0.4192923523} %
\newcommand{\DemoTOneRowHKSeE}{0.2188884708} %
\newcommand{\DemoTOneRowHKRCrit}{7} %
\newcommand{\DemoTOneRowHLRejections}{0} %
\newcommand{\DemoTOneRowHLK}{32} %
\newcommand{\DemoTOneRowHLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHLMeanE}{1.023358409} %
\newcommand{\DemoTOneRowHLSeE}{0.02464139607} %
\newcommand{\DemoTOneRowHLRCrit}{7} %
\newcommand{\DemoTOneRowHMRejections}{0} %
\newcommand{\DemoTOneRowHMK}{32} %
\newcommand{\DemoTOneRowHMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHMMeanE}{0.9972183844} %
\newcommand{\DemoTOneRowHMSeE}{0.002425832207} %
\newcommand{\DemoTOneRowHMRCrit}{7} %
\newcommand{\DemoTOneRowHNRejections}{0} %
\newcommand{\DemoTOneRowHNK}{32} %
\newcommand{\DemoTOneRowHNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHNMeanE}{0.2139667081} %
\newcommand{\DemoTOneRowHNSeE}{0.08885473068} %
\newcommand{\DemoTOneRowHNRCrit}{7} %
\newcommand{\DemoTOneRowHORejections}{0} %
\newcommand{\DemoTOneRowHOK}{32} %
\newcommand{\DemoTOneRowHOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHOMeanE}{3.507714892e-31} %
\newcommand{\DemoTOneRowHOSeE}{3.498877386e-31} %
\newcommand{\DemoTOneRowHORCrit}{7} %
\newcommand{\DemoTOneRowHPRejections}{0} %
\newcommand{\DemoTOneRowHPK}{32} %
\newcommand{\DemoTOneRowHPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHPMeanE}{3.507714892e-31} %
\newcommand{\DemoTOneRowHPSeE}{3.498877386e-31} %
\newcommand{\DemoTOneRowHPRCrit}{7} %
\newcommand{\DemoTOneRowHQRejections}{0} %
\newcommand{\DemoTOneRowHQK}{32} %
\newcommand{\DemoTOneRowHQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHQMeanE}{0.9772754832} %
\newcommand{\DemoTOneRowHQSeE}{0.3156367125} %
\newcommand{\DemoTOneRowHQRCrit}{7} %
\newcommand{\DemoTOneRowHRRejections}{1} %
\newcommand{\DemoTOneRowHRK}{32} %
\newcommand{\DemoTOneRowHRCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowHRCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowHRMeanE}{2.527794229} %
\newcommand{\DemoTOneRowHRSeE}{1.349678716} %
\newcommand{\DemoTOneRowHRRCrit}{7} %
\newcommand{\DemoTOneRowHSRejections}{0} %
\newcommand{\DemoTOneRowHSK}{32} %
\newcommand{\DemoTOneRowHSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHSMeanE}{1.002464618} %
\newcommand{\DemoTOneRowHSSeE}{0.009385160487} %
\newcommand{\DemoTOneRowHSRCrit}{7} %
\newcommand{\DemoTOneRowHTRejections}{0} %
\newcommand{\DemoTOneRowHTK}{32} %
\newcommand{\DemoTOneRowHTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHTMeanE}{0.0004417415903} %
\newcommand{\DemoTOneRowHTSeE}{0.0002713173045} %
\newcommand{\DemoTOneRowHTRCrit}{7} %
\newcommand{\DemoTOneRowHURejections}{0} %
\newcommand{\DemoTOneRowHUK}{32} %
\newcommand{\DemoTOneRowHUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHUMeanE}{1} %
\newcommand{\DemoTOneRowHUSeE}{0} %
\newcommand{\DemoTOneRowHURCrit}{7} %
\newcommand{\DemoTOneRowHVRejections}{0} %
\newcommand{\DemoTOneRowHVK}{32} %
\newcommand{\DemoTOneRowHVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHVMeanE}{1} %
\newcommand{\DemoTOneRowHVSeE}{0} %
\newcommand{\DemoTOneRowHVRCrit}{7} %
\newcommand{\DemoTOneRowHWRejections}{0} %
\newcommand{\DemoTOneRowHWK}{32} %
\newcommand{\DemoTOneRowHWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHWMeanE}{1} %
\newcommand{\DemoTOneRowHWSeE}{0} %
\newcommand{\DemoTOneRowHWRCrit}{7} %
\newcommand{\DemoTOneRowHXRejections}{0} %
\newcommand{\DemoTOneRowHXK}{32} %
\newcommand{\DemoTOneRowHXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHXMeanE}{1} %
\newcommand{\DemoTOneRowHXSeE}{0} %
\newcommand{\DemoTOneRowHXRCrit}{7} %
\newcommand{\DemoTOneRowHYRejections}{0} %
\newcommand{\DemoTOneRowHYK}{32} %
\newcommand{\DemoTOneRowHYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHYMeanE}{0.001480927208} %
\newcommand{\DemoTOneRowHYSeE}{0.001404204011} %
\newcommand{\DemoTOneRowHYRCrit}{7} %
\newcommand{\DemoTOneRowHZRejections}{0} %
\newcommand{\DemoTOneRowHZK}{32} %
\newcommand{\DemoTOneRowHZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowHZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowHZMeanE}{0.001480927208} %
\newcommand{\DemoTOneRowHZSeE}{0.001404204011} %
\newcommand{\DemoTOneRowHZRCrit}{7} %
\newcommand{\DemoTOneRowIARejections}{0} %
\newcommand{\DemoTOneRowIAK}{32} %
\newcommand{\DemoTOneRowIACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIAMeanE}{0.6982839177} %
\newcommand{\DemoTOneRowIASeE}{0.1880700573} %
\newcommand{\DemoTOneRowIARCrit}{7} %
\newcommand{\DemoTOneRowIBRejections}{1} %
\newcommand{\DemoTOneRowIBK}{32} %
\newcommand{\DemoTOneRowIBCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowIBCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowIBMeanE}{1.775576319} %
\newcommand{\DemoTOneRowIBSeE}{0.6727553215} %
\newcommand{\DemoTOneRowIBRCrit}{7} %
\newcommand{\DemoTOneRowICRejections}{0} %
\newcommand{\DemoTOneRowICK}{32} %
\newcommand{\DemoTOneRowICCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowICCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowICMeanE}{0.9998415013} %
\newcommand{\DemoTOneRowICSeE}{0.005364037705} %
\newcommand{\DemoTOneRowICRCrit}{7} %
\newcommand{\DemoTOneRowIDRejections}{0} %
\newcommand{\DemoTOneRowIDK}{32} %
\newcommand{\DemoTOneRowIDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIDMeanE}{0.1072042248} %
\newcommand{\DemoTOneRowIDSeE}{0.04441918843} %
\newcommand{\DemoTOneRowIDRCrit}{7} %
\newcommand{\DemoTOneRowIERejections}{0} %
\newcommand{\DemoTOneRowIEK}{32} %
\newcommand{\DemoTOneRowIECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIEMeanE}{8.241953991e-11} %
\newcommand{\DemoTOneRowIESeE}{6.928675398e-11} %
\newcommand{\DemoTOneRowIERCrit}{7} %
\newcommand{\DemoTOneRowIFRejections}{0} %
\newcommand{\DemoTOneRowIFK}{32} %
\newcommand{\DemoTOneRowIFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIFMeanE}{1.014646895} %
\newcommand{\DemoTOneRowIFSeE}{0.02485790233} %
\newcommand{\DemoTOneRowIFRCrit}{7} %
\newcommand{\DemoTOneRowIGRejections}{0} %
\newcommand{\DemoTOneRowIGK}{32} %
\newcommand{\DemoTOneRowIGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIGMeanE}{1.057325881} %
\newcommand{\DemoTOneRowIGSeE}{0.1830587328} %
\newcommand{\DemoTOneRowIGRCrit}{7} %
\newcommand{\DemoTOneRowIHRejections}{0} %
\newcommand{\DemoTOneRowIHK}{32} %
\newcommand{\DemoTOneRowIHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIHMeanE}{1.012798693} %
\newcommand{\DemoTOneRowIHSeE}{0.02182711542} %
\newcommand{\DemoTOneRowIHRCrit}{7} %
\newcommand{\DemoTOneRowIIRejections}{0} %
\newcommand{\DemoTOneRowIIK}{32} %
\newcommand{\DemoTOneRowIICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIIMeanE}{1.00271156} %
\newcommand{\DemoTOneRowIISeE}{0.004334902009} %
\newcommand{\DemoTOneRowIIRCrit}{7} %
\newcommand{\DemoTOneRowIJRejections}{1} %
\newcommand{\DemoTOneRowIJK}{32} %
\newcommand{\DemoTOneRowIJCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowIJCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowIJMeanE}{1.396844335} %
\newcommand{\DemoTOneRowIJSeE}{1.368086617} %
\newcommand{\DemoTOneRowIJRCrit}{7} %
\newcommand{\DemoTOneRowIKRejections}{0} %
\newcommand{\DemoTOneRowIKK}{32} %
\newcommand{\DemoTOneRowIKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIKMeanE}{1.194232793e-75} %
\newcommand{\DemoTOneRowIKSeE}{8.385930076e-76} %
\newcommand{\DemoTOneRowIKRCrit}{7} %
\newcommand{\DemoTOneRowILRejections}{0} %
\newcommand{\DemoTOneRowILK}{32} %
\newcommand{\DemoTOneRowILCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowILCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowILMeanE}{1.086326626} %
\newcommand{\DemoTOneRowILSeE}{0.06571320629} %
\newcommand{\DemoTOneRowILRCrit}{7} %
\newcommand{\DemoTOneRowIMRejections}{0} %
\newcommand{\DemoTOneRowIMK}{32} %
\newcommand{\DemoTOneRowIMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIMMeanE}{1.106756565} %
\newcommand{\DemoTOneRowIMSeE}{0.1256150074} %
\newcommand{\DemoTOneRowIMRCrit}{7} %
\newcommand{\DemoTOneRowINRejections}{0} %
\newcommand{\DemoTOneRowINK}{32} %
\newcommand{\DemoTOneRowINCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowINCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowINMeanE}{1.089293454} %
\newcommand{\DemoTOneRowINSeE}{0.07023583467} %
\newcommand{\DemoTOneRowINRCrit}{7} %
\newcommand{\DemoTOneRowIORejections}{0} %
\newcommand{\DemoTOneRowIOK}{32} %
\newcommand{\DemoTOneRowIOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIOMeanE}{1.018649852} %
\newcommand{\DemoTOneRowIOSeE}{0.01064009733} %
\newcommand{\DemoTOneRowIORCrit}{7} %
\newcommand{\DemoTOneRowIPRejections}{0} %
\newcommand{\DemoTOneRowIPK}{32} %
\newcommand{\DemoTOneRowIPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIPMeanE}{4.768765337e-05} %
\newcommand{\DemoTOneRowIPSeE}{3.537638926e-05} %
\newcommand{\DemoTOneRowIPRCrit}{7} %
\newcommand{\DemoTOneRowIQRejections}{0} %
\newcommand{\DemoTOneRowIQK}{32} %
\newcommand{\DemoTOneRowIQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIQMeanE}{1} %
\newcommand{\DemoTOneRowIQSeE}{0} %
\newcommand{\DemoTOneRowIQRCrit}{7} %
\newcommand{\DemoTOneRowIRRejections}{0} %
\newcommand{\DemoTOneRowIRK}{32} %
\newcommand{\DemoTOneRowIRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIRMeanE}{1} %
\newcommand{\DemoTOneRowIRSeE}{0} %
\newcommand{\DemoTOneRowIRRCrit}{7} %
\newcommand{\DemoTOneRowISRejections}{0} %
\newcommand{\DemoTOneRowISK}{32} %
\newcommand{\DemoTOneRowISCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowISCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowISMeanE}{1} %
\newcommand{\DemoTOneRowISSeE}{0} %
\newcommand{\DemoTOneRowISRCrit}{7} %
\newcommand{\DemoTOneRowITRejections}{0} %
\newcommand{\DemoTOneRowITK}{32} %
\newcommand{\DemoTOneRowITCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowITCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowITMeanE}{1} %
\newcommand{\DemoTOneRowITSeE}{0} %
\newcommand{\DemoTOneRowITRCrit}{7} %
\newcommand{\DemoTOneRowIURejections}{0} %
\newcommand{\DemoTOneRowIUK}{32} %
\newcommand{\DemoTOneRowIUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIUMeanE}{4.120976995e-11} %
\newcommand{\DemoTOneRowIUSeE}{3.464337699e-11} %
\newcommand{\DemoTOneRowIURCrit}{7} %
\newcommand{\DemoTOneRowIVRejections}{0} %
\newcommand{\DemoTOneRowIVK}{32} %
\newcommand{\DemoTOneRowIVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIVMeanE}{1.050486761} %
\newcommand{\DemoTOneRowIVSeE}{0.03926578907} %
\newcommand{\DemoTOneRowIVRCrit}{7} %
\newcommand{\DemoTOneRowIWRejections}{0} %
\newcommand{\DemoTOneRowIWK}{32} %
\newcommand{\DemoTOneRowIWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIWMeanE}{1.082041223} %
\newcommand{\DemoTOneRowIWSeE}{0.1291001782} %
\newcommand{\DemoTOneRowIWRCrit}{7} %
\newcommand{\DemoTOneRowIXRejections}{0} %
\newcommand{\DemoTOneRowIXK}{32} %
\newcommand{\DemoTOneRowIXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIXMeanE}{1.051046074} %
\newcommand{\DemoTOneRowIXSeE}{0.04243984704} %
\newcommand{\DemoTOneRowIXRCrit}{7} %
\newcommand{\DemoTOneRowIYRejections}{0} %
\newcommand{\DemoTOneRowIYK}{32} %
\newcommand{\DemoTOneRowIYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowIYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowIYMeanE}{1.010680706} %
\newcommand{\DemoTOneRowIYSeE}{0.00646444166} %
\newcommand{\DemoTOneRowIYRCrit}{7} %
\newcommand{\DemoTOneRowIZRejections}{1} %
\newcommand{\DemoTOneRowIZK}{32} %
\newcommand{\DemoTOneRowIZCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowIZCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowIZMeanE}{0.6984460115} %
\newcommand{\DemoTOneRowIZSeE}{0.6840425295} %
\newcommand{\DemoTOneRowIZRCrit}{7} %
\newcommand{\DemoTOneRowJARejections}{0} %
\newcommand{\DemoTOneRowJAK}{32} %
\newcommand{\DemoTOneRowJACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJAMeanE}{0.0006120671662} %
\newcommand{\DemoTOneRowJASeE}{0.000458670381} %
\newcommand{\DemoTOneRowJARCrit}{7} %
\newcommand{\DemoTOneRowJBRejections}{0} %
\newcommand{\DemoTOneRowJBK}{32} %
\newcommand{\DemoTOneRowJBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJBMeanE}{0.0006120671662} %
\newcommand{\DemoTOneRowJBSeE}{0.000458670381} %
\newcommand{\DemoTOneRowJBRCrit}{7} %
\newcommand{\DemoTOneRowJCRejections}{1} %
\newcommand{\DemoTOneRowJCK}{32} %
\newcommand{\DemoTOneRowJCCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowJCCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowJCMeanE}{1.66273057} %
\newcommand{\DemoTOneRowJCSeE}{1.148752149} %
\newcommand{\DemoTOneRowJCRCrit}{7} %
\newcommand{\DemoTOneRowJDRejections}{0} %
\newcommand{\DemoTOneRowJDK}{32} %
\newcommand{\DemoTOneRowJDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJDMeanE}{1.030500912} %
\newcommand{\DemoTOneRowJDSeE}{0.05816775063} %
\newcommand{\DemoTOneRowJDRCrit}{7} %
\newcommand{\DemoTOneRowJERejections}{0} %
\newcommand{\DemoTOneRowJEK}{32} %
\newcommand{\DemoTOneRowJECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJEMeanE}{0.9999533888} %
\newcommand{\DemoTOneRowJESeE}{0.004083297542} %
\newcommand{\DemoTOneRowJERCrit}{7} %
\newcommand{\DemoTOneRowJFRejections}{0} %
\newcommand{\DemoTOneRowJFK}{32} %
\newcommand{\DemoTOneRowJFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJFMeanE}{0.5633232942} %
\newcommand{\DemoTOneRowJFSeE}{0.3560849528} %
\newcommand{\DemoTOneRowJFRCrit}{7} %
\newcommand{\DemoTOneRowJGRejections}{0} %
\newcommand{\DemoTOneRowJGK}{32} %
\newcommand{\DemoTOneRowJGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJGMeanE}{1.605327795e-19} %
\newcommand{\DemoTOneRowJGSeE}{1.545232289e-19} %
\newcommand{\DemoTOneRowJGRCrit}{7} %
\newcommand{\DemoTOneRowJHRejections}{0} %
\newcommand{\DemoTOneRowJHK}{32} %
\newcommand{\DemoTOneRowJHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJHMeanE}{2.504991416e-17} %
\newcommand{\DemoTOneRowJHSeE}{2.367566183e-17} %
\newcommand{\DemoTOneRowJHRCrit}{7} %
\newcommand{\DemoTOneRowJIRejections}{0} %
\newcommand{\DemoTOneRowJIK}{32} %
\newcommand{\DemoTOneRowJICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJIMeanE}{1.208119975} %
\newcommand{\DemoTOneRowJISeE}{0.3769141327} %
\newcommand{\DemoTOneRowJIRCrit}{7} %
\newcommand{\DemoTOneRowJJRejections}{0} %
\newcommand{\DemoTOneRowJJK}{32} %
\newcommand{\DemoTOneRowJJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJJMeanE}{0.2638002604} %
\newcommand{\DemoTOneRowJJSeE}{0.06855814558} %
\newcommand{\DemoTOneRowJJRCrit}{7} %
\newcommand{\DemoTOneRowJKRejections}{0} %
\newcommand{\DemoTOneRowJKK}{32} %
\newcommand{\DemoTOneRowJKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJKMeanE}{1.007428737} %
\newcommand{\DemoTOneRowJKSeE}{0.00637777747} %
\newcommand{\DemoTOneRowJKRCrit}{7} %
\newcommand{\DemoTOneRowJLRejections}{0} %
\newcommand{\DemoTOneRowJLK}{32} %
\newcommand{\DemoTOneRowJLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJLMeanE}{0.004887738789} %
\newcommand{\DemoTOneRowJLSeE}{0.00377565195} %
\newcommand{\DemoTOneRowJLRCrit}{7} %
\newcommand{\DemoTOneRowJMRejections}{0} %
\newcommand{\DemoTOneRowJMK}{32} %
\newcommand{\DemoTOneRowJMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJMMeanE}{1} %
\newcommand{\DemoTOneRowJMSeE}{0} %
\newcommand{\DemoTOneRowJMRCrit}{7} %
\newcommand{\DemoTOneRowJNRejections}{0} %
\newcommand{\DemoTOneRowJNK}{32} %
\newcommand{\DemoTOneRowJNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJNMeanE}{1} %
\newcommand{\DemoTOneRowJNSeE}{0} %
\newcommand{\DemoTOneRowJNRCrit}{7} %
\newcommand{\DemoTOneRowJORejections}{0} %
\newcommand{\DemoTOneRowJOK}{32} %
\newcommand{\DemoTOneRowJOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJOMeanE}{1} %
\newcommand{\DemoTOneRowJOSeE}{0} %
\newcommand{\DemoTOneRowJORCrit}{7} %
\newcommand{\DemoTOneRowJPRejections}{0} %
\newcommand{\DemoTOneRowJPK}{32} %
\newcommand{\DemoTOneRowJPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJPMeanE}{1} %
\newcommand{\DemoTOneRowJPSeE}{0} %
\newcommand{\DemoTOneRowJPRCrit}{7} %
\newcommand{\DemoTOneRowJQRejections}{0} %
\newcommand{\DemoTOneRowJQK}{32} %
\newcommand{\DemoTOneRowJQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJQMeanE}{0.0003060335831} %
\newcommand{\DemoTOneRowJQSeE}{0.0002293351905} %
\newcommand{\DemoTOneRowJQRCrit}{7} %
\newcommand{\DemoTOneRowJRRejections}{0} %
\newcommand{\DemoTOneRowJRK}{32} %
\newcommand{\DemoTOneRowJRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJRMeanE}{0.0003060335831} %
\newcommand{\DemoTOneRowJRSeE}{0.0002293351905} %
\newcommand{\DemoTOneRowJRRCrit}{7} %
\newcommand{\DemoTOneRowJSRejections}{0} %
\newcommand{\DemoTOneRowJSK}{32} %
\newcommand{\DemoTOneRowJSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJSMeanE}{1.435425272} %
\newcommand{\DemoTOneRowJSSeE}{0.6243277129} %
\newcommand{\DemoTOneRowJSRCrit}{7} %
\newcommand{\DemoTOneRowJTRejections}{0} %
\newcommand{\DemoTOneRowJTK}{32} %
\newcommand{\DemoTOneRowJTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJTMeanE}{0.647150586} %
\newcommand{\DemoTOneRowJTSeE}{0.04096807815} %
\newcommand{\DemoTOneRowJTRCrit}{7} %
\newcommand{\DemoTOneRowJURejections}{0} %
\newcommand{\DemoTOneRowJUK}{32} %
\newcommand{\DemoTOneRowJUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJUMeanE}{1.003691063} %
\newcommand{\DemoTOneRowJUSeE}{0.004465984069} %
\newcommand{\DemoTOneRowJURCrit}{7} %
\newcommand{\DemoTOneRowJVRejections}{0} %
\newcommand{\DemoTOneRowJVK}{32} %
\newcommand{\DemoTOneRowJVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJVMeanE}{0.2841055165} %
\newcommand{\DemoTOneRowJVSeE}{0.1779650769} %
\newcommand{\DemoTOneRowJVRCrit}{7} %
\newcommand{\DemoTOneRowJWRejections}{0} %
\newcommand{\DemoTOneRowJWK}{32} %
\newcommand{\DemoTOneRowJWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJWMeanE}{3.143685884e-42} %
\newcommand{\DemoTOneRowJWSeE}{2.20291207e-42} %
\newcommand{\DemoTOneRowJWRCrit}{7} %
\newcommand{\DemoTOneRowJXRejections}{0} %
\newcommand{\DemoTOneRowJXK}{32} %
\newcommand{\DemoTOneRowJXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJXMeanE}{3.143685884e-42} %
\newcommand{\DemoTOneRowJXSeE}{2.20291207e-42} %
\newcommand{\DemoTOneRowJXRCrit}{7} %
\newcommand{\DemoTOneRowJYRejections}{0} %
\newcommand{\DemoTOneRowJYK}{32} %
\newcommand{\DemoTOneRowJYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJYMeanE}{0.4394108718} %
\newcommand{\DemoTOneRowJYSeE}{0.2557168407} %
\newcommand{\DemoTOneRowJYRCrit}{7} %
\newcommand{\DemoTOneRowJZRejections}{0} %
\newcommand{\DemoTOneRowJZK}{32} %
\newcommand{\DemoTOneRowJZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowJZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowJZMeanE}{0.9635577338} %
\newcommand{\DemoTOneRowJZSeE}{0.02627738669} %
\newcommand{\DemoTOneRowJZRCrit}{7} %
\newcommand{\DemoTOneRowKARejections}{0} %
\newcommand{\DemoTOneRowKAK}{32} %
\newcommand{\DemoTOneRowKACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKAMeanE}{0.9991683904} %
\newcommand{\DemoTOneRowKASeE}{0.002673788596} %
\newcommand{\DemoTOneRowKARCrit}{7} %
\newcommand{\DemoTOneRowKBRejections}{0} %
\newcommand{\DemoTOneRowKBK}{32} %
\newcommand{\DemoTOneRowKBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKBMeanE}{0.0006129419188} %
\newcommand{\DemoTOneRowKBSeE}{0.0005860613931} %
\newcommand{\DemoTOneRowKBRCrit}{7} %
\newcommand{\DemoTOneRowKCRejections}{0} %
\newcommand{\DemoTOneRowKCK}{32} %
\newcommand{\DemoTOneRowKCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKCMeanE}{2.989955538e-97} %
\newcommand{\DemoTOneRowKCSeE}{2.917722963e-97} %
\newcommand{\DemoTOneRowKCRCrit}{7} %
\newcommand{\DemoTOneRowKDRejections}{0} %
\newcommand{\DemoTOneRowKDK}{32} %
\newcommand{\DemoTOneRowKDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKDMeanE}{2.989955538e-97} %
\newcommand{\DemoTOneRowKDSeE}{2.917722963e-97} %
\newcommand{\DemoTOneRowKDRCrit}{7} %
\newcommand{\DemoTOneRowKERejections}{0} %
\newcommand{\DemoTOneRowKEK}{32} %
\newcommand{\DemoTOneRowKECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKEMeanE}{0.6684403369} %
\newcommand{\DemoTOneRowKESeE}{0.1058553513} %
\newcommand{\DemoTOneRowKERCrit}{7} %
\newcommand{\DemoTOneRowKFRejections}{0} %
\newcommand{\DemoTOneRowKFK}{32} %
\newcommand{\DemoTOneRowKFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKFMeanE}{0.08983709413} %
\newcommand{\DemoTOneRowKFSeE}{0.02309037268} %
\newcommand{\DemoTOneRowKFRCrit}{7} %
\newcommand{\DemoTOneRowKGRejections}{0} %
\newcommand{\DemoTOneRowKGK}{32} %
\newcommand{\DemoTOneRowKGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKGMeanE}{0.9958035907} %
\newcommand{\DemoTOneRowKGSeE}{0.003279655518} %
\newcommand{\DemoTOneRowKGRCrit}{7} %
\newcommand{\DemoTOneRowKHRejections}{0} %
\newcommand{\DemoTOneRowKHK}{32} %
\newcommand{\DemoTOneRowKHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKHMeanE}{1.583059406e-08} %
\newcommand{\DemoTOneRowKHSeE}{1.035702554e-08} %
\newcommand{\DemoTOneRowKHRCrit}{7} %
\newcommand{\DemoTOneRowKIRejections}{0} %
\newcommand{\DemoTOneRowKIK}{32} %
\newcommand{\DemoTOneRowKICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKIMeanE}{1} %
\newcommand{\DemoTOneRowKISeE}{0} %
\newcommand{\DemoTOneRowKIRCrit}{7} %
\newcommand{\DemoTOneRowKJRejections}{0} %
\newcommand{\DemoTOneRowKJK}{32} %
\newcommand{\DemoTOneRowKJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKJMeanE}{1} %
\newcommand{\DemoTOneRowKJSeE}{0} %
\newcommand{\DemoTOneRowKJRCrit}{7} %
\newcommand{\DemoTOneRowKKRejections}{0} %
\newcommand{\DemoTOneRowKKK}{32} %
\newcommand{\DemoTOneRowKKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKKMeanE}{1} %
\newcommand{\DemoTOneRowKKSeE}{0} %
\newcommand{\DemoTOneRowKKRCrit}{7} %
\newcommand{\DemoTOneRowKLRejections}{0} %
\newcommand{\DemoTOneRowKLK}{32} %
\newcommand{\DemoTOneRowKLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKLMeanE}{1} %
\newcommand{\DemoTOneRowKLSeE}{0} %
\newcommand{\DemoTOneRowKLRCrit}{7} %
\newcommand{\DemoTOneRowKMRejections}{0} %
\newcommand{\DemoTOneRowKMK}{32} %
\newcommand{\DemoTOneRowKMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKMMeanE}{1.571842942e-42} %
\newcommand{\DemoTOneRowKMSeE}{1.101456035e-42} %
\newcommand{\DemoTOneRowKMRCrit}{7} %
\newcommand{\DemoTOneRowKNRejections}{0} %
\newcommand{\DemoTOneRowKNK}{32} %
\newcommand{\DemoTOneRowKNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKNMeanE}{1.571842942e-42} %
\newcommand{\DemoTOneRowKNSeE}{1.101456035e-42} %
\newcommand{\DemoTOneRowKNRCrit}{7} %
\newcommand{\DemoTOneRowKORejections}{0} %
\newcommand{\DemoTOneRowKOK}{32} %
\newcommand{\DemoTOneRowKOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKOMeanE}{0.5539256043} %
\newcommand{\DemoTOneRowKOSeE}{0.1332758067} %
\newcommand{\DemoTOneRowKORCrit}{7} %
\newcommand{\DemoTOneRowKPRejections}{0} %
\newcommand{\DemoTOneRowKPK}{32} %
\newcommand{\DemoTOneRowKPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKPMeanE}{0.526697414} %
\newcommand{\DemoTOneRowKPSeE}{0.01612992819} %
\newcommand{\DemoTOneRowKPRCrit}{7} %
\newcommand{\DemoTOneRowKQRejections}{0} %
\newcommand{\DemoTOneRowKQK}{32} %
\newcommand{\DemoTOneRowKQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKQMeanE}{0.9974859905} %
\newcommand{\DemoTOneRowKQSeE}{0.002360640868} %
\newcommand{\DemoTOneRowKQRCrit}{7} %
\newcommand{\DemoTOneRowKRRejections}{0} %
\newcommand{\DemoTOneRowKRK}{32} %
\newcommand{\DemoTOneRowKRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKRMeanE}{0.0003064788747} %
\newcommand{\DemoTOneRowKRSeE}{0.0002930304375} %
\newcommand{\DemoTOneRowKRRCrit}{7} %
\newcommand{\DemoTOneRowKSRejections}{0} %
\newcommand{\DemoTOneRowKSK}{32} %
\newcommand{\DemoTOneRowKSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKSMeanE}{4.231287359e-162} %
\newcommand{\DemoTOneRowKSSeE}{4.231287279e-162} %
\newcommand{\DemoTOneRowKSRCrit}{7} %
\newcommand{\DemoTOneRowKTRejections}{0} %
\newcommand{\DemoTOneRowKTK}{32} %
\newcommand{\DemoTOneRowKTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKTMeanE}{1.055685234} %
\newcommand{\DemoTOneRowKTSeE}{0.02645827365} %
\newcommand{\DemoTOneRowKTRCrit}{7} %
\newcommand{\DemoTOneRowKURejections}{0} %
\newcommand{\DemoTOneRowKUK}{32} %
\newcommand{\DemoTOneRowKUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKUMeanE}{1.090566845} %
\newcommand{\DemoTOneRowKUSeE}{0.1148692952} %
\newcommand{\DemoTOneRowKURCrit}{7} %
\newcommand{\DemoTOneRowKVRejections}{0} %
\newcommand{\DemoTOneRowKVK}{32} %
\newcommand{\DemoTOneRowKVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKVMeanE}{1.060623662} %
\newcommand{\DemoTOneRowKVSeE}{0.02277738054} %
\newcommand{\DemoTOneRowKVRCrit}{7} %
\newcommand{\DemoTOneRowKWRejections}{0} %
\newcommand{\DemoTOneRowKWK}{32} %
\newcommand{\DemoTOneRowKWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKWMeanE}{1.011047215} %
\newcommand{\DemoTOneRowKWSeE}{0.004545280135} %
\newcommand{\DemoTOneRowKWRCrit}{7} %
\newcommand{\DemoTOneRowKXRejections}{0} %
\newcommand{\DemoTOneRowKXK}{32} %
\newcommand{\DemoTOneRowKXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKXMeanE}{7.421473772e-08} %
\newcommand{\DemoTOneRowKXSeE}{6.744323291e-08} %
\newcommand{\DemoTOneRowKXRCrit}{7} %
\newcommand{\DemoTOneRowKYRejections}{0} %
\newcommand{\DemoTOneRowKYK}{32} %
\newcommand{\DemoTOneRowKYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKYMeanE}{0} %
\newcommand{\DemoTOneRowKYSeE}{0} %
\newcommand{\DemoTOneRowKYRCrit}{7} %
\newcommand{\DemoTOneRowKZRejections}{0} %
\newcommand{\DemoTOneRowKZK}{32} %
\newcommand{\DemoTOneRowKZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowKZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowKZMeanE}{1.049604157} %
\newcommand{\DemoTOneRowKZSeE}{0.1191934085} %
\newcommand{\DemoTOneRowKZRCrit}{7} %
\newcommand{\DemoTOneRowLARejections}{0} %
\newcommand{\DemoTOneRowLAK}{32} %
\newcommand{\DemoTOneRowLACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLAMeanE}{1.042920314} %
\newcommand{\DemoTOneRowLASeE}{0.167973376} %
\newcommand{\DemoTOneRowLARCrit}{7} %
\newcommand{\DemoTOneRowLBRejections}{0} %
\newcommand{\DemoTOneRowLBK}{32} %
\newcommand{\DemoTOneRowLBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLBMeanE}{1.087082757} %
\newcommand{\DemoTOneRowLBSeE}{0.1121803079} %
\newcommand{\DemoTOneRowLBRCrit}{7} %
\newcommand{\DemoTOneRowLCRejections}{0} %
\newcommand{\DemoTOneRowLCK}{32} %
\newcommand{\DemoTOneRowLCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLCMeanE}{1.004675745} %
\newcommand{\DemoTOneRowLCSeE}{0.02015989039} %
\newcommand{\DemoTOneRowLCRCrit}{7} %
\newcommand{\DemoTOneRowLDRejections}{0} %
\newcommand{\DemoTOneRowLDK}{32} %
\newcommand{\DemoTOneRowLDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLDMeanE}{1.326750878e-11} %
\newcommand{\DemoTOneRowLDSeE}{8.188098382e-12} %
\newcommand{\DemoTOneRowLDRCrit}{7} %
\newcommand{\DemoTOneRowLERejections}{0} %
\newcommand{\DemoTOneRowLEK}{32} %
\newcommand{\DemoTOneRowLECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLEMeanE}{1} %
\newcommand{\DemoTOneRowLESeE}{0} %
\newcommand{\DemoTOneRowLERCrit}{7} %
\newcommand{\DemoTOneRowLFRejections}{0} %
\newcommand{\DemoTOneRowLFK}{32} %
\newcommand{\DemoTOneRowLFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLFMeanE}{1} %
\newcommand{\DemoTOneRowLFSeE}{0} %
\newcommand{\DemoTOneRowLFRCrit}{7} %
\newcommand{\DemoTOneRowLGRejections}{0} %
\newcommand{\DemoTOneRowLGK}{32} %
\newcommand{\DemoTOneRowLGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLGMeanE}{1} %
\newcommand{\DemoTOneRowLGSeE}{0} %
\newcommand{\DemoTOneRowLGRCrit}{7} %
\newcommand{\DemoTOneRowLHRejections}{0} %
\newcommand{\DemoTOneRowLHK}{32} %
\newcommand{\DemoTOneRowLHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLHMeanE}{1} %
\newcommand{\DemoTOneRowLHSeE}{0} %
\newcommand{\DemoTOneRowLHRCrit}{7} %
\newcommand{\DemoTOneRowLIRejections}{0} %
\newcommand{\DemoTOneRowLIK}{32} %
\newcommand{\DemoTOneRowLICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLIMeanE}{2.115643679e-162} %
\newcommand{\DemoTOneRowLISeE}{2.11564364e-162} %
\newcommand{\DemoTOneRowLIRCrit}{7} %
\newcommand{\DemoTOneRowLJRejections}{0} %
\newcommand{\DemoTOneRowLJK}{32} %
\newcommand{\DemoTOneRowLJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLJMeanE}{1.052644695} %
\newcommand{\DemoTOneRowLJSeE}{0.0657862185} %
\newcommand{\DemoTOneRowLJRCrit}{7} %
\newcommand{\DemoTOneRowLKRejections}{0} %
\newcommand{\DemoTOneRowLKK}{32} %
\newcommand{\DemoTOneRowLKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLKMeanE}{1.06674358} %
\newcommand{\DemoTOneRowLKSeE}{0.1167587124} %
\newcommand{\DemoTOneRowLKRCrit}{7} %
\newcommand{\DemoTOneRowLLRejections}{0} %
\newcommand{\DemoTOneRowLLK}{32} %
\newcommand{\DemoTOneRowLLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLLMeanE}{1.073853209} %
\newcommand{\DemoTOneRowLLSeE}{0.06112118773} %
\newcommand{\DemoTOneRowLLRCrit}{7} %
\newcommand{\DemoTOneRowLMRejections}{0} %
\newcommand{\DemoTOneRowLMK}{32} %
\newcommand{\DemoTOneRowLMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLMMeanE}{1.00786148} %
\newcommand{\DemoTOneRowLMSeE}{0.01119962633} %
\newcommand{\DemoTOneRowLMRCrit}{7} %
\newcommand{\DemoTOneRowLNRejections}{0} %
\newcommand{\DemoTOneRowLNK}{32} %
\newcommand{\DemoTOneRowLNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLNMeanE}{3.711400261e-08} %
\newcommand{\DemoTOneRowLNSeE}{3.372138915e-08} %
\newcommand{\DemoTOneRowLNRCrit}{7} %
\newcommand{\DemoTOneRowLORejections}{0} %
\newcommand{\DemoTOneRowLOK}{32} %
\newcommand{\DemoTOneRowLOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLOMeanE}{4.732932821e-18} %
\newcommand{\DemoTOneRowLOSeE}{4.732932821e-18} %
\newcommand{\DemoTOneRowLORCrit}{7} %
\newcommand{\DemoTOneRowLPRejections}{0} %
\newcommand{\DemoTOneRowLPK}{32} %
\newcommand{\DemoTOneRowLPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLPMeanE}{4.732932821e-18} %
\newcommand{\DemoTOneRowLPSeE}{4.732932821e-18} %
\newcommand{\DemoTOneRowLPRCrit}{7} %
\newcommand{\DemoTOneRowLQRejections}{0} %
\newcommand{\DemoTOneRowLQK}{32} %
\newcommand{\DemoTOneRowLQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLQMeanE}{1.178841135} %
\newcommand{\DemoTOneRowLQSeE}{0.6115925952} %
\newcommand{\DemoTOneRowLQRCrit}{7} %
\newcommand{\DemoTOneRowLRRejections}{0} %
\newcommand{\DemoTOneRowLRK}{32} %
\newcommand{\DemoTOneRowLRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLRMeanE}{0.8246110727} %
\newcommand{\DemoTOneRowLRSeE}{0.06741238833} %
\newcommand{\DemoTOneRowLRRCrit}{7} %
\newcommand{\DemoTOneRowLSRejections}{0} %
\newcommand{\DemoTOneRowLSK}{32} %
\newcommand{\DemoTOneRowLSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLSMeanE}{1.00069149} %
\newcommand{\DemoTOneRowLSSeE}{0.001776765794} %
\newcommand{\DemoTOneRowLSRCrit}{7} %
\newcommand{\DemoTOneRowLTRejections}{0} %
\newcommand{\DemoTOneRowLTK}{32} %
\newcommand{\DemoTOneRowLTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLTMeanE}{0.003587156029} %
\newcommand{\DemoTOneRowLTSeE}{0.00176701198} %
\newcommand{\DemoTOneRowLTRCrit}{7} %
\newcommand{\DemoTOneRowLURejections}{0} %
\newcommand{\DemoTOneRowLUK}{32} %
\newcommand{\DemoTOneRowLUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLUMeanE}{8.011861319e-167} %
\newcommand{\DemoTOneRowLUSeE}{8.011861319e-167} %
\newcommand{\DemoTOneRowLURCrit}{7} %
\newcommand{\DemoTOneRowLVRejections}{0} %
\newcommand{\DemoTOneRowLVK}{32} %
\newcommand{\DemoTOneRowLVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLVMeanE}{8.011861319e-167} %
\newcommand{\DemoTOneRowLVSeE}{8.011861319e-167} %
\newcommand{\DemoTOneRowLVRCrit}{7} %
\newcommand{\DemoTOneRowLWRejections}{0} %
\newcommand{\DemoTOneRowLWK}{32} %
\newcommand{\DemoTOneRowLWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLWMeanE}{0.9613898922} %
\newcommand{\DemoTOneRowLWSeE}{0.2039976043} %
\newcommand{\DemoTOneRowLWRCrit}{7} %
\newcommand{\DemoTOneRowLXRejections}{0} %
\newcommand{\DemoTOneRowLXK}{32} %
\newcommand{\DemoTOneRowLXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLXMeanE}{4.537606966e-05} %
\newcommand{\DemoTOneRowLXSeE}{4.27376468e-05} %
\newcommand{\DemoTOneRowLXRCrit}{7} %
\newcommand{\DemoTOneRowLYRejections}{0} %
\newcommand{\DemoTOneRowLYK}{32} %
\newcommand{\DemoTOneRowLYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLYMeanE}{0.9996250481} %
\newcommand{\DemoTOneRowLYSeE}{0.004843378058} %
\newcommand{\DemoTOneRowLYRCrit}{7} %
\newcommand{\DemoTOneRowLZRejections}{0} %
\newcommand{\DemoTOneRowLZK}{32} %
\newcommand{\DemoTOneRowLZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowLZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowLZMeanE}{1.35047215e-09} %
\newcommand{\DemoTOneRowLZSeE}{8.864259886e-10} %
\newcommand{\DemoTOneRowLZRCrit}{7} %
\newcommand{\DemoTOneRowMARejections}{0} %
\newcommand{\DemoTOneRowMAK}{32} %
\newcommand{\DemoTOneRowMACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMAMeanE}{1} %
\newcommand{\DemoTOneRowMASeE}{0} %
\newcommand{\DemoTOneRowMARCrit}{7} %
\newcommand{\DemoTOneRowMBRejections}{0} %
\newcommand{\DemoTOneRowMBK}{32} %
\newcommand{\DemoTOneRowMBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMBMeanE}{1} %
\newcommand{\DemoTOneRowMBSeE}{0} %
\newcommand{\DemoTOneRowMBRCrit}{7} %
\newcommand{\DemoTOneRowMCRejections}{0} %
\newcommand{\DemoTOneRowMCK}{32} %
\newcommand{\DemoTOneRowMCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMCMeanE}{1} %
\newcommand{\DemoTOneRowMCSeE}{0} %
\newcommand{\DemoTOneRowMCRCrit}{7} %
\newcommand{\DemoTOneRowMDRejections}{0} %
\newcommand{\DemoTOneRowMDK}{32} %
\newcommand{\DemoTOneRowMDCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMDMeanE}{1} %
\newcommand{\DemoTOneRowMDSeE}{0} %
\newcommand{\DemoTOneRowMDRCrit}{7} %
\newcommand{\DemoTOneRowMERejections}{0} %
\newcommand{\DemoTOneRowMEK}{32} %
\newcommand{\DemoTOneRowMECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMEMeanE}{2.36646641e-18} %
\newcommand{\DemoTOneRowMESeE}{2.36646641e-18} %
\newcommand{\DemoTOneRowMERCrit}{7} %
\newcommand{\DemoTOneRowMFRejections}{0} %
\newcommand{\DemoTOneRowMFK}{32} %
\newcommand{\DemoTOneRowMFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMFMeanE}{2.36646641e-18} %
\newcommand{\DemoTOneRowMFSeE}{2.36646641e-18} %
\newcommand{\DemoTOneRowMFRCrit}{7} %
\newcommand{\DemoTOneRowMGRejections}{0} %
\newcommand{\DemoTOneRowMGK}{32} %
\newcommand{\DemoTOneRowMGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMGMeanE}{1.070115514} %
\newcommand{\DemoTOneRowMGSeE}{0.3249543247} %
\newcommand{\DemoTOneRowMGRCrit}{7} %
\newcommand{\DemoTOneRowMHRejections}{0} %
\newcommand{\DemoTOneRowMHK}{32} %
\newcommand{\DemoTOneRowMHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMHMeanE}{0.4123282244} %
\newcommand{\DemoTOneRowMHSeE}{0.03371039413} %
\newcommand{\DemoTOneRowMHRCrit}{7} %
\newcommand{\DemoTOneRowMIRejections}{0} %
\newcommand{\DemoTOneRowMIK}{32} %
\newcommand{\DemoTOneRowMICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMIMeanE}{1.000158269} %
\newcommand{\DemoTOneRowMISeE}{0.002634606231} %
\newcommand{\DemoTOneRowMIRCrit}{7} %
\newcommand{\DemoTOneRowMJRejections}{0} %
\newcommand{\DemoTOneRowMJK}{32} %
\newcommand{\DemoTOneRowMJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMJMeanE}{0.00179357869} %
\newcommand{\DemoTOneRowMJSeE}{0.0008835059465} %
\newcommand{\DemoTOneRowMJRCrit}{7} %
\newcommand{\DemoTOneRowMKRejections}{0} %
\newcommand{\DemoTOneRowMKK}{32} %
\newcommand{\DemoTOneRowMKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMKMeanE}{5.59432259e-184} %
\newcommand{\DemoTOneRowMKSeE}{5.59432259e-184} %
\newcommand{\DemoTOneRowMKRCrit}{7} %
\newcommand{\DemoTOneRowMLRejections}{0} %
\newcommand{\DemoTOneRowMLK}{32} %
\newcommand{\DemoTOneRowMLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMLMeanE}{5.59432259e-184} %
\newcommand{\DemoTOneRowMLSeE}{5.59432259e-184} %
\newcommand{\DemoTOneRowMLRCrit}{7} %
\newcommand{\DemoTOneRowMMRejections}{0} %
\newcommand{\DemoTOneRowMMK}{32} %
\newcommand{\DemoTOneRowMMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMMMeanE}{0.1923351507} %
\newcommand{\DemoTOneRowMMSeE}{0.1135384145} %
\newcommand{\DemoTOneRowMMRCrit}{7} %
\newcommand{\DemoTOneRowMNRejections}{0} %
\newcommand{\DemoTOneRowMNK}{32} %
\newcommand{\DemoTOneRowMNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMNMeanE}{1.015006032} %
\newcommand{\DemoTOneRowMNSeE}{0.03475480611} %
\newcommand{\DemoTOneRowMNRCrit}{7} %
\newcommand{\DemoTOneRowMORejections}{0} %
\newcommand{\DemoTOneRowMOK}{32} %
\newcommand{\DemoTOneRowMOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMOMeanE}{1.001284712} %
\newcommand{\DemoTOneRowMOSeE}{0.002320920003} %
\newcommand{\DemoTOneRowMORCrit}{7} %
\newcommand{\DemoTOneRowMPRejections}{0} %
\newcommand{\DemoTOneRowMPK}{32} %
\newcommand{\DemoTOneRowMPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMPMeanE}{8.062790274e-06} %
\newcommand{\DemoTOneRowMPSeE}{5.701357506e-06} %
\newcommand{\DemoTOneRowMPRCrit}{7} %
\newcommand{\DemoTOneRowMQRejections}{0} %
\newcommand{\DemoTOneRowMQK}{32} %
\newcommand{\DemoTOneRowMQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMQMeanE}{0} %
\newcommand{\DemoTOneRowMQSeE}{0} %
\newcommand{\DemoTOneRowMQRCrit}{7} %
\newcommand{\DemoTOneRowMRRejections}{0} %
\newcommand{\DemoTOneRowMRK}{32} %
\newcommand{\DemoTOneRowMRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMRMeanE}{0} %
\newcommand{\DemoTOneRowMRSeE}{0} %
\newcommand{\DemoTOneRowMRRCrit}{7} %
\newcommand{\DemoTOneRowMSRejections}{0} %
\newcommand{\DemoTOneRowMSK}{32} %
\newcommand{\DemoTOneRowMSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMSMeanE}{0.897411009} %
\newcommand{\DemoTOneRowMSSeE}{0.1914762971} %
\newcommand{\DemoTOneRowMSRCrit}{7} %
\newcommand{\DemoTOneRowMTRejections}{1} %
\newcommand{\DemoTOneRowMTK}{32} %
\newcommand{\DemoTOneRowMTCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowMTCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowMTMeanE}{3.612691245} %
\newcommand{\DemoTOneRowMTSeE}{3.466629162} %
\newcommand{\DemoTOneRowMTRCrit}{7} %
\newcommand{\DemoTOneRowMURejections}{0} %
\newcommand{\DemoTOneRowMUK}{32} %
\newcommand{\DemoTOneRowMUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMUMeanE}{1.002447383} %
\newcommand{\DemoTOneRowMUSeE}{0.002936937439} %
\newcommand{\DemoTOneRowMURCrit}{7} %
\newcommand{\DemoTOneRowMVRejections}{0} %
\newcommand{\DemoTOneRowMVK}{32} %
\newcommand{\DemoTOneRowMVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMVMeanE}{1.177056595e-09} %
\newcommand{\DemoTOneRowMVSeE}{1.047621897e-09} %
\newcommand{\DemoTOneRowMVRCrit}{7} %
\newcommand{\DemoTOneRowMWRejections}{0} %
\newcommand{\DemoTOneRowMWK}{32} %
\newcommand{\DemoTOneRowMWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMWMeanE}{1} %
\newcommand{\DemoTOneRowMWSeE}{0} %
\newcommand{\DemoTOneRowMWRCrit}{7} %
\newcommand{\DemoTOneRowMXRejections}{0} %
\newcommand{\DemoTOneRowMXK}{32} %
\newcommand{\DemoTOneRowMXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMXMeanE}{1} %
\newcommand{\DemoTOneRowMXSeE}{0} %
\newcommand{\DemoTOneRowMXRCrit}{7} %
\newcommand{\DemoTOneRowMYRejections}{0} %
\newcommand{\DemoTOneRowMYK}{32} %
\newcommand{\DemoTOneRowMYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMYMeanE}{1} %
\newcommand{\DemoTOneRowMYSeE}{0} %
\newcommand{\DemoTOneRowMYRCrit}{7} %
\newcommand{\DemoTOneRowMZRejections}{0} %
\newcommand{\DemoTOneRowMZK}{32} %
\newcommand{\DemoTOneRowMZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowMZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowMZMeanE}{1} %
\newcommand{\DemoTOneRowMZSeE}{0} %
\newcommand{\DemoTOneRowMZRCrit}{7} %
\newcommand{\DemoTOneRowNARejections}{0} %
\newcommand{\DemoTOneRowNAK}{32} %
\newcommand{\DemoTOneRowNACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNAMeanE}{2.797161295e-184} %
\newcommand{\DemoTOneRowNASeE}{2.797161295e-184} %
\newcommand{\DemoTOneRowNARCrit}{7} %
\newcommand{\DemoTOneRowNBRejections}{0} %
\newcommand{\DemoTOneRowNBK}{32} %
\newcommand{\DemoTOneRowNBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNBMeanE}{2.797161295e-184} %
\newcommand{\DemoTOneRowNBSeE}{2.797161295e-184} %
\newcommand{\DemoTOneRowNBRCrit}{7} %
\newcommand{\DemoTOneRowNCRejections}{0} %
\newcommand{\DemoTOneRowNCK}{32} %
\newcommand{\DemoTOneRowNCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNCMeanE}{0.5448730798} %
\newcommand{\DemoTOneRowNCSeE}{0.1075405928} %
\newcommand{\DemoTOneRowNCRCrit}{7} %
\newcommand{\DemoTOneRowNDRejections}{1} %
\newcommand{\DemoTOneRowNDK}{32} %
\newcommand{\DemoTOneRowNDCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowNDCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowNDMeanE}{2.313848639} %
\newcommand{\DemoTOneRowNDSeE}{1.731762827} %
\newcommand{\DemoTOneRowNDRCrit}{7} %
\newcommand{\DemoTOneRowNERejections}{0} %
\newcommand{\DemoTOneRowNEK}{32} %
\newcommand{\DemoTOneRowNECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNEMeanE}{1.001866048} %
\newcommand{\DemoTOneRowNESeE}{0.001986709976} %
\newcommand{\DemoTOneRowNERCrit}{7} %
\newcommand{\DemoTOneRowNFRejections}{0} %
\newcommand{\DemoTOneRowNFK}{32} %
\newcommand{\DemoTOneRowNFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNFMeanE}{4.031983665e-06} %
\newcommand{\DemoTOneRowNFSeE}{2.850652293e-06} %
\newcommand{\DemoTOneRowNFRCrit}{7} %
\newcommand{\DemoTOneRowNGRejections}{0} %
\newcommand{\DemoTOneRowNGK}{32} %
\newcommand{\DemoTOneRowNGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNGMeanE}{0} %
\newcommand{\DemoTOneRowNGSeE}{0} %
\newcommand{\DemoTOneRowNGRCrit}{7} %
\newcommand{\DemoTOneRowNHRejections}{0} %
\newcommand{\DemoTOneRowNHK}{32} %
\newcommand{\DemoTOneRowNHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNHMeanE}{0.9987294223} %
\newcommand{\DemoTOneRowNHSeE}{0.02518192334} %
\newcommand{\DemoTOneRowNHRCrit}{7} %
\newcommand{\DemoTOneRowNIRejections}{0} %
\newcommand{\DemoTOneRowNIK}{32} %
\newcommand{\DemoTOneRowNICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNIMeanE}{0.9791809431} %
\newcommand{\DemoTOneRowNISeE}{0.2075230607} %
\newcommand{\DemoTOneRowNIRCrit}{7} %
\newcommand{\DemoTOneRowNJRejections}{0} %
\newcommand{\DemoTOneRowNJK}{32} %
\newcommand{\DemoTOneRowNJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNJMeanE}{1.019983392} %
\newcommand{\DemoTOneRowNJSeE}{0.02096710344} %
\newcommand{\DemoTOneRowNJRCrit}{7} %
\newcommand{\DemoTOneRowNKRejections}{0} %
\newcommand{\DemoTOneRowNKK}{32} %
\newcommand{\DemoTOneRowNKCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNKCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNKMeanE}{1.000000462} %
\newcommand{\DemoTOneRowNKSeE}{0.004125989384} %
\newcommand{\DemoTOneRowNKRCrit}{7} %
\newcommand{\DemoTOneRowNLRejections}{0} %
\newcommand{\DemoTOneRowNLK}{32} %
\newcommand{\DemoTOneRowNLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNLMeanE}{1.130991404e-11} %
\newcommand{\DemoTOneRowNLSeE}{7.045511134e-12} %
\newcommand{\DemoTOneRowNLRCrit}{7} %
\newcommand{\DemoTOneRowNMRejections}{0} %
\newcommand{\DemoTOneRowNMK}{32} %
\newcommand{\DemoTOneRowNMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNMMeanE}{0} %
\newcommand{\DemoTOneRowNMSeE}{0} %
\newcommand{\DemoTOneRowNMRCrit}{7} %
\newcommand{\DemoTOneRowNNRejections}{0} %
\newcommand{\DemoTOneRowNNK}{32} %
\newcommand{\DemoTOneRowNNCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNNCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNNMeanE}{1.131194261} %
\newcommand{\DemoTOneRowNNSeE}{0.1274263961} %
\newcommand{\DemoTOneRowNNRCrit}{7} %
\newcommand{\DemoTOneRowNORejections}{0} %
\newcommand{\DemoTOneRowNOK}{32} %
\newcommand{\DemoTOneRowNOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNOMeanE}{1.206213593} %
\newcommand{\DemoTOneRowNOSeE}{0.2511398464} %
\newcommand{\DemoTOneRowNORCrit}{7} %
\newcommand{\DemoTOneRowNPRejections}{0} %
\newcommand{\DemoTOneRowNPK}{32} %
\newcommand{\DemoTOneRowNPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNPMeanE}{1.088015665} %
\newcommand{\DemoTOneRowNPSeE}{0.1028842843} %
\newcommand{\DemoTOneRowNPRCrit}{7} %
\newcommand{\DemoTOneRowNQRejections}{0} %
\newcommand{\DemoTOneRowNQK}{32} %
\newcommand{\DemoTOneRowNQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNQMeanE}{1.016198693} %
\newcommand{\DemoTOneRowNQSeE}{0.0181865149} %
\newcommand{\DemoTOneRowNQRCrit}{7} %
\newcommand{\DemoTOneRowNRRejections}{0} %
\newcommand{\DemoTOneRowNRK}{32} %
\newcommand{\DemoTOneRowNRCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNRMeanE}{2.034447436e-11} %
\newcommand{\DemoTOneRowNRSeE}{1.299036492e-11} %
\newcommand{\DemoTOneRowNRRCrit}{7} %
\newcommand{\DemoTOneRowNSRejections}{0} %
\newcommand{\DemoTOneRowNSK}{32} %
\newcommand{\DemoTOneRowNSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNSMeanE}{1} %
\newcommand{\DemoTOneRowNSSeE}{0} %
\newcommand{\DemoTOneRowNSRCrit}{7} %
\newcommand{\DemoTOneRowNTRejections}{0} %
\newcommand{\DemoTOneRowNTK}{32} %
\newcommand{\DemoTOneRowNTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNTMeanE}{1} %
\newcommand{\DemoTOneRowNTSeE}{0} %
\newcommand{\DemoTOneRowNTRCrit}{7} %
\newcommand{\DemoTOneRowNURejections}{0} %
\newcommand{\DemoTOneRowNUK}{32} %
\newcommand{\DemoTOneRowNUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNUMeanE}{1} %
\newcommand{\DemoTOneRowNUSeE}{0} %
\newcommand{\DemoTOneRowNURCrit}{7} %
\newcommand{\DemoTOneRowNVRejections}{0} %
\newcommand{\DemoTOneRowNVK}{32} %
\newcommand{\DemoTOneRowNVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNVMeanE}{1} %
\newcommand{\DemoTOneRowNVSeE}{0} %
\newcommand{\DemoTOneRowNVRCrit}{7} %
\newcommand{\DemoTOneRowNWRejections}{0} %
\newcommand{\DemoTOneRowNWK}{32} %
\newcommand{\DemoTOneRowNWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNWMeanE}{0} %
\newcommand{\DemoTOneRowNWSeE}{0} %
\newcommand{\DemoTOneRowNWRCrit}{7} %
\newcommand{\DemoTOneRowNXRejections}{0} %
\newcommand{\DemoTOneRowNXK}{32} %
\newcommand{\DemoTOneRowNXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNXMeanE}{1.064961842} %
\newcommand{\DemoTOneRowNXSeE}{0.06709127713} %
\newcommand{\DemoTOneRowNXRCrit}{7} %
\newcommand{\DemoTOneRowNYRejections}{0} %
\newcommand{\DemoTOneRowNYK}{32} %
\newcommand{\DemoTOneRowNYCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNYMeanE}{1.092697268} %
\newcommand{\DemoTOneRowNYSeE}{0.163824993} %
\newcommand{\DemoTOneRowNYRCrit}{7} %
\newcommand{\DemoTOneRowNZRejections}{0} %
\newcommand{\DemoTOneRowNZK}{32} %
\newcommand{\DemoTOneRowNZCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowNZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowNZMeanE}{1.053999529} %
\newcommand{\DemoTOneRowNZSeE}{0.0517150246} %
\newcommand{\DemoTOneRowNZRCrit}{7} %
\newcommand{\DemoTOneRowOARejections}{0} %
\newcommand{\DemoTOneRowOAK}{32} %
\newcommand{\DemoTOneRowOACpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOAMeanE}{1.008099578} %
\newcommand{\DemoTOneRowOASeE}{0.009685138815} %
\newcommand{\DemoTOneRowOARCrit}{7} %
\newcommand{\DemoTOneRowOBRejections}{0} %
\newcommand{\DemoTOneRowOBK}{32} %
\newcommand{\DemoTOneRowOBCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOBMeanE}{1.58271942e-11} %
\newcommand{\DemoTOneRowOBSeE}{7.180098555e-12} %
\newcommand{\DemoTOneRowOBRCrit}{7} %
\newcommand{\DemoTOneRowOCRejections}{0} %
\newcommand{\DemoTOneRowOCK}{32} %
\newcommand{\DemoTOneRowOCCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOCMeanE}{3.178482516e-287} %
\newcommand{\DemoTOneRowOCSeE}{3.178482516e-287} %
\newcommand{\DemoTOneRowOCRCrit}{7} %
\newcommand{\DemoTOneRowODRejections}{0} %
\newcommand{\DemoTOneRowODK}{32} %
\newcommand{\DemoTOneRowODCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowODCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowODMeanE}{3.178482516e-287} %
\newcommand{\DemoTOneRowODSeE}{3.178482516e-287} %
\newcommand{\DemoTOneRowODRCrit}{7} %
\newcommand{\DemoTOneRowOERejections}{0} %
\newcommand{\DemoTOneRowOEK}{32} %
\newcommand{\DemoTOneRowOECpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOECpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOEMeanE}{0.4499275932} %
\newcommand{\DemoTOneRowOESeE}{0.2542386644} %
\newcommand{\DemoTOneRowOERCrit}{7} %
\newcommand{\DemoTOneRowOFRejections}{0} %
\newcommand{\DemoTOneRowOFK}{32} %
\newcommand{\DemoTOneRowOFCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOFMeanE}{0.1711596835} %
\newcommand{\DemoTOneRowOFSeE}{0.06892859288} %
\newcommand{\DemoTOneRowOFRCrit}{7} %
\newcommand{\DemoTOneRowOGRejections}{0} %
\newcommand{\DemoTOneRowOGK}{32} %
\newcommand{\DemoTOneRowOGCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOGMeanE}{1.002668857} %
\newcommand{\DemoTOneRowOGSeE}{0.00235344911} %
\newcommand{\DemoTOneRowOGRCrit}{7} %
\newcommand{\DemoTOneRowOHRejections}{0} %
\newcommand{\DemoTOneRowOHK}{32} %
\newcommand{\DemoTOneRowOHCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOHMeanE}{9.81465793e-08} %
\newcommand{\DemoTOneRowOHSeE}{9.774544589e-08} %
\newcommand{\DemoTOneRowOHRCrit}{7} %
\newcommand{\DemoTOneRowOIRejections}{0} %
\newcommand{\DemoTOneRowOIK}{32} %
\newcommand{\DemoTOneRowOICpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOIMeanE}{0} %
\newcommand{\DemoTOneRowOISeE}{0} %
\newcommand{\DemoTOneRowOIRCrit}{7} %
\newcommand{\DemoTOneRowOJRejections}{0} %
\newcommand{\DemoTOneRowOJK}{32} %
\newcommand{\DemoTOneRowOJCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOJMeanE}{5.698905071e-225} %
\newcommand{\DemoTOneRowOJSeE}{4.098191229e-225} %
\newcommand{\DemoTOneRowOJRCrit}{7} %
\newcommand{\DemoTOneRowOKRejections}{1} %
\newcommand{\DemoTOneRowOKK}{32} %
\newcommand{\DemoTOneRowOKCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTOneRowOKCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTOneRowOKMeanE}{1.782312878} %
\newcommand{\DemoTOneRowOKSeE}{1.029840335} %
\newcommand{\DemoTOneRowOKRCrit}{7} %
\newcommand{\DemoTOneRowOLRejections}{0} %
\newcommand{\DemoTOneRowOLK}{32} %
\newcommand{\DemoTOneRowOLCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOLMeanE}{6.018396611e-07} %
\newcommand{\DemoTOneRowOLSeE}{3.297034099e-07} %
\newcommand{\DemoTOneRowOLRCrit}{7} %
\newcommand{\DemoTOneRowOMRejections}{0} %
\newcommand{\DemoTOneRowOMK}{32} %
\newcommand{\DemoTOneRowOMCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOMCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOMMeanE}{1.004710772} %
\newcommand{\DemoTOneRowOMSeE}{0.005914528767} %
\newcommand{\DemoTOneRowOMRCrit}{7} %
\newcommand{\DemoTOneRowONRejections}{0} %
\newcommand{\DemoTOneRowONK}{32} %
\newcommand{\DemoTOneRowONCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowONCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowONMeanE}{4.255297715e-12} %
\newcommand{\DemoTOneRowONSeE}{2.426376321e-12} %
\newcommand{\DemoTOneRowONRCrit}{7} %
\newcommand{\DemoTOneRowOORejections}{0} %
\newcommand{\DemoTOneRowOOK}{32} %
\newcommand{\DemoTOneRowOOCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOOCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOOMeanE}{1} %
\newcommand{\DemoTOneRowOOSeE}{0} %
\newcommand{\DemoTOneRowOORCrit}{7} %
\newcommand{\DemoTOneRowOPRejections}{0} %
\newcommand{\DemoTOneRowOPK}{32} %
\newcommand{\DemoTOneRowOPCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOPMeanE}{1} %
\newcommand{\DemoTOneRowOPSeE}{0} %
\newcommand{\DemoTOneRowOPRCrit}{7} %
\newcommand{\DemoTOneRowOQRejections}{0} %
\newcommand{\DemoTOneRowOQK}{32} %
\newcommand{\DemoTOneRowOQCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOQMeanE}{1} %
\newcommand{\DemoTOneRowOQSeE}{0} %
\newcommand{\DemoTOneRowOQRCrit}{7} %
\newcommand{\DemoTOneRowORRejections}{0} %
\newcommand{\DemoTOneRowORK}{32} %
\newcommand{\DemoTOneRowORCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowORCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowORMeanE}{1} %
\newcommand{\DemoTOneRowORSeE}{0} %
\newcommand{\DemoTOneRowORRCrit}{7} %
\newcommand{\DemoTOneRowOSRejections}{0} %
\newcommand{\DemoTOneRowOSK}{32} %
\newcommand{\DemoTOneRowOSCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOSMeanE}{1.589241258e-287} %
\newcommand{\DemoTOneRowOSSeE}{1.589241258e-287} %
\newcommand{\DemoTOneRowOSRCrit}{7} %
\newcommand{\DemoTOneRowOTRejections}{0} %
\newcommand{\DemoTOneRowOTK}{32} %
\newcommand{\DemoTOneRowOTCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOTMeanE}{2.849452535e-225} %
\newcommand{\DemoTOneRowOTSeE}{2.049095614e-225} %
\newcommand{\DemoTOneRowOTRCrit}{7} %
\newcommand{\DemoTOneRowOURejections}{0} %
\newcommand{\DemoTOneRowOUK}{32} %
\newcommand{\DemoTOneRowOUCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOUMeanE}{1.116120236} %
\newcommand{\DemoTOneRowOUSeE}{0.5278703444} %
\newcommand{\DemoTOneRowOURCrit}{7} %
\newcommand{\DemoTOneRowOVRejections}{0} %
\newcommand{\DemoTOneRowOVK}{32} %
\newcommand{\DemoTOneRowOVCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOVMeanE}{0.08558014268} %
\newcommand{\DemoTOneRowOVSeE}{0.03446428319} %
\newcommand{\DemoTOneRowOVRCrit}{7} %
\newcommand{\DemoTOneRowOWRejections}{0} %
\newcommand{\DemoTOneRowOWK}{32} %
\newcommand{\DemoTOneRowOWCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOWMeanE}{1.003689815} %
\newcommand{\DemoTOneRowOWSeE}{0.003327415331} %
\newcommand{\DemoTOneRowOWRCrit}{7} %
\newcommand{\DemoTOneRowOXRejections}{0} %
\newcommand{\DemoTOneRowOXK}{32} %
\newcommand{\DemoTOneRowOXCpNineFiveLower}{0} %
\newcommand{\DemoTOneRowOXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTOneRowOXMeanE}{4.90754173e-08} %
\newcommand{\DemoTOneRowOXSeE}{4.8872691e-08} %
\newcommand{\DemoTOneRowOXRCrit}{7} %
\newcommand{\DemoTTwoRowAMedianLogE}{-5.51038097} %
\newcommand{\DemoTTwoRowAQTwoFiveLogE}{-7.523514872} %
\newcommand{\DemoTTwoRowAQSevenFiveLogE}{-1.971219935} %
\newcommand{\DemoTTwoRowARate}{0.0625} %
\newcommand{\DemoTTwoRowACpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowACpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowAMedianLogRatioToExactBound}{-0.01748424317} %
\newcommand{\DemoTTwoRowBMedianLogE}{-5.51038097} %
\newcommand{\DemoTTwoRowBQTwoFiveLogE}{-7.523514872} %
\newcommand{\DemoTTwoRowBQSevenFiveLogE}{-1.971219935} %
\newcommand{\DemoTTwoRowBRate}{0.0625} %
\newcommand{\DemoTTwoRowBCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowBCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowBMedianLogRatioToExactBound}{-0.01748424317} %
\newcommand{\DemoTTwoRowCMedianLogE}{0.2149451334} %
\newcommand{\DemoTTwoRowCQTwoFiveLogE}{-0.5564076837} %
\newcommand{\DemoTTwoRowCQSevenFiveLogE}{1.415924289} %
\newcommand{\DemoTTwoRowCRate}{0.125} %
\newcommand{\DemoTTwoRowCCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowCCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowCMedianLogRatioToExactBound}{0.0006820132766} %
\newcommand{\DemoTTwoRowDMedianLogE}{-0.01668481993} %
\newcommand{\DemoTTwoRowDQTwoFiveLogE}{-0.1059446031} %
\newcommand{\DemoTTwoRowDQSevenFiveLogE}{0.1515394371} %
\newcommand{\DemoTTwoRowDRate}{0} %
\newcommand{\DemoTTwoRowDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDMedianLogRatioToExactBound}{-5.294034125e-05} %
\newcommand{\DemoTTwoRowEMedianLogE}{0.06490501313} %
\newcommand{\DemoTTwoRowEQTwoFiveLogE}{0.03311607987} %
\newcommand{\DemoTTwoRowEQSevenFiveLogE}{0.1176800027} %
\newcommand{\DemoTTwoRowERate}{0} %
\newcommand{\DemoTTwoRowECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEMedianLogRatioToExactBound}{0.0002059413022} %
\newcommand{\DemoTTwoRowFMedianLogE}{-0.04683584515} %
\newcommand{\DemoTTwoRowFQTwoFiveLogE}{-1.207367737} %
\newcommand{\DemoTTwoRowFQSevenFiveLogE}{1.812836191} %
\newcommand{\DemoTTwoRowFRate}{0.125} %
\newcommand{\DemoTTwoRowFCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowFCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowFMedianLogRatioToExactBound}{-0.0001486084738} %
\newcommand{\DemoTTwoRowGMedianLogE}{-10.68536586} %
\newcommand{\DemoTTwoRowGQTwoFiveLogE}{-13.73116326} %
\newcommand{\DemoTTwoRowGQSevenFiveLogE}{-7.587721541} %
\newcommand{\DemoTTwoRowGRate}{0} %
\newcommand{\DemoTTwoRowGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGMedianLogRatioToExactBound}{-0.03390428649} %
\newcommand{\DemoTTwoRowHMedianLogE}{-10.68536586} %
\newcommand{\DemoTTwoRowHQTwoFiveLogE}{-13.73116326} %
\newcommand{\DemoTTwoRowHQSevenFiveLogE}{-7.587721541} %
\newcommand{\DemoTTwoRowHRate}{0} %
\newcommand{\DemoTTwoRowHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHMedianLogRatioToExactBound}{-0.03390428649} %
\newcommand{\DemoTTwoRowIMedianLogE}{0.5771850592} %
\newcommand{\DemoTTwoRowIQTwoFiveLogE}{-0.4487951142} %
\newcommand{\DemoTTwoRowIQSevenFiveLogE}{1.273650023} %
\newcommand{\DemoTTwoRowIRate}{0.0625} %
\newcommand{\DemoTTwoRowICpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowICpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowIMedianLogRatioToExactBound}{0.0018313877} %
\newcommand{\DemoTTwoRowJMedianLogE}{-0.5221814705} %
\newcommand{\DemoTTwoRowJQTwoFiveLogE}{-0.6966937568} %
\newcommand{\DemoTTwoRowJQSevenFiveLogE}{0.04230089466} %
\newcommand{\DemoTTwoRowJRate}{0} %
\newcommand{\DemoTTwoRowJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJMedianLogRatioToExactBound}{-0.001656863266} %
\newcommand{\DemoTTwoRowKMedianLogE}{0.1103683659} %
\newcommand{\DemoTTwoRowKQTwoFiveLogE}{0.04872131859} %
\newcommand{\DemoTTwoRowKQSevenFiveLogE}{0.1461007173} %
\newcommand{\DemoTTwoRowKRate}{0} %
\newcommand{\DemoTTwoRowKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKMedianLogRatioToExactBound}{0.0003501949064} %
\newcommand{\DemoTTwoRowLMedianLogE}{-0.001551819229} %
\newcommand{\DemoTTwoRowLQTwoFiveLogE}{-1.254683988} %
\newcommand{\DemoTTwoRowLQSevenFiveLogE}{1.038485843} %
\newcommand{\DemoTTwoRowLRate}{0.0625} %
\newcommand{\DemoTTwoRowLCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowLCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowLMedianLogRatioToExactBound}{-4.923867318e-06} %
\newcommand{\DemoTTwoRowMMedianLogE}{14.76878982} %
\newcommand{\DemoTTwoRowMQTwoFiveLogE}{12.97775702} %
\newcommand{\DemoTTwoRowMQSevenFiveLogE}{17.59234515} %
\newcommand{\DemoTTwoRowMRate}{1} %
\newcommand{\DemoTTwoRowMCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowMCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowMMedianLogRatioToExactBound}{0.04686084573} %
\newcommand{\DemoTTwoRowNMedianLogE}{14.76878982} %
\newcommand{\DemoTTwoRowNQTwoFiveLogE}{12.97775702} %
\newcommand{\DemoTTwoRowNQSevenFiveLogE}{17.59234515} %
\newcommand{\DemoTTwoRowNRate}{1} %
\newcommand{\DemoTTwoRowNCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNMedianLogRatioToExactBound}{0.04686084573} %
\newcommand{\DemoTTwoRowOMedianLogE}{14.76878982} %
\newcommand{\DemoTTwoRowOQTwoFiveLogE}{12.97775702} %
\newcommand{\DemoTTwoRowOQSevenFiveLogE}{17.59234515} %
\newcommand{\DemoTTwoRowORate}{1} %
\newcommand{\DemoTTwoRowOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOMedianLogRatioToExactBound}{0.04686084573} %
\newcommand{\DemoTTwoRowPMedianLogE}{14.76878982} %
\newcommand{\DemoTTwoRowPQTwoFiveLogE}{12.97775702} %
\newcommand{\DemoTTwoRowPQSevenFiveLogE}{17.59234515} %
\newcommand{\DemoTTwoRowPRate}{1} %
\newcommand{\DemoTTwoRowPCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowPCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowPMedianLogRatioToExactBound}{0.04686084573} %
\newcommand{\DemoTTwoRowQMedianLogE}{-6.107626351} %
\newcommand{\DemoTTwoRowQQTwoFiveLogE}{-7.880125533} %
\newcommand{\DemoTTwoRowQQSevenFiveLogE}{-2.664244022} %
\newcommand{\DemoTTwoRowQRate}{0} %
\newcommand{\DemoTTwoRowQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQMedianLogRatioToExactBound}{-0.01937928156} %
\newcommand{\DemoTTwoRowRMedianLogE}{-6.107626351} %
\newcommand{\DemoTTwoRowRQTwoFiveLogE}{-7.880125533} %
\newcommand{\DemoTTwoRowRQSevenFiveLogE}{-2.664244022} %
\newcommand{\DemoTTwoRowRRate}{0} %
\newcommand{\DemoTTwoRowRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRMedianLogRatioToExactBound}{-0.01937928156} %
\newcommand{\DemoTTwoRowSMedianLogE}{0.5317283464} %
\newcommand{\DemoTTwoRowSQTwoFiveLogE}{-0.148046621} %
\newcommand{\DemoTTwoRowSQSevenFiveLogE}{1.511656586} %
\newcommand{\DemoTTwoRowSRate}{0.125} %
\newcommand{\DemoTTwoRowSCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowSCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowSMedianLogRatioToExactBound}{0.001687155164} %
\newcommand{\DemoTTwoRowTMedianLogE}{-0.1797546252} %
\newcommand{\DemoTTwoRowTQTwoFiveLogE}{-0.3567116247} %
\newcommand{\DemoTTwoRowTQSevenFiveLogE}{0.05240693812} %
\newcommand{\DemoTTwoRowTRate}{0} %
\newcommand{\DemoTTwoRowTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTMedianLogRatioToExactBound}{-0.0005703550437} %
\newcommand{\DemoTTwoRowUMedianLogE}{0.08530028018} %
\newcommand{\DemoTTwoRowUQTwoFiveLogE}{0.05044115603} %
\newcommand{\DemoTTwoRowUQSevenFiveLogE}{0.1291728974} %
\newcommand{\DemoTTwoRowURate}{0} %
\newcommand{\DemoTTwoRowUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowUMedianLogRatioToExactBound}{0.0002706547604} %
\newcommand{\DemoTTwoRowVMedianLogE}{0.4900723767} %
\newcommand{\DemoTTwoRowVQTwoFiveLogE}{-0.7702934765} %
\newcommand{\DemoTTwoRowVQSevenFiveLogE}{1.615009438} %
\newcommand{\DemoTTwoRowVRate}{0.125} %
\newcommand{\DemoTTwoRowVCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowVCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowVMedianLogRatioToExactBound}{0.001554982251} %
\newcommand{\DemoTTwoRowWMedianLogE}{-4.453438323} %
\newcommand{\DemoTTwoRowWQTwoFiveLogE}{-9.003174015} %
\newcommand{\DemoTTwoRowWQSevenFiveLogE}{0.003113169524} %
\newcommand{\DemoTTwoRowWRate}{0} %
\newcommand{\DemoTTwoRowWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowWMedianLogRatioToExactBound}{-0.01413060168} %
\newcommand{\DemoTTwoRowXMedianLogE}{0.4879594382} %
\newcommand{\DemoTTwoRowXQTwoFiveLogE}{0.4057957891} %
\newcommand{\DemoTTwoRowXQSevenFiveLogE}{0.783726667} %
\newcommand{\DemoTTwoRowXRate}{0} %
\newcommand{\DemoTTwoRowXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowXMedianLogRatioToExactBound}{0.001548277972} %
\newcommand{\DemoTTwoRowYMedianLogE}{0.9102531814} %
\newcommand{\DemoTTwoRowYQTwoFiveLogE}{0.3084540736} %
\newcommand{\DemoTTwoRowYQSevenFiveLogE}{2.461444173} %
\newcommand{\DemoTTwoRowYRate}{0.125} %
\newcommand{\DemoTTwoRowYCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowYCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowYMedianLogRatioToExactBound}{0.002888201026} %
\newcommand{\DemoTTwoRowZMedianLogE}{0.03421833366} %
\newcommand{\DemoTTwoRowZQTwoFiveLogE}{-0.04728715467} %
\newcommand{\DemoTTwoRowZQSevenFiveLogE}{0.11453799} %
\newcommand{\DemoTTwoRowZRate}{0} %
\newcommand{\DemoTTwoRowZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowZMedianLogRatioToExactBound}{0.0001085735578} %
\newcommand{\DemoTTwoRowAAMedianLogE}{0.1003676762} %
\newcommand{\DemoTTwoRowAAQTwoFiveLogE}{0.08358481158} %
\newcommand{\DemoTTwoRowAAQSevenFiveLogE}{0.1518686841} %
\newcommand{\DemoTTwoRowAARate}{0} %
\newcommand{\DemoTTwoRowAACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAAMedianLogRatioToExactBound}{0.0003184630729} %
\newcommand{\DemoTTwoRowABMedianLogE}{0.0902023682} %
\newcommand{\DemoTTwoRowABQTwoFiveLogE}{-0.797810774} %
\newcommand{\DemoTTwoRowABQSevenFiveLogE}{2.494258735} %
\newcommand{\DemoTTwoRowABRate}{0.1875} %
\newcommand{\DemoTTwoRowABCpNineFiveLower}{0.04047373391} %
\newcommand{\DemoTTwoRowABCpNineFiveUpper}{0.4564565462} %
\newcommand{\DemoTTwoRowABMedianLogRatioToExactBound}{0.0002862089117} %
\newcommand{\DemoTTwoRowACMedianLogE}{-31.2222107} %
\newcommand{\DemoTTwoRowACQTwoFiveLogE}{-40.05018589} %
\newcommand{\DemoTTwoRowACQSevenFiveLogE}{-24.50363413} %
\newcommand{\DemoTTwoRowACRate}{0} %
\newcommand{\DemoTTwoRowACCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowACCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowACMedianLogRatioToExactBound}{-0.09906696599} %
\newcommand{\DemoTTwoRowADMedianLogE}{0.2549701685} %
\newcommand{\DemoTTwoRowADQTwoFiveLogE}{0.04250516965} %
\newcommand{\DemoTTwoRowADQSevenFiveLogE}{0.5779938453} %
\newcommand{\DemoTTwoRowADRate}{0} %
\newcommand{\DemoTTwoRowADCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowADCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowADMedianLogRatioToExactBound}{0.000809011292} %
\newcommand{\DemoTTwoRowAEMedianLogE}{-0.1278387652} %
\newcommand{\DemoTTwoRowAEQTwoFiveLogE}{-0.4677380963} %
\newcommand{\DemoTTwoRowAEQSevenFiveLogE}{0.8672504378} %
\newcommand{\DemoTTwoRowAERate}{0} %
\newcommand{\DemoTTwoRowAECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAEMedianLogRatioToExactBound}{-0.000405627863} %
\newcommand{\DemoTTwoRowAFMedianLogE}{-0.1139394145} %
\newcommand{\DemoTTwoRowAFQTwoFiveLogE}{-0.3799753101} %
\newcommand{\DemoTTwoRowAFQSevenFiveLogE}{0.02001043181} %
\newcommand{\DemoTTwoRowAFRate}{0} %
\newcommand{\DemoTTwoRowAFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAFMedianLogRatioToExactBound}{-0.0003615257168} %
\newcommand{\DemoTTwoRowAGMedianLogE}{0.07581721914} %
\newcommand{\DemoTTwoRowAGQTwoFiveLogE}{0.0339086648} %
\newcommand{\DemoTTwoRowAGQSevenFiveLogE}{0.1475880085} %
\newcommand{\DemoTTwoRowAGRate}{0} %
\newcommand{\DemoTTwoRowAGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAGMedianLogRatioToExactBound}{0.0002405653444} %
\newcommand{\DemoTTwoRowAHMedianLogE}{-3.968492329} %
\newcommand{\DemoTTwoRowAHQTwoFiveLogE}{-5.958910218} %
\newcommand{\DemoTTwoRowAHQSevenFiveLogE}{-2.758088547} %
\newcommand{\DemoTTwoRowAHRate}{0} %
\newcommand{\DemoTTwoRowAHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAHMedianLogRatioToExactBound}{-0.01259188526} %
\newcommand{\DemoTTwoRowAIMedianLogE}{13.55071527} %
\newcommand{\DemoTTwoRowAIQTwoFiveLogE}{10.49107898} %
\newcommand{\DemoTTwoRowAIQSevenFiveLogE}{14.6133092} %
\newcommand{\DemoTTwoRowAIRate}{1} %
\newcommand{\DemoTTwoRowAICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowAICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowAIMedianLogRatioToExactBound}{0.04299593842} %
\newcommand{\DemoTTwoRowAJMedianLogE}{1.439474138} %
\newcommand{\DemoTTwoRowAJQTwoFiveLogE}{1.327524301} %
\newcommand{\DemoTTwoRowAJQSevenFiveLogE}{1.53552873} %
\newcommand{\DemoTTwoRowAJRate}{0} %
\newcommand{\DemoTTwoRowAJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAJMedianLogRatioToExactBound}{0.004567400333} %
\newcommand{\DemoTTwoRowAKMedianLogE}{13.55071527} %
\newcommand{\DemoTTwoRowAKQTwoFiveLogE}{10.49107898} %
\newcommand{\DemoTTwoRowAKQSevenFiveLogE}{14.6133092} %
\newcommand{\DemoTTwoRowAKRate}{1} %
\newcommand{\DemoTTwoRowAKCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowAKCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowAKMedianLogRatioToExactBound}{0.04299593842} %
\newcommand{\DemoTTwoRowALMedianLogE}{14.44168183} %
\newcommand{\DemoTTwoRowALQTwoFiveLogE}{11.02681042} %
\newcommand{\DemoTTwoRowALQSevenFiveLogE}{16.1494472} %
\newcommand{\DemoTTwoRowALRate}{1} %
\newcommand{\DemoTTwoRowALCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowALCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowALMedianLogRatioToExactBound}{0.04582294369} %
\newcommand{\DemoTTwoRowAMMedianLogE}{-5.146585504} %
\newcommand{\DemoTTwoRowAMQTwoFiveLogE}{-9.696314985} %
\newcommand{\DemoTTwoRowAMQSevenFiveLogE}{-0.690034011} %
\newcommand{\DemoTTwoRowAMRate}{0} %
\newcommand{\DemoTTwoRowAMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAMMedianLogRatioToExactBound}{-0.01632993307} %
\newcommand{\DemoTTwoRowANMedianLogE}{0.4739413403} %
\newcommand{\DemoTTwoRowANQTwoFiveLogE}{0.3416461941} %
\newcommand{\DemoTTwoRowANQSevenFiveLogE}{0.7039989573} %
\newcommand{\DemoTTwoRowANRate}{0} %
\newcommand{\DemoTTwoRowANCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowANCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowANMedianLogRatioToExactBound}{0.001503799046} %
\newcommand{\DemoTTwoRowAOMedianLogE}{1.35614482} %
\newcommand{\DemoTTwoRowAOQTwoFiveLogE}{0.3585297803} %
\newcommand{\DemoTTwoRowAOQSevenFiveLogE}{1.924218182} %
\newcommand{\DemoTTwoRowAORate}{0.0625} %
\newcommand{\DemoTTwoRowAOCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowAOCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowAOMedianLogRatioToExactBound}{0.004302999363} %
\newcommand{\DemoTTwoRowAPMedianLogE}{-0.02822971858} %
\newcommand{\DemoTTwoRowAPQTwoFiveLogE}{-0.1184192051} %
\newcommand{\DemoTTwoRowAPQSevenFiveLogE}{0.08197555315} %
\newcommand{\DemoTTwoRowAPRate}{0} %
\newcommand{\DemoTTwoRowAPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAPMedianLogRatioToExactBound}{-8.957189476e-05} %
\newcommand{\DemoTTwoRowAQMedianLogE}{0.08639715751} %
\newcommand{\DemoTTwoRowAQQTwoFiveLogE}{0.0692529925} %
\newcommand{\DemoTTwoRowAQQSevenFiveLogE}{0.158014351} %
\newcommand{\DemoTTwoRowAQRate}{0} %
\newcommand{\DemoTTwoRowAQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAQMedianLogRatioToExactBound}{0.0002741351133} %
\newcommand{\DemoTTwoRowARMedianLogE}{0.3203112849} %
\newcommand{\DemoTTwoRowARQTwoFiveLogE}{-1.41975379} %
\newcommand{\DemoTTwoRowARQSevenFiveLogE}{2.176015095} %
\newcommand{\DemoTTwoRowARRate}{0.0625} %
\newcommand{\DemoTTwoRowARCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowARCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowARMedianLogRatioToExactBound}{0.001016336334} %
\newcommand{\DemoTTwoRowASMedianLogE}{-4.178522578} %
\newcommand{\DemoTTwoRowASQTwoFiveLogE}{-5.66313126} %
\newcommand{\DemoTTwoRowASQSevenFiveLogE}{-1.64466517} %
\newcommand{\DemoTTwoRowASRate}{0} %
\newcommand{\DemoTTwoRowASCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowASCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowASMedianLogRatioToExactBound}{-0.01325830378} %
\newcommand{\DemoTTwoRowATMedianLogE}{-4.178522578} %
\newcommand{\DemoTTwoRowATQTwoFiveLogE}{-5.66313126} %
\newcommand{\DemoTTwoRowATQSevenFiveLogE}{-1.64466517} %
\newcommand{\DemoTTwoRowATRate}{0} %
\newcommand{\DemoTTwoRowATCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowATCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowATMedianLogRatioToExactBound}{-0.01325830378} %
\newcommand{\DemoTTwoRowAUMedianLogE}{0.5598895486} %
\newcommand{\DemoTTwoRowAUQTwoFiveLogE}{-0.1597456893} %
\newcommand{\DemoTTwoRowAUQSevenFiveLogE}{1.548991435} %
\newcommand{\DemoTTwoRowAURate}{0} %
\newcommand{\DemoTTwoRowAUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAUMedianLogRatioToExactBound}{0.001776509659} %
\newcommand{\DemoTTwoRowAVMedianLogE}{-0.05161479501} %
\newcommand{\DemoTTwoRowAVQTwoFiveLogE}{-0.2045815646} %
\newcommand{\DemoTTwoRowAVQSevenFiveLogE}{0.07359193339} %
\newcommand{\DemoTTwoRowAVRate}{0} %
\newcommand{\DemoTTwoRowAVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAVMedianLogRatioToExactBound}{-0.000163771912} %
\newcommand{\DemoTTwoRowAWMedianLogE}{0.07802346919} %
\newcommand{\DemoTTwoRowAWQTwoFiveLogE}{0.04492982559} %
\newcommand{\DemoTTwoRowAWQSevenFiveLogE}{0.09744679746} %
\newcommand{\DemoTTwoRowAWRate}{0} %
\newcommand{\DemoTTwoRowAWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAWMedianLogRatioToExactBound}{0.0002475656975} %
\newcommand{\DemoTTwoRowAXMedianLogE}{0.05636358334} %
\newcommand{\DemoTTwoRowAXQTwoFiveLogE}{-0.4092286752} %
\newcommand{\DemoTTwoRowAXQSevenFiveLogE}{1.613833287} %
\newcommand{\DemoTTwoRowAXRate}{0.0625} %
\newcommand{\DemoTTwoRowAXCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowAXCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowAXMedianLogRatioToExactBound}{0.0001788396488} %
\newcommand{\DemoTTwoRowAYMedianLogE}{-6.647886509} %
\newcommand{\DemoTTwoRowAYQTwoFiveLogE}{-9.50821168} %
\newcommand{\DemoTTwoRowAYQSevenFiveLogE}{-4.73390671} %
\newcommand{\DemoTTwoRowAYRate}{0} %
\newcommand{\DemoTTwoRowAYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAYMedianLogRatioToExactBound}{-0.02109350786} %
\newcommand{\DemoTTwoRowAZMedianLogE}{-6.647886509} %
\newcommand{\DemoTTwoRowAZQTwoFiveLogE}{-9.50821168} %
\newcommand{\DemoTTwoRowAZQSevenFiveLogE}{-4.73390671} %
\newcommand{\DemoTTwoRowAZRate}{0} %
\newcommand{\DemoTTwoRowAZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowAZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowAZMedianLogRatioToExactBound}{-0.02109350786} %
\newcommand{\DemoTTwoRowBAMedianLogE}{1.153384931} %
\newcommand{\DemoTTwoRowBAQTwoFiveLogE}{-0.1050010529} %
\newcommand{\DemoTTwoRowBAQSevenFiveLogE}{1.580644101} %
\newcommand{\DemoTTwoRowBARate}{0} %
\newcommand{\DemoTTwoRowBACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBAMedianLogRatioToExactBound}{0.003659649435} %
\newcommand{\DemoTTwoRowBBMedianLogE}{-0.2192892424} %
\newcommand{\DemoTTwoRowBBQTwoFiveLogE}{-0.6307723623} %
\newcommand{\DemoTTwoRowBBQSevenFiveLogE}{0.1414235461} %
\newcommand{\DemoTTwoRowBBRate}{0} %
\newcommand{\DemoTTwoRowBBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBBMedianLogRatioToExactBound}{-0.0006957969804} %
\newcommand{\DemoTTwoRowBCMedianLogE}{0.09023772782} %
\newcommand{\DemoTTwoRowBCQTwoFiveLogE}{0.05282914258} %
\newcommand{\DemoTTwoRowBCQSevenFiveLogE}{0.1484155375} %
\newcommand{\DemoTTwoRowBCRate}{0} %
\newcommand{\DemoTTwoRowBCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBCMedianLogRatioToExactBound}{0.0002863211065} %
\newcommand{\DemoTTwoRowBDMedianLogE}{0.4387164639} %
\newcommand{\DemoTTwoRowBDQTwoFiveLogE}{-1.648866736} %
\newcommand{\DemoTTwoRowBDQSevenFiveLogE}{1.157977186} %
\newcommand{\DemoTTwoRowBDRate}{0.0625} %
\newcommand{\DemoTTwoRowBDCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowBDCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowBDMedianLogRatioToExactBound}{0.001392031763} %
\newcommand{\DemoTTwoRowBEMedianLogE}{13.45993373} %
\newcommand{\DemoTTwoRowBEQTwoFiveLogE}{12.31186581} %
\newcommand{\DemoTTwoRowBEQSevenFiveLogE}{15.18914677} %
\newcommand{\DemoTTwoRowBERate}{1} %
\newcommand{\DemoTTwoRowBECpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBECpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBEMedianLogRatioToExactBound}{0.04270789184} %
\newcommand{\DemoTTwoRowBFMedianLogE}{12.006521} %
\newcommand{\DemoTTwoRowBFQTwoFiveLogE}{11.27745014} %
\newcommand{\DemoTTwoRowBFQSevenFiveLogE}{13.52319888} %
\newcommand{\DemoTTwoRowBFRate}{1} %
\newcommand{\DemoTTwoRowBFCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBFCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBFMedianLogRatioToExactBound}{0.03809626485} %
\newcommand{\DemoTTwoRowBGMedianLogE}{13.45993373} %
\newcommand{\DemoTTwoRowBGQTwoFiveLogE}{12.31186581} %
\newcommand{\DemoTTwoRowBGQSevenFiveLogE}{15.18914677} %
\newcommand{\DemoTTwoRowBGRate}{1} %
\newcommand{\DemoTTwoRowBGCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBGCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBGMedianLogRatioToExactBound}{0.04270789184} %
\newcommand{\DemoTTwoRowBHMedianLogE}{14.60761889} %
\newcommand{\DemoTTwoRowBHQTwoFiveLogE}{12.54437566} %
\newcommand{\DemoTTwoRowBHQSevenFiveLogE}{16.65032601} %
\newcommand{\DemoTTwoRowBHRate}{1} %
\newcommand{\DemoTTwoRowBHCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBHCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBHMedianLogRatioToExactBound}{0.0463494561} %
\newcommand{\DemoTTwoRowBIMedianLogE}{-4.655636977} %
\newcommand{\DemoTTwoRowBIQTwoFiveLogE}{-6.058201198} %
\newcommand{\DemoTTwoRowBIQSevenFiveLogE}{-2.026348326} %
\newcommand{\DemoTTwoRowBIRate}{0} %
\newcommand{\DemoTTwoRowBICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBIMedianLogRatioToExactBound}{-0.01477217083} %
\newcommand{\DemoTTwoRowBJMedianLogE}{-4.655636977} %
\newcommand{\DemoTTwoRowBJQTwoFiveLogE}{-6.058201198} %
\newcommand{\DemoTTwoRowBJQSevenFiveLogE}{-2.026348326} %
\newcommand{\DemoTTwoRowBJRate}{0} %
\newcommand{\DemoTTwoRowBJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBJMedianLogRatioToExactBound}{-0.01477217083} %
\newcommand{\DemoTTwoRowBKMedianLogE}{1.107259949} %
\newcommand{\DemoTTwoRowBKQTwoFiveLogE}{0.05215386361} %
\newcommand{\DemoTTwoRowBKQSevenFiveLogE}{1.636508856} %
\newcommand{\DemoTTwoRowBKRate}{0} %
\newcommand{\DemoTTwoRowBKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBKMedianLogRatioToExactBound}{0.003513296506} %
\newcommand{\DemoTTwoRowBLMedianLogE}{-0.1085559222} %
\newcommand{\DemoTTwoRowBLQTwoFiveLogE}{-0.2882785756} %
\newcommand{\DemoTTwoRowBLQSevenFiveLogE}{0.132713754} %
\newcommand{\DemoTTwoRowBLRate}{0} %
\newcommand{\DemoTTwoRowBLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBLMedianLogRatioToExactBound}{-0.0003444440868} %
\newcommand{\DemoTTwoRowBMMedianLogE}{0.08375230713} %
\newcommand{\DemoTTwoRowBMQTwoFiveLogE}{0.05647159292} %
\newcommand{\DemoTTwoRowBMQSevenFiveLogE}{0.1135018946} %
\newcommand{\DemoTTwoRowBMRate}{0} %
\newcommand{\DemoTTwoRowBMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBMMedianLogRatioToExactBound}{0.0002657430969} %
\newcommand{\DemoTTwoRowBNMedianLogE}{0.3209368059} %
\newcommand{\DemoTTwoRowBNQTwoFiveLogE}{-0.574467155} %
\newcommand{\DemoTTwoRowBNQSevenFiveLogE}{1.470509021} %
\newcommand{\DemoTTwoRowBNRate}{0.0625} %
\newcommand{\DemoTTwoRowBNCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowBNCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowBNMedianLogRatioToExactBound}{0.00101832109} %
\newcommand{\DemoTTwoRowBOMedianLogE}{-16.56234149} %
\newcommand{\DemoTTwoRowBOQTwoFiveLogE}{-21.51591067} %
\newcommand{\DemoTTwoRowBOQSevenFiveLogE}{-11.32520123} %
\newcommand{\DemoTTwoRowBORate}{0.0625} %
\newcommand{\DemoTTwoRowBOCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowBOCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowBOMedianLogRatioToExactBound}{-0.05255172151} %
\newcommand{\DemoTTwoRowBPMedianLogE}{-16.56234149} %
\newcommand{\DemoTTwoRowBPQTwoFiveLogE}{-21.51591067} %
\newcommand{\DemoTTwoRowBPQSevenFiveLogE}{-11.32520123} %
\newcommand{\DemoTTwoRowBPRate}{0.0625} %
\newcommand{\DemoTTwoRowBPCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowBPCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowBPMedianLogRatioToExactBound}{-0.05255172151} %
\newcommand{\DemoTTwoRowBQMedianLogE}{8.030145509} %
\newcommand{\DemoTTwoRowBQQTwoFiveLogE}{7.043228006} %
\newcommand{\DemoTTwoRowBQQSevenFiveLogE}{9.432759608} %
\newcommand{\DemoTTwoRowBQRate}{1} %
\newcommand{\DemoTTwoRowBQCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBQCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBQMedianLogRatioToExactBound}{0.02547936659} %
\newcommand{\DemoTTwoRowBRMedianLogE}{-0.01928412657} %
\newcommand{\DemoTTwoRowBRQTwoFiveLogE}{-0.08302590213} %
\newcommand{\DemoTTwoRowBRQSevenFiveLogE}{0.1208204094} %
\newcommand{\DemoTTwoRowBRRate}{0} %
\newcommand{\DemoTTwoRowBRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBRMedianLogRatioToExactBound}{-6.118784891e-05} %
\newcommand{\DemoTTwoRowBSMedianLogE}{0.7820750788} %
\newcommand{\DemoTTwoRowBSQTwoFiveLogE}{0.6809524793} %
\newcommand{\DemoTTwoRowBSQSevenFiveLogE}{0.829387188} %
\newcommand{\DemoTTwoRowBSRate}{0} %
\newcommand{\DemoTTwoRowBSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBSMedianLogRatioToExactBound}{0.002481496457} %
\newcommand{\DemoTTwoRowBTMedianLogE}{4.572494089} %
\newcommand{\DemoTTwoRowBTQTwoFiveLogE}{3.378292306} %
\newcommand{\DemoTTwoRowBTQSevenFiveLogE}{7.239625008} %
\newcommand{\DemoTTwoRowBTRate}{0.8125} %
\newcommand{\DemoTTwoRowBTCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowBTCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowBTMedianLogRatioToExactBound}{0.0145083614} %
\newcommand{\DemoTTwoRowBUMedianLogE}{-38.89826694} %
\newcommand{\DemoTTwoRowBUQTwoFiveLogE}{-51.59383409} %
\newcommand{\DemoTTwoRowBUQSevenFiveLogE}{-33.60541969} %
\newcommand{\DemoTTwoRowBURate}{0} %
\newcommand{\DemoTTwoRowBUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBUMedianLogRatioToExactBound}{-0.1234228199} %
\newcommand{\DemoTTwoRowBVMedianLogE}{-38.89826694} %
\newcommand{\DemoTTwoRowBVQTwoFiveLogE}{-51.59383409} %
\newcommand{\DemoTTwoRowBVQSevenFiveLogE}{-33.60541969} %
\newcommand{\DemoTTwoRowBVRate}{0} %
\newcommand{\DemoTTwoRowBVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBVMedianLogRatioToExactBound}{-0.1234228199} %
\newcommand{\DemoTTwoRowBWMedianLogE}{10.66524182} %
\newcommand{\DemoTTwoRowBWQTwoFiveLogE}{9.507359779} %
\newcommand{\DemoTTwoRowBWQSevenFiveLogE}{13.04764379} %
\newcommand{\DemoTTwoRowBWRate}{1} %
\newcommand{\DemoTTwoRowBWCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowBWCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowBWMedianLogRatioToExactBound}{0.03384043364} %
\newcommand{\DemoTTwoRowBXMedianLogE}{-0.2948177743} %
\newcommand{\DemoTTwoRowBXQTwoFiveLogE}{-0.5770650887} %
\newcommand{\DemoTTwoRowBXQSevenFiveLogE}{0.1478272188} %
\newcommand{\DemoTTwoRowBXRate}{0} %
\newcommand{\DemoTTwoRowBXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBXMedianLogRatioToExactBound}{-0.0009354463305} %
\newcommand{\DemoTTwoRowBYMedianLogE}{1.446518979} %
\newcommand{\DemoTTwoRowBYQTwoFiveLogE}{1.288594999} %
\newcommand{\DemoTTwoRowBYQSevenFiveLogE}{1.53455783} %
\newcommand{\DemoTTwoRowBYRate}{0} %
\newcommand{\DemoTTwoRowBYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowBYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowBYMedianLogRatioToExactBound}{0.004589753363} %
\newcommand{\DemoTTwoRowBZMedianLogE}{4.117974787} %
\newcommand{\DemoTTwoRowBZQTwoFiveLogE}{1.165647432} %
\newcommand{\DemoTTwoRowBZQSevenFiveLogE}{6.654646777} %
\newcommand{\DemoTTwoRowBZRate}{0.6875} %
\newcommand{\DemoTTwoRowBZCpNineFiveLower}{0.4133793635} %
\newcommand{\DemoTTwoRowBZCpNineFiveUpper}{0.8898300453} %
\newcommand{\DemoTTwoRowBZMedianLogRatioToExactBound}{0.01306618779} %
\newcommand{\DemoTTwoRowCAMedianLogE}{78.97784709} %
\newcommand{\DemoTTwoRowCAQTwoFiveLogE}{76.71755329} %
\newcommand{\DemoTTwoRowCAQSevenFiveLogE}{82.04519821} %
\newcommand{\DemoTTwoRowCARate}{1} %
\newcommand{\DemoTTwoRowCACpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCACpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCAMedianLogRatioToExactBound}{0.2505939047} %
\newcommand{\DemoTTwoRowCBMedianLogE}{78.97784709} %
\newcommand{\DemoTTwoRowCBQTwoFiveLogE}{76.71755329} %
\newcommand{\DemoTTwoRowCBQSevenFiveLogE}{82.04519821} %
\newcommand{\DemoTTwoRowCBRate}{1} %
\newcommand{\DemoTTwoRowCBCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCBCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCBMedianLogRatioToExactBound}{0.2505939047} %
\newcommand{\DemoTTwoRowCCMedianLogE}{78.97784709} %
\newcommand{\DemoTTwoRowCCQTwoFiveLogE}{76.71755329} %
\newcommand{\DemoTTwoRowCCQSevenFiveLogE}{82.04519821} %
\newcommand{\DemoTTwoRowCCRate}{1} %
\newcommand{\DemoTTwoRowCCCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCCCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCCMedianLogRatioToExactBound}{0.2505939047} %
\newcommand{\DemoTTwoRowCDMedianLogE}{78.97784709} %
\newcommand{\DemoTTwoRowCDQTwoFiveLogE}{76.71755329} %
\newcommand{\DemoTTwoRowCDQSevenFiveLogE}{82.04519821} %
\newcommand{\DemoTTwoRowCDRate}{1} %
\newcommand{\DemoTTwoRowCDCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCDCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCDMedianLogRatioToExactBound}{0.2505939047} %
\newcommand{\DemoTTwoRowCEMedianLogE}{-17.25548847} %
\newcommand{\DemoTTwoRowCEQTwoFiveLogE}{-22.20905785} %
\newcommand{\DemoTTwoRowCEQSevenFiveLogE}{-12.01834841} %
\newcommand{\DemoTTwoRowCERate}{0.0625} %
\newcommand{\DemoTTwoRowCECpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowCECpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowCEMedianLogRatioToExactBound}{-0.05475105225} %
\newcommand{\DemoTTwoRowCFMedianLogE}{-17.25548847} %
\newcommand{\DemoTTwoRowCFQTwoFiveLogE}{-22.20905785} %
\newcommand{\DemoTTwoRowCFQSevenFiveLogE}{-12.01834841} %
\newcommand{\DemoTTwoRowCFRate}{0.0625} %
\newcommand{\DemoTTwoRowCFCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowCFCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowCFMedianLogRatioToExactBound}{-0.05475105225} %
\newcommand{\DemoTTwoRowCGMedianLogE}{10.24401966} %
\newcommand{\DemoTTwoRowCGQTwoFiveLogE}{9.019331417} %
\newcommand{\DemoTTwoRowCGQSevenFiveLogE}{12.36881021} %
\newcommand{\DemoTTwoRowCGRate}{1} %
\newcommand{\DemoTTwoRowCGCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCGCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCGMedianLogRatioToExactBound}{0.03250391068} %
\newcommand{\DemoTTwoRowCHMedianLogE}{-0.1752547819} %
\newcommand{\DemoTTwoRowCHQTwoFiveLogE}{-0.2942465217} %
\newcommand{\DemoTTwoRowCHQSevenFiveLogE}{0.079861971} %
\newcommand{\DemoTTwoRowCHRate}{0} %
\newcommand{\DemoTTwoRowCHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCHMedianLogRatioToExactBound}{-0.0005560772006} %
\newcommand{\DemoTTwoRowCIMedianLogE}{1.13250629} %
\newcommand{\DemoTTwoRowCIQTwoFiveLogE}{1.043238874} %
\newcommand{\DemoTTwoRowCIQSevenFiveLogE}{1.231900912} %
\newcommand{\DemoTTwoRowCIRate}{0} %
\newcommand{\DemoTTwoRowCICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCIMedianLogRatioToExactBound}{0.003593402248} %
\newcommand{\DemoTTwoRowCJMedianLogE}{5.605156358} %
\newcommand{\DemoTTwoRowCJQTwoFiveLogE}{3.399199428} %
\newcommand{\DemoTTwoRowCJQSevenFiveLogE}{8.041380335} %
\newcommand{\DemoTTwoRowCJRate}{0.75} %
\newcommand{\DemoTTwoRowCJCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowCJCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowCJMedianLogRatioToExactBound}{0.01778496211} %
\newcommand{\DemoTTwoRowCKMedianLogE}{-10.46351348} %
\newcommand{\DemoTTwoRowCKQTwoFiveLogE}{-22.38839623} %
\newcommand{\DemoTTwoRowCKQSevenFiveLogE}{-5.298243624} %
\newcommand{\DemoTTwoRowCKRate}{0} %
\newcommand{\DemoTTwoRowCKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCKMedianLogRatioToExactBound}{-0.03320035677} %
\newcommand{\DemoTTwoRowCLMedianLogE}{3.767391903} %
\newcommand{\DemoTTwoRowCLQTwoFiveLogE}{2.883745249} %
\newcommand{\DemoTTwoRowCLQSevenFiveLogE}{3.910188775} %
\newcommand{\DemoTTwoRowCLRate}{0.6875} %
\newcommand{\DemoTTwoRowCLCpNineFiveLower}{0.4133793635} %
\newcommand{\DemoTTwoRowCLCpNineFiveUpper}{0.8898300453} %
\newcommand{\DemoTTwoRowCLMedianLogRatioToExactBound}{0.01195380075} %
\newcommand{\DemoTTwoRowCMMedianLogE}{7.860416714} %
\newcommand{\DemoTTwoRowCMQTwoFiveLogE}{5.08101008} %
\newcommand{\DemoTTwoRowCMQSevenFiveLogE}{9.829956649} %
\newcommand{\DemoTTwoRowCMRate}{0.875} %
\newcommand{\DemoTTwoRowCMCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowCMCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowCMMedianLogRatioToExactBound}{0.02494082315} %
\newcommand{\DemoTTwoRowCNMedianLogE}{0.09220319253} %
\newcommand{\DemoTTwoRowCNQTwoFiveLogE}{-0.07664583005} %
\newcommand{\DemoTTwoRowCNQSevenFiveLogE}{0.1216932332} %
\newcommand{\DemoTTwoRowCNRate}{0} %
\newcommand{\DemoTTwoRowCNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCNMedianLogRatioToExactBound}{0.0002925574562} %
\newcommand{\DemoTTwoRowCOMedianLogE}{0.6950820642} %
\newcommand{\DemoTTwoRowCOQTwoFiveLogE}{0.5900636284} %
\newcommand{\DemoTTwoRowCOQSevenFiveLogE}{0.7389718885} %
\newcommand{\DemoTTwoRowCORate}{0} %
\newcommand{\DemoTTwoRowCOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCOMedianLogRatioToExactBound}{0.002205470711} %
\newcommand{\DemoTTwoRowCPMedianLogE}{5.554616741} %
\newcommand{\DemoTTwoRowCPQTwoFiveLogE}{3.035462365} %
\newcommand{\DemoTTwoRowCPQSevenFiveLogE}{8.00242621} %
\newcommand{\DemoTTwoRowCPRate}{0.75} %
\newcommand{\DemoTTwoRowCPCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowCPCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowCPMedianLogRatioToExactBound}{0.0176246017} %
\newcommand{\DemoTTwoRowCQMedianLogE}{-48.28818176} %
\newcommand{\DemoTTwoRowCQQTwoFiveLogE}{-67.27053378} %
\newcommand{\DemoTTwoRowCQQSevenFiveLogE}{-38.29286074} %
\newcommand{\DemoTTwoRowCQRate}{0} %
\newcommand{\DemoTTwoRowCQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCQMedianLogRatioToExactBound}{-0.1532166863} %
\newcommand{\DemoTTwoRowCRMedianLogE}{5.928609001} %
\newcommand{\DemoTTwoRowCRQTwoFiveLogE}{5.401208229} %
\newcommand{\DemoTTwoRowCRQSevenFiveLogE}{6.472990296} %
\newcommand{\DemoTTwoRowCRRate}{1} %
\newcommand{\DemoTTwoRowCRCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCRCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCRMedianLogRatioToExactBound}{0.01881126587} %
\newcommand{\DemoTTwoRowCSMedianLogE}{10.30289627} %
\newcommand{\DemoTTwoRowCSQTwoFiveLogE}{6.718348723} %
\newcommand{\DemoTTwoRowCSQSevenFiveLogE}{11.35083828} %
\newcommand{\DemoTTwoRowCSRate}{0.875} %
\newcommand{\DemoTTwoRowCSCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowCSCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowCSMedianLogRatioToExactBound}{0.03269072406} %
\newcommand{\DemoTTwoRowCTMedianLogE}{2.022986242e-05} %
\newcommand{\DemoTTwoRowCTQTwoFiveLogE}{-0.231648501} %
\newcommand{\DemoTTwoRowCTQSevenFiveLogE}{0.3510483606} %
\newcommand{\DemoTTwoRowCTRate}{0} %
\newcommand{\DemoTTwoRowCTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCTMedianLogRatioToExactBound}{6.418863518e-08} %
\newcommand{\DemoTTwoRowCUMedianLogE}{1.101598009} %
\newcommand{\DemoTTwoRowCUQTwoFiveLogE}{1.039929674} %
\newcommand{\DemoTTwoRowCUQSevenFiveLogE}{1.264032306} %
\newcommand{\DemoTTwoRowCURate}{0} %
\newcommand{\DemoTTwoRowCUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowCUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowCUMedianLogRatioToExactBound}{0.003495331371} %
\newcommand{\DemoTTwoRowCVMedianLogE}{1.051421217} %
\newcommand{\DemoTTwoRowCVQTwoFiveLogE}{-0.7240785114} %
\newcommand{\DemoTTwoRowCVQSevenFiveLogE}{4.308591652} %
\newcommand{\DemoTTwoRowCVRate}{0.375} %
\newcommand{\DemoTTwoRowCVCpNineFiveLower}{0.1519836751} %
\newcommand{\DemoTTwoRowCVCpNineFiveUpper}{0.6456539057} %
\newcommand{\DemoTTwoRowCVMedianLogRatioToExactBound}{0.003336122191} %
\newcommand{\DemoTTwoRowCWMedianLogE}{79.99630046} %
\newcommand{\DemoTTwoRowCWQTwoFiveLogE}{75.69354385} %
\newcommand{\DemoTTwoRowCWQSevenFiveLogE}{82.0968023} %
\newcommand{\DemoTTwoRowCWRate}{1} %
\newcommand{\DemoTTwoRowCWCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCWCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCWMedianLogRatioToExactBound}{0.2538254211} %
\newcommand{\DemoTTwoRowCXMedianLogE}{18.54850033} %
\newcommand{\DemoTTwoRowCXQTwoFiveLogE}{17.66295198} %
\newcommand{\DemoTTwoRowCXQSevenFiveLogE}{19.18674887} %
\newcommand{\DemoTTwoRowCXRate}{1} %
\newcommand{\DemoTTwoRowCXCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCXCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCXMedianLogRatioToExactBound}{0.05885373298} %
\newcommand{\DemoTTwoRowCYMedianLogE}{79.99630046} %
\newcommand{\DemoTTwoRowCYQTwoFiveLogE}{75.69354385} %
\newcommand{\DemoTTwoRowCYQSevenFiveLogE}{82.0968023} %
\newcommand{\DemoTTwoRowCYRate}{1} %
\newcommand{\DemoTTwoRowCYCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCYCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCYMedianLogRatioToExactBound}{0.2538254211} %
\newcommand{\DemoTTwoRowCZMedianLogE}{82.1296036} %
\newcommand{\DemoTTwoRowCZQTwoFiveLogE}{76.97839845} %
\newcommand{\DemoTTwoRowCZQSevenFiveLogE}{84.67903225} %
\newcommand{\DemoTTwoRowCZRate}{1} %
\newcommand{\DemoTTwoRowCZCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowCZCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowCZMedianLogRatioToExactBound}{0.2605943162} %
\newcommand{\DemoTTwoRowDAMedianLogE}{-11.15666066} %
\newcommand{\DemoTTwoRowDAQTwoFiveLogE}{-23.08154333} %
\newcommand{\DemoTTwoRowDAQSevenFiveLogE}{-5.991390804} %
\newcommand{\DemoTTwoRowDARate}{0} %
\newcommand{\DemoTTwoRowDACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDAMedianLogRatioToExactBound}{-0.03539968817} %
\newcommand{\DemoTTwoRowDBMedianLogE}{5.290089489} %
\newcommand{\DemoTTwoRowDBQTwoFiveLogE}{4.913023206} %
\newcommand{\DemoTTwoRowDBQSevenFiveLogE}{5.881640701} %
\newcommand{\DemoTTwoRowDBRate}{0.875} %
\newcommand{\DemoTTwoRowDBCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowDBCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowDBMedianLogRatioToExactBound}{0.01678526612} %
\newcommand{\DemoTTwoRowDCMedianLogE}{10.2902171} %
\newcommand{\DemoTTwoRowDCQTwoFiveLogE}{8.039285427} %
\newcommand{\DemoTTwoRowDCQSevenFiveLogE}{10.77683626} %
\newcommand{\DemoTTwoRowDCRate}{0.875} %
\newcommand{\DemoTTwoRowDCCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowDCCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowDCMedianLogRatioToExactBound}{0.03265049349} %
\newcommand{\DemoTTwoRowDDMedianLogE}{0.08019197246} %
\newcommand{\DemoTTwoRowDDQTwoFiveLogE}{-0.07617730806} %
\newcommand{\DemoTTwoRowDDQSevenFiveLogE}{0.2079733941} %
\newcommand{\DemoTTwoRowDDRate}{0} %
\newcommand{\DemoTTwoRowDDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDDMedianLogRatioToExactBound}{0.0002544462814} %
\newcommand{\DemoTTwoRowDEMedianLogE}{0.9399500157} %
\newcommand{\DemoTTwoRowDEQTwoFiveLogE}{0.8649640215} %
\newcommand{\DemoTTwoRowDEQSevenFiveLogE}{1.025276897} %
\newcommand{\DemoTTwoRowDERate}{0} %
\newcommand{\DemoTTwoRowDECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDEMedianLogRatioToExactBound}{0.002982428027} %
\newcommand{\DemoTTwoRowDFMedianLogE}{4.865120702} %
\newcommand{\DemoTTwoRowDFQTwoFiveLogE}{2.746016879} %
\newcommand{\DemoTTwoRowDFQSevenFiveLogE}{7.309738734} %
\newcommand{\DemoTTwoRowDFRate}{0.75} %
\newcommand{\DemoTTwoRowDFCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowDFCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowDFMedianLogRatioToExactBound}{0.01543685525} %
\newcommand{\DemoTTwoRowDGMedianLogE}{-12.1296799} %
\newcommand{\DemoTTwoRowDGQTwoFiveLogE}{-14.93754426} %
\newcommand{\DemoTTwoRowDGQSevenFiveLogE}{-2.717373967} %
\newcommand{\DemoTTwoRowDGRate}{0.0625} %
\newcommand{\DemoTTwoRowDGCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowDGCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowDGMedianLogRatioToExactBound}{-0.03848704367} %
\newcommand{\DemoTTwoRowDHMedianLogE}{-12.1296799} %
\newcommand{\DemoTTwoRowDHQTwoFiveLogE}{-14.93754426} %
\newcommand{\DemoTTwoRowDHQSevenFiveLogE}{-2.717373967} %
\newcommand{\DemoTTwoRowDHRate}{0.0625} %
\newcommand{\DemoTTwoRowDHCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowDHCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowDHMedianLogRatioToExactBound}{-0.03848704367} %
\newcommand{\DemoTTwoRowDIMedianLogE}{8.280255634} %
\newcommand{\DemoTTwoRowDIQTwoFiveLogE}{6.653474962} %
\newcommand{\DemoTTwoRowDIQSevenFiveLogE}{9.705711614} %
\newcommand{\DemoTTwoRowDIRate}{0.9375} %
\newcommand{\DemoTTwoRowDICpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowDICpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowDIMedianLogRatioToExactBound}{0.02627295713} %
\newcommand{\DemoTTwoRowDJMedianLogE}{0.0355058292} %
\newcommand{\DemoTTwoRowDJQTwoFiveLogE}{-0.1415326321} %
\newcommand{\DemoTTwoRowDJQSevenFiveLogE}{0.09200439183} %
\newcommand{\DemoTTwoRowDJRate}{0} %
\newcommand{\DemoTTwoRowDJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDJMedianLogRatioToExactBound}{0.0001126587354} %
\newcommand{\DemoTTwoRowDKMedianLogE}{0.7811490706} %
\newcommand{\DemoTTwoRowDKQTwoFiveLogE}{0.6847562366} %
\newcommand{\DemoTTwoRowDKQSevenFiveLogE}{0.8257572225} %
\newcommand{\DemoTTwoRowDKRate}{0} %
\newcommand{\DemoTTwoRowDKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDKMedianLogRatioToExactBound}{0.002478558266} %
\newcommand{\DemoTTwoRowDLMedianLogE}{6.135665811} %
\newcommand{\DemoTTwoRowDLQTwoFiveLogE}{3.563660407} %
\newcommand{\DemoTTwoRowDLQSevenFiveLogE}{9.208954041} %
\newcommand{\DemoTTwoRowDLRate}{0.8125} %
\newcommand{\DemoTTwoRowDLCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowDLCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowDLMedianLogRatioToExactBound}{0.01946824977} %
\newcommand{\DemoTTwoRowDMMedianLogE}{-33.31068265} %
\newcommand{\DemoTTwoRowDMQTwoFiveLogE}{-42.36648072} %
\newcommand{\DemoTTwoRowDMQSevenFiveLogE}{-18.32654789} %
\newcommand{\DemoTTwoRowDMRate}{0} %
\newcommand{\DemoTTwoRowDMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDMMedianLogRatioToExactBound}{-0.1056936133} %
\newcommand{\DemoTTwoRowDNMedianLogE}{-33.31068265} %
\newcommand{\DemoTTwoRowDNQTwoFiveLogE}{-42.36648072} %
\newcommand{\DemoTTwoRowDNQSevenFiveLogE}{-18.32654789} %
\newcommand{\DemoTTwoRowDNRate}{0} %
\newcommand{\DemoTTwoRowDNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDNMedianLogRatioToExactBound}{-0.1056936133} %
\newcommand{\DemoTTwoRowDOMedianLogE}{8.546777381} %
\newcommand{\DemoTTwoRowDOQTwoFiveLogE}{6.975677201} %
\newcommand{\DemoTTwoRowDOQSevenFiveLogE}{13.77509919} %
\newcommand{\DemoTTwoRowDORate}{1} %
\newcommand{\DemoTTwoRowDOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDOMedianLogRatioToExactBound}{0.02711862118} %
\newcommand{\DemoTTwoRowDPMedianLogE}{-0.4527131508} %
\newcommand{\DemoTTwoRowDPQTwoFiveLogE}{-0.7748634505} %
\newcommand{\DemoTTwoRowDPQSevenFiveLogE}{-0.1154480715} %
\newcommand{\DemoTTwoRowDPRate}{0} %
\newcommand{\DemoTTwoRowDPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDPMedianLogRatioToExactBound}{-0.001436442754} %
\newcommand{\DemoTTwoRowDQMedianLogE}{1.044107632} %
\newcommand{\DemoTTwoRowDQQTwoFiveLogE}{0.9857003251} %
\newcommand{\DemoTTwoRowDQQSevenFiveLogE}{1.289868895} %
\newcommand{\DemoTTwoRowDQRate}{0} %
\newcommand{\DemoTTwoRowDQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDQMedianLogRatioToExactBound}{0.003312916446} %
\newcommand{\DemoTTwoRowDRMedianLogE}{4.289044491} %
\newcommand{\DemoTTwoRowDRQTwoFiveLogE}{1.367455101} %
\newcommand{\DemoTTwoRowDRQSevenFiveLogE}{10.49227841} %
\newcommand{\DemoTTwoRowDRRate}{0.5625} %
\newcommand{\DemoTTwoRowDRCpNineFiveLower}{0.2987768991} %
\newcommand{\DemoTTwoRowDRCpNineFiveUpper}{0.8024658595} %
\newcommand{\DemoTTwoRowDRMedianLogRatioToExactBound}{0.01360898589} %
\newcommand{\DemoTTwoRowDSMedianLogE}{82.03098858} %
\newcommand{\DemoTTwoRowDSQTwoFiveLogE}{77.15734513} %
\newcommand{\DemoTTwoRowDSQSevenFiveLogE}{85.2876907} %
\newcommand{\DemoTTwoRowDSRate}{1} %
\newcommand{\DemoTTwoRowDSCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDSCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDSMedianLogRatioToExactBound}{0.2602814143} %
\newcommand{\DemoTTwoRowDTMedianLogE}{80.77688402} %
\newcommand{\DemoTTwoRowDTQTwoFiveLogE}{76.37698542} %
\newcommand{\DemoTTwoRowDTQSevenFiveLogE}{84.27067984} %
\newcommand{\DemoTTwoRowDTRate}{1} %
\newcommand{\DemoTTwoRowDTCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDTCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDTMedianLogRatioToExactBound}{0.256302185} %
\newcommand{\DemoTTwoRowDUMedianLogE}{82.03098858} %
\newcommand{\DemoTTwoRowDUQTwoFiveLogE}{77.15734513} %
\newcommand{\DemoTTwoRowDUQSevenFiveLogE}{85.2876907} %
\newcommand{\DemoTTwoRowDURate}{1} %
\newcommand{\DemoTTwoRowDUCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDUCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDUMedianLogRatioToExactBound}{0.2602814143} %
\newcommand{\DemoTTwoRowDVMedianLogE}{82.86303058} %
\newcommand{\DemoTTwoRowDVQTwoFiveLogE}{78.05747385} %
\newcommand{\DemoTTwoRowDVQSevenFiveLogE}{86.51682285} %
\newcommand{\DemoTTwoRowDVRate}{1} %
\newcommand{\DemoTTwoRowDVCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDVCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDVMedianLogRatioToExactBound}{0.262921454} %
\newcommand{\DemoTTwoRowDWMedianLogE}{-12.82282708} %
\newcommand{\DemoTTwoRowDWQTwoFiveLogE}{-15.62978045} %
\newcommand{\DemoTTwoRowDWQSevenFiveLogE}{-3.409822611} %
\newcommand{\DemoTTwoRowDWRate}{0.0625} %
\newcommand{\DemoTTwoRowDWCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowDWCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowDWMedianLogRatioToExactBound}{-0.04068637506} %
\newcommand{\DemoTTwoRowDXMedianLogE}{-12.82282708} %
\newcommand{\DemoTTwoRowDXQTwoFiveLogE}{-15.62978045} %
\newcommand{\DemoTTwoRowDXQSevenFiveLogE}{-3.409822611} %
\newcommand{\DemoTTwoRowDXRate}{0.0625} %
\newcommand{\DemoTTwoRowDXCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowDXCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowDXMedianLogRatioToExactBound}{-0.04068637506} %
\newcommand{\DemoTTwoRowDYMedianLogE}{8.855715382} %
\newcommand{\DemoTTwoRowDYQTwoFiveLogE}{6.752307123} %
\newcommand{\DemoTTwoRowDYQSevenFiveLogE}{13.08621239} %
\newcommand{\DemoTTwoRowDYRate}{1} %
\newcommand{\DemoTTwoRowDYCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowDYCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowDYMedianLogRatioToExactBound}{0.02809887049} %
\newcommand{\DemoTTwoRowDZMedianLogE}{-0.1922123325} %
\newcommand{\DemoTTwoRowDZQTwoFiveLogE}{-0.2784831343} %
\newcommand{\DemoTTwoRowDZQSevenFiveLogE}{-0.1244321921} %
\newcommand{\DemoTTwoRowDZRate}{0} %
\newcommand{\DemoTTwoRowDZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowDZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowDZMedianLogRatioToExactBound}{-0.0006098829064} %
\newcommand{\DemoTTwoRowEAMedianLogE}{0.9072845819} %
\newcommand{\DemoTTwoRowEAQTwoFiveLogE}{0.8197407958} %
\newcommand{\DemoTTwoRowEAQSevenFiveLogE}{1.090232427} %
\newcommand{\DemoTTwoRowEARate}{0} %
\newcommand{\DemoTTwoRowEACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEAMedianLogRatioToExactBound}{0.002878781765} %
\newcommand{\DemoTTwoRowEBMedianLogE}{6.288535487} %
\newcommand{\DemoTTwoRowEBQTwoFiveLogE}{3.198174162} %
\newcommand{\DemoTTwoRowEBQSevenFiveLogE}{10.83394866} %
\newcommand{\DemoTTwoRowEBRate}{0.75} %
\newcommand{\DemoTTwoRowEBCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowEBCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowEBMedianLogRatioToExactBound}{0.01995329983} %
\newcommand{\DemoTTwoRowECMedianLogE}{-82.30326827} %
\newcommand{\DemoTTwoRowECQTwoFiveLogE}{-100.0562551} %
\newcommand{\DemoTTwoRowECQSevenFiveLogE}{-66.35337502} %
\newcommand{\DemoTTwoRowECRate}{0} %
\newcommand{\DemoTTwoRowECCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowECCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowECMedianLogRatioToExactBound}{-0.261145348} %
\newcommand{\DemoTTwoRowEDMedianLogE}{-82.30326827} %
\newcommand{\DemoTTwoRowEDQTwoFiveLogE}{-100.0562551} %
\newcommand{\DemoTTwoRowEDQSevenFiveLogE}{-66.35337502} %
\newcommand{\DemoTTwoRowEDRate}{0} %
\newcommand{\DemoTTwoRowEDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEDMedianLogRatioToExactBound}{-0.261145348} %
\newcommand{\DemoTTwoRowEEMedianLogE}{0.3444532037} %
\newcommand{\DemoTTwoRowEEQTwoFiveLogE}{-1.348324778} %
\newcommand{\DemoTTwoRowEEQSevenFiveLogE}{1.706856595} %
\newcommand{\DemoTTwoRowEERate}{0.1875} %
\newcommand{\DemoTTwoRowEECpNineFiveLower}{0.04047373391} %
\newcommand{\DemoTTwoRowEECpNineFiveUpper}{0.4564565462} %
\newcommand{\DemoTTwoRowEEMedianLogRatioToExactBound}{0.001092937785} %
\newcommand{\DemoTTwoRowEFMedianLogE}{0.004471079991} %
\newcommand{\DemoTTwoRowEFQTwoFiveLogE}{-0.1140710645} %
\newcommand{\DemoTTwoRowEFQSevenFiveLogE}{0.06284922731} %
\newcommand{\DemoTTwoRowEFRate}{0} %
\newcommand{\DemoTTwoRowEFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEFMedianLogRatioToExactBound}{1.418657807e-05} %
\newcommand{\DemoTTwoRowEGMedianLogE}{0.06159037249} %
\newcommand{\DemoTTwoRowEGQTwoFiveLogE}{0.02255607062} %
\newcommand{\DemoTTwoRowEGQSevenFiveLogE}{0.1087417381} %
\newcommand{\DemoTTwoRowEGRate}{0} %
\newcommand{\DemoTTwoRowEGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEGMedianLogRatioToExactBound}{0.0001954240651} %
\newcommand{\DemoTTwoRowEHMedianLogE}{-9.241663516} %
\newcommand{\DemoTTwoRowEHQTwoFiveLogE}{-12.78311672} %
\newcommand{\DemoTTwoRowEHQSevenFiveLogE}{-5.04386288} %
\newcommand{\DemoTTwoRowEHRate}{0} %
\newcommand{\DemoTTwoRowEHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEHMedianLogRatioToExactBound}{-0.02932347021} %
\newcommand{\DemoTTwoRowEIMedianLogE}{-176.7927335} %
\newcommand{\DemoTTwoRowEIQTwoFiveLogE}{-205.9502313} %
\newcommand{\DemoTTwoRowEIQSevenFiveLogE}{-154.4650626} %
\newcommand{\DemoTTwoRowEIRate}{0} %
\newcommand{\DemoTTwoRowEICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEIMedianLogRatioToExactBound}{-0.5609570665} %
\newcommand{\DemoTTwoRowEJMedianLogE}{-176.7927335} %
\newcommand{\DemoTTwoRowEJQTwoFiveLogE}{-205.9502313} %
\newcommand{\DemoTTwoRowEJQSevenFiveLogE}{-154.4650626} %
\newcommand{\DemoTTwoRowEJRate}{0} %
\newcommand{\DemoTTwoRowEJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEJMedianLogRatioToExactBound}{-0.5609570665} %
\newcommand{\DemoTTwoRowEKMedianLogE}{-0.5231792133} %
\newcommand{\DemoTTwoRowEKQTwoFiveLogE}{-1.45162473} %
\newcommand{\DemoTTwoRowEKQSevenFiveLogE}{0.9828425286} %
\newcommand{\DemoTTwoRowEKRate}{0.0625} %
\newcommand{\DemoTTwoRowEKCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowEKCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowEKMedianLogRatioToExactBound}{-0.001660029068} %
\newcommand{\DemoTTwoRowELMedianLogE}{-1.138939988} %
\newcommand{\DemoTTwoRowELQTwoFiveLogE}{-1.663321676} %
\newcommand{\DemoTTwoRowELQSevenFiveLogE}{-0.3669931311} %
\newcommand{\DemoTTwoRowELRate}{0} %
\newcommand{\DemoTTwoRowELCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowELCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowELMedianLogRatioToExactBound}{-0.003613816145} %
\newcommand{\DemoTTwoRowEMMedianLogE}{0.06755777408} %
\newcommand{\DemoTTwoRowEMQTwoFiveLogE}{0.03511045733} %
\newcommand{\DemoTTwoRowEMQSevenFiveLogE}{0.1226172365} %
\newcommand{\DemoTTwoRowEMRate}{0} %
\newcommand{\DemoTTwoRowEMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEMMedianLogRatioToExactBound}{0.0002143584185} %
\newcommand{\DemoTTwoRowENMedianLogE}{-13.43786974} %
\newcommand{\DemoTTwoRowENQTwoFiveLogE}{-15.21421268} %
\newcommand{\DemoTTwoRowENQSevenFiveLogE}{-12.19428272} %
\newcommand{\DemoTTwoRowENRate}{0} %
\newcommand{\DemoTTwoRowENCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowENCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowENMedianLogRatioToExactBound}{-0.04263788358} %
\newcommand{\DemoTTwoRowEOMedianLogE}{37.94805031} %
\newcommand{\DemoTTwoRowEOQTwoFiveLogE}{35.42543839} %
\newcommand{\DemoTTwoRowEOQSevenFiveLogE}{41.55700596} %
\newcommand{\DemoTTwoRowEORate}{1} %
\newcommand{\DemoTTwoRowEOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowEOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowEOMedianLogRatioToExactBound}{0.1204078163} %
\newcommand{\DemoTTwoRowEPMedianLogE}{37.61014007} %
\newcommand{\DemoTTwoRowEPQTwoFiveLogE}{35.34610809} %
\newcommand{\DemoTTwoRowEPQSevenFiveLogE}{41.04340319} %
\newcommand{\DemoTTwoRowEPRate}{1} %
\newcommand{\DemoTTwoRowEPCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowEPCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowEPMedianLogRatioToExactBound}{0.1193356391} %
\newcommand{\DemoTTwoRowEQMedianLogE}{37.85764977} %
\newcommand{\DemoTTwoRowEQQTwoFiveLogE}{35.41744295} %
\newcommand{\DemoTTwoRowEQQSevenFiveLogE}{41.40404583} %
\newcommand{\DemoTTwoRowEQRate}{1} %
\newcommand{\DemoTTwoRowEQCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowEQCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowEQMedianLogRatioToExactBound}{0.1201209786} %
\newcommand{\DemoTTwoRowERMedianLogE}{37.94805031} %
\newcommand{\DemoTTwoRowERQTwoFiveLogE}{35.42543839} %
\newcommand{\DemoTTwoRowERQSevenFiveLogE}{41.55700596} %
\newcommand{\DemoTTwoRowERRate}{1} %
\newcommand{\DemoTTwoRowERCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowERCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowERMedianLogRatioToExactBound}{0.1204078163} %
\newcommand{\DemoTTwoRowESMedianLogE}{-82.99641545} %
\newcommand{\DemoTTwoRowESQTwoFiveLogE}{-100.7494023} %
\newcommand{\DemoTTwoRowESQSevenFiveLogE}{-67.0465222} %
\newcommand{\DemoTTwoRowESRate}{0} %
\newcommand{\DemoTTwoRowESCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowESCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowESMedianLogRatioToExactBound}{-0.2633446794} %
\newcommand{\DemoTTwoRowETMedianLogE}{-82.99641545} %
\newcommand{\DemoTTwoRowETQTwoFiveLogE}{-100.7494023} %
\newcommand{\DemoTTwoRowETQSevenFiveLogE}{-67.0465222} %
\newcommand{\DemoTTwoRowETRate}{0} %
\newcommand{\DemoTTwoRowETCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowETCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowETMedianLogRatioToExactBound}{-0.2633446794} %
\newcommand{\DemoTTwoRowEUMedianLogE}{0.5901373273} %
\newcommand{\DemoTTwoRowEUQTwoFiveLogE}{-0.8665508809} %
\newcommand{\DemoTTwoRowEUQSevenFiveLogE}{1.819561241} %
\newcommand{\DemoTTwoRowEURate}{0.0625} %
\newcommand{\DemoTTwoRowEUCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowEUCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowEUMedianLogRatioToExactBound}{0.001872484787} %
\newcommand{\DemoTTwoRowEVMedianLogE}{-0.4100377923} %
\newcommand{\DemoTTwoRowEVQTwoFiveLogE}{-0.6071063245} %
\newcommand{\DemoTTwoRowEVQSevenFiveLogE}{-0.08249815418} %
\newcommand{\DemoTTwoRowEVRate}{0} %
\newcommand{\DemoTTwoRowEVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEVMedianLogRatioToExactBound}{-0.001301035357} %
\newcommand{\DemoTTwoRowEWMedianLogE}{0.06923138577} %
\newcommand{\DemoTTwoRowEWQTwoFiveLogE}{0.03212523462} %
\newcommand{\DemoTTwoRowEWQSevenFiveLogE}{0.1205674136} %
\newcommand{\DemoTTwoRowEWRate}{0} %
\newcommand{\DemoTTwoRowEWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEWMedianLogRatioToExactBound}{0.000219668729} %
\newcommand{\DemoTTwoRowEXMedianLogE}{-9.36993619} %
\newcommand{\DemoTTwoRowEXQTwoFiveLogE}{-11.6716072} %
\newcommand{\DemoTTwoRowEXQSevenFiveLogE}{-4.623132229} %
\newcommand{\DemoTTwoRowEXRate}{0} %
\newcommand{\DemoTTwoRowEXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEXMedianLogRatioToExactBound}{-0.02973047485} %
\newcommand{\DemoTTwoRowEYMedianLogE}{-106.4842621} %
\newcommand{\DemoTTwoRowEYQTwoFiveLogE}{-127.0314369} %
\newcommand{\DemoTTwoRowEYQSevenFiveLogE}{-88.58642401} %
\newcommand{\DemoTTwoRowEYRate}{0} %
\newcommand{\DemoTTwoRowEYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEYMedianLogRatioToExactBound}{-0.337870783} %
\newcommand{\DemoTTwoRowEZMedianLogE}{0.4160885826} %
\newcommand{\DemoTTwoRowEZQTwoFiveLogE}{0.2970828006} %
\newcommand{\DemoTTwoRowEZQSevenFiveLogE}{0.7869850291} %
\newcommand{\DemoTTwoRowEZRate}{0} %
\newcommand{\DemoTTwoRowEZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowEZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowEZMedianLogRatioToExactBound}{0.001320234299} %
\newcommand{\DemoTTwoRowFAMedianLogE}{0.9241301645} %
\newcommand{\DemoTTwoRowFAQTwoFiveLogE}{0.1562690569} %
\newcommand{\DemoTTwoRowFAQSevenFiveLogE}{2.657967021} %
\newcommand{\DemoTTwoRowFARate}{0.25} %
\newcommand{\DemoTTwoRowFACpNineFiveLower}{0.07266203825} %
\newcommand{\DemoTTwoRowFACpNineFiveUpper}{0.5237708199} %
\newcommand{\DemoTTwoRowFAMedianLogRatioToExactBound}{0.002932232201} %
\newcommand{\DemoTTwoRowFBMedianLogE}{0.000766964046} %
\newcommand{\DemoTTwoRowFBQTwoFiveLogE}{-0.02694525647} %
\newcommand{\DemoTTwoRowFBQSevenFiveLogE}{0.06303890043} %
\newcommand{\DemoTTwoRowFBRate}{0} %
\newcommand{\DemoTTwoRowFBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFBMedianLogRatioToExactBound}{2.433549687e-06} %
\newcommand{\DemoTTwoRowFCMedianLogE}{0.08544116712} %
\newcommand{\DemoTTwoRowFCQTwoFiveLogE}{0.05567283606} %
\newcommand{\DemoTTwoRowFCQSevenFiveLogE}{0.1491482692} %
\newcommand{\DemoTTwoRowFCRate}{0} %
\newcommand{\DemoTTwoRowFCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFCMedianLogRatioToExactBound}{0.0002711017897} %
\newcommand{\DemoTTwoRowFDMedianLogE}{-8.696460033} %
\newcommand{\DemoTTwoRowFDQTwoFiveLogE}{-12.96646943} %
\newcommand{\DemoTTwoRowFDQSevenFiveLogE}{-5.99549483} %
\newcommand{\DemoTTwoRowFDRate}{0} %
\newcommand{\DemoTTwoRowFDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFDMedianLogRatioToExactBound}{-0.02759355892} %
\newcommand{\DemoTTwoRowFEMedianLogE}{-331.6192632} %
\newcommand{\DemoTTwoRowFEQTwoFiveLogE}{-344.1879127} %
\newcommand{\DemoTTwoRowFEQSevenFiveLogE}{-300.8446864} %
\newcommand{\DemoTTwoRowFERate}{0} %
\newcommand{\DemoTTwoRowFECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFEMedianLogRatioToExactBound}{-1.052216148} %
\newcommand{\DemoTTwoRowFFMedianLogE}{0.4006468961} %
\newcommand{\DemoTTwoRowFFQTwoFiveLogE}{-0.01520481637} %
\newcommand{\DemoTTwoRowFFQSevenFiveLogE}{0.6139867535} %
\newcommand{\DemoTTwoRowFFRate}{0} %
\newcommand{\DemoTTwoRowFFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFFMedianLogRatioToExactBound}{0.001271238376} %
\newcommand{\DemoTTwoRowFGMedianLogE}{0.3375970826} %
\newcommand{\DemoTTwoRowFGQTwoFiveLogE}{-0.7446147344} %
\newcommand{\DemoTTwoRowFGQSevenFiveLogE}{0.871107157} %
\newcommand{\DemoTTwoRowFGRate}{0} %
\newcommand{\DemoTTwoRowFGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFGMedianLogRatioToExactBound}{0.001071183557} %
\newcommand{\DemoTTwoRowFHMedianLogE}{-0.1504256215} %
\newcommand{\DemoTTwoRowFHQTwoFiveLogE}{-0.3245715955} %
\newcommand{\DemoTTwoRowFHQSevenFiveLogE}{0.1115352159} %
\newcommand{\DemoTTwoRowFHRate}{0} %
\newcommand{\DemoTTwoRowFHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFHMedianLogRatioToExactBound}{-0.0004772951562} %
\newcommand{\DemoTTwoRowFIMedianLogE}{0.07605561678} %
\newcommand{\DemoTTwoRowFIQTwoFiveLogE}{0.01631568284} %
\newcommand{\DemoTTwoRowFIQSevenFiveLogE}{0.1230198171} %
\newcommand{\DemoTTwoRowFIRate}{0} %
\newcommand{\DemoTTwoRowFICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFIMedianLogRatioToExactBound}{0.0002413217717} %
\newcommand{\DemoTTwoRowFJMedianLogE}{-19.03281526} %
\newcommand{\DemoTTwoRowFJQTwoFiveLogE}{-21.25589528} %
\newcommand{\DemoTTwoRowFJQSevenFiveLogE}{-16.77093209} %
\newcommand{\DemoTTwoRowFJRate}{0} %
\newcommand{\DemoTTwoRowFJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFJMedianLogRatioToExactBound}{-0.06039044706} %
\newcommand{\DemoTTwoRowFKMedianLogE}{36.36045079} %
\newcommand{\DemoTTwoRowFKQTwoFiveLogE}{32.3236859} %
\newcommand{\DemoTTwoRowFKQSevenFiveLogE}{39.05802341} %
\newcommand{\DemoTTwoRowFKRate}{1} %
\newcommand{\DemoTTwoRowFKCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowFKCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowFKMedianLogRatioToExactBound}{0.1153704194} %
\newcommand{\DemoTTwoRowFLMedianLogE}{1.435468192} %
\newcommand{\DemoTTwoRowFLQTwoFiveLogE}{1.393842689} %
\newcommand{\DemoTTwoRowFLQSevenFiveLogE}{1.49779633} %
\newcommand{\DemoTTwoRowFLRate}{0} %
\newcommand{\DemoTTwoRowFLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFLMedianLogRatioToExactBound}{0.004554689606} %
\newcommand{\DemoTTwoRowFMMedianLogE}{36.36045079} %
\newcommand{\DemoTTwoRowFMQTwoFiveLogE}{32.3236859} %
\newcommand{\DemoTTwoRowFMQSevenFiveLogE}{39.05802341} %
\newcommand{\DemoTTwoRowFMRate}{1} %
\newcommand{\DemoTTwoRowFMCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowFMCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowFMMedianLogRatioToExactBound}{0.1153704194} %
\newcommand{\DemoTTwoRowFNMedianLogE}{38.0849207} %
\newcommand{\DemoTTwoRowFNQTwoFiveLogE}{33.47059199} %
\newcommand{\DemoTTwoRowFNQSevenFiveLogE}{40.72477581} %
\newcommand{\DemoTTwoRowFNRate}{1} %
\newcommand{\DemoTTwoRowFNCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowFNCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowFNMedianLogRatioToExactBound}{0.1208421012} %
\newcommand{\DemoTTwoRowFOMedianLogE}{-107.1774093} %
\newcommand{\DemoTTwoRowFOQTwoFiveLogE}{-127.7245841} %
\newcommand{\DemoTTwoRowFOQSevenFiveLogE}{-89.27957119} %
\newcommand{\DemoTTwoRowFORate}{0} %
\newcommand{\DemoTTwoRowFOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFOMedianLogRatioToExactBound}{-0.3400701144} %
\newcommand{\DemoTTwoRowFPMedianLogE}{0.466685394} %
\newcommand{\DemoTTwoRowFPQTwoFiveLogE}{0.2765457204} %
\newcommand{\DemoTTwoRowFPQSevenFiveLogE}{0.6312830096} %
\newcommand{\DemoTTwoRowFPRate}{0} %
\newcommand{\DemoTTwoRowFPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFPMedianLogRatioToExactBound}{0.001480776186} %
\newcommand{\DemoTTwoRowFQMedianLogE}{0.7765624061} %
\newcommand{\DemoTTwoRowFQQTwoFiveLogE}{0.4294271791} %
\newcommand{\DemoTTwoRowFQQSevenFiveLogE}{1.980513935} %
\newcommand{\DemoTTwoRowFQRate}{0.125} %
\newcommand{\DemoTTwoRowFQCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowFQCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowFQMedianLogRatioToExactBound}{0.002464004943} %
\newcommand{\DemoTTwoRowFRMedianLogE}{-0.074773443} %
\newcommand{\DemoTTwoRowFRQTwoFiveLogE}{-0.132590682} %
\newcommand{\DemoTTwoRowFRQSevenFiveLogE}{0.05023649303} %
\newcommand{\DemoTTwoRowFRRate}{0} %
\newcommand{\DemoTTwoRowFRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFRMedianLogRatioToExactBound}{-0.0002372534798} %
\newcommand{\DemoTTwoRowFSMedianLogE}{0.09548403603} %
\newcommand{\DemoTTwoRowFSQTwoFiveLogE}{0.05512483105} %
\newcommand{\DemoTTwoRowFSQSevenFiveLogE}{0.11942689} %
\newcommand{\DemoTTwoRowFSRate}{0} %
\newcommand{\DemoTTwoRowFSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFSMedianLogRatioToExactBound}{0.0003029674562} %
\newcommand{\DemoTTwoRowFTMedianLogE}{-9.385216391} %
\newcommand{\DemoTTwoRowFTQTwoFiveLogE}{-13.59184449} %
\newcommand{\DemoTTwoRowFTQSevenFiveLogE}{-6.688641769} %
\newcommand{\DemoTTwoRowFTRate}{0} %
\newcommand{\DemoTTwoRowFTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFTMedianLogRatioToExactBound}{-0.02977895839} %
\newcommand{\DemoTTwoRowFUMedianLogE}{-100.3220158} %
\newcommand{\DemoTTwoRowFUQTwoFiveLogE}{-107.0877631} %
\newcommand{\DemoTTwoRowFUQSevenFiveLogE}{-75.21607118} %
\newcommand{\DemoTTwoRowFURate}{0} %
\newcommand{\DemoTTwoRowFUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFUMedianLogRatioToExactBound}{-0.3183181941} %
\newcommand{\DemoTTwoRowFVMedianLogE}{-100.3220158} %
\newcommand{\DemoTTwoRowFVQTwoFiveLogE}{-107.0877631} %
\newcommand{\DemoTTwoRowFVQSevenFiveLogE}{-75.21607118} %
\newcommand{\DemoTTwoRowFVRate}{0} %
\newcommand{\DemoTTwoRowFVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFVMedianLogRatioToExactBound}{-0.3183181941} %
\newcommand{\DemoTTwoRowFWMedianLogE}{0.1179801605} %
\newcommand{\DemoTTwoRowFWQTwoFiveLogE}{-0.670792596} %
\newcommand{\DemoTTwoRowFWQSevenFiveLogE}{0.7655441929} %
\newcommand{\DemoTTwoRowFWRate}{0} %
\newcommand{\DemoTTwoRowFWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFWMedianLogRatioToExactBound}{0.0003743468604} %
\newcommand{\DemoTTwoRowFXMedianLogE}{-0.09081407341} %
\newcommand{\DemoTTwoRowFXQTwoFiveLogE}{-0.4423774652} %
\newcommand{\DemoTTwoRowFXQSevenFiveLogE}{0.0130422318} %
\newcommand{\DemoTTwoRowFXRate}{0} %
\newcommand{\DemoTTwoRowFXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFXMedianLogRatioToExactBound}{-0.0002881498306} %
\newcommand{\DemoTTwoRowFYMedianLogE}{0.06891693526} %
\newcommand{\DemoTTwoRowFYQTwoFiveLogE}{0.03450223071} %
\newcommand{\DemoTTwoRowFYQSevenFiveLogE}{0.09642497478} %
\newcommand{\DemoTTwoRowFYRate}{0} %
\newcommand{\DemoTTwoRowFYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFYMedianLogRatioToExactBound}{0.0002186709887} %
\newcommand{\DemoTTwoRowFZMedianLogE}{-9.375917939} %
\newcommand{\DemoTTwoRowFZQTwoFiveLogE}{-11.16417559} %
\newcommand{\DemoTTwoRowFZQSevenFiveLogE}{-5.849046811} %
\newcommand{\DemoTTwoRowFZRate}{0} %
\newcommand{\DemoTTwoRowFZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowFZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowFZMedianLogRatioToExactBound}{-0.02974945473} %
\newcommand{\DemoTTwoRowGAMedianLogE}{-122.2988412} %
\newcommand{\DemoTTwoRowGAQTwoFiveLogE}{-139.8526623} %
\newcommand{\DemoTTwoRowGAQSevenFiveLogE}{-112.7201084} %
\newcommand{\DemoTTwoRowGARate}{0} %
\newcommand{\DemoTTwoRowGACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGAMedianLogRatioToExactBound}{-0.3880498808} %
\newcommand{\DemoTTwoRowGBMedianLogE}{-122.2988412} %
\newcommand{\DemoTTwoRowGBQTwoFiveLogE}{-139.8526623} %
\newcommand{\DemoTTwoRowGBQSevenFiveLogE}{-112.7201084} %
\newcommand{\DemoTTwoRowGBRate}{0} %
\newcommand{\DemoTTwoRowGBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGBMedianLogRatioToExactBound}{-0.3880498808} %
\newcommand{\DemoTTwoRowGCMedianLogE}{0.09477559083} %
\newcommand{\DemoTTwoRowGCQTwoFiveLogE}{-0.7754698065} %
\newcommand{\DemoTTwoRowGCQSevenFiveLogE}{0.7603034828} %
\newcommand{\DemoTTwoRowGCRate}{0.0625} %
\newcommand{\DemoTTwoRowGCCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowGCCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowGCMedianLogRatioToExactBound}{0.0003007195847} %
\newcommand{\DemoTTwoRowGDMedianLogE}{-2.647351177} %
\newcommand{\DemoTTwoRowGDQTwoFiveLogE}{-3.808172548} %
\newcommand{\DemoTTwoRowGDQSevenFiveLogE}{-0.9516391967} %
\newcommand{\DemoTTwoRowGDRate}{0} %
\newcommand{\DemoTTwoRowGDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGDMedianLogRatioToExactBound}{-0.008399951289} %
\newcommand{\DemoTTwoRowGEMedianLogE}{0.07032868937} %
\newcommand{\DemoTTwoRowGEQTwoFiveLogE}{0.04086893692} %
\newcommand{\DemoTTwoRowGEQSevenFiveLogE}{0.1077835642} %
\newcommand{\DemoTTwoRowGERate}{0} %
\newcommand{\DemoTTwoRowGECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGEMedianLogRatioToExactBound}{0.0002231504344} %
\newcommand{\DemoTTwoRowGFMedianLogE}{-11.34307392} %
\newcommand{\DemoTTwoRowGFQTwoFiveLogE}{-13.22401115} %
\newcommand{\DemoTTwoRowGFQSevenFiveLogE}{-8.602529934} %
\newcommand{\DemoTTwoRowGFRate}{0} %
\newcommand{\DemoTTwoRowGFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGFMedianLogRatioToExactBound}{-0.03599117081} %
\newcommand{\DemoTTwoRowGGMedianLogE}{38.08982209} %
\newcommand{\DemoTTwoRowGGQTwoFiveLogE}{34.80573282} %
\newcommand{\DemoTTwoRowGGQSevenFiveLogE}{40.40948414} %
\newcommand{\DemoTTwoRowGGRate}{1} %
\newcommand{\DemoTTwoRowGGCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowGGCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowGGMedianLogRatioToExactBound}{0.1208576531} %
\newcommand{\DemoTTwoRowGHMedianLogE}{30.60534145} %
\newcommand{\DemoTTwoRowGHQTwoFiveLogE}{28.71900833} %
\newcommand{\DemoTTwoRowGHQSevenFiveLogE}{32.75116164} %
\newcommand{\DemoTTwoRowGHRate}{1} %
\newcommand{\DemoTTwoRowGHCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowGHCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowGHMedianLogRatioToExactBound}{0.09710966177} %
\newcommand{\DemoTTwoRowGIMedianLogE}{38.08982209} %
\newcommand{\DemoTTwoRowGIQTwoFiveLogE}{34.80573282} %
\newcommand{\DemoTTwoRowGIQSevenFiveLogE}{40.40948414} %
\newcommand{\DemoTTwoRowGIRate}{1} %
\newcommand{\DemoTTwoRowGICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowGICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowGIMedianLogRatioToExactBound}{0.1208576531} %
\newcommand{\DemoTTwoRowGJMedianLogE}{38.67844172} %
\newcommand{\DemoTTwoRowGJQTwoFiveLogE}{36.28478577} %
\newcommand{\DemoTTwoRowGJQSevenFiveLogE}{42.40098086} %
\newcommand{\DemoTTwoRowGJRate}{1} %
\newcommand{\DemoTTwoRowGJCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowGJCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowGJMedianLogRatioToExactBound}{0.1227253223} %
\newcommand{\DemoTTwoRowGKMedianLogE}{-101.015163} %
\newcommand{\DemoTTwoRowGKQTwoFiveLogE}{-107.7806898} %
\newcommand{\DemoTTwoRowGKQSevenFiveLogE}{-75.90921836} %
\newcommand{\DemoTTwoRowGKRate}{0} %
\newcommand{\DemoTTwoRowGKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGKMedianLogRatioToExactBound}{-0.3205175255} %
\newcommand{\DemoTTwoRowGLMedianLogE}{-101.015163} %
\newcommand{\DemoTTwoRowGLQTwoFiveLogE}{-107.7806898} %
\newcommand{\DemoTTwoRowGLQSevenFiveLogE}{-75.90921836} %
\newcommand{\DemoTTwoRowGLRate}{0} %
\newcommand{\DemoTTwoRowGLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGLMedianLogRatioToExactBound}{-0.3205175255} %
\newcommand{\DemoTTwoRowGMMedianLogE}{0.1251042162} %
\newcommand{\DemoTTwoRowGMQTwoFiveLogE}{-0.46399718} %
\newcommand{\DemoTTwoRowGMQSevenFiveLogE}{0.6461059459} %
\newcommand{\DemoTTwoRowGMRate}{0.0625} %
\newcommand{\DemoTTwoRowGMCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowGMCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowGMMedianLogRatioToExactBound}{0.0003969512362} %
\newcommand{\DemoTTwoRowGNMedianLogE}{-0.6424202439} %
\newcommand{\DemoTTwoRowGNQTwoFiveLogE}{-1.08121115} %
\newcommand{\DemoTTwoRowGNQSevenFiveLogE}{-0.2948136252} %
\newcommand{\DemoTTwoRowGNRate}{0} %
\newcommand{\DemoTTwoRowGNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGNMedianLogRatioToExactBound}{-0.002038376625} %
\newcommand{\DemoTTwoRowGOMedianLogE}{0.06906983172} %
\newcommand{\DemoTTwoRowGOQTwoFiveLogE}{0.03783695976} %
\newcommand{\DemoTTwoRowGOQSevenFiveLogE}{0.09366012583} %
\newcommand{\DemoTTwoRowGORate}{0} %
\newcommand{\DemoTTwoRowGOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGOMedianLogRatioToExactBound}{0.0002191561237} %
\newcommand{\DemoTTwoRowGPMedianLogE}{-9.798708903} %
\newcommand{\DemoTTwoRowGPQTwoFiveLogE}{-11.3769962} %
\newcommand{\DemoTTwoRowGPQSevenFiveLogE}{-6.508656512} %
\newcommand{\DemoTTwoRowGPRate}{0} %
\newcommand{\DemoTTwoRowGPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGPMedianLogRatioToExactBound}{-0.03109095545} %
\newcommand{\DemoTTwoRowGQMedianLogE}{-270.6132476} %
\newcommand{\DemoTTwoRowGQQTwoFiveLogE}{-308.2178867} %
\newcommand{\DemoTTwoRowGQQSevenFiveLogE}{-195.2342277} %
\newcommand{\DemoTTwoRowGQRate}{0} %
\newcommand{\DemoTTwoRowGQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGQMedianLogRatioToExactBound}{-0.8586462266} %
\newcommand{\DemoTTwoRowGRMedianLogE}{-270.6132476} %
\newcommand{\DemoTTwoRowGRQTwoFiveLogE}{-308.2178867} %
\newcommand{\DemoTTwoRowGRQSevenFiveLogE}{-195.2342277} %
\newcommand{\DemoTTwoRowGRRate}{0} %
\newcommand{\DemoTTwoRowGRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGRMedianLogRatioToExactBound}{-0.8586462266} %
\newcommand{\DemoTTwoRowGSMedianLogE}{7.471202165} %
\newcommand{\DemoTTwoRowGSQTwoFiveLogE}{5.329381941} %
\newcommand{\DemoTTwoRowGSQSevenFiveLogE}{9.886979891} %
\newcommand{\DemoTTwoRowGSRate}{0.875} %
\newcommand{\DemoTTwoRowGSCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowGSCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowGSMedianLogRatioToExactBound}{0.02370585921} %
\newcommand{\DemoTTwoRowGTMedianLogE}{0.04500510693} %
\newcommand{\DemoTTwoRowGTQTwoFiveLogE}{-0.1114006903} %
\newcommand{\DemoTTwoRowGTQSevenFiveLogE}{0.1271950441} %
\newcommand{\DemoTTwoRowGTRate}{0} %
\newcommand{\DemoTTwoRowGTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGTMedianLogRatioToExactBound}{0.0001427996064} %
\newcommand{\DemoTTwoRowGUMedianLogE}{0.6934976653} %
\newcommand{\DemoTTwoRowGUQTwoFiveLogE}{0.5643578063} %
\newcommand{\DemoTTwoRowGUQSevenFiveLogE}{0.7689884218} %
\newcommand{\DemoTTwoRowGURate}{0} %
\newcommand{\DemoTTwoRowGUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGUMedianLogRatioToExactBound}{0.002200443469} %
\newcommand{\DemoTTwoRowGVMedianLogE}{-10.07372892} %
\newcommand{\DemoTTwoRowGVQTwoFiveLogE}{-15.82802045} %
\newcommand{\DemoTTwoRowGVQSevenFiveLogE}{-6.134691068} %
\newcommand{\DemoTTwoRowGVRate}{0} %
\newcommand{\DemoTTwoRowGVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGVMedianLogRatioToExactBound}{-0.03196358418} %
\newcommand{\DemoTTwoRowGWMedianLogE}{-400.3766149} %
\newcommand{\DemoTTwoRowGWQTwoFiveLogE}{-472.4492763} %
\newcommand{\DemoTTwoRowGWQSevenFiveLogE}{-350.4533131} %
\newcommand{\DemoTTwoRowGWRate}{0} %
\newcommand{\DemoTTwoRowGWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGWMedianLogRatioToExactBound}{-1.270380784} %
\newcommand{\DemoTTwoRowGXMedianLogE}{-400.3766149} %
\newcommand{\DemoTTwoRowGXQTwoFiveLogE}{-472.4492763} %
\newcommand{\DemoTTwoRowGXQSevenFiveLogE}{-350.4533131} %
\newcommand{\DemoTTwoRowGXRate}{0} %
\newcommand{\DemoTTwoRowGXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGXMedianLogRatioToExactBound}{-1.270380784} %
\newcommand{\DemoTTwoRowGYMedianLogE}{10.48661492} %
\newcommand{\DemoTTwoRowGYQTwoFiveLogE}{6.600314411} %
\newcommand{\DemoTTwoRowGYQSevenFiveLogE}{11.16819173} %
\newcommand{\DemoTTwoRowGYRate}{0.875} %
\newcommand{\DemoTTwoRowGYCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowGYCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowGYMedianLogRatioToExactBound}{0.03327365681} %
\newcommand{\DemoTTwoRowGZMedianLogE}{-3.032434995} %
\newcommand{\DemoTTwoRowGZQTwoFiveLogE}{-3.771163738} %
\newcommand{\DemoTTwoRowGZQSevenFiveLogE}{-2.029377583} %
\newcommand{\DemoTTwoRowGZRate}{0} %
\newcommand{\DemoTTwoRowGZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowGZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowGZMedianLogRatioToExactBound}{-0.009621808571} %
\newcommand{\DemoTTwoRowHAMedianLogE}{1.112578715} %
\newcommand{\DemoTTwoRowHAQTwoFiveLogE}{0.8997636869} %
\newcommand{\DemoTTwoRowHAQSevenFiveLogE}{1.161868982} %
\newcommand{\DemoTTwoRowHARate}{0} %
\newcommand{\DemoTTwoRowHACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHAMedianLogRatioToExactBound}{0.00353017276} %
\newcommand{\DemoTTwoRowHBMedianLogE}{-11.00134652} %
\newcommand{\DemoTTwoRowHBQTwoFiveLogE}{-14.76766144} %
\newcommand{\DemoTTwoRowHBQSevenFiveLogE}{-6.0216071} %
\newcommand{\DemoTTwoRowHBRate}{0} %
\newcommand{\DemoTTwoRowHBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHBMedianLogRatioToExactBound}{-0.0349068819} %
\newcommand{\DemoTTwoRowHCMedianLogE}{134.5178138} %
\newcommand{\DemoTTwoRowHCQTwoFiveLogE}{131.0440006} %
\newcommand{\DemoTTwoRowHCQSevenFiveLogE}{137.9005233} %
\newcommand{\DemoTTwoRowHCRate}{1} %
\newcommand{\DemoTTwoRowHCCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHCCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHCMedianLogRatioToExactBound}{0.4268202472} %
\newcommand{\DemoTTwoRowHDMedianLogE}{134.1566053} %
\newcommand{\DemoTTwoRowHDQTwoFiveLogE}{130.9636603} %
\newcommand{\DemoTTwoRowHDQSevenFiveLogE}{137.5732962} %
\newcommand{\DemoTTwoRowHDRate}{1} %
\newcommand{\DemoTTwoRowHDCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHDCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHDMedianLogRatioToExactBound}{0.4256741455} %
\newcommand{\DemoTTwoRowHEMedianLogE}{134.4978895} %
\newcommand{\DemoTTwoRowHEQTwoFiveLogE}{131.0417575} %
\newcommand{\DemoTTwoRowHEQSevenFiveLogE}{137.8830565} %
\newcommand{\DemoTTwoRowHERate}{1} %
\newcommand{\DemoTTwoRowHECpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHECpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHEMedianLogRatioToExactBound}{0.4267570279} %
\newcommand{\DemoTTwoRowHFMedianLogE}{134.5178138} %
\newcommand{\DemoTTwoRowHFQTwoFiveLogE}{131.0440006} %
\newcommand{\DemoTTwoRowHFQSevenFiveLogE}{137.9005233} %
\newcommand{\DemoTTwoRowHFRate}{1} %
\newcommand{\DemoTTwoRowHFCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHFCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHFMedianLogRatioToExactBound}{0.4268202472} %
\newcommand{\DemoTTwoRowHGMedianLogE}{-271.3063948} %
\newcommand{\DemoTTwoRowHGQTwoFiveLogE}{-308.9110338} %
\newcommand{\DemoTTwoRowHGQSevenFiveLogE}{-195.9273749} %
\newcommand{\DemoTTwoRowHGRate}{0} %
\newcommand{\DemoTTwoRowHGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHGMedianLogRatioToExactBound}{-0.860845558} %
\newcommand{\DemoTTwoRowHHMedianLogE}{-271.3063948} %
\newcommand{\DemoTTwoRowHHQTwoFiveLogE}{-308.9110338} %
\newcommand{\DemoTTwoRowHHQSevenFiveLogE}{-195.9273749} %
\newcommand{\DemoTTwoRowHHRate}{0} %
\newcommand{\DemoTTwoRowHHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHHMedianLogRatioToExactBound}{-0.860845558} %
\newcommand{\DemoTTwoRowHIMedianLogE}{10.24225605} %
\newcommand{\DemoTTwoRowHIQTwoFiveLogE}{7.859770566} %
\newcommand{\DemoTTwoRowHIQSevenFiveLogE}{11.28929406} %
\newcommand{\DemoTTwoRowHIRate}{1} %
\newcommand{\DemoTTwoRowHICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHIMedianLogRatioToExactBound}{0.03249831478} %
\newcommand{\DemoTTwoRowHJMedianLogE}{-0.5744534416} %
\newcommand{\DemoTTwoRowHJQTwoFiveLogE}{-0.6740935712} %
\newcommand{\DemoTTwoRowHJQSevenFiveLogE}{-0.3395189204} %
\newcommand{\DemoTTwoRowHJRate}{0} %
\newcommand{\DemoTTwoRowHJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHJMedianLogRatioToExactBound}{-0.001822720374} %
\newcommand{\DemoTTwoRowHKMedianLogE}{0.9451499029} %
\newcommand{\DemoTTwoRowHKQTwoFiveLogE}{0.720419158} %
\newcommand{\DemoTTwoRowHKQSevenFiveLogE}{0.997118016} %
\newcommand{\DemoTTwoRowHKRate}{0} %
\newcommand{\DemoTTwoRowHKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHKMedianLogRatioToExactBound}{0.002998927084} %
\newcommand{\DemoTTwoRowHLMedianLogE}{-8.72437376} %
\newcommand{\DemoTTwoRowHLQTwoFiveLogE}{-13.28193728} %
\newcommand{\DemoTTwoRowHLQSevenFiveLogE}{-4.50393981} %
\newcommand{\DemoTTwoRowHLRate}{0} %
\newcommand{\DemoTTwoRowHLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHLMedianLogRatioToExactBound}{-0.02768212818} %
\newcommand{\DemoTTwoRowHMMedianLogE}{-227.5251635} %
\newcommand{\DemoTTwoRowHMQTwoFiveLogE}{-265.4779818} %
\newcommand{\DemoTTwoRowHMQSevenFiveLogE}{-197.2218051} %
\newcommand{\DemoTTwoRowHMRate}{0} %
\newcommand{\DemoTTwoRowHMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHMMedianLogRatioToExactBound}{-0.7219292654} %
\newcommand{\DemoTTwoRowHNMedianLogE}{3.843124438} %
\newcommand{\DemoTTwoRowHNQTwoFiveLogE}{3.111135445} %
\newcommand{\DemoTTwoRowHNQSevenFiveLogE}{4.570942566} %
\newcommand{\DemoTTwoRowHNRate}{0.8125} %
\newcommand{\DemoTTwoRowHNCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowHNCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowHNMedianLogRatioToExactBound}{0.01219409739} %
\newcommand{\DemoTTwoRowHOMedianLogE}{7.926765034} %
\newcommand{\DemoTTwoRowHOQTwoFiveLogE}{5.792883619} %
\newcommand{\DemoTTwoRowHOQSevenFiveLogE}{12.15009822} %
\newcommand{\DemoTTwoRowHORate}{0.875} %
\newcommand{\DemoTTwoRowHOCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowHOCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowHOMedianLogRatioToExactBound}{0.02515134401} %
\newcommand{\DemoTTwoRowHPMedianLogE}{-0.04367134519} %
\newcommand{\DemoTTwoRowHPQTwoFiveLogE}{-0.07279776429} %
\newcommand{\DemoTTwoRowHPQSevenFiveLogE}{0.03037024209} %
\newcommand{\DemoTTwoRowHPRate}{0} %
\newcommand{\DemoTTwoRowHPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHPMedianLogRatioToExactBound}{-0.0001385676277} %
\newcommand{\DemoTTwoRowHQMedianLogE}{0.7352315404} %
\newcommand{\DemoTTwoRowHQQTwoFiveLogE}{0.6177271926} %
\newcommand{\DemoTTwoRowHQQSevenFiveLogE}{0.8727777408} %
\newcommand{\DemoTTwoRowHQRate}{0} %
\newcommand{\DemoTTwoRowHQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHQMedianLogRatioToExactBound}{0.002332863573} %
\newcommand{\DemoTTwoRowHRMedianLogE}{-9.577653324} %
\newcommand{\DemoTTwoRowHRQTwoFiveLogE}{-12.09322015} %
\newcommand{\DemoTTwoRowHRQSevenFiveLogE}{-6.813614809} %
\newcommand{\DemoTTwoRowHRRate}{0.0625} %
\newcommand{\DemoTTwoRowHRCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowHRCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowHRMedianLogRatioToExactBound}{-0.03038955394} %
\newcommand{\DemoTTwoRowHSMedianLogE}{-467.8859836} %
\newcommand{\DemoTTwoRowHSQTwoFiveLogE}{-492.9880647} %
\newcommand{\DemoTTwoRowHSQSevenFiveLogE}{-414.4583399} %
\newcommand{\DemoTTwoRowHSRate}{0} %
\newcommand{\DemoTTwoRowHSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHSMedianLogRatioToExactBound}{-1.484585614} %
\newcommand{\DemoTTwoRowHTMedianLogE}{5.219266061} %
\newcommand{\DemoTTwoRowHTQTwoFiveLogE}{4.092360178} %
\newcommand{\DemoTTwoRowHTQSevenFiveLogE}{5.934753688} %
\newcommand{\DemoTTwoRowHTRate}{1} %
\newcommand{\DemoTTwoRowHTCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHTCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHTMedianLogRatioToExactBound}{0.0165605459} %
\newcommand{\DemoTTwoRowHUMedianLogE}{8.544062476} %
\newcommand{\DemoTTwoRowHUQTwoFiveLogE}{5.210390463} %
\newcommand{\DemoTTwoRowHUQSevenFiveLogE}{11.80721995} %
\newcommand{\DemoTTwoRowHURate}{0.8125} %
\newcommand{\DemoTTwoRowHUCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowHUCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowHUMedianLogRatioToExactBound}{0.02711000688} %
\newcommand{\DemoTTwoRowHVMedianLogE}{-0.1197028911} %
\newcommand{\DemoTTwoRowHVQTwoFiveLogE}{-0.4618811246} %
\newcommand{\DemoTTwoRowHVQSevenFiveLogE}{0.2337530962} %
\newcommand{\DemoTTwoRowHVRate}{0} %
\newcommand{\DemoTTwoRowHVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHVMedianLogRatioToExactBound}{-0.0003798130234} %
\newcommand{\DemoTTwoRowHWMedianLogE}{1.020399393} %
\newcommand{\DemoTTwoRowHWQTwoFiveLogE}{0.9125665614} %
\newcommand{\DemoTTwoRowHWQSevenFiveLogE}{1.184228032} %
\newcommand{\DemoTTwoRowHWRate}{0} %
\newcommand{\DemoTTwoRowHWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHWMedianLogRatioToExactBound}{0.003237691044} %
\newcommand{\DemoTTwoRowHXMedianLogE}{-12.5668468} %
\newcommand{\DemoTTwoRowHXQTwoFiveLogE}{-14.91548831} %
\newcommand{\DemoTTwoRowHXQSevenFiveLogE}{-8.475747636} %
\newcommand{\DemoTTwoRowHXRate}{0} %
\newcommand{\DemoTTwoRowHXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowHXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowHXMedianLogRatioToExactBound}{-0.03987415871} %
\newcommand{\DemoTTwoRowHYMedianLogE}{137.7106775} %
\newcommand{\DemoTTwoRowHYQTwoFiveLogE}{133.1678846} %
\newcommand{\DemoTTwoRowHYQSevenFiveLogE}{138.9474222} %
\newcommand{\DemoTTwoRowHYRate}{1} %
\newcommand{\DemoTTwoRowHYCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHYCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHYMedianLogRatioToExactBound}{0.4369510904} %
\newcommand{\DemoTTwoRowHZMedianLogE}{19.55105584} %
\newcommand{\DemoTTwoRowHZQTwoFiveLogE}{18.87144975} %
\newcommand{\DemoTTwoRowHZQSevenFiveLogE}{20.40732008} %
\newcommand{\DemoTTwoRowHZRate}{1} %
\newcommand{\DemoTTwoRowHZCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowHZCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowHZMedianLogRatioToExactBound}{0.06203480601} %
\newcommand{\DemoTTwoRowIAMedianLogE}{137.7106775} %
\newcommand{\DemoTTwoRowIAQTwoFiveLogE}{133.1678846} %
\newcommand{\DemoTTwoRowIAQSevenFiveLogE}{138.9474222} %
\newcommand{\DemoTTwoRowIARate}{1} %
\newcommand{\DemoTTwoRowIACpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIACpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIAMedianLogRatioToExactBound}{0.4369510904} %
\newcommand{\DemoTTwoRowIBMedianLogE}{139.7408712} %
\newcommand{\DemoTTwoRowIBQTwoFiveLogE}{134.2224622} %
\newcommand{\DemoTTwoRowIBQSevenFiveLogE}{140.9535536} %
\newcommand{\DemoTTwoRowIBRate}{1} %
\newcommand{\DemoTTwoRowIBCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIBCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIBMedianLogRatioToExactBound}{0.443392823} %
\newcommand{\DemoTTwoRowICMedianLogE}{-228.2183106} %
\newcommand{\DemoTTwoRowICQTwoFiveLogE}{-266.1711289} %
\newcommand{\DemoTTwoRowICQSevenFiveLogE}{-197.9149523} %
\newcommand{\DemoTTwoRowICRate}{0} %
\newcommand{\DemoTTwoRowICCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowICCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowICMedianLogRatioToExactBound}{-0.7241285968} %
\newcommand{\DemoTTwoRowIDMedianLogE}{4.736320112} %
\newcommand{\DemoTTwoRowIDQTwoFiveLogE}{3.862485171} %
\newcommand{\DemoTTwoRowIDQSevenFiveLogE}{5.487151699} %
\newcommand{\DemoTTwoRowIDRate}{1} %
\newcommand{\DemoTTwoRowIDCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIDCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIDMedianLogRatioToExactBound}{0.01502817555} %
\newcommand{\DemoTTwoRowIEMedianLogE}{9.750907363} %
\newcommand{\DemoTTwoRowIEQTwoFiveLogE}{6.479807688} %
\newcommand{\DemoTTwoRowIEQSevenFiveLogE}{13.29518132} %
\newcommand{\DemoTTwoRowIERate}{0.9375} %
\newcommand{\DemoTTwoRowIECpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowIECpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowIEMedianLogRatioToExactBound}{0.03093928286} %
\newcommand{\DemoTTwoRowIFMedianLogE}{-0.07149684484} %
\newcommand{\DemoTTwoRowIFQTwoFiveLogE}{-0.2367899469} %
\newcommand{\DemoTTwoRowIFQSevenFiveLogE}{0.1037840332} %
\newcommand{\DemoTTwoRowIFRate}{0} %
\newcommand{\DemoTTwoRowIFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIFMedianLogRatioToExactBound}{-0.0002268569502} %
\newcommand{\DemoTTwoRowIGMedianLogE}{0.8800962106} %
\newcommand{\DemoTTwoRowIGQTwoFiveLogE}{0.7672766758} %
\newcommand{\DemoTTwoRowIGQSevenFiveLogE}{1.049395207} %
\newcommand{\DemoTTwoRowIGRate}{0} %
\newcommand{\DemoTTwoRowIGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIGMedianLogRatioToExactBound}{0.002792514028} %
\newcommand{\DemoTTwoRowIHMedianLogE}{-9.387439732} %
\newcommand{\DemoTTwoRowIHQTwoFiveLogE}{-11.59882973} %
\newcommand{\DemoTTwoRowIHQSevenFiveLogE}{-4.763310058} %
\newcommand{\DemoTTwoRowIHRate}{0.0625} %
\newcommand{\DemoTTwoRowIHCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowIHCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowIHMedianLogRatioToExactBound}{-0.02978601297} %
\newcommand{\DemoTTwoRowIIMedianLogE}{-284.7859509} %
\newcommand{\DemoTTwoRowIIQTwoFiveLogE}{-311.1974416} %
\newcommand{\DemoTTwoRowIIQSevenFiveLogE}{-218.5430966} %
\newcommand{\DemoTTwoRowIIRate}{0} %
\newcommand{\DemoTTwoRowIICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIIMedianLogRatioToExactBound}{-0.9036157109} %
\newcommand{\DemoTTwoRowIJMedianLogE}{-284.7859509} %
\newcommand{\DemoTTwoRowIJQTwoFiveLogE}{-311.1974416} %
\newcommand{\DemoTTwoRowIJQSevenFiveLogE}{-218.5430966} %
\newcommand{\DemoTTwoRowIJRate}{0} %
\newcommand{\DemoTTwoRowIJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIJMedianLogRatioToExactBound}{-0.9036157109} %
\newcommand{\DemoTTwoRowIKMedianLogE}{6.367875261} %
\newcommand{\DemoTTwoRowIKQTwoFiveLogE}{3.769103153} %
\newcommand{\DemoTTwoRowIKQSevenFiveLogE}{8.2476462} %
\newcommand{\DemoTTwoRowIKRate}{0.875} %
\newcommand{\DemoTTwoRowIKCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowIKCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowIKMedianLogRatioToExactBound}{0.02020504211} %
\newcommand{\DemoTTwoRowILMedianLogE}{0.05062434953} %
\newcommand{\DemoTTwoRowILQTwoFiveLogE}{-0.05079853176} %
\newcommand{\DemoTTwoRowILQSevenFiveLogE}{0.1504834584} %
\newcommand{\DemoTTwoRowILRate}{0} %
\newcommand{\DemoTTwoRowILCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowILCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowILMedianLogRatioToExactBound}{0.0001606292636} %
\newcommand{\DemoTTwoRowIMMedianLogE}{0.6127441789} %
\newcommand{\DemoTTwoRowIMQTwoFiveLogE}{0.5712572126} %
\newcommand{\DemoTTwoRowIMQSevenFiveLogE}{0.6850343341} %
\newcommand{\DemoTTwoRowIMRate}{0} %
\newcommand{\DemoTTwoRowIMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIMMedianLogRatioToExactBound}{0.001944215524} %
\newcommand{\DemoTTwoRowINMedianLogE}{-9.02329712} %
\newcommand{\DemoTTwoRowINQTwoFiveLogE}{-13.52702465} %
\newcommand{\DemoTTwoRowINQSevenFiveLogE}{-7.124698134} %
\newcommand{\DemoTTwoRowINRate}{0} %
\newcommand{\DemoTTwoRowINCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowINCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowINMedianLogRatioToExactBound}{-0.02863060139} %
\newcommand{\DemoTTwoRowIOMedianLogE}{-420.2760726} %
\newcommand{\DemoTTwoRowIOQTwoFiveLogE}{-475.2813234} %
\newcommand{\DemoTTwoRowIOQSevenFiveLogE}{-326.5331021} %
\newcommand{\DemoTTwoRowIORate}{0} %
\newcommand{\DemoTTwoRowIOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIOMedianLogRatioToExactBound}{-1.333521056} %
\newcommand{\DemoTTwoRowIPMedianLogE}{-420.2760726} %
\newcommand{\DemoTTwoRowIPQTwoFiveLogE}{-475.2813234} %
\newcommand{\DemoTTwoRowIPQSevenFiveLogE}{-326.5331021} %
\newcommand{\DemoTTwoRowIPRate}{0} %
\newcommand{\DemoTTwoRowIPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIPMedianLogRatioToExactBound}{-1.333521056} %
\newcommand{\DemoTTwoRowIQMedianLogE}{7.210952936} %
\newcommand{\DemoTTwoRowIQQTwoFiveLogE}{4.143666181} %
\newcommand{\DemoTTwoRowIQQSevenFiveLogE}{8.59671598} %
\newcommand{\DemoTTwoRowIQRate}{0.875} %
\newcommand{\DemoTTwoRowIQCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowIQCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowIQMedianLogRatioToExactBound}{0.02288009764} %
\newcommand{\DemoTTwoRowIRMedianLogE}{-6.643918697} %
\newcommand{\DemoTTwoRowIRQTwoFiveLogE}{-8.245835105} %
\newcommand{\DemoTTwoRowIRQSevenFiveLogE}{-3.666472502} %
\newcommand{\DemoTTwoRowIRRate}{0} %
\newcommand{\DemoTTwoRowIRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIRMedianLogRatioToExactBound}{-0.02108091813} %
\newcommand{\DemoTTwoRowISMedianLogE}{0.938050505} %
\newcommand{\DemoTTwoRowISQTwoFiveLogE}{0.8910279064} %
\newcommand{\DemoTTwoRowISQSevenFiveLogE}{1.040158868} %
\newcommand{\DemoTTwoRowISRate}{0} %
\newcommand{\DemoTTwoRowISCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowISCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowISMedianLogRatioToExactBound}{0.002976400947} %
\newcommand{\DemoTTwoRowITMedianLogE}{-11.76184628} %
\newcommand{\DemoTTwoRowITQTwoFiveLogE}{-16.78965338} %
\newcommand{\DemoTTwoRowITQSevenFiveLogE}{-8.603471033} %
\newcommand{\DemoTTwoRowITRate}{0} %
\newcommand{\DemoTTwoRowITCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowITCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowITMedianLogRatioToExactBound}{-0.03731992064} %
\newcommand{\DemoTTwoRowIUMedianLogE}{131.4897913} %
\newcommand{\DemoTTwoRowIUQTwoFiveLogE}{129.7762184} %
\newcommand{\DemoTTwoRowIUQSevenFiveLogE}{135.4502881} %
\newcommand{\DemoTTwoRowIURate}{1} %
\newcommand{\DemoTTwoRowIUCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIUCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIUMedianLogRatioToExactBound}{0.4172124392} %
\newcommand{\DemoTTwoRowIVMedianLogE}{120.9760306} %
\newcommand{\DemoTTwoRowIVQTwoFiveLogE}{119.5731576} %
\newcommand{\DemoTTwoRowIVQSevenFiveLogE}{125.2792934} %
\newcommand{\DemoTTwoRowIVRate}{1} %
\newcommand{\DemoTTwoRowIVCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIVCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIVMedianLogRatioToExactBound}{0.3838526499} %
\newcommand{\DemoTTwoRowIWMedianLogE}{128.1872483} %
\newcommand{\DemoTTwoRowIWQTwoFiveLogE}{126.7272301} %
\newcommand{\DemoTTwoRowIWQSevenFiveLogE}{132.4155481} %
\newcommand{\DemoTTwoRowIWRate}{1} %
\newcommand{\DemoTTwoRowIWCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIWCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIWMedianLogRatioToExactBound}{0.4067335874} %
\newcommand{\DemoTTwoRowIXMedianLogE}{132.7397764} %
\newcommand{\DemoTTwoRowIXQTwoFiveLogE}{129.568517} %
\newcommand{\DemoTTwoRowIXQSevenFiveLogE}{136.4426407} %
\newcommand{\DemoTTwoRowIXRate}{1} %
\newcommand{\DemoTTwoRowIXCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowIXCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowIXMedianLogRatioToExactBound}{0.4211785976} %
\newcommand{\DemoTTwoRowIYMedianLogE}{-285.4790981} %
\newcommand{\DemoTTwoRowIYQTwoFiveLogE}{-311.8905888} %
\newcommand{\DemoTTwoRowIYQSevenFiveLogE}{-219.2362438} %
\newcommand{\DemoTTwoRowIYRate}{0} %
\newcommand{\DemoTTwoRowIYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIYMedianLogRatioToExactBound}{-0.9058150423} %
\newcommand{\DemoTTwoRowIZMedianLogE}{-285.4790981} %
\newcommand{\DemoTTwoRowIZQTwoFiveLogE}{-311.8905888} %
\newcommand{\DemoTTwoRowIZQSevenFiveLogE}{-219.2362438} %
\newcommand{\DemoTTwoRowIZRate}{0} %
\newcommand{\DemoTTwoRowIZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowIZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowIZMedianLogRatioToExactBound}{-0.9058150423} %
\newcommand{\DemoTTwoRowJAMedianLogE}{7.156692565} %
\newcommand{\DemoTTwoRowJAQTwoFiveLogE}{4.955205439} %
\newcommand{\DemoTTwoRowJAQSevenFiveLogE}{8.963278429} %
\newcommand{\DemoTTwoRowJARate}{0.875} %
\newcommand{\DemoTTwoRowJACpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowJACpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowJAMedianLogRatioToExactBound}{0.02270793141} %
\newcommand{\DemoTTwoRowJBMedianLogE}{-0.6416672513} %
\newcommand{\DemoTTwoRowJBQTwoFiveLogE}{-0.725153732} %
\newcommand{\DemoTTwoRowJBQSevenFiveLogE}{-0.525381871} %
\newcommand{\DemoTTwoRowJBRate}{0} %
\newcommand{\DemoTTwoRowJBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJBMedianLogRatioToExactBound}{-0.002035987406} %
\newcommand{\DemoTTwoRowJCMedianLogE}{0.7932696464} %
\newcommand{\DemoTTwoRowJCQTwoFiveLogE}{0.771940611} %
\newcommand{\DemoTTwoRowJCQSevenFiveLogE}{0.8528004016} %
\newcommand{\DemoTTwoRowJCRate}{0} %
\newcommand{\DemoTTwoRowJCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJCMedianLogRatioToExactBound}{0.002517016423} %
\newcommand{\DemoTTwoRowJDMedianLogE}{-8.934766305} %
\newcommand{\DemoTTwoRowJDQTwoFiveLogE}{-12.82489977} %
\newcommand{\DemoTTwoRowJDQSevenFiveLogE}{-6.805816411} %
\newcommand{\DemoTTwoRowJDRate}{0} %
\newcommand{\DemoTTwoRowJDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJDMedianLogRatioToExactBound}{-0.02834969626} %
\newcommand{\DemoTTwoRowJEMedianLogE}{-655.9466091} %
\newcommand{\DemoTTwoRowJEQTwoFiveLogE}{-704.9634283} %
\newcommand{\DemoTTwoRowJEQSevenFiveLogE}{-587.2217905} %
\newcommand{\DemoTTwoRowJERate}{0} %
\newcommand{\DemoTTwoRowJECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJEMedianLogRatioToExactBound}{-2.081295301} %
\newcommand{\DemoTTwoRowJFMedianLogE}{-655.9466091} %
\newcommand{\DemoTTwoRowJFQTwoFiveLogE}{-704.9634283} %
\newcommand{\DemoTTwoRowJFQSevenFiveLogE}{-587.2217905} %
\newcommand{\DemoTTwoRowJFRate}{0} %
\newcommand{\DemoTTwoRowJFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJFMedianLogRatioToExactBound}{-2.081295301} %
\newcommand{\DemoTTwoRowJGMedianLogE}{0.9992892048} %
\newcommand{\DemoTTwoRowJGQTwoFiveLogE}{-1.177868422} %
\newcommand{\DemoTTwoRowJGQSevenFiveLogE}{1.9046128} %
\newcommand{\DemoTTwoRowJGRate}{0.0625} %
\newcommand{\DemoTTwoRowJGCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowJGCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowJGMedianLogRatioToExactBound}{0.003170709167} %
\newcommand{\DemoTTwoRowJHMedianLogE}{-0.01505767202} %
\newcommand{\DemoTTwoRowJHQTwoFiveLogE}{-0.1787561284} %
\newcommand{\DemoTTwoRowJHQSevenFiveLogE}{0.09247307052} %
\newcommand{\DemoTTwoRowJHRate}{0} %
\newcommand{\DemoTTwoRowJHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJHMedianLogRatioToExactBound}{-4.777745869e-05} %
\newcommand{\DemoTTwoRowJIMedianLogE}{0.08331711991} %
\newcommand{\DemoTTwoRowJIQTwoFiveLogE}{0.02667471874} %
\newcommand{\DemoTTwoRowJIQSevenFiveLogE}{0.1244392194} %
\newcommand{\DemoTTwoRowJIRate}{0} %
\newcommand{\DemoTTwoRowJICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJIMedianLogRatioToExactBound}{0.0002643622633} %
\newcommand{\DemoTTwoRowJJMedianLogE}{-21.41068884} %
\newcommand{\DemoTTwoRowJJQTwoFiveLogE}{-22.7733738} %
\newcommand{\DemoTTwoRowJJQSevenFiveLogE}{-18.43455232} %
\newcommand{\DemoTTwoRowJJRate}{0} %
\newcommand{\DemoTTwoRowJJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJJMedianLogRatioToExactBound}{-0.0679353555} %
\newcommand{\DemoTTwoRowJKMedianLogE}{-954.9753786} %
\newcommand{\DemoTTwoRowJKQTwoFiveLogE}{-1106.324946} %
\newcommand{\DemoTTwoRowJKQSevenFiveLogE}{-899.4235071} %
\newcommand{\DemoTTwoRowJKRate}{0} %
\newcommand{\DemoTTwoRowJKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJKMedianLogRatioToExactBound}{-3.03010297} %
\newcommand{\DemoTTwoRowJLMedianLogE}{-954.9753786} %
\newcommand{\DemoTTwoRowJLQTwoFiveLogE}{-1106.324946} %
\newcommand{\DemoTTwoRowJLQSevenFiveLogE}{-899.4235071} %
\newcommand{\DemoTTwoRowJLRate}{0} %
\newcommand{\DemoTTwoRowJLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJLMedianLogRatioToExactBound}{-3.03010297} %
\newcommand{\DemoTTwoRowJMMedianLogE}{-0.1961743174} %
\newcommand{\DemoTTwoRowJMQTwoFiveLogE}{-0.6605774279} %
\newcommand{\DemoTTwoRowJMQSevenFiveLogE}{0.7839695649} %
\newcommand{\DemoTTwoRowJMRate}{0.0625} %
\newcommand{\DemoTTwoRowJMCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowJMCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowJMMedianLogRatioToExactBound}{-0.0006224541438} %
\newcommand{\DemoTTwoRowJNMedianLogE}{-3.814315154} %
\newcommand{\DemoTTwoRowJNQTwoFiveLogE}{-6.044863032} %
\newcommand{\DemoTTwoRowJNQSevenFiveLogE}{-3.649358471} %
\newcommand{\DemoTTwoRowJNRate}{0} %
\newcommand{\DemoTTwoRowJNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJNMedianLogRatioToExactBound}{-0.01210268656} %
\newcommand{\DemoTTwoRowJOMedianLogE}{0.06621077324} %
\newcommand{\DemoTTwoRowJOQTwoFiveLogE}{0.047895717} %
\newcommand{\DemoTTwoRowJOQSevenFiveLogE}{0.1054881638} %
\newcommand{\DemoTTwoRowJORate}{0} %
\newcommand{\DemoTTwoRowJOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJOMedianLogRatioToExactBound}{0.0002100844327} %
\newcommand{\DemoTTwoRowJPMedianLogE}{-23.25306492} %
\newcommand{\DemoTTwoRowJPQTwoFiveLogE}{-25.48405833} %
\newcommand{\DemoTTwoRowJPQSevenFiveLogE}{-20.19617156} %
\newcommand{\DemoTTwoRowJPRate}{0} %
\newcommand{\DemoTTwoRowJPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJPMedianLogRatioToExactBound}{-0.07378114938} %
\newcommand{\DemoTTwoRowJQMedianLogE}{85.95493325} %
\newcommand{\DemoTTwoRowJQQTwoFiveLogE}{83.00895782} %
\newcommand{\DemoTTwoRowJQQSevenFiveLogE}{89.10302539} %
\newcommand{\DemoTTwoRowJQRate}{1} %
\newcommand{\DemoTTwoRowJQCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowJQCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowJQMedianLogRatioToExactBound}{0.2727319514} %
\newcommand{\DemoTTwoRowJRMedianLogE}{85.90592124} %
\newcommand{\DemoTTwoRowJRQTwoFiveLogE}{82.95736356} %
\newcommand{\DemoTTwoRowJRQSevenFiveLogE}{89.03200088} %
\newcommand{\DemoTTwoRowJRRate}{1} %
\newcommand{\DemoTTwoRowJRCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowJRCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowJRMedianLogRatioToExactBound}{0.272576438} %
\newcommand{\DemoTTwoRowJSMedianLogE}{85.56667804} %
\newcommand{\DemoTTwoRowJSQTwoFiveLogE}{82.6002098} %
\newcommand{\DemoTTwoRowJSQSevenFiveLogE}{88.56349611} %
\newcommand{\DemoTTwoRowJSRate}{1} %
\newcommand{\DemoTTwoRowJSCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowJSCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowJSMedianLogRatioToExactBound}{0.2715000314} %
\newcommand{\DemoTTwoRowJTMedianLogE}{85.95493325} %
\newcommand{\DemoTTwoRowJTQTwoFiveLogE}{83.00895782} %
\newcommand{\DemoTTwoRowJTQSevenFiveLogE}{89.10302539} %
\newcommand{\DemoTTwoRowJTRate}{1} %
\newcommand{\DemoTTwoRowJTCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowJTCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowJTMedianLogRatioToExactBound}{0.2727319514} %
\newcommand{\DemoTTwoRowJUMedianLogE}{-656.6397563} %
\newcommand{\DemoTTwoRowJUQTwoFiveLogE}{-705.6565755} %
\newcommand{\DemoTTwoRowJUQSevenFiveLogE}{-587.9149376} %
\newcommand{\DemoTTwoRowJURate}{0} %
\newcommand{\DemoTTwoRowJUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJUMedianLogRatioToExactBound}{-2.083494633} %
\newcommand{\DemoTTwoRowJVMedianLogE}{-656.6397563} %
\newcommand{\DemoTTwoRowJVQTwoFiveLogE}{-705.6565755} %
\newcommand{\DemoTTwoRowJVQSevenFiveLogE}{-587.9149376} %
\newcommand{\DemoTTwoRowJVRate}{0} %
\newcommand{\DemoTTwoRowJVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJVMedianLogRatioToExactBound}{-2.083494633} %
\newcommand{\DemoTTwoRowJWMedianLogE}{0.7603027126} %
\newcommand{\DemoTTwoRowJWQTwoFiveLogE}{-0.7997055781} %
\newcommand{\DemoTTwoRowJWQSevenFiveLogE}{2.156736617} %
\newcommand{\DemoTTwoRowJWRate}{0.0625} %
\newcommand{\DemoTTwoRowJWCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowJWCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowJWMedianLogRatioToExactBound}{0.002412413512} %
\newcommand{\DemoTTwoRowJXMedianLogE}{-0.6762722863} %
\newcommand{\DemoTTwoRowJXQTwoFiveLogE}{-0.8445464251} %
\newcommand{\DemoTTwoRowJXQSevenFiveLogE}{-0.599409703} %
\newcommand{\DemoTTwoRowJXRate}{0} %
\newcommand{\DemoTTwoRowJXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJXMedianLogRatioToExactBound}{-0.002145787953} %
\newcommand{\DemoTTwoRowJYMedianLogE}{0.07584384211} %
\newcommand{\DemoTTwoRowJYQTwoFiveLogE}{0.04415663576} %
\newcommand{\DemoTTwoRowJYQSevenFiveLogE}{0.1252165843} %
\newcommand{\DemoTTwoRowJYRate}{0} %
\newcommand{\DemoTTwoRowJYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJYMedianLogRatioToExactBound}{0.0002406498182} %
\newcommand{\DemoTTwoRowJZMedianLogE}{-21.24626023} %
\newcommand{\DemoTTwoRowJZQTwoFiveLogE}{-23.42216867} %
\newcommand{\DemoTTwoRowJZQSevenFiveLogE}{-18.93928756} %
\newcommand{\DemoTTwoRowJZRate}{0} %
\newcommand{\DemoTTwoRowJZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowJZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowJZMedianLogRatioToExactBound}{-0.06741362937} %
\newcommand{\DemoTTwoRowKAMedianLogE}{-608.4973198} %
\newcommand{\DemoTTwoRowKAQTwoFiveLogE}{-702.1174131} %
\newcommand{\DemoTTwoRowKAQSevenFiveLogE}{-578.5958088} %
\newcommand{\DemoTTwoRowKARate}{0} %
\newcommand{\DemoTTwoRowKACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKAMedianLogRatioToExactBound}{-1.930740391} %
\newcommand{\DemoTTwoRowKBMedianLogE}{0.3244817031} %
\newcommand{\DemoTTwoRowKBQTwoFiveLogE}{0.1280468987} %
\newcommand{\DemoTTwoRowKBQSevenFiveLogE}{0.652639335} %
\newcommand{\DemoTTwoRowKBRate}{0} %
\newcommand{\DemoTTwoRowKBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKBMedianLogRatioToExactBound}{0.001029568923} %
\newcommand{\DemoTTwoRowKCMedianLogE}{1.00624034} %
\newcommand{\DemoTTwoRowKCQTwoFiveLogE}{-0.02894043365} %
\newcommand{\DemoTTwoRowKCQSevenFiveLogE}{2.201304508} %
\newcommand{\DemoTTwoRowKCRate}{0.0625} %
\newcommand{\DemoTTwoRowKCCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowKCCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowKCMedianLogRatioToExactBound}{0.003192764873} %
\newcommand{\DemoTTwoRowKDMedianLogE}{-0.05028471685} %
\newcommand{\DemoTTwoRowKDQTwoFiveLogE}{-0.08888517349} %
\newcommand{\DemoTTwoRowKDQSevenFiveLogE}{-0.004668587077} %
\newcommand{\DemoTTwoRowKDRate}{0} %
\newcommand{\DemoTTwoRowKDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKDMedianLogRatioToExactBound}{-0.0001595516212} %
\newcommand{\DemoTTwoRowKEMedianLogE}{0.0600810814} %
\newcommand{\DemoTTwoRowKEQTwoFiveLogE}{0.02500618563} %
\newcommand{\DemoTTwoRowKEQSevenFiveLogE}{0.1138260405} %
\newcommand{\DemoTTwoRowKERate}{0} %
\newcommand{\DemoTTwoRowKECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKEMedianLogRatioToExactBound}{0.0001906351381} %
\newcommand{\DemoTTwoRowKFMedianLogE}{-21.92658444} %
\newcommand{\DemoTTwoRowKFQTwoFiveLogE}{-23.63576889} %
\newcommand{\DemoTTwoRowKFQSevenFiveLogE}{-19.53912057} %
\newcommand{\DemoTTwoRowKFRate}{0} %
\newcommand{\DemoTTwoRowKFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKFMedianLogRatioToExactBound}{-0.06957227392} %
\newcommand{\DemoTTwoRowKGMedianLogE}{-2012.894423} %
\newcommand{\DemoTTwoRowKGQTwoFiveLogE}{-2104.583958} %
\newcommand{\DemoTTwoRowKGQSevenFiveLogE}{-1897.48992} %
\newcommand{\DemoTTwoRowKGRate}{0} %
\newcommand{\DemoTTwoRowKGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKGMedianLogRatioToExactBound}{-6.386842536} %
\newcommand{\DemoTTwoRowKHMedianLogE}{0.08111780104} %
\newcommand{\DemoTTwoRowKHQTwoFiveLogE}{-0.2719042581} %
\newcommand{\DemoTTwoRowKHQSevenFiveLogE}{0.437610603} %
\newcommand{\DemoTTwoRowKHRate}{0} %
\newcommand{\DemoTTwoRowKHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKHMedianLogRatioToExactBound}{0.0002573839026} %
\newcommand{\DemoTTwoRowKIMedianLogE}{-0.448375265} %
\newcommand{\DemoTTwoRowKIQTwoFiveLogE}{-0.88846509} %
\newcommand{\DemoTTwoRowKIQSevenFiveLogE}{0.4030504682} %
\newcommand{\DemoTTwoRowKIRate}{0} %
\newcommand{\DemoTTwoRowKICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKIMedianLogRatioToExactBound}{-0.001422678796} %
\newcommand{\DemoTTwoRowKJMedianLogE}{-0.2608773524} %
\newcommand{\DemoTTwoRowKJQTwoFiveLogE}{-0.5238802417} %
\newcommand{\DemoTTwoRowKJQSevenFiveLogE}{-0.07261053148} %
\newcommand{\DemoTTwoRowKJRate}{0} %
\newcommand{\DemoTTwoRowKJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKJMedianLogRatioToExactBound}{-0.0008277545766} %
\newcommand{\DemoTTwoRowKKMedianLogE}{0.01970737868} %
\newcommand{\DemoTTwoRowKKQTwoFiveLogE}{-0.009653727212} %
\newcommand{\DemoTTwoRowKKQSevenFiveLogE}{0.1004370459} %
\newcommand{\DemoTTwoRowKKRate}{0} %
\newcommand{\DemoTTwoRowKKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKKMedianLogRatioToExactBound}{6.253081284e-05} %
\newcommand{\DemoTTwoRowKLMedianLogE}{-25.75209708} %
\newcommand{\DemoTTwoRowKLQTwoFiveLogE}{-28.78475569} %
\newcommand{\DemoTTwoRowKLQSevenFiveLogE}{-23.57333964} %
\newcommand{\DemoTTwoRowKLRate}{0} %
\newcommand{\DemoTTwoRowKLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKLMedianLogRatioToExactBound}{-0.0817104897} %
\newcommand{\DemoTTwoRowKMMedianLogE}{81.3953534} %
\newcommand{\DemoTTwoRowKMQTwoFiveLogE}{79.7893537} %
\newcommand{\DemoTTwoRowKMQSevenFiveLogE}{84.02335182} %
\newcommand{\DemoTTwoRowKMRate}{1} %
\newcommand{\DemoTTwoRowKMCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowKMCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowKMMedianLogRatioToExactBound}{0.2582645664} %
\newcommand{\DemoTTwoRowKNMedianLogE}{1.483313584} %
\newcommand{\DemoTTwoRowKNQTwoFiveLogE}{1.451651703} %
\newcommand{\DemoTTwoRowKNQSevenFiveLogE}{1.563111241} %
\newcommand{\DemoTTwoRowKNRate}{0} %
\newcommand{\DemoTTwoRowKNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKNMedianLogRatioToExactBound}{0.004706501336} %
\newcommand{\DemoTTwoRowKOMedianLogE}{81.3953534} %
\newcommand{\DemoTTwoRowKOQTwoFiveLogE}{79.7893537} %
\newcommand{\DemoTTwoRowKOQSevenFiveLogE}{84.02335182} %
\newcommand{\DemoTTwoRowKORate}{1} %
\newcommand{\DemoTTwoRowKOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowKOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowKOMedianLogRatioToExactBound}{0.2582645664} %
\newcommand{\DemoTTwoRowKPMedianLogE}{84.16632998} %
\newcommand{\DemoTTwoRowKPQTwoFiveLogE}{82.05526714} %
\newcommand{\DemoTTwoRowKPQSevenFiveLogE}{86.29773625} %
\newcommand{\DemoTTwoRowKPRate}{1} %
\newcommand{\DemoTTwoRowKPCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowKPCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowKPMedianLogRatioToExactBound}{0.2670567767} %
\newcommand{\DemoTTwoRowKQMedianLogE}{-609.190467} %
\newcommand{\DemoTTwoRowKQQTwoFiveLogE}{-702.8105603} %
\newcommand{\DemoTTwoRowKQQSevenFiveLogE}{-579.288956} %
\newcommand{\DemoTTwoRowKQRate}{0} %
\newcommand{\DemoTTwoRowKQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKQMedianLogRatioToExactBound}{-1.932939722} %
\newcommand{\DemoTTwoRowKRMedianLogE}{0.3275994103} %
\newcommand{\DemoTTwoRowKRQTwoFiveLogE}{-0.0476232725} %
\newcommand{\DemoTTwoRowKRQSevenFiveLogE}{0.4730067215} %
\newcommand{\DemoTTwoRowKRRate}{0} %
\newcommand{\DemoTTwoRowKRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKRMedianLogRatioToExactBound}{0.001039461297} %
\newcommand{\DemoTTwoRowKSMedianLogE}{0.6337807526} %
\newcommand{\DemoTTwoRowKSQTwoFiveLogE}{0.03082927294} %
\newcommand{\DemoTTwoRowKSQSevenFiveLogE}{1.628374376} %
\newcommand{\DemoTTwoRowKSRate}{0} %
\newcommand{\DemoTTwoRowKSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKSMedianLogRatioToExactBound}{0.002010963825} %
\newcommand{\DemoTTwoRowKTMedianLogE}{-0.1729238058} %
\newcommand{\DemoTTwoRowKTQTwoFiveLogE}{-0.276433048} %
\newcommand{\DemoTTwoRowKTQSevenFiveLogE}{-0.09733260185} %
\newcommand{\DemoTTwoRowKTRate}{0} %
\newcommand{\DemoTTwoRowKTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKTMedianLogRatioToExactBound}{-0.0005486810963} %
\newcommand{\DemoTTwoRowKUMedianLogE}{0.06627532345} %
\newcommand{\DemoTTwoRowKUQTwoFiveLogE}{0.008225161315} %
\newcommand{\DemoTTwoRowKUQSevenFiveLogE}{0.08602832648} %
\newcommand{\DemoTTwoRowKURate}{0} %
\newcommand{\DemoTTwoRowKUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKUMedianLogRatioToExactBound}{0.0002102892482} %
\newcommand{\DemoTTwoRowKVMedianLogE}{-21.65372534} %
\newcommand{\DemoTTwoRowKVQTwoFiveLogE}{-23.76131493} %
\newcommand{\DemoTTwoRowKVQSevenFiveLogE}{-19.71181916} %
\newcommand{\DemoTTwoRowKVRate}{0} %
\newcommand{\DemoTTwoRowKVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKVMedianLogRatioToExactBound}{-0.0687065017} %
\newcommand{\DemoTTwoRowKWMedianLogE}{-619.2664545} %
\newcommand{\DemoTTwoRowKWQTwoFiveLogE}{-681.3748537} %
\newcommand{\DemoTTwoRowKWQSevenFiveLogE}{-474.5508826} %
\newcommand{\DemoTTwoRowKWRate}{0} %
\newcommand{\DemoTTwoRowKWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKWMedianLogRatioToExactBound}{-1.964910473} %
\newcommand{\DemoTTwoRowKXMedianLogE}{-619.2664545} %
\newcommand{\DemoTTwoRowKXQTwoFiveLogE}{-681.3748537} %
\newcommand{\DemoTTwoRowKXQSevenFiveLogE}{-474.5508826} %
\newcommand{\DemoTTwoRowKXRate}{0} %
\newcommand{\DemoTTwoRowKXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKXMedianLogRatioToExactBound}{-1.964910473} %
\newcommand{\DemoTTwoRowKYMedianLogE}{-0.07204574323} %
\newcommand{\DemoTTwoRowKYQTwoFiveLogE}{-2.797447509} %
\newcommand{\DemoTTwoRowKYQSevenFiveLogE}{1.777198801} %
\newcommand{\DemoTTwoRowKYRate}{0.125} %
\newcommand{\DemoTTwoRowKYCpNineFiveLower}{0.01551360382} %
\newcommand{\DemoTTwoRowKYCpNineFiveUpper}{0.3834762368} %
\newcommand{\DemoTTwoRowKYMedianLogRatioToExactBound}{-0.0002285985853} %
\newcommand{\DemoTTwoRowKZMedianLogE}{-0.2410261224} %
\newcommand{\DemoTTwoRowKZQTwoFiveLogE}{-0.7629892114} %
\newcommand{\DemoTTwoRowKZQSevenFiveLogE}{0.2972495825} %
\newcommand{\DemoTTwoRowKZRate}{0} %
\newcommand{\DemoTTwoRowKZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowKZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowKZMedianLogRatioToExactBound}{-0.0007647673288} %
\newcommand{\DemoTTwoRowLAMedianLogE}{0.06074525535} %
\newcommand{\DemoTTwoRowLAQTwoFiveLogE}{0.006841560113} %
\newcommand{\DemoTTwoRowLAQSevenFiveLogE}{0.105102891} %
\newcommand{\DemoTTwoRowLARate}{0} %
\newcommand{\DemoTTwoRowLACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLAMedianLogRatioToExactBound}{0.0001927425385} %
\newcommand{\DemoTTwoRowLBMedianLogE}{-22.36304378} %
\newcommand{\DemoTTwoRowLBQTwoFiveLogE}{-24.67841566} %
\newcommand{\DemoTTwoRowLBQSevenFiveLogE}{-21.07173803} %
\newcommand{\DemoTTwoRowLBRate}{0} %
\newcommand{\DemoTTwoRowLBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLBMedianLogRatioToExactBound}{-0.07095714392} %
\newcommand{\DemoTTwoRowLCMedianLogE}{-995.6173368} %
\newcommand{\DemoTTwoRowLCQTwoFiveLogE}{-1146.391839} %
\newcommand{\DemoTTwoRowLCQSevenFiveLogE}{-862.0873461} %
\newcommand{\DemoTTwoRowLCRate}{0} %
\newcommand{\DemoTTwoRowLCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLCMedianLogRatioToExactBound}{-3.15905846} %
\newcommand{\DemoTTwoRowLDMedianLogE}{-595.5752223} %
\newcommand{\DemoTTwoRowLDQTwoFiveLogE}{-692.9842161} %
\newcommand{\DemoTTwoRowLDQSevenFiveLogE}{-509.1480504} %
\newcommand{\DemoTTwoRowLDRate}{0} %
\newcommand{\DemoTTwoRowLDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLDMedianLogRatioToExactBound}{-1.889739035} %
\newcommand{\DemoTTwoRowLEMedianLogE}{-0.4747307282} %
\newcommand{\DemoTTwoRowLEQTwoFiveLogE}{-2.231947351} %
\newcommand{\DemoTTwoRowLEQSevenFiveLogE}{1.39384425} %
\newcommand{\DemoTTwoRowLERate}{0.0625} %
\newcommand{\DemoTTwoRowLECpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowLECpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowLEMedianLogRatioToExactBound}{-0.001506303745} %
\newcommand{\DemoTTwoRowLFMedianLogE}{-9.282259246} %
\newcommand{\DemoTTwoRowLFQTwoFiveLogE}{-10.59297189} %
\newcommand{\DemoTTwoRowLFQSevenFiveLogE}{-7.230629871} %
\newcommand{\DemoTTwoRowLFRate}{0} %
\newcommand{\DemoTTwoRowLFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLFMedianLogRatioToExactBound}{-0.02945227902} %
\newcommand{\DemoTTwoRowLGMedianLogE}{0.05486701924} %
\newcommand{\DemoTTwoRowLGQTwoFiveLogE}{0.006788709969} %
\newcommand{\DemoTTwoRowLGQSevenFiveLogE}{0.1105025373} %
\newcommand{\DemoTTwoRowLGRate}{0} %
\newcommand{\DemoTTwoRowLGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLGMedianLogRatioToExactBound}{0.000174091104} %
\newcommand{\DemoTTwoRowLHMedianLogE}{-22.97853167} %
\newcommand{\DemoTTwoRowLHQTwoFiveLogE}{-27.39754806} %
\newcommand{\DemoTTwoRowLHQSevenFiveLogE}{-21.20926628} %
\newcommand{\DemoTTwoRowLHRate}{0} %
\newcommand{\DemoTTwoRowLHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLHMedianLogRatioToExactBound}{-0.07291006514} %
\newcommand{\DemoTTwoRowLIMedianLogE}{82.9940366} %
\newcommand{\DemoTTwoRowLIQTwoFiveLogE}{79.62357458} %
\newcommand{\DemoTTwoRowLIQSevenFiveLogE}{86.7738243} %
\newcommand{\DemoTTwoRowLIRate}{1} %
\newcommand{\DemoTTwoRowLICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowLICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowLIMedianLogRatioToExactBound}{0.2633371314} %
\newcommand{\DemoTTwoRowLJMedianLogE}{46.23357686} %
\newcommand{\DemoTTwoRowLJQTwoFiveLogE}{44.80473449} %
\newcommand{\DemoTTwoRowLJQSevenFiveLogE}{46.95539803} %
\newcommand{\DemoTTwoRowLJRate}{1} %
\newcommand{\DemoTTwoRowLJCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowLJCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowLJMedianLogRatioToExactBound}{0.1466974979} %
\newcommand{\DemoTTwoRowLKMedianLogE}{82.3621147} %
\newcommand{\DemoTTwoRowLKQTwoFiveLogE}{79.27067596} %
\newcommand{\DemoTTwoRowLKQSevenFiveLogE}{85.85194424} %
\newcommand{\DemoTTwoRowLKRate}{1} %
\newcommand{\DemoTTwoRowLKCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowLKCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowLKMedianLogRatioToExactBound}{0.2613320657} %
\newcommand{\DemoTTwoRowLLMedianLogE}{84.25082433} %
\newcommand{\DemoTTwoRowLLQTwoFiveLogE}{80.10742465} %
\newcommand{\DemoTTwoRowLLQSevenFiveLogE}{88.57859845} %
\newcommand{\DemoTTwoRowLLRate}{1} %
\newcommand{\DemoTTwoRowLLCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowLLCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowLLMedianLogRatioToExactBound}{0.2673248743} %
\newcommand{\DemoTTwoRowLMMedianLogE}{-619.9596016} %
\newcommand{\DemoTTwoRowLMQTwoFiveLogE}{-682.0680009} %
\newcommand{\DemoTTwoRowLMQSevenFiveLogE}{-475.2440298} %
\newcommand{\DemoTTwoRowLMRate}{0} %
\newcommand{\DemoTTwoRowLMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLMMedianLogRatioToExactBound}{-1.967109804} %
\newcommand{\DemoTTwoRowLNMedianLogE}{-595.8076297} %
\newcommand{\DemoTTwoRowLNQTwoFiveLogE}{-659.5773507} %
\newcommand{\DemoTTwoRowLNQSevenFiveLogE}{-467.4241058} %
\newcommand{\DemoTTwoRowLNRate}{0} %
\newcommand{\DemoTTwoRowLNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLNMedianLogRatioToExactBound}{-1.890476455} %
\newcommand{\DemoTTwoRowLOMedianLogE}{0.2091894718} %
\newcommand{\DemoTTwoRowLOQTwoFiveLogE}{-2.551983167} %
\newcommand{\DemoTTwoRowLOQSevenFiveLogE}{1.818345972} %
\newcommand{\DemoTTwoRowLORate}{0.0625} %
\newcommand{\DemoTTwoRowLOCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowLOCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowLOMedianLogRatioToExactBound}{0.0006637507666} %
\newcommand{\DemoTTwoRowLPMedianLogE}{-0.7693684992} %
\newcommand{\DemoTTwoRowLPQTwoFiveLogE}{-1.298442314} %
\newcommand{\DemoTTwoRowLPQSevenFiveLogE}{-0.3929970818} %
\newcommand{\DemoTTwoRowLPRate}{0} %
\newcommand{\DemoTTwoRowLPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLPMedianLogRatioToExactBound}{-0.002441178932} %
\newcommand{\DemoTTwoRowLQMedianLogE}{0.05395822377} %
\newcommand{\DemoTTwoRowLQQTwoFiveLogE}{0.003438302087} %
\newcommand{\DemoTTwoRowLQQSevenFiveLogE}{0.1011414279} %
\newcommand{\DemoTTwoRowLQRate}{0} %
\newcommand{\DemoTTwoRowLQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLQMedianLogRatioToExactBound}{0.0001712075282} %
\newcommand{\DemoTTwoRowLRMedianLogE}{-22.87649034} %
\newcommand{\DemoTTwoRowLRQTwoFiveLogE}{-23.61910065} %
\newcommand{\DemoTTwoRowLRQSevenFiveLogE}{-18.91935397} %
\newcommand{\DemoTTwoRowLRRate}{0} %
\newcommand{\DemoTTwoRowLRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLRMedianLogRatioToExactBound}{-0.07258629163} %
\newcommand{\DemoTTwoRowLSMedianLogE}{-1429.677389} %
\newcommand{\DemoTTwoRowLSQTwoFiveLogE}{-1545.101705} %
\newcommand{\DemoTTwoRowLSQSevenFiveLogE}{-1355.384072} %
\newcommand{\DemoTTwoRowLSRate}{0} %
\newcommand{\DemoTTwoRowLSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLSMedianLogRatioToExactBound}{-4.536315594} %
\newcommand{\DemoTTwoRowLTMedianLogE}{-1429.677389} %
\newcommand{\DemoTTwoRowLTQTwoFiveLogE}{-1545.101705} %
\newcommand{\DemoTTwoRowLTQSevenFiveLogE}{-1355.384072} %
\newcommand{\DemoTTwoRowLTRate}{0} %
\newcommand{\DemoTTwoRowLTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLTMedianLogRatioToExactBound}{-4.536315594} %
\newcommand{\DemoTTwoRowLUMedianLogE}{6.82198916} %
\newcommand{\DemoTTwoRowLUQTwoFiveLogE}{5.507421459} %
\newcommand{\DemoTTwoRowLUQSevenFiveLogE}{7.769764117} %
\newcommand{\DemoTTwoRowLURate}{0.875} %
\newcommand{\DemoTTwoRowLUCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowLUCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowLUMedianLogRatioToExactBound}{0.02164592939} %
\newcommand{\DemoTTwoRowLVMedianLogE}{-0.03685276587} %
\newcommand{\DemoTTwoRowLVQTwoFiveLogE}{-0.1104345678} %
\newcommand{\DemoTTwoRowLVQSevenFiveLogE}{0.05696670958} %
\newcommand{\DemoTTwoRowLVRate}{0} %
\newcommand{\DemoTTwoRowLVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLVMedianLogRatioToExactBound}{-0.0001169325176} %
\newcommand{\DemoTTwoRowLWMedianLogE}{0.5764380057} %
\newcommand{\DemoTTwoRowLWQTwoFiveLogE}{0.5115824248} %
\newcommand{\DemoTTwoRowLWQSevenFiveLogE}{0.6322442842} %
\newcommand{\DemoTTwoRowLWRate}{0} %
\newcommand{\DemoTTwoRowLWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLWMedianLogRatioToExactBound}{0.001829017326} %
\newcommand{\DemoTTwoRowLXMedianLogE}{-24.43287118} %
\newcommand{\DemoTTwoRowLXQTwoFiveLogE}{-26.88511347} %
\newcommand{\DemoTTwoRowLXQSevenFiveLogE}{-21.42049896} %
\newcommand{\DemoTTwoRowLXRate}{0} %
\newcommand{\DemoTTwoRowLXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLXMedianLogRatioToExactBound}{-0.07752463277} %
\newcommand{\DemoTTwoRowLYMedianLogE}{-2022.615168} %
\newcommand{\DemoTTwoRowLYQTwoFiveLogE}{-2326.783176} %
\newcommand{\DemoTTwoRowLYQSevenFiveLogE}{-1879.429331} %
\newcommand{\DemoTTwoRowLYRate}{0} %
\newcommand{\DemoTTwoRowLYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLYMedianLogRatioToExactBound}{-6.417686114} %
\newcommand{\DemoTTwoRowLZMedianLogE}{-2022.615168} %
\newcommand{\DemoTTwoRowLZQTwoFiveLogE}{-2326.783176} %
\newcommand{\DemoTTwoRowLZQSevenFiveLogE}{-1879.429331} %
\newcommand{\DemoTTwoRowLZRate}{0} %
\newcommand{\DemoTTwoRowLZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowLZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowLZMedianLogRatioToExactBound}{-6.417686114} %
\newcommand{\DemoTTwoRowMAMedianLogE}{4.247955674} %
\newcommand{\DemoTTwoRowMAQTwoFiveLogE}{-0.2433628632} %
\newcommand{\DemoTTwoRowMAQSevenFiveLogE}{8.839522} %
\newcommand{\DemoTTwoRowMARate}{0.5625} %
\newcommand{\DemoTTwoRowMACpNineFiveLower}{0.2987768991} %
\newcommand{\DemoTTwoRowMACpNineFiveUpper}{0.8024658595} %
\newcommand{\DemoTTwoRowMAMedianLogRatioToExactBound}{0.01347861253} %
\newcommand{\DemoTTwoRowMBMedianLogE}{-9.112974427} %
\newcommand{\DemoTTwoRowMBQTwoFiveLogE}{-10.08409143} %
\newcommand{\DemoTTwoRowMBQSevenFiveLogE}{-7.000115091} %
\newcommand{\DemoTTwoRowMBRate}{0} %
\newcommand{\DemoTTwoRowMBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMBMedianLogRatioToExactBound}{-0.0289151443} %
\newcommand{\DemoTTwoRowMCMedianLogE}{0.7984228219} %
\newcommand{\DemoTTwoRowMCQTwoFiveLogE}{0.6415240298} %
\newcommand{\DemoTTwoRowMCQSevenFiveLogE}{0.9545647364} %
\newcommand{\DemoTTwoRowMCRate}{0} %
\newcommand{\DemoTTwoRowMCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMCMedianLogRatioToExactBound}{0.002533367266} %
\newcommand{\DemoTTwoRowMDMedianLogE}{-22.88954978} %
\newcommand{\DemoTTwoRowMDQTwoFiveLogE}{-28.04913521} %
\newcommand{\DemoTTwoRowMDQSevenFiveLogE}{-18.68547103} %
\newcommand{\DemoTTwoRowMDRate}{0} %
\newcommand{\DemoTTwoRowMDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMDMedianLogRatioToExactBound}{-0.07262772876} %
\newcommand{\DemoTTwoRowMEMedianLogE}{152.7515237} %
\newcommand{\DemoTTwoRowMEQTwoFiveLogE}{149.1282329} %
\newcommand{\DemoTTwoRowMEQSevenFiveLogE}{156.4897718} %
\newcommand{\DemoTTwoRowMERate}{1} %
\newcommand{\DemoTTwoRowMECpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowMECpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowMEMedianLogRatioToExactBound}{0.4846751612} %
\newcommand{\DemoTTwoRowMFMedianLogE}{152.7394102} %
\newcommand{\DemoTTwoRowMFQTwoFiveLogE}{149.1235713} %
\newcommand{\DemoTTwoRowMFQSevenFiveLogE}{156.4869246} %
\newcommand{\DemoTTwoRowMFRate}{1} %
\newcommand{\DemoTTwoRowMFCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowMFCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowMFMedianLogRatioToExactBound}{0.4846367254} %
\newcommand{\DemoTTwoRowMGMedianLogE}{152.7439386} %
\newcommand{\DemoTTwoRowMGQTwoFiveLogE}{149.1253348} %
\newcommand{\DemoTTwoRowMGQSevenFiveLogE}{156.4880124} %
\newcommand{\DemoTTwoRowMGRate}{1} %
\newcommand{\DemoTTwoRowMGCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowMGCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowMGMedianLogRatioToExactBound}{0.4846510939} %
\newcommand{\DemoTTwoRowMHMedianLogE}{152.7515237} %
\newcommand{\DemoTTwoRowMHQTwoFiveLogE}{149.1282329} %
\newcommand{\DemoTTwoRowMHQSevenFiveLogE}{156.4897718} %
\newcommand{\DemoTTwoRowMHRate}{1} %
\newcommand{\DemoTTwoRowMHCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowMHCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowMHMedianLogRatioToExactBound}{0.4846751612} %
\newcommand{\DemoTTwoRowMIMedianLogE}{-1430.370536} %
\newcommand{\DemoTTwoRowMIQTwoFiveLogE}{-1545.794852} %
\newcommand{\DemoTTwoRowMIQSevenFiveLogE}{-1356.077219} %
\newcommand{\DemoTTwoRowMIRate}{0} %
\newcommand{\DemoTTwoRowMICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMIMedianLogRatioToExactBound}{-4.538514925} %
\newcommand{\DemoTTwoRowMJMedianLogE}{-1430.370536} %
\newcommand{\DemoTTwoRowMJQTwoFiveLogE}{-1545.794852} %
\newcommand{\DemoTTwoRowMJQSevenFiveLogE}{-1356.077219} %
\newcommand{\DemoTTwoRowMJRate}{0} %
\newcommand{\DemoTTwoRowMJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMJMedianLogRatioToExactBound}{-4.538514925} %
\newcommand{\DemoTTwoRowMKMedianLogE}{7.151587385} %
\newcommand{\DemoTTwoRowMKQTwoFiveLogE}{5.518721976} %
\newcommand{\DemoTTwoRowMKQSevenFiveLogE}{9.042362738} %
\newcommand{\DemoTTwoRowMKRate}{0.8125} %
\newcommand{\DemoTTwoRowMKCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowMKCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowMKMedianLogRatioToExactBound}{0.02269173286} %
\newcommand{\DemoTTwoRowMLMedianLogE}{-0.7298640686} %
\newcommand{\DemoTTwoRowMLQTwoFiveLogE}{-0.8029661749} %
\newcommand{\DemoTTwoRowMLQSevenFiveLogE}{-0.635715573} %
\newcommand{\DemoTTwoRowMLRate}{0} %
\newcommand{\DemoTTwoRowMLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMLMedianLogRatioToExactBound}{-0.002315832776} %
\newcommand{\DemoTTwoRowMMMedianLogE}{0.7118390492} %
\newcommand{\DemoTTwoRowMMQTwoFiveLogE}{0.6270738793} %
\newcommand{\DemoTTwoRowMMQSevenFiveLogE}{0.7701062413} %
\newcommand{\DemoTTwoRowMMRate}{0} %
\newcommand{\DemoTTwoRowMMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMMMedianLogRatioToExactBound}{0.002258640029} %
\newcommand{\DemoTTwoRowMNMedianLogE}{-21.59083206} %
\newcommand{\DemoTTwoRowMNQTwoFiveLogE}{-23.97938083} %
\newcommand{\DemoTTwoRowMNQSevenFiveLogE}{-17.69773573} %
\newcommand{\DemoTTwoRowMNRate}{0} %
\newcommand{\DemoTTwoRowMNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMNMedianLogRatioToExactBound}{-0.06850694355} %
\newcommand{\DemoTTwoRowMOMedianLogE}{-1553.899541} %
\newcommand{\DemoTTwoRowMOQTwoFiveLogE}{-1627.878901} %
\newcommand{\DemoTTwoRowMOQSevenFiveLogE}{-1344.218351} %
\newcommand{\DemoTTwoRowMORate}{0} %
\newcommand{\DemoTTwoRowMOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMOMedianLogRatioToExactBound}{-4.930468072} %
\newcommand{\DemoTTwoRowMPMedianLogE}{3.074872956} %
\newcommand{\DemoTTwoRowMPQTwoFiveLogE}{2.834610132} %
\newcommand{\DemoTTwoRowMPQSevenFiveLogE}{3.839117025} %
\newcommand{\DemoTTwoRowMPRate}{0.5625} %
\newcommand{\DemoTTwoRowMPCpNineFiveLower}{0.2987768991} %
\newcommand{\DemoTTwoRowMPCpNineFiveUpper}{0.8024658595} %
\newcommand{\DemoTTwoRowMPMedianLogRatioToExactBound}{0.009756462717} %
\newcommand{\DemoTTwoRowMQMedianLogE}{7.789374294} %
\newcommand{\DemoTTwoRowMQQTwoFiveLogE}{4.921248578} %
\newcommand{\DemoTTwoRowMQQSevenFiveLogE}{8.981358292} %
\newcommand{\DemoTTwoRowMQRate}{0.9375} %
\newcommand{\DemoTTwoRowMQCpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowMQCpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowMQMedianLogRatioToExactBound}{0.02471540807} %
\newcommand{\DemoTTwoRowMRMedianLogE}{-0.0009927726839} %
\newcommand{\DemoTTwoRowMRQTwoFiveLogE}{-0.09912744901} %
\newcommand{\DemoTTwoRowMRQSevenFiveLogE}{0.04747468542} %
\newcommand{\DemoTTwoRowMRRate}{0} %
\newcommand{\DemoTTwoRowMRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMRMedianLogRatioToExactBound}{-3.150032478e-06} %
\newcommand{\DemoTTwoRowMSMedianLogE}{0.638786755} %
\newcommand{\DemoTTwoRowMSQTwoFiveLogE}{0.5401511929} %
\newcommand{\DemoTTwoRowMSQSevenFiveLogE}{0.7272034849} %
\newcommand{\DemoTTwoRowMSRate}{0} %
\newcommand{\DemoTTwoRowMSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMSMedianLogRatioToExactBound}{0.002026847694} %
\newcommand{\DemoTTwoRowMTMedianLogE}{-23.69367146} %
\newcommand{\DemoTTwoRowMTQTwoFiveLogE}{-25.03035656} %
\newcommand{\DemoTTwoRowMTQSevenFiveLogE}{-21.66854235} %
\newcommand{\DemoTTwoRowMTRate}{0} %
\newcommand{\DemoTTwoRowMTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMTMedianLogRatioToExactBound}{-0.07517917829} %
\newcommand{\DemoTTwoRowMUMedianLogE}{-2723.018367} %
\newcommand{\DemoTTwoRowMUQTwoFiveLogE}{-2809.539442} %
\newcommand{\DemoTTwoRowMUQSevenFiveLogE}{-2483.854137} %
\newcommand{\DemoTTwoRowMURate}{0} %
\newcommand{\DemoTTwoRowMUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMUMedianLogRatioToExactBound}{-8.640040599} %
\newcommand{\DemoTTwoRowMVMedianLogE}{4.399949453} %
\newcommand{\DemoTTwoRowMVQTwoFiveLogE}{3.877727663} %
\newcommand{\DemoTTwoRowMVQSevenFiveLogE}{4.873160404} %
\newcommand{\DemoTTwoRowMVRate}{0.9375} %
\newcommand{\DemoTTwoRowMVCpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowMVCpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowMVMedianLogRatioToExactBound}{0.01396088339} %
\newcommand{\DemoTTwoRowMWMedianLogE}{6.681728322} %
\newcommand{\DemoTTwoRowMWQTwoFiveLogE}{4.288071717} %
\newcommand{\DemoTTwoRowMWQSevenFiveLogE}{7.920879957} %
\newcommand{\DemoTTwoRowMWRate}{0.875} %
\newcommand{\DemoTTwoRowMWCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowMWCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowMWMedianLogRatioToExactBound}{0.02120088673} %
\newcommand{\DemoTTwoRowMXMedianLogE}{-0.09493835727} %
\newcommand{\DemoTTwoRowMXQTwoFiveLogE}{-0.3185894953} %
\newcommand{\DemoTTwoRowMXQSevenFiveLogE}{0.1190001166} %
\newcommand{\DemoTTwoRowMXRate}{0} %
\newcommand{\DemoTTwoRowMXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMXMedianLogRatioToExactBound}{-0.0003012360368} %
\newcommand{\DemoTTwoRowMYMedianLogE}{0.8304612654} %
\newcommand{\DemoTTwoRowMYQTwoFiveLogE}{0.7747841353} %
\newcommand{\DemoTTwoRowMYQSevenFiveLogE}{1.004139268} %
\newcommand{\DemoTTwoRowMYRate}{0} %
\newcommand{\DemoTTwoRowMYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMYMedianLogRatioToExactBound}{0.00263502411} %
\newcommand{\DemoTTwoRowMZMedianLogE}{-24.56618087} %
\newcommand{\DemoTTwoRowMZQTwoFiveLogE}{-26.17096179} %
\newcommand{\DemoTTwoRowMZQSevenFiveLogE}{-20.99724999} %
\newcommand{\DemoTTwoRowMZRate}{0} %
\newcommand{\DemoTTwoRowMZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowMZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowMZMedianLogRatioToExactBound}{-0.07794761968} %
\newcommand{\DemoTTwoRowNAMedianLogE}{153.8486874} %
\newcommand{\DemoTTwoRowNAQTwoFiveLogE}{151.7794857} %
\newcommand{\DemoTTwoRowNAQSevenFiveLogE}{155.3305576} %
\newcommand{\DemoTTwoRowNARate}{1} %
\newcommand{\DemoTTwoRowNACpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNACpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNAMedianLogRatioToExactBound}{0.4881564227} %
\newcommand{\DemoTTwoRowNBMedianLogE}{19.15735086} %
\newcommand{\DemoTTwoRowNBQTwoFiveLogE}{18.32590847} %
\newcommand{\DemoTTwoRowNBQSevenFiveLogE}{19.58382892} %
\newcommand{\DemoTTwoRowNBRate}{1} %
\newcommand{\DemoTTwoRowNBCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNBCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNBMedianLogRatioToExactBound}{0.06078559408} %
\newcommand{\DemoTTwoRowNCMedianLogE}{153.8486874} %
\newcommand{\DemoTTwoRowNCQTwoFiveLogE}{151.7794857} %
\newcommand{\DemoTTwoRowNCQSevenFiveLogE}{155.3305576} %
\newcommand{\DemoTTwoRowNCRate}{1} %
\newcommand{\DemoTTwoRowNCCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNCCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNCMedianLogRatioToExactBound}{0.4881564227} %
\newcommand{\DemoTTwoRowNDMedianLogE}{153.9831147} %
\newcommand{\DemoTTwoRowNDQTwoFiveLogE}{153.2668181} %
\newcommand{\DemoTTwoRowNDQSevenFiveLogE}{156.8093473} %
\newcommand{\DemoTTwoRowNDRate}{1} %
\newcommand{\DemoTTwoRowNDCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNDCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNDMedianLogRatioToExactBound}{0.4885829558} %
\newcommand{\DemoTTwoRowNEMedianLogE}{-1554.592688} %
\newcommand{\DemoTTwoRowNEQTwoFiveLogE}{-1628.572048} %
\newcommand{\DemoTTwoRowNEQSevenFiveLogE}{-1344.911498} %
\newcommand{\DemoTTwoRowNERate}{0} %
\newcommand{\DemoTTwoRowNECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNEMedianLogRatioToExactBound}{-4.932667404} %
\newcommand{\DemoTTwoRowNFMedianLogE}{4.030945798} %
\newcommand{\DemoTTwoRowNFQTwoFiveLogE}{3.603780906} %
\newcommand{\DemoTTwoRowNFQSevenFiveLogE}{4.471862323} %
\newcommand{\DemoTTwoRowNFRate}{0.9375} %
\newcommand{\DemoTTwoRowNFCpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowNFCpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowNFMedianLogRatioToExactBound}{0.0127900479} %
\newcommand{\DemoTTwoRowNGMedianLogE}{7.901538478} %
\newcommand{\DemoTTwoRowNGQTwoFiveLogE}{5.116900585} %
\newcommand{\DemoTTwoRowNGQSevenFiveLogE}{9.010258999} %
\newcommand{\DemoTTwoRowNGRate}{0.875} %
\newcommand{\DemoTTwoRowNGCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowNGCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowNGMedianLogRatioToExactBound}{0.02507130105} %
\newcommand{\DemoTTwoRowNHMedianLogE}{-0.07023467597} %
\newcommand{\DemoTTwoRowNHQTwoFiveLogE}{-0.2284406135} %
\newcommand{\DemoTTwoRowNHQSevenFiveLogE}{0.08267978311} %
\newcommand{\DemoTTwoRowNHRate}{0} %
\newcommand{\DemoTTwoRowNHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNHMedianLogRatioToExactBound}{-0.0002228521332} %
\newcommand{\DemoTTwoRowNIMedianLogE}{0.7647814337} %
\newcommand{\DemoTTwoRowNIQTwoFiveLogE}{0.685843793} %
\newcommand{\DemoTTwoRowNIQSevenFiveLogE}{0.8322839954} %
\newcommand{\DemoTTwoRowNIRate}{0} %
\newcommand{\DemoTTwoRowNICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNIMedianLogRatioToExactBound}{0.002426624336} %
\newcommand{\DemoTTwoRowNJMedianLogE}{-22.01676553} %
\newcommand{\DemoTTwoRowNJQTwoFiveLogE}{-24.10099219} %
\newcommand{\DemoTTwoRowNJQSevenFiveLogE}{-17.7166043} %
\newcommand{\DemoTTwoRowNJRate}{0} %
\newcommand{\DemoTTwoRowNJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNJMedianLogRatioToExactBound}{-0.06985841533} %
\newcommand{\DemoTTwoRowNKMedianLogE}{-1580.585166} %
\newcommand{\DemoTTwoRowNKQTwoFiveLogE}{-1713.825001} %
\newcommand{\DemoTTwoRowNKQSevenFiveLogE}{-1454.166997} %
\newcommand{\DemoTTwoRowNKRate}{0} %
\newcommand{\DemoTTwoRowNKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNKMedianLogRatioToExactBound}{-5.015140613} %
\newcommand{\DemoTTwoRowNLMedianLogE}{-1580.585166} %
\newcommand{\DemoTTwoRowNLQTwoFiveLogE}{-1713.825001} %
\newcommand{\DemoTTwoRowNLQSevenFiveLogE}{-1454.166997} %
\newcommand{\DemoTTwoRowNLRate}{0} %
\newcommand{\DemoTTwoRowNLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNLMedianLogRatioToExactBound}{-5.015140613} %
\newcommand{\DemoTTwoRowNMMedianLogE}{8.36238162} %
\newcommand{\DemoTTwoRowNMQTwoFiveLogE}{5.730205187} %
\newcommand{\DemoTTwoRowNMQSevenFiveLogE}{11.55407516} %
\newcommand{\DemoTTwoRowNMRate}{0.9375} %
\newcommand{\DemoTTwoRowNMCpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowNMCpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowNMMedianLogRatioToExactBound}{0.02653353997} %
\newcommand{\DemoTTwoRowNNMedianLogE}{-0.147098281} %
\newcommand{\DemoTTwoRowNNQTwoFiveLogE}{-0.7070585863} %
\newcommand{\DemoTTwoRowNNQSevenFiveLogE}{0.02840319851} %
\newcommand{\DemoTTwoRowNNRate}{0} %
\newcommand{\DemoTTwoRowNNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNNMedianLogRatioToExactBound}{-0.0004667376229} %
\newcommand{\DemoTTwoRowNOMedianLogE}{0.7589269012} %
\newcommand{\DemoTTwoRowNOQTwoFiveLogE}{0.6532731733} %
\newcommand{\DemoTTwoRowNOQSevenFiveLogE}{0.8579447094} %
\newcommand{\DemoTTwoRowNORate}{0} %
\newcommand{\DemoTTwoRowNOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNOMedianLogRatioToExactBound}{0.002408048112} %
\newcommand{\DemoTTwoRowNPMedianLogE}{-21.23883934} %
\newcommand{\DemoTTwoRowNPQTwoFiveLogE}{-23.8549073} %
\newcommand{\DemoTTwoRowNPQSevenFiveLogE}{-17.26406347} %
\newcommand{\DemoTTwoRowNPRate}{0} %
\newcommand{\DemoTTwoRowNPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNPMedianLogRatioToExactBound}{-0.06739008314} %
\newcommand{\DemoTTwoRowNQMedianLogE}{-2173.817136} %
\newcommand{\DemoTTwoRowNQQTwoFiveLogE}{-2313.390368} %
\newcommand{\DemoTTwoRowNQQSevenFiveLogE}{-1834.560231} %
\newcommand{\DemoTTwoRowNQRate}{0} %
\newcommand{\DemoTTwoRowNQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNQMedianLogRatioToExactBound}{-6.897444592} %
\newcommand{\DemoTTwoRowNRMedianLogE}{-2173.817136} %
\newcommand{\DemoTTwoRowNRQTwoFiveLogE}{-2313.390368} %
\newcommand{\DemoTTwoRowNRQSevenFiveLogE}{-1834.560231} %
\newcommand{\DemoTTwoRowNRRate}{0} %
\newcommand{\DemoTTwoRowNRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNRMedianLogRatioToExactBound}{-6.897444592} %
\newcommand{\DemoTTwoRowNSMedianLogE}{7.060080056} %
\newcommand{\DemoTTwoRowNSQTwoFiveLogE}{3.611296794} %
\newcommand{\DemoTTwoRowNSQSevenFiveLogE}{12.10789513} %
\newcommand{\DemoTTwoRowNSRate}{0.75} %
\newcommand{\DemoTTwoRowNSCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowNSCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowNSMedianLogRatioToExactBound}{0.02240138335} %
\newcommand{\DemoTTwoRowNTMedianLogE}{-31.59482457} %
\newcommand{\DemoTTwoRowNTQTwoFiveLogE}{-40.5275644} %
\newcommand{\DemoTTwoRowNTQSevenFiveLogE}{-28.12122943} %
\newcommand{\DemoTTwoRowNTRate}{0} %
\newcommand{\DemoTTwoRowNTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNTMedianLogRatioToExactBound}{-0.1002492566} %
\newcommand{\DemoTTwoRowNUMedianLogE}{0.9707351382} %
\newcommand{\DemoTTwoRowNUQTwoFiveLogE}{0.7649590761} %
\newcommand{\DemoTTwoRowNUQSevenFiveLogE}{1.109022677} %
\newcommand{\DemoTTwoRowNURate}{0} %
\newcommand{\DemoTTwoRowNUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNUMedianLogRatioToExactBound}{0.003080108128} %
\newcommand{\DemoTTwoRowNVMedianLogE}{-24.22419465} %
\newcommand{\DemoTTwoRowNVQTwoFiveLogE}{-27.07529301} %
\newcommand{\DemoTTwoRowNVQSevenFiveLogE}{-21.30001998} %
\newcommand{\DemoTTwoRowNVRate}{0} %
\newcommand{\DemoTTwoRowNVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowNVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowNVMedianLogRatioToExactBound}{-0.07686250956} %
\newcommand{\DemoTTwoRowNWMedianLogE}{155.0801913} %
\newcommand{\DemoTTwoRowNWQTwoFiveLogE}{152.6398988} %
\newcommand{\DemoTTwoRowNWQSevenFiveLogE}{158.0209695} %
\newcommand{\DemoTTwoRowNWRate}{1} %
\newcommand{\DemoTTwoRowNWCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNWCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNWMedianLogRatioToExactBound}{0.4920639408} %
\newcommand{\DemoTTwoRowNXMedianLogE}{146.7406746} %
\newcommand{\DemoTTwoRowNXQTwoFiveLogE}{144.5736659} %
\newcommand{\DemoTTwoRowNXQSevenFiveLogE}{148.8580584} %
\newcommand{\DemoTTwoRowNXRate}{1} %
\newcommand{\DemoTTwoRowNXCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNXCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNXMedianLogRatioToExactBound}{0.4656029504} %
\newcommand{\DemoTTwoRowNYMedianLogE}{152.9930607} %
\newcommand{\DemoTTwoRowNYQTwoFiveLogE}{150.6014239} %
\newcommand{\DemoTTwoRowNYQSevenFiveLogE}{154.7804456} %
\newcommand{\DemoTTwoRowNYRate}{1} %
\newcommand{\DemoTTwoRowNYCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNYCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNYMedianLogRatioToExactBound}{0.4854415495} %
\newcommand{\DemoTTwoRowNZMedianLogE}{155.1347119} %
\newcommand{\DemoTTwoRowNZQTwoFiveLogE}{152.3426147} %
\newcommand{\DemoTTwoRowNZQSevenFiveLogE}{157.8774744} %
\newcommand{\DemoTTwoRowNZRate}{1} %
\newcommand{\DemoTTwoRowNZCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowNZCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowNZMedianLogRatioToExactBound}{0.4922369327} %
\newcommand{\DemoTTwoRowOAMedianLogE}{-1542.49843} %
\newcommand{\DemoTTwoRowOAQTwoFiveLogE}{-1654.814277} %
\newcommand{\DemoTTwoRowOAQSevenFiveLogE}{-1454.860145} %
\newcommand{\DemoTTwoRowOARate}{0} %
\newcommand{\DemoTTwoRowOACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOAMedianLogRatioToExactBound}{-4.894292752} %
\newcommand{\DemoTTwoRowOBMedianLogE}{-1542.49843} %
\newcommand{\DemoTTwoRowOBQTwoFiveLogE}{-1654.814277} %
\newcommand{\DemoTTwoRowOBQSevenFiveLogE}{-1454.860145} %
\newcommand{\DemoTTwoRowOBRate}{0} %
\newcommand{\DemoTTwoRowOBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOBMedianLogRatioToExactBound}{-4.894292752} %
\newcommand{\DemoTTwoRowOCMedianLogE}{9.250546157} %
\newcommand{\DemoTTwoRowOCQTwoFiveLogE}{6.252291636} %
\newcommand{\DemoTTwoRowOCQSevenFiveLogE}{12.16118875} %
\newcommand{\DemoTTwoRowOCRate}{1} %
\newcommand{\DemoTTwoRowOCCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOCCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOCMedianLogRatioToExactBound}{0.02935165452} %
\newcommand{\DemoTTwoRowODMedianLogE}{-0.8402454615} %
\newcommand{\DemoTTwoRowODQTwoFiveLogE}{-1.400205763} %
\newcommand{\DemoTTwoRowODQSevenFiveLogE}{-0.6647439821} %
\newcommand{\DemoTTwoRowODRate}{0} %
\newcommand{\DemoTTwoRowODCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowODCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowODMedianLogRatioToExactBound}{-0.002666069017} %
\newcommand{\DemoTTwoRowOEMedianLogE}{0.8619844683} %
\newcommand{\DemoTTwoRowOEQTwoFiveLogE}{0.7059698704} %
\newcommand{\DemoTTwoRowOEQSevenFiveLogE}{1.026630847} %
\newcommand{\DemoTTwoRowOERate}{0} %
\newcommand{\DemoTTwoRowOECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOEMedianLogRatioToExactBound}{0.002735046113} %
\newcommand{\DemoTTwoRowOFMedianLogE}{-21.26866582} %
\newcommand{\DemoTTwoRowOFQTwoFiveLogE}{-23.78805219} %
\newcommand{\DemoTTwoRowOFQSevenFiveLogE}{-17.93956638} %
\newcommand{\DemoTTwoRowOFRate}{0} %
\newcommand{\DemoTTwoRowOFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOFMedianLogRatioToExactBound}{-0.0674847215} %
\newcommand{\DemoTTwoRowOGMedianLogE}{-2676.633511} %
\newcommand{\DemoTTwoRowOGQTwoFiveLogE}{-3046.519124} %
\newcommand{\DemoTTwoRowOGQSevenFiveLogE}{-2447.167548} %
\newcommand{\DemoTTwoRowOGRate}{0} %
\newcommand{\DemoTTwoRowOGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOGMedianLogRatioToExactBound}{-8.492863098} %
\newcommand{\DemoTTwoRowOHMedianLogE}{-2676.633511} %
\newcommand{\DemoTTwoRowOHQTwoFiveLogE}{-3046.519124} %
\newcommand{\DemoTTwoRowOHQSevenFiveLogE}{-2447.167548} %
\newcommand{\DemoTTwoRowOHRate}{0} %
\newcommand{\DemoTTwoRowOHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOHMedianLogRatioToExactBound}{-8.492863098} %
\newcommand{\DemoTTwoRowOIMedianLogE}{0.7553814641} %
\newcommand{\DemoTTwoRowOIQTwoFiveLogE}{-0.4136041523} %
\newcommand{\DemoTTwoRowOIQSevenFiveLogE}{1.832421417} %
\newcommand{\DemoTTwoRowOIRate}{0.0625} %
\newcommand{\DemoTTwoRowOICpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowOICpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowOIMedianLogRatioToExactBound}{0.002396798566} %
\newcommand{\DemoTTwoRowOJMedianLogE}{-0.03144883796} %
\newcommand{\DemoTTwoRowOJQTwoFiveLogE}{-0.1670239361} %
\newcommand{\DemoTTwoRowOJQSevenFiveLogE}{0.1057399675} %
\newcommand{\DemoTTwoRowOJRate}{0} %
\newcommand{\DemoTTwoRowOJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOJMedianLogRatioToExactBound}{-9.978604627e-05} %
\newcommand{\DemoTTwoRowOKMedianLogE}{0.07389335758} %
\newcommand{\DemoTTwoRowOKQTwoFiveLogE}{0.04195738028} %
\newcommand{\DemoTTwoRowOKQSevenFiveLogE}{0.09611768512} %
\newcommand{\DemoTTwoRowOKRate}{0} %
\newcommand{\DemoTTwoRowOKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOKMedianLogRatioToExactBound}{0.000234461} %
\newcommand{\DemoTTwoRowOLMedianLogE}{-27.06328774} %
\newcommand{\DemoTTwoRowOLQTwoFiveLogE}{-28.60833649} %
\newcommand{\DemoTTwoRowOLQSevenFiveLogE}{-25.02033646} %
\newcommand{\DemoTTwoRowOLRate}{0} %
\newcommand{\DemoTTwoRowOLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOLMedianLogRatioToExactBound}{-0.08587085113} %
\newcommand{\DemoTTwoRowOMMedianLogE}{-3419.034467} %
\newcommand{\DemoTTwoRowOMQTwoFiveLogE}{-3843.474074} %
\newcommand{\DemoTTwoRowOMQSevenFiveLogE}{-3127.379596} %
\newcommand{\DemoTTwoRowOMRate}{0} %
\newcommand{\DemoTTwoRowOMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOMMedianLogRatioToExactBound}{-10.84847497} %
\newcommand{\DemoTTwoRowONMedianLogE}{-3419.034467} %
\newcommand{\DemoTTwoRowONQTwoFiveLogE}{-3843.474074} %
\newcommand{\DemoTTwoRowONQSevenFiveLogE}{-3127.379596} %
\newcommand{\DemoTTwoRowONRate}{0} %
\newcommand{\DemoTTwoRowONCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowONCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowONMedianLogRatioToExactBound}{-10.84847497} %
\newcommand{\DemoTTwoRowOOMedianLogE}{0.3043237883} %
\newcommand{\DemoTTwoRowOOQTwoFiveLogE}{-1.555808266} %
\newcommand{\DemoTTwoRowOOQSevenFiveLogE}{3.302070295} %
\newcommand{\DemoTTwoRowOORate}{0.3125} %
\newcommand{\DemoTTwoRowOOCpNineFiveLower}{0.1101699547} %
\newcommand{\DemoTTwoRowOOCpNineFiveUpper}{0.5866206365} %
\newcommand{\DemoTTwoRowOOMedianLogRatioToExactBound}{0.0009656085753} %
\newcommand{\DemoTTwoRowOPMedianLogE}{-10.98934469} %
\newcommand{\DemoTTwoRowOPQTwoFiveLogE}{-17.67075767} %
\newcommand{\DemoTTwoRowOPQSevenFiveLogE}{-7.134171269} %
\newcommand{\DemoTTwoRowOPRate}{0} %
\newcommand{\DemoTTwoRowOPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOPMedianLogRatioToExactBound}{-0.03486880052} %
\newcommand{\DemoTTwoRowOQMedianLogE}{0.07321082803} %
\newcommand{\DemoTTwoRowOQQTwoFiveLogE}{0.01831223583} %
\newcommand{\DemoTTwoRowOQQSevenFiveLogE}{0.1398793094} %
\newcommand{\DemoTTwoRowOQRate}{0} %
\newcommand{\DemoTTwoRowOQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOQMedianLogRatioToExactBound}{0.000232295358} %
\newcommand{\DemoTTwoRowORMedianLogE}{-26.9676015} %
\newcommand{\DemoTTwoRowORQTwoFiveLogE}{-29.53903526} %
\newcommand{\DemoTTwoRowORQSevenFiveLogE}{-25.62531955} %
\newcommand{\DemoTTwoRowORRate}{0} %
\newcommand{\DemoTTwoRowORCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowORCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowORMedianLogRatioToExactBound}{-0.08556724207} %
\newcommand{\DemoTTwoRowOSMedianLogE}{135.4222888} %
\newcommand{\DemoTTwoRowOSQTwoFiveLogE}{132.6833226} %
\newcommand{\DemoTTwoRowOSQSevenFiveLogE}{138.9674829} %
\newcommand{\DemoTTwoRowOSRate}{1} %
\newcommand{\DemoTTwoRowOSCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOSCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOSMedianLogRatioToExactBound}{0.4296901143} %
\newcommand{\DemoTTwoRowOTMedianLogE}{135.4021661} %
\newcommand{\DemoTTwoRowOTQTwoFiveLogE}{132.6804687} %
\newcommand{\DemoTTwoRowOTQSevenFiveLogE}{138.9713827} %
\newcommand{\DemoTTwoRowOTRate}{1} %
\newcommand{\DemoTTwoRowOTCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOTCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOTMedianLogRatioToExactBound}{0.4296262655} %
\newcommand{\DemoTTwoRowOUMedianLogE}{135.2075983} %
\newcommand{\DemoTTwoRowOUQTwoFiveLogE}{132.6434077} %
\newcommand{\DemoTTwoRowOUQSevenFiveLogE}{138.9971215} %
\newcommand{\DemoTTwoRowOURate}{1} %
\newcommand{\DemoTTwoRowOUCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOUCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOUMedianLogRatioToExactBound}{0.429008909} %
\newcommand{\DemoTTwoRowOVMedianLogE}{135.4222888} %
\newcommand{\DemoTTwoRowOVQTwoFiveLogE}{132.6833226} %
\newcommand{\DemoTTwoRowOVQSevenFiveLogE}{138.9674829} %
\newcommand{\DemoTTwoRowOVRate}{1} %
\newcommand{\DemoTTwoRowOVCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowOVCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowOVMedianLogRatioToExactBound}{0.4296901143} %
\newcommand{\DemoTTwoRowOWMedianLogE}{-2677.326659} %
\newcommand{\DemoTTwoRowOWQTwoFiveLogE}{-3047.212271} %
\newcommand{\DemoTTwoRowOWQSevenFiveLogE}{-2447.860695} %
\newcommand{\DemoTTwoRowOWRate}{0} %
\newcommand{\DemoTTwoRowOWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOWMedianLogRatioToExactBound}{-8.495062429} %
\newcommand{\DemoTTwoRowOXMedianLogE}{-2677.326659} %
\newcommand{\DemoTTwoRowOXQTwoFiveLogE}{-3047.212271} %
\newcommand{\DemoTTwoRowOXQSevenFiveLogE}{-2447.860695} %
\newcommand{\DemoTTwoRowOXRate}{0} %
\newcommand{\DemoTTwoRowOXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOXMedianLogRatioToExactBound}{-8.495062429} %
\newcommand{\DemoTTwoRowOYMedianLogE}{0.3086364197} %
\newcommand{\DemoTTwoRowOYQTwoFiveLogE}{-0.1837726516} %
\newcommand{\DemoTTwoRowOYQSevenFiveLogE}{2.825595668} %
\newcommand{\DemoTTwoRowOYRate}{0.25} %
\newcommand{\DemoTTwoRowOYCpNineFiveLower}{0.07266203825} %
\newcommand{\DemoTTwoRowOYCpNineFiveUpper}{0.5237708199} %
\newcommand{\DemoTTwoRowOYMedianLogRatioToExactBound}{0.0009792924015} %
\newcommand{\DemoTTwoRowOZMedianLogE}{-0.7132422355} %
\newcommand{\DemoTTwoRowOZQTwoFiveLogE}{-0.8585411732} %
\newcommand{\DemoTTwoRowOZQSevenFiveLogE}{-0.5855091788} %
\newcommand{\DemoTTwoRowOZRate}{0} %
\newcommand{\DemoTTwoRowOZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowOZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowOZMedianLogRatioToExactBound}{-0.00226309229} %
\newcommand{\DemoTTwoRowPAMedianLogE}{0.05803118891} %
\newcommand{\DemoTTwoRowPAQTwoFiveLogE}{0.03275907846} %
\newcommand{\DemoTTwoRowPAQSevenFiveLogE}{0.1170491062} %
\newcommand{\DemoTTwoRowPARate}{0} %
\newcommand{\DemoTTwoRowPACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPAMedianLogRatioToExactBound}{0.000184130902} %
\newcommand{\DemoTTwoRowPBMedianLogE}{-25.99745585} %
\newcommand{\DemoTTwoRowPBQTwoFiveLogE}{-27.61985415} %
\newcommand{\DemoTTwoRowPBQSevenFiveLogE}{-24.96501056} %
\newcommand{\DemoTTwoRowPBRate}{0} %
\newcommand{\DemoTTwoRowPBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPBMedianLogRatioToExactBound}{-0.08248900437} %
\newcommand{\DemoTTwoRowPCMedianLogE}{-3235.13383} %
\newcommand{\DemoTTwoRowPCQTwoFiveLogE}{-3480.38871} %
\newcommand{\DemoTTwoRowPCQSevenFiveLogE}{-2886.589772} %
\newcommand{\DemoTTwoRowPCRate}{0} %
\newcommand{\DemoTTwoRowPCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPCMedianLogRatioToExactBound}{-10.26496478} %
\newcommand{\DemoTTwoRowPDMedianLogE}{0.2597978623} %
\newcommand{\DemoTTwoRowPDQTwoFiveLogE}{0.1445370921} %
\newcommand{\DemoTTwoRowPDQSevenFiveLogE}{0.5146644725} %
\newcommand{\DemoTTwoRowPDRate}{0} %
\newcommand{\DemoTTwoRowPDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPDMedianLogRatioToExactBound}{0.0008243293931} %
\newcommand{\DemoTTwoRowPEMedianLogE}{0.6621980794} %
\newcommand{\DemoTTwoRowPEQTwoFiveLogE}{-0.04599374594} %
\newcommand{\DemoTTwoRowPEQSevenFiveLogE}{1.432169176} %
\newcommand{\DemoTTwoRowPERate}{0.0625} %
\newcommand{\DemoTTwoRowPECpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowPECpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowPEMedianLogRatioToExactBound}{0.002101130995} %
\newcommand{\DemoTTwoRowPFMedianLogE}{0.1046759714} %
\newcommand{\DemoTTwoRowPFQTwoFiveLogE}{0.01949815646} %
\newcommand{\DemoTTwoRowPFQSevenFiveLogE}{0.2105466693} %
\newcommand{\DemoTTwoRowPFRate}{0} %
\newcommand{\DemoTTwoRowPFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPFMedianLogRatioToExactBound}{0.0003321331408} %
\newcommand{\DemoTTwoRowPGMedianLogE}{0.04626335489} %
\newcommand{\DemoTTwoRowPGQTwoFiveLogE}{0.03065146663} %
\newcommand{\DemoTTwoRowPGQSevenFiveLogE}{0.09519590877} %
\newcommand{\DemoTTwoRowPGRate}{0} %
\newcommand{\DemoTTwoRowPGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPGMedianLogRatioToExactBound}{0.0001467919825} %
\newcommand{\DemoTTwoRowPHMedianLogE}{-26.32899277} %
\newcommand{\DemoTTwoRowPHQTwoFiveLogE}{-29.65483651} %
\newcommand{\DemoTTwoRowPHQSevenFiveLogE}{-25.97167987} %
\newcommand{\DemoTTwoRowPHRate}{0} %
\newcommand{\DemoTTwoRowPHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPHMedianLogRatioToExactBound}{-0.08354095926} %
\newcommand{\DemoTTwoRowPIMedianLogE}{-7636.389357} %
\newcommand{\DemoTTwoRowPIQTwoFiveLogE}{-8062.792458} %
\newcommand{\DemoTTwoRowPIQSevenFiveLogE}{-6780.132772} %
\newcommand{\DemoTTwoRowPIRate}{0} %
\newcommand{\DemoTTwoRowPICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPIMedianLogRatioToExactBound}{-24.2299923} %
\newcommand{\DemoTTwoRowPJMedianLogE}{0.0460944172} %
\newcommand{\DemoTTwoRowPJQTwoFiveLogE}{-0.5577332636} %
\newcommand{\DemoTTwoRowPJQSevenFiveLogE}{0.4716477676} %
\newcommand{\DemoTTwoRowPJRate}{0} %
\newcommand{\DemoTTwoRowPJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPJMedianLogRatioToExactBound}{0.0001462559492} %
\newcommand{\DemoTTwoRowPKMedianLogE}{-0.14416679} %
\newcommand{\DemoTTwoRowPKQTwoFiveLogE}{-0.9846514004} %
\newcommand{\DemoTTwoRowPKQSevenFiveLogE}{0.6214390614} %
\newcommand{\DemoTTwoRowPKRate}{0} %
\newcommand{\DemoTTwoRowPKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPKMedianLogRatioToExactBound}{-0.0004574361059} %
\newcommand{\DemoTTwoRowPLMedianLogE}{-0.09289267306} %
\newcommand{\DemoTTwoRowPLQTwoFiveLogE}{-0.5394865375} %
\newcommand{\DemoTTwoRowPLQSevenFiveLogE}{0.2285761774} %
\newcommand{\DemoTTwoRowPLRate}{0} %
\newcommand{\DemoTTwoRowPLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPLMedianLogRatioToExactBound}{-0.0002947451535} %
\newcommand{\DemoTTwoRowPMMedianLogE}{0.02619628954} %
\newcommand{\DemoTTwoRowPMQTwoFiveLogE}{-0.07676643415} %
\newcommand{\DemoTTwoRowPMQSevenFiveLogE}{0.07480448067} %
\newcommand{\DemoTTwoRowPMRate}{0} %
\newcommand{\DemoTTwoRowPMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPMMedianLogRatioToExactBound}{8.311989662e-05} %
\newcommand{\DemoTTwoRowPNMedianLogE}{-29.09780566} %
\newcommand{\DemoTTwoRowPNQTwoFiveLogE}{-30.46772313} %
\newcommand{\DemoTTwoRowPNQSevenFiveLogE}{-26.56813138} %
\newcommand{\DemoTTwoRowPNRate}{0} %
\newcommand{\DemoTTwoRowPNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPNMedianLogRatioToExactBound}{-0.09232630425} %
\newcommand{\DemoTTwoRowPOMedianLogE}{132.996121} %
\newcommand{\DemoTTwoRowPOQTwoFiveLogE}{129.4214401} %
\newcommand{\DemoTTwoRowPOQSevenFiveLogE}{137.0290456} %
\newcommand{\DemoTTwoRowPORate}{1} %
\newcommand{\DemoTTwoRowPOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowPOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowPOMedianLogRatioToExactBound}{0.4219919699} %
\newcommand{\DemoTTwoRowPPMedianLogE}{1.550331566} %
\newcommand{\DemoTTwoRowPPQTwoFiveLogE}{1.503760667} %
\newcommand{\DemoTTwoRowPPQSevenFiveLogE}{1.607526383} %
\newcommand{\DemoTTwoRowPPRate}{0} %
\newcommand{\DemoTTwoRowPPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPPMedianLogRatioToExactBound}{0.004919147015} %
\newcommand{\DemoTTwoRowPQMedianLogE}{132.996121} %
\newcommand{\DemoTTwoRowPQQTwoFiveLogE}{129.4214401} %
\newcommand{\DemoTTwoRowPQQSevenFiveLogE}{137.0290456} %
\newcommand{\DemoTTwoRowPQRate}{1} %
\newcommand{\DemoTTwoRowPQCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowPQCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowPQMedianLogRatioToExactBound}{0.4219919699} %
\newcommand{\DemoTTwoRowPRMedianLogE}{134.9241579} %
\newcommand{\DemoTTwoRowPRQTwoFiveLogE}{131.4386113} %
\newcommand{\DemoTTwoRowPRQSevenFiveLogE}{140.8387137} %
\newcommand{\DemoTTwoRowPRRate}{1} %
\newcommand{\DemoTTwoRowPRCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowPRCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowPRMedianLogRatioToExactBound}{0.4281095626} %
\newcommand{\DemoTTwoRowPSMedianLogE}{-3235.826978} %
\newcommand{\DemoTTwoRowPSQTwoFiveLogE}{-3481.081857} %
\newcommand{\DemoTTwoRowPSQSevenFiveLogE}{-2887.28292} %
\newcommand{\DemoTTwoRowPSRate}{0} %
\newcommand{\DemoTTwoRowPSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPSMedianLogRatioToExactBound}{-10.26716411} %
\newcommand{\DemoTTwoRowPTMedianLogE}{0.1534062189} %
\newcommand{\DemoTTwoRowPTQTwoFiveLogE}{0.07124234174} %
\newcommand{\DemoTTwoRowPTQSevenFiveLogE}{0.4549165111} %
\newcommand{\DemoTTwoRowPTRate}{0} %
\newcommand{\DemoTTwoRowPTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPTMedianLogRatioToExactBound}{0.000486752486} %
\newcommand{\DemoTTwoRowPUMedianLogE}{0.4486704274} %
\newcommand{\DemoTTwoRowPUQTwoFiveLogE}{-0.0343386467} %
\newcommand{\DemoTTwoRowPUQSevenFiveLogE}{1.101507301} %
\newcommand{\DemoTTwoRowPURate}{0.0625} %
\newcommand{\DemoTTwoRowPUCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowPUCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowPUMedianLogRatioToExactBound}{0.001423615336} %
\newcommand{\DemoTTwoRowPVMedianLogE}{-0.01419722078} %
\newcommand{\DemoTTwoRowPVQTwoFiveLogE}{-0.1775285285} %
\newcommand{\DemoTTwoRowPVQSevenFiveLogE}{0.2046361157} %
\newcommand{\DemoTTwoRowPVRate}{0} %
\newcommand{\DemoTTwoRowPVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPVMedianLogRatioToExactBound}{-4.504727746e-05} %
\newcommand{\DemoTTwoRowPWMedianLogE}{0.03305222348} %
\newcommand{\DemoTTwoRowPWQTwoFiveLogE}{-0.003854449538} %
\newcommand{\DemoTTwoRowPWQSevenFiveLogE}{0.0800114812} %
\newcommand{\DemoTTwoRowPWRate}{0} %
\newcommand{\DemoTTwoRowPWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPWMedianLogRatioToExactBound}{0.0001048735316} %
\newcommand{\DemoTTwoRowPXMedianLogE}{-26.56752393} %
\newcommand{\DemoTTwoRowPXQTwoFiveLogE}{-28.36816039} %
\newcommand{\DemoTTwoRowPXQSevenFiveLogE}{-25.37515228} %
\newcommand{\DemoTTwoRowPXRate}{0} %
\newcommand{\DemoTTwoRowPXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPXMedianLogRatioToExactBound}{-0.08429781016} %
\newcommand{\DemoTTwoRowPYMedianLogE}{-2468.129354} %
\newcommand{\DemoTTwoRowPYQTwoFiveLogE}{-2661.379389} %
\newcommand{\DemoTTwoRowPYQSevenFiveLogE}{-2236.31435} %
\newcommand{\DemoTTwoRowPYRate}{0} %
\newcommand{\DemoTTwoRowPYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPYMedianLogRatioToExactBound}{-7.83128681} %
\newcommand{\DemoTTwoRowPZMedianLogE}{-2468.129354} %
\newcommand{\DemoTTwoRowPZQTwoFiveLogE}{-2661.379389} %
\newcommand{\DemoTTwoRowPZQSevenFiveLogE}{-2236.31435} %
\newcommand{\DemoTTwoRowPZRate}{0} %
\newcommand{\DemoTTwoRowPZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowPZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowPZMedianLogRatioToExactBound}{-7.83128681} %
\newcommand{\DemoTTwoRowQAMedianLogE}{0.01700640682} %
\newcommand{\DemoTTwoRowQAQTwoFiveLogE}{-0.9515709058} %
\newcommand{\DemoTTwoRowQAQSevenFiveLogE}{1.431157695} %
\newcommand{\DemoTTwoRowQARate}{0.0625} %
\newcommand{\DemoTTwoRowQACpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowQACpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowQAMedianLogRatioToExactBound}{5.396072502e-05} %
\newcommand{\DemoTTwoRowQBMedianLogE}{-6.523780211} %
\newcommand{\DemoTTwoRowQBQTwoFiveLogE}{-7.958416082} %
\newcommand{\DemoTTwoRowQBQSevenFiveLogE}{-4.574089037} %
\newcommand{\DemoTTwoRowQBRate}{0.0625} %
\newcommand{\DemoTTwoRowQBCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowQBCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowQBMedianLogRatioToExactBound}{-0.02069972298} %
\newcommand{\DemoTTwoRowQCMedianLogE}{0.04049844435} %
\newcommand{\DemoTTwoRowQCQTwoFiveLogE}{0.02193734977} %
\newcommand{\DemoTTwoRowQCQSevenFiveLogE}{0.08223986225} %
\newcommand{\DemoTTwoRowQCRate}{0} %
\newcommand{\DemoTTwoRowQCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQCMedianLogRatioToExactBound}{0.000128500126} %
\newcommand{\DemoTTwoRowQDMedianLogE}{-28.4032402} %
\newcommand{\DemoTTwoRowQDQTwoFiveLogE}{-29.14062099} %
\newcommand{\DemoTTwoRowQDQSevenFiveLogE}{-25.51368907} %
\newcommand{\DemoTTwoRowQDRate}{0} %
\newcommand{\DemoTTwoRowQDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQDMedianLogRatioToExactBound}{-0.09012247271} %
\newcommand{\DemoTTwoRowQEMedianLogE}{-2805.788599} %
\newcommand{\DemoTTwoRowQEQTwoFiveLogE}{-3034.345412} %
\newcommand{\DemoTTwoRowQEQSevenFiveLogE}{-2730.122909} %
\newcommand{\DemoTTwoRowQERate}{0} %
\newcommand{\DemoTTwoRowQECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQEMedianLogRatioToExactBound}{-8.902667606} %
\newcommand{\DemoTTwoRowQFMedianLogE}{-1244.737434} %
\newcommand{\DemoTTwoRowQFQTwoFiveLogE}{-1353.924343} %
\newcommand{\DemoTTwoRowQFQSevenFiveLogE}{-1208.337859} %
\newcommand{\DemoTTwoRowQFRate}{0} %
\newcommand{\DemoTTwoRowQFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQFMedianLogRatioToExactBound}{-3.949507683} %
\newcommand{\DemoTTwoRowQGMedianLogE}{0.3490344619} %
\newcommand{\DemoTTwoRowQGQTwoFiveLogE}{-0.1389531256} %
\newcommand{\DemoTTwoRowQGQSevenFiveLogE}{1.523721623} %
\newcommand{\DemoTTwoRowQGRate}{0.0625} %
\newcommand{\DemoTTwoRowQGCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowQGCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowQGMedianLogRatioToExactBound}{0.001107473955} %
\newcommand{\DemoTTwoRowQHMedianLogE}{-93.79946699} %
\newcommand{\DemoTTwoRowQHQTwoFiveLogE}{-105.0256383} %
\newcommand{\DemoTTwoRowQHQSevenFiveLogE}{-82.93037256} %
\newcommand{\DemoTTwoRowQHRate}{0} %
\newcommand{\DemoTTwoRowQHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQHMedianLogRatioToExactBound}{-0.2976223784} %
\newcommand{\DemoTTwoRowQIMedianLogE}{0.05155022224} %
\newcommand{\DemoTTwoRowQIQTwoFiveLogE}{0.03834695319} %
\newcommand{\DemoTTwoRowQIQSevenFiveLogE}{0.07633088571} %
\newcommand{\DemoTTwoRowQIRate}{0} %
\newcommand{\DemoTTwoRowQICpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQICpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQIMedianLogRatioToExactBound}{0.0001635670249} %
\newcommand{\DemoTTwoRowQJMedianLogE}{-26.39009769} %
\newcommand{\DemoTTwoRowQJQTwoFiveLogE}{-30.10067374} %
\newcommand{\DemoTTwoRowQJQSevenFiveLogE}{-25.63631206} %
\newcommand{\DemoTTwoRowQJRate}{0} %
\newcommand{\DemoTTwoRowQJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQJMedianLogRatioToExactBound}{-0.08373484299} %
\newcommand{\DemoTTwoRowQKMedianLogE}{132.4062601} %
\newcommand{\DemoTTwoRowQKQTwoFiveLogE}{129.0144189} %
\newcommand{\DemoTTwoRowQKQSevenFiveLogE}{136.5064377} %
\newcommand{\DemoTTwoRowQKRate}{1} %
\newcommand{\DemoTTwoRowQKCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowQKCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowQKMedianLogRatioToExactBound}{0.4201203622} %
\newcommand{\DemoTTwoRowQLMedianLogE}{52.61269802} %
\newcommand{\DemoTTwoRowQLQTwoFiveLogE}{51.34048486} %
\newcommand{\DemoTTwoRowQLQSevenFiveLogE}{53.60410718} %
\newcommand{\DemoTTwoRowQLRate}{1} %
\newcommand{\DemoTTwoRowQLCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowQLCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowQLMedianLogRatioToExactBound}{0.1669382228} %
\newcommand{\DemoTTwoRowQMMedianLogE}{126.1829019} %
\newcommand{\DemoTTwoRowQMQTwoFiveLogE}{124.1618703} %
\newcommand{\DemoTTwoRowQMQSevenFiveLogE}{131.2977921} %
\newcommand{\DemoTTwoRowQMRate}{1} %
\newcommand{\DemoTTwoRowQMCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowQMCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowQMMedianLogRatioToExactBound}{0.4003738677} %
\newcommand{\DemoTTwoRowQNMedianLogE}{133.5630088} %
\newcommand{\DemoTTwoRowQNQTwoFiveLogE}{130.5185636} %
\newcommand{\DemoTTwoRowQNQSevenFiveLogE}{136.7489138} %
\newcommand{\DemoTTwoRowQNRate}{1} %
\newcommand{\DemoTTwoRowQNCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowQNCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowQNMedianLogRatioToExactBound}{0.4237906847} %
\newcommand{\DemoTTwoRowQOMedianLogE}{-2468.822501} %
\newcommand{\DemoTTwoRowQOQTwoFiveLogE}{-2662.072536} %
\newcommand{\DemoTTwoRowQOQSevenFiveLogE}{-2237.007497} %
\newcommand{\DemoTTwoRowQORate}{0} %
\newcommand{\DemoTTwoRowQOCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQOCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQOMedianLogRatioToExactBound}{-7.833486141} %
\newcommand{\DemoTTwoRowQPMedianLogE}{-1245.430581} %
\newcommand{\DemoTTwoRowQPQTwoFiveLogE}{-1354.61749} %
\newcommand{\DemoTTwoRowQPQSevenFiveLogE}{-1209.031006} %
\newcommand{\DemoTTwoRowQPRate}{0} %
\newcommand{\DemoTTwoRowQPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQPMedianLogRatioToExactBound}{-3.951707014} %
\newcommand{\DemoTTwoRowQQMedianLogE}{0.622180527} %
\newcommand{\DemoTTwoRowQQQTwoFiveLogE}{-0.1828968843} %
\newcommand{\DemoTTwoRowQQQSevenFiveLogE}{1.200429722} %
\newcommand{\DemoTTwoRowQQRate}{0.0625} %
\newcommand{\DemoTTwoRowQQCpNineFiveLower}{0.001581111723} %
\newcommand{\DemoTTwoRowQQCpNineFiveUpper}{0.3023207384} %
\newcommand{\DemoTTwoRowQQMedianLogRatioToExactBound}{0.001974156722} %
\newcommand{\DemoTTwoRowQRMedianLogE}{-7.216927392} %
\newcommand{\DemoTTwoRowQRQTwoFiveLogE}{-8.651563262} %
\newcommand{\DemoTTwoRowQRQSevenFiveLogE}{-5.267236218} %
\newcommand{\DemoTTwoRowQRRate}{0} %
\newcommand{\DemoTTwoRowQRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQRMedianLogRatioToExactBound}{-0.02289905438} %
\newcommand{\DemoTTwoRowQSMedianLogE}{0.05037790649} %
\newcommand{\DemoTTwoRowQSQTwoFiveLogE}{0.03671323031} %
\newcommand{\DemoTTwoRowQSQSevenFiveLogE}{0.06951975299} %
\newcommand{\DemoTTwoRowQSRate}{0} %
\newcommand{\DemoTTwoRowQSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQSMedianLogRatioToExactBound}{0.0001598473086} %
\newcommand{\DemoTTwoRowQTMedianLogE}{-26.28939474} %
\newcommand{\DemoTTwoRowQTQTwoFiveLogE}{-27.27927883} %
\newcommand{\DemoTTwoRowQTQSevenFiveLogE}{-23.76866924} %
\newcommand{\DemoTTwoRowQTRate}{0} %
\newcommand{\DemoTTwoRowQTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQTMedianLogRatioToExactBound}{-0.08341531609} %
\newcommand{\DemoTTwoRowQUMedianLogE}{-6831.059864} %
\newcommand{\DemoTTwoRowQUQTwoFiveLogE}{-7662.093434} %
\newcommand{\DemoTTwoRowQUQSevenFiveLogE}{-5908.088803} %
\newcommand{\DemoTTwoRowQURate}{0} %
\newcommand{\DemoTTwoRowQUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQUMedianLogRatioToExactBound}{-21.67471041} %
\newcommand{\DemoTTwoRowQVMedianLogE}{-6831.059864} %
\newcommand{\DemoTTwoRowQVQTwoFiveLogE}{-7662.093434} %
\newcommand{\DemoTTwoRowQVQSevenFiveLogE}{-5908.088803} %
\newcommand{\DemoTTwoRowQVRate}{0} %
\newcommand{\DemoTTwoRowQVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQVMedianLogRatioToExactBound}{-21.67471041} %
\newcommand{\DemoTTwoRowQWMedianLogE}{6.726987648} %
\newcommand{\DemoTTwoRowQWQTwoFiveLogE}{3.222309152} %
\newcommand{\DemoTTwoRowQWQSevenFiveLogE}{11.56125501} %
\newcommand{\DemoTTwoRowQWRate}{0.8125} %
\newcommand{\DemoTTwoRowQWCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowQWCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowQWMedianLogRatioToExactBound}{0.02134449297} %
\newcommand{\DemoTTwoRowQXMedianLogE}{0.02073131495} %
\newcommand{\DemoTTwoRowQXQTwoFiveLogE}{-0.1426872018} %
\newcommand{\DemoTTwoRowQXQSevenFiveLogE}{0.3481887353} %
\newcommand{\DemoTTwoRowQXRate}{0} %
\newcommand{\DemoTTwoRowQXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQXMedianLogRatioToExactBound}{6.577972628e-05} %
\newcommand{\DemoTTwoRowQYMedianLogE}{0.7001863175} %
\newcommand{\DemoTTwoRowQYQTwoFiveLogE}{0.6299665435} %
\newcommand{\DemoTTwoRowQYQSevenFiveLogE}{0.8904345138} %
\newcommand{\DemoTTwoRowQYRate}{0} %
\newcommand{\DemoTTwoRowQYCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQYCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQYMedianLogRatioToExactBound}{0.002221666325} %
\newcommand{\DemoTTwoRowQZMedianLogE}{-25.15671606} %
\newcommand{\DemoTTwoRowQZQTwoFiveLogE}{-28.62621096} %
\newcommand{\DemoTTwoRowQZQSevenFiveLogE}{-20.71239295} %
\newcommand{\DemoTTwoRowQZRate}{0} %
\newcommand{\DemoTTwoRowQZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowQZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowQZMedianLogRatioToExactBound}{-0.07982136686} %
\newcommand{\DemoTTwoRowRAMedianLogE}{-8061.399382} %
\newcommand{\DemoTTwoRowRAQTwoFiveLogE}{-8879.266249} %
\newcommand{\DemoTTwoRowRAQSevenFiveLogE}{-7550.958565} %
\newcommand{\DemoTTwoRowRARate}{0} %
\newcommand{\DemoTTwoRowRACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRAMedianLogRatioToExactBound}{-25.57853402} %
\newcommand{\DemoTTwoRowRBMedianLogE}{-8061.399382} %
\newcommand{\DemoTTwoRowRBQTwoFiveLogE}{-8879.266249} %
\newcommand{\DemoTTwoRowRBQSevenFiveLogE}{-7550.958565} %
\newcommand{\DemoTTwoRowRBRate}{0} %
\newcommand{\DemoTTwoRowRBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRBMedianLogRatioToExactBound}{-25.57853402} %
\newcommand{\DemoTTwoRowRCMedianLogE}{8.067389225} %
\newcommand{\DemoTTwoRowRCQTwoFiveLogE}{3.911361882} %
\newcommand{\DemoTTwoRowRCQSevenFiveLogE}{10.02124263} %
\newcommand{\DemoTTwoRowRCRate}{0.8125} %
\newcommand{\DemoTTwoRowRCCpNineFiveLower}{0.5435434538} %
\newcommand{\DemoTTwoRowRCCpNineFiveUpper}{0.9595262661} %
\newcommand{\DemoTTwoRowRCMedianLogRatioToExactBound}{0.02559753958} %
\newcommand{\DemoTTwoRowRDMedianLogE}{-14.64725084} %
\newcommand{\DemoTTwoRowRDQTwoFiveLogE}{-19.72668555} %
\newcommand{\DemoTTwoRowRDQSevenFiveLogE}{-8.54322871} %
\newcommand{\DemoTTwoRowRDRate}{0} %
\newcommand{\DemoTTwoRowRDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRDMedianLogRatioToExactBound}{-0.04647520687} %
\newcommand{\DemoTTwoRowREMedianLogE}{0.9412302321} %
\newcommand{\DemoTTwoRowREQTwoFiveLogE}{0.7996138281} %
\newcommand{\DemoTTwoRowREQSevenFiveLogE}{1.011000636} %
\newcommand{\DemoTTwoRowRERate}{0} %
\newcommand{\DemoTTwoRowRECpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRECpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowREMedianLogRatioToExactBound}{0.002986490108} %
\newcommand{\DemoTTwoRowRFMedianLogE}{-25.24946536} %
\newcommand{\DemoTTwoRowRFQTwoFiveLogE}{-27.74091259} %
\newcommand{\DemoTTwoRowRFQSevenFiveLogE}{-21.21434677} %
\newcommand{\DemoTTwoRowRFRate}{0} %
\newcommand{\DemoTTwoRowRFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRFMedianLogRatioToExactBound}{-0.08011565711} %
\newcommand{\DemoTTwoRowRGMedianLogE}{157.1348315} %
\newcommand{\DemoTTwoRowRGQTwoFiveLogE}{152.6163855} %
\newcommand{\DemoTTwoRowRGQSevenFiveLogE}{158.2075704} %
\newcommand{\DemoTTwoRowRGRate}{1} %
\newcommand{\DemoTTwoRowRGCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowRGCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowRGMedianLogRatioToExactBound}{0.4985832412} %
\newcommand{\DemoTTwoRowRHMedianLogE}{157.1344296} %
\newcommand{\DemoTTwoRowRHQTwoFiveLogE}{152.594968} %
\newcommand{\DemoTTwoRowRHQSevenFiveLogE}{158.2070698} %
\newcommand{\DemoTTwoRowRHRate}{1} %
\newcommand{\DemoTTwoRowRHCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowRHCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowRHMedianLogRatioToExactBound}{0.4985819661} %
\newcommand{\DemoTTwoRowRIMedianLogE}{157.1346167} %
\newcommand{\DemoTTwoRowRIQTwoFiveLogE}{152.6046938} %
\newcommand{\DemoTTwoRowRIQSevenFiveLogE}{158.2073505} %
\newcommand{\DemoTTwoRowRIRate}{1} %
\newcommand{\DemoTTwoRowRICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowRICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowRIMedianLogRatioToExactBound}{0.4985825598} %
\newcommand{\DemoTTwoRowRJMedianLogE}{157.1348315} %
\newcommand{\DemoTTwoRowRJQTwoFiveLogE}{152.6163855} %
\newcommand{\DemoTTwoRowRJQSevenFiveLogE}{158.2075704} %
\newcommand{\DemoTTwoRowRJRate}{1} %
\newcommand{\DemoTTwoRowRJCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowRJCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowRJMedianLogRatioToExactBound}{0.4985832412} %
\newcommand{\DemoTTwoRowRKMedianLogE}{-6831.753011} %
\newcommand{\DemoTTwoRowRKQTwoFiveLogE}{-7662.786582} %
\newcommand{\DemoTTwoRowRKQSevenFiveLogE}{-5739.880101} %
\newcommand{\DemoTTwoRowRKRate}{0} %
\newcommand{\DemoTTwoRowRKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRKMedianLogRatioToExactBound}{-21.67690974} %
\newcommand{\DemoTTwoRowRLMedianLogE}{-6831.753011} %
\newcommand{\DemoTTwoRowRLQTwoFiveLogE}{-7662.786582} %
\newcommand{\DemoTTwoRowRLQSevenFiveLogE}{-5739.880101} %
\newcommand{\DemoTTwoRowRLRate}{0} %
\newcommand{\DemoTTwoRowRLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRLMedianLogRatioToExactBound}{-21.67690974} %
\newcommand{\DemoTTwoRowRMMedianLogE}{9.231423093} %
\newcommand{\DemoTTwoRowRMQTwoFiveLogE}{4.370059644} %
\newcommand{\DemoTTwoRowRMQSevenFiveLogE}{11.98174392} %
\newcommand{\DemoTTwoRowRMRate}{0.875} %
\newcommand{\DemoTTwoRowRMCpNineFiveLower}{0.6165237632} %
\newcommand{\DemoTTwoRowRMCpNineFiveUpper}{0.9844863962} %
\newcommand{\DemoTTwoRowRMMedianLogRatioToExactBound}{0.02929097771} %
\newcommand{\DemoTTwoRowRNMedianLogE}{-0.6712434638} %
\newcommand{\DemoTTwoRowRNQTwoFiveLogE}{-0.8358343788} %
\newcommand{\DemoTTwoRowRNQSevenFiveLogE}{-0.3447769464} %
\newcommand{\DemoTTwoRowRNRate}{0} %
\newcommand{\DemoTTwoRowRNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRNMedianLogRatioToExactBound}{-0.002129831678} %
\newcommand{\DemoTTwoRowROMedianLogE}{0.8369029388} %
\newcommand{\DemoTTwoRowROQTwoFiveLogE}{0.736740261} %
\newcommand{\DemoTTwoRowROQSevenFiveLogE}{0.9480762847} %
\newcommand{\DemoTTwoRowRORate}{0} %
\newcommand{\DemoTTwoRowROCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowROCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowROMedianLogRatioToExactBound}{0.002655463311} %
\newcommand{\DemoTTwoRowRPMedianLogE}{-23.42937934} %
\newcommand{\DemoTTwoRowRPQTwoFiveLogE}{-26.94439895} %
\newcommand{\DemoTTwoRowRPQSevenFiveLogE}{-18.7655389} %
\newcommand{\DemoTTwoRowRPRate}{0} %
\newcommand{\DemoTTwoRowRPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRPMedianLogRatioToExactBound}{-0.07434058879} %
\newcommand{\DemoTTwoRowRQMedianLogE}{-5995.33473} %
\newcommand{\DemoTTwoRowRQQTwoFiveLogE}{-6428.127092} %
\newcommand{\DemoTTwoRowRQQSevenFiveLogE}{-5717.821014} %
\newcommand{\DemoTTwoRowRQRate}{0} %
\newcommand{\DemoTTwoRowRQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRQMedianLogRatioToExactBound}{-19.02298423} %
\newcommand{\DemoTTwoRowRRMedianLogE}{3.037639496} %
\newcommand{\DemoTTwoRowRRQTwoFiveLogE}{2.54216267} %
\newcommand{\DemoTTwoRowRRQSevenFiveLogE}{3.247536494} %
\newcommand{\DemoTTwoRowRRRate}{0.5} %
\newcommand{\DemoTTwoRowRRCpNineFiveLower}{0.2465101115} %
\newcommand{\DemoTTwoRowRRCpNineFiveUpper}{0.7534898885} %
\newcommand{\DemoTTwoRowRRMedianLogRatioToExactBound}{0.009638322268} %
\newcommand{\DemoTTwoRowRSMedianLogE}{7.327963536} %
\newcommand{\DemoTTwoRowRSQTwoFiveLogE}{5.434753014} %
\newcommand{\DemoTTwoRowRSQSevenFiveLogE}{8.073471924} %
\newcommand{\DemoTTwoRowRSRate}{0.9375} %
\newcommand{\DemoTTwoRowRSCpNineFiveLower}{0.6976792616} %
\newcommand{\DemoTTwoRowRSCpNineFiveUpper}{0.9984188883} %
\newcommand{\DemoTTwoRowRSMedianLogRatioToExactBound}{0.02325136812} %
\newcommand{\DemoTTwoRowRTMedianLogE}{0.0231807874} %
\newcommand{\DemoTTwoRowRTQTwoFiveLogE}{-0.05714703623} %
\newcommand{\DemoTTwoRowRTQSevenFiveLogE}{0.04638375108} %
\newcommand{\DemoTTwoRowRTRate}{0} %
\newcommand{\DemoTTwoRowRTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRTMedianLogRatioToExactBound}{7.355181538e-05} %
\newcommand{\DemoTTwoRowRUMedianLogE}{0.5849295303} %
\newcommand{\DemoTTwoRowRUQTwoFiveLogE}{0.4770572273} %
\newcommand{\DemoTTwoRowRUQSevenFiveLogE}{0.6382276737} %
\newcommand{\DemoTTwoRowRURate}{0} %
\newcommand{\DemoTTwoRowRUCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRUCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRUMedianLogRatioToExactBound}{0.001855960632} %
\newcommand{\DemoTTwoRowRVMedianLogE}{-25.01374162} %
\newcommand{\DemoTTwoRowRVQTwoFiveLogE}{-27.56888618} %
\newcommand{\DemoTTwoRowRVQSevenFiveLogE}{-20.79065889} %
\newcommand{\DemoTTwoRowRVRate}{0} %
\newcommand{\DemoTTwoRowRVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRVMedianLogRatioToExactBound}{-0.07936771406} %
\newcommand{\DemoTTwoRowRWMedianLogE}{-8833.407383} %
\newcommand{\DemoTTwoRowRWQTwoFiveLogE}{-9242.638819} %
\newcommand{\DemoTTwoRowRWQSevenFiveLogE}{-8712.058958} %
\newcommand{\DemoTTwoRowRWRate}{0} %
\newcommand{\DemoTTwoRowRWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRWMedianLogRatioToExactBound}{-28.028088} %
\newcommand{\DemoTTwoRowRXMedianLogE}{2.583185022} %
\newcommand{\DemoTTwoRowRXQTwoFiveLogE}{2.322135451} %
\newcommand{\DemoTTwoRowRXQSevenFiveLogE}{3.114932485} %
\newcommand{\DemoTTwoRowRXRate}{0.3125} %
\newcommand{\DemoTTwoRowRXCpNineFiveLower}{0.1101699547} %
\newcommand{\DemoTTwoRowRXCpNineFiveUpper}{0.5866206365} %
\newcommand{\DemoTTwoRowRXMedianLogRatioToExactBound}{0.008196354358} %
\newcommand{\DemoTTwoRowRYMedianLogE}{4.604537274} %
\newcommand{\DemoTTwoRowRYQTwoFiveLogE}{3.485587108} %
\newcommand{\DemoTTwoRowRYQSevenFiveLogE}{5.970021924} %
\newcommand{\DemoTTwoRowRYRate}{0.75} %
\newcommand{\DemoTTwoRowRYCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowRYCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowRYMedianLogRatioToExactBound}{0.01461003329} %
\newcommand{\DemoTTwoRowRZMedianLogE}{-0.08731990722} %
\newcommand{\DemoTTwoRowRZQTwoFiveLogE}{-0.2556327052} %
\newcommand{\DemoTTwoRowRZQSevenFiveLogE}{0.1725565721} %
\newcommand{\DemoTTwoRowRZRate}{0} %
\newcommand{\DemoTTwoRowRZCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowRZCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowRZMedianLogRatioToExactBound}{-0.0002770629653} %
\newcommand{\DemoTTwoRowSAMedianLogE}{0.5413814052} %
\newcommand{\DemoTTwoRowSAQTwoFiveLogE}{0.4557906939} %
\newcommand{\DemoTTwoRowSAQSevenFiveLogE}{0.6072486939} %
\newcommand{\DemoTTwoRowSARate}{0} %
\newcommand{\DemoTTwoRowSACpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSACpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSAMedianLogRatioToExactBound}{0.001717783977} %
\newcommand{\DemoTTwoRowSBMedianLogE}{-25.81743503} %
\newcommand{\DemoTTwoRowSBQTwoFiveLogE}{-28.86404811} %
\newcommand{\DemoTTwoRowSBQSevenFiveLogE}{-23.86146208} %
\newcommand{\DemoTTwoRowSBRate}{0} %
\newcommand{\DemoTTwoRowSBCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSBCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSBMedianLogRatioToExactBound}{-0.08191780469} %
\newcommand{\DemoTTwoRowSCMedianLogE}{155.1492257} %
\newcommand{\DemoTTwoRowSCQTwoFiveLogE}{153.7393453} %
\newcommand{\DemoTTwoRowSCQSevenFiveLogE}{157.8935696} %
\newcommand{\DemoTTwoRowSCRate}{1} %
\newcommand{\DemoTTwoRowSCCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSCCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSCMedianLogRatioToExactBound}{0.4922829845} %
\newcommand{\DemoTTwoRowSDMedianLogE}{18.99609639} %
\newcommand{\DemoTTwoRowSDQTwoFiveLogE}{18.54034701} %
\newcommand{\DemoTTwoRowSDQSevenFiveLogE}{19.50533527} %
\newcommand{\DemoTTwoRowSDRate}{1} %
\newcommand{\DemoTTwoRowSDCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSDCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSDMedianLogRatioToExactBound}{0.06027393937} %
\newcommand{\DemoTTwoRowSEMedianLogE}{155.1492257} %
\newcommand{\DemoTTwoRowSEQTwoFiveLogE}{153.7393453} %
\newcommand{\DemoTTwoRowSEQSevenFiveLogE}{157.8935696} %
\newcommand{\DemoTTwoRowSERate}{1} %
\newcommand{\DemoTTwoRowSECpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSECpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSEMedianLogRatioToExactBound}{0.4922829845} %
\newcommand{\DemoTTwoRowSFMedianLogE}{155.3740595} %
\newcommand{\DemoTTwoRowSFQTwoFiveLogE}{154.4164696} %
\newcommand{\DemoTTwoRowSFQSevenFiveLogE}{157.9083344} %
\newcommand{\DemoTTwoRowSFRate}{1} %
\newcommand{\DemoTTwoRowSFCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSFCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSFMedianLogRatioToExactBound}{0.4929963741} %
\newcommand{\DemoTTwoRowSGMedianLogE}{-5996.027877} %
\newcommand{\DemoTTwoRowSGQTwoFiveLogE}{-6428.820239} %
\newcommand{\DemoTTwoRowSGQSevenFiveLogE}{-5718.514162} %
\newcommand{\DemoTTwoRowSGRate}{0} %
\newcommand{\DemoTTwoRowSGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSGMedianLogRatioToExactBound}{-19.02518357} %
\newcommand{\DemoTTwoRowSHMedianLogE}{2.885218232} %
\newcommand{\DemoTTwoRowSHQTwoFiveLogE}{2.420158032} %
\newcommand{\DemoTTwoRowSHQSevenFiveLogE}{3.319215674} %
\newcommand{\DemoTTwoRowSHRate}{0.4375} %
\newcommand{\DemoTTwoRowSHCpNineFiveLower}{0.1975341405} %
\newcommand{\DemoTTwoRowSHCpNineFiveUpper}{0.7012231009} %
\newcommand{\DemoTTwoRowSHMedianLogRatioToExactBound}{0.009154695009} %
\newcommand{\DemoTTwoRowSIMedianLogE}{7.056378966} %
\newcommand{\DemoTTwoRowSIQTwoFiveLogE}{5.535391711} %
\newcommand{\DemoTTwoRowSIQSevenFiveLogE}{7.646840873} %
\newcommand{\DemoTTwoRowSIRate}{1} %
\newcommand{\DemoTTwoRowSICpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSICpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSIMedianLogRatioToExactBound}{0.02238963992} %
\newcommand{\DemoTTwoRowSJMedianLogE}{-0.0207706784} %
\newcommand{\DemoTTwoRowSJQTwoFiveLogE}{-0.159721755} %
\newcommand{\DemoTTwoRowSJQSevenFiveLogE}{0.08510022631} %
\newcommand{\DemoTTwoRowSJRate}{0} %
\newcommand{\DemoTTwoRowSJCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSJCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSJMedianLogRatioToExactBound}{-6.59046251e-05} %
\newcommand{\DemoTTwoRowSKMedianLogE}{0.569065413} %
\newcommand{\DemoTTwoRowSKQTwoFiveLogE}{0.4600963825} %
\newcommand{\DemoTTwoRowSKQSevenFiveLogE}{0.6516876942} %
\newcommand{\DemoTTwoRowSKRate}{0} %
\newcommand{\DemoTTwoRowSKCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSKCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSKMedianLogRatioToExactBound}{0.001805624351} %
\newcommand{\DemoTTwoRowSLMedianLogE}{-23.55693196} %
\newcommand{\DemoTTwoRowSLQTwoFiveLogE}{-26.35881602} %
\newcommand{\DemoTTwoRowSLQSevenFiveLogE}{-20.88336787} %
\newcommand{\DemoTTwoRowSLRate}{0} %
\newcommand{\DemoTTwoRowSLCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSLCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSLMedianLogRatioToExactBound}{-0.07474530872} %
\newcommand{\DemoTTwoRowSMMedianLogE}{-6755.164436} %
\newcommand{\DemoTTwoRowSMQTwoFiveLogE}{-7287.365119} %
\newcommand{\DemoTTwoRowSMQSevenFiveLogE}{-6241.388764} %
\newcommand{\DemoTTwoRowSMRate}{0} %
\newcommand{\DemoTTwoRowSMCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSMCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSMMedianLogRatioToExactBound}{-21.43389691} %
\newcommand{\DemoTTwoRowSNMedianLogE}{-6755.164436} %
\newcommand{\DemoTTwoRowSNQTwoFiveLogE}{-7287.365119} %
\newcommand{\DemoTTwoRowSNQSevenFiveLogE}{-6241.388764} %
\newcommand{\DemoTTwoRowSNRate}{0} %
\newcommand{\DemoTTwoRowSNCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSNCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSNMedianLogRatioToExactBound}{-21.43389691} %
\newcommand{\DemoTTwoRowSOMedianLogE}{8.674810083} %
\newcommand{\DemoTTwoRowSOQTwoFiveLogE}{5.438392269} %
\newcommand{\DemoTTwoRowSOQSevenFiveLogE}{10.64172411} %
\newcommand{\DemoTTwoRowSORate}{1} %
\newcommand{\DemoTTwoRowSOCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSOCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSOMedianLogRatioToExactBound}{0.02752486439} %
\newcommand{\DemoTTwoRowSPMedianLogE}{-6.218870796} %
\newcommand{\DemoTTwoRowSPQTwoFiveLogE}{-7.765327091} %
\newcommand{\DemoTTwoRowSPQSevenFiveLogE}{-3.443065145} %
\newcommand{\DemoTTwoRowSPRate}{0} %
\newcommand{\DemoTTwoRowSPCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSPCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSPMedianLogRatioToExactBound}{-0.01973225623} %
\newcommand{\DemoTTwoRowSQMedianLogE}{0.7706829967} %
\newcommand{\DemoTTwoRowSQQTwoFiveLogE}{0.7023129981} %
\newcommand{\DemoTTwoRowSQQSevenFiveLogE}{0.8483881075} %
\newcommand{\DemoTTwoRowSQRate}{0} %
\newcommand{\DemoTTwoRowSQCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSQCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSQMedianLogRatioToExactBound}{0.002445349785} %
\newcommand{\DemoTTwoRowSRMedianLogE}{-21.24990283} %
\newcommand{\DemoTTwoRowSRQTwoFiveLogE}{-24.66045653} %
\newcommand{\DemoTTwoRowSRQSevenFiveLogE}{-18.98149133} %
\newcommand{\DemoTTwoRowSRRate}{0} %
\newcommand{\DemoTTwoRowSRCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSRCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSRMedianLogRatioToExactBound}{-0.06742518719} %
\newcommand{\DemoTTwoRowSSMedianLogE}{-7295.374983} %
\newcommand{\DemoTTwoRowSSQTwoFiveLogE}{-8250.704717} %
\newcommand{\DemoTTwoRowSSQSevenFiveLogE}{-6683.788705} %
\newcommand{\DemoTTwoRowSSRate}{0} %
\newcommand{\DemoTTwoRowSSCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSSCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSSMedianLogRatioToExactBound}{-23.1479658} %
\newcommand{\DemoTTwoRowSTMedianLogE}{-7295.374983} %
\newcommand{\DemoTTwoRowSTQTwoFiveLogE}{-8250.704717} %
\newcommand{\DemoTTwoRowSTQSevenFiveLogE}{-6683.788705} %
\newcommand{\DemoTTwoRowSTRate}{0} %
\newcommand{\DemoTTwoRowSTCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSTCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSTMedianLogRatioToExactBound}{-23.1479658} %
\newcommand{\DemoTTwoRowSUMedianLogE}{6.969843847} %
\newcommand{\DemoTTwoRowSUQTwoFiveLogE}{4.668598057} %
\newcommand{\DemoTTwoRowSUQSevenFiveLogE}{8.519341007} %
\newcommand{\DemoTTwoRowSURate}{0.75} %
\newcommand{\DemoTTwoRowSUCpNineFiveLower}{0.4762291801} %
\newcommand{\DemoTTwoRowSUCpNineFiveUpper}{0.9273379617} %
\newcommand{\DemoTTwoRowSUMedianLogRatioToExactBound}{0.02211506706} %
\newcommand{\DemoTTwoRowSVMedianLogE}{-158.8404} %
\newcommand{\DemoTTwoRowSVQTwoFiveLogE}{-171.3906918} %
\newcommand{\DemoTTwoRowSVQSevenFiveLogE}{-150.0252457} %
\newcommand{\DemoTTwoRowSVRate}{0} %
\newcommand{\DemoTTwoRowSVCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSVCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSVMedianLogRatioToExactBound}{-0.5039949496} %
\newcommand{\DemoTTwoRowSWMedianLogE}{0.7142058877} %
\newcommand{\DemoTTwoRowSWQTwoFiveLogE}{0.7039063363} %
\newcommand{\DemoTTwoRowSWQSevenFiveLogE}{0.7648248504} %
\newcommand{\DemoTTwoRowSWRate}{0} %
\newcommand{\DemoTTwoRowSWCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSWCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSWMedianLogRatioToExactBound}{0.002266149924} %
\newcommand{\DemoTTwoRowSXMedianLogE}{-25.35498371} %
\newcommand{\DemoTTwoRowSXQTwoFiveLogE}{-27.64129728} %
\newcommand{\DemoTTwoRowSXQSevenFiveLogE}{-21.45288792} %
\newcommand{\DemoTTwoRowSXRate}{0} %
\newcommand{\DemoTTwoRowSXCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowSXCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowSXMedianLogRatioToExactBound}{-0.08045046307} %
\newcommand{\DemoTTwoRowSYMedianLogE}{156.6888061} %
\newcommand{\DemoTTwoRowSYQTwoFiveLogE}{154.1487564} %
\newcommand{\DemoTTwoRowSYQSevenFiveLogE}{159.7834972} %
\newcommand{\DemoTTwoRowSYRate}{1} %
\newcommand{\DemoTTwoRowSYCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSYCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSYMedianLogRatioToExactBound}{0.4971680185} %
\newcommand{\DemoTTwoRowSZMedianLogE}{153.1439382} %
\newcommand{\DemoTTwoRowSZQTwoFiveLogE}{150.9492367} %
\newcommand{\DemoTTwoRowSZQSevenFiveLogE}{155.6200517} %
\newcommand{\DemoTTwoRowSZRate}{1} %
\newcommand{\DemoTTwoRowSZCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowSZCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowSZMedianLogRatioToExactBound}{0.4859202787} %
\newcommand{\DemoTTwoRowTAMedianLogE}{156.9466635} %
\newcommand{\DemoTTwoRowTAQTwoFiveLogE}{153.8059181} %
\newcommand{\DemoTTwoRowTAQSevenFiveLogE}{159.1654231} %
\newcommand{\DemoTTwoRowTARate}{1} %
\newcommand{\DemoTTwoRowTACpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowTACpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowTAMedianLogRatioToExactBound}{0.4979861909} %
\newcommand{\DemoTTwoRowTBMedianLogE}{157.5970899} %
\newcommand{\DemoTTwoRowTBQTwoFiveLogE}{154.1487563} %
\newcommand{\DemoTTwoRowTBQSevenFiveLogE}{160.1950976} %
\newcommand{\DemoTTwoRowTBRate}{1} %
\newcommand{\DemoTTwoRowTBCpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowTBCpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowTBMedianLogRatioToExactBound}{0.5000499707} %
\newcommand{\DemoTTwoRowTCMedianLogE}{-6567.325552} %
\newcommand{\DemoTTwoRowTCQTwoFiveLogE}{-7288.058266} %
\newcommand{\DemoTTwoRowTCQSevenFiveLogE}{-6242.081911} %
\newcommand{\DemoTTwoRowTCRate}{0} %
\newcommand{\DemoTTwoRowTCCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTCCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTCMedianLogRatioToExactBound}{-20.8378908} %
\newcommand{\DemoTTwoRowTDMedianLogE}{-6567.325552} %
\newcommand{\DemoTTwoRowTDQTwoFiveLogE}{-7288.058266} %
\newcommand{\DemoTTwoRowTDQSevenFiveLogE}{-6242.081911} %
\newcommand{\DemoTTwoRowTDRate}{0} %
\newcommand{\DemoTTwoRowTDCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTDCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTDMedianLogRatioToExactBound}{-20.8378908} %
\newcommand{\DemoTTwoRowTEMedianLogE}{9.062769084} %
\newcommand{\DemoTTwoRowTEQTwoFiveLogE}{6.552721237} %
\newcommand{\DemoTTwoRowTEQSevenFiveLogE}{10.40384127} %
\newcommand{\DemoTTwoRowTERate}{1} %
\newcommand{\DemoTTwoRowTECpNineFiveLower}{0.7940927858} %
\newcommand{\DemoTTwoRowTECpNineFiveUpper}{1} %
\newcommand{\DemoTTwoRowTEMedianLogRatioToExactBound}{0.02875584453} %
\newcommand{\DemoTTwoRowTFMedianLogE}{-6.912017976} %
\newcommand{\DemoTTwoRowTFQTwoFiveLogE}{-8.458474271} %
\newcommand{\DemoTTwoRowTFQSevenFiveLogE}{-4.136212325} %
\newcommand{\DemoTTwoRowTFRate}{0} %
\newcommand{\DemoTTwoRowTFCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTFCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTFMedianLogRatioToExactBound}{-0.02193158763} %
\newcommand{\DemoTTwoRowTGMedianLogE}{0.7509242623} %
\newcommand{\DemoTTwoRowTGQTwoFiveLogE}{0.7106006627} %
\newcommand{\DemoTTwoRowTGQSevenFiveLogE}{0.8055256951} %
\newcommand{\DemoTTwoRowTGRate}{0} %
\newcommand{\DemoTTwoRowTGCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTGCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTGMedianLogRatioToExactBound}{0.002382656023} %
\newcommand{\DemoTTwoRowTHMedianLogE}{-20.69425354} %
\newcommand{\DemoTTwoRowTHQTwoFiveLogE}{-22.22264223} %
\newcommand{\DemoTTwoRowTHQSevenFiveLogE}{-18.0878044} %
\newcommand{\DemoTTwoRowTHRate}{0} %
\newcommand{\DemoTTwoRowTHCpNineFiveLower}{0} %
\newcommand{\DemoTTwoRowTHCpNineFiveUpper}{0.2059072142} %
\newcommand{\DemoTTwoRowTHMedianLogRatioToExactBound}{-0.06566213175} %
\newcommand{\DemoTThreeRowAEffectReports}{41} %
\newcommand{\DemoTThreeRowAK}{64} %
\newcommand{\DemoTThreeRowARate}{0.640625} %
\newcommand{\DemoTThreeRowACpNineFiveLower}{0.5109625982} %
\newcommand{\DemoTThreeRowACpNineFiveUpper}{0.756809709} %
\newcommand{\DemoTThreeRowBEffectReports}{42} %
\newcommand{\DemoTThreeRowBK}{64} %
\newcommand{\DemoTThreeRowBRate}{0.65625} %
\newcommand{\DemoTThreeRowBCpNineFiveLower}{0.5269769612} %
\newcommand{\DemoTThreeRowBCpNineFiveUpper}{0.7705367575} %
\newcommand{\DemoTThreeRowCEffectReports}{64} %
\newcommand{\DemoTThreeRowCK}{64} %
\newcommand{\DemoTThreeRowCRate}{1} %
\newcommand{\DemoTThreeRowCCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowCCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowDEffectReports}{59} %
\newcommand{\DemoTThreeRowDK}{64} %
\newcommand{\DemoTThreeRowDRate}{0.921875} %
\newcommand{\DemoTThreeRowDCpNineFiveLower}{0.827021671} %
\newcommand{\DemoTThreeRowDCpNineFiveUpper}{0.9741461598} %
\newcommand{\DemoTThreeRowEEffectReports}{63} %
\newcommand{\DemoTThreeRowEK}{64} %
\newcommand{\DemoTThreeRowERate}{0.984375} %
\newcommand{\DemoTThreeRowECpNineFiveLower}{0.9159896736} %
\newcommand{\DemoTThreeRowECpNineFiveUpper}{0.9996044875} %
\newcommand{\DemoTThreeRowFEffectReports}{64} %
\newcommand{\DemoTThreeRowFK}{64} %
\newcommand{\DemoTThreeRowFRate}{1} %
\newcommand{\DemoTThreeRowFCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowFCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowGEffectReports}{58} %
\newcommand{\DemoTThreeRowGK}{64} %
\newcommand{\DemoTThreeRowGRate}{0.90625} %
\newcommand{\DemoTThreeRowGCpNineFiveLower}{0.8070308956} %
\newcommand{\DemoTThreeRowGCpNineFiveUpper}{0.9648126671} %
\newcommand{\DemoTThreeRowHEffectReports}{60} %
\newcommand{\DemoTThreeRowHK}{64} %
\newcommand{\DemoTThreeRowHRate}{0.9375} %
\newcommand{\DemoTThreeRowHCpNineFiveLower}{0.8476365266} %
\newcommand{\DemoTThreeRowHCpNineFiveUpper}{0.9827099726} %
\newcommand{\DemoTThreeRowIEffectReports}{63} %
\newcommand{\DemoTThreeRowIK}{64} %
\newcommand{\DemoTThreeRowIRate}{0.984375} %
\newcommand{\DemoTThreeRowICpNineFiveLower}{0.9159896736} %
\newcommand{\DemoTThreeRowICpNineFiveUpper}{0.9996044875} %
\newcommand{\DemoTThreeRowJEffectReports}{59} %
\newcommand{\DemoTThreeRowJK}{64} %
\newcommand{\DemoTThreeRowJRate}{0.921875} %
\newcommand{\DemoTThreeRowJCpNineFiveLower}{0.827021671} %
\newcommand{\DemoTThreeRowJCpNineFiveUpper}{0.9741461598} %
\newcommand{\DemoTThreeRowKEffectReports}{63} %
\newcommand{\DemoTThreeRowKK}{64} %
\newcommand{\DemoTThreeRowKRate}{0.984375} %
\newcommand{\DemoTThreeRowKCpNineFiveLower}{0.9159896736} %
\newcommand{\DemoTThreeRowKCpNineFiveUpper}{0.9996044875} %
\newcommand{\DemoTThreeRowLEffectReports}{64} %
\newcommand{\DemoTThreeRowLK}{64} %
\newcommand{\DemoTThreeRowLRate}{1} %
\newcommand{\DemoTThreeRowLCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowLCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowMEffectReports}{56} %
\newcommand{\DemoTThreeRowMK}{64} %
\newcommand{\DemoTThreeRowMRate}{0.875} %
\newcommand{\DemoTThreeRowMCpNineFiveLower}{0.768473694} %
\newcommand{\DemoTThreeRowMCpNineFiveUpper}{0.9444572088} %
\newcommand{\DemoTThreeRowNEffectReports}{56} %
\newcommand{\DemoTThreeRowNK}{64} %
\newcommand{\DemoTThreeRowNRate}{0.875} %
\newcommand{\DemoTThreeRowNCpNineFiveLower}{0.768473694} %
\newcommand{\DemoTThreeRowNCpNineFiveUpper}{0.9444572088} %
\newcommand{\DemoTThreeRowOEffectReports}{64} %
\newcommand{\DemoTThreeRowOK}{64} %
\newcommand{\DemoTThreeRowORate}{1} %
\newcommand{\DemoTThreeRowOCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowOCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowPEffectReports}{63} %
\newcommand{\DemoTThreeRowPK}{64} %
\newcommand{\DemoTThreeRowPRate}{0.984375} %
\newcommand{\DemoTThreeRowPCpNineFiveLower}{0.9159896736} %
\newcommand{\DemoTThreeRowPCpNineFiveUpper}{0.9996044875} %
\newcommand{\DemoTThreeRowQEffectReports}{64} %
\newcommand{\DemoTThreeRowQK}{64} %
\newcommand{\DemoTThreeRowQRate}{1} %
\newcommand{\DemoTThreeRowQCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowQCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowREffectReports}{64} %
\newcommand{\DemoTThreeRowRK}{64} %
\newcommand{\DemoTThreeRowRRate}{1} %
\newcommand{\DemoTThreeRowRCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowRCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowSEffectReports}{51} %
\newcommand{\DemoTThreeRowSK}{64} %
\newcommand{\DemoTThreeRowSRate}{0.796875} %
\newcommand{\DemoTThreeRowSCpNineFiveLower}{0.6777356933} %
\newcommand{\DemoTThreeRowSCpNineFiveUpper}{0.8871711405} %
\newcommand{\DemoTThreeRowTEffectReports}{51} %
\newcommand{\DemoTThreeRowTK}{64} %
\newcommand{\DemoTThreeRowTRate}{0.796875} %
\newcommand{\DemoTThreeRowTCpNineFiveLower}{0.6777356933} %
\newcommand{\DemoTThreeRowTCpNineFiveUpper}{0.8871711405} %
\newcommand{\DemoTThreeRowUEffectReports}{64} %
\newcommand{\DemoTThreeRowUK}{64} %
\newcommand{\DemoTThreeRowURate}{1} %
\newcommand{\DemoTThreeRowUCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowUCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowVEffectReports}{58} %
\newcommand{\DemoTThreeRowVK}{64} %
\newcommand{\DemoTThreeRowVRate}{0.90625} %
\newcommand{\DemoTThreeRowVCpNineFiveLower}{0.8070308956} %
\newcommand{\DemoTThreeRowVCpNineFiveUpper}{0.9648126671} %
\newcommand{\DemoTThreeRowWEffectReports}{64} %
\newcommand{\DemoTThreeRowWK}{64} %
\newcommand{\DemoTThreeRowWRate}{1} %
\newcommand{\DemoTThreeRowWCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowWCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowXEffectReports}{64} %
\newcommand{\DemoTThreeRowXK}{64} %
\newcommand{\DemoTThreeRowXRate}{1} %
\newcommand{\DemoTThreeRowXCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowXCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowYEffectReports}{49} %
\newcommand{\DemoTThreeRowYK}{64} %
\newcommand{\DemoTThreeRowYRate}{0.765625} %
\newcommand{\DemoTThreeRowYCpNineFiveLower}{0.6430658896} %
\newcommand{\DemoTThreeRowYCpNineFiveUpper}{0.8624845216} %
\newcommand{\DemoTThreeRowZEffectReports}{52} %
\newcommand{\DemoTThreeRowZK}{64} %
\newcommand{\DemoTThreeRowZRate}{0.8125} %
\newcommand{\DemoTThreeRowZCpNineFiveLower}{0.6953771263} %
\newcommand{\DemoTThreeRowZCpNineFiveUpper}{0.8991848406} %
\newcommand{\DemoTThreeRowAAEffectReports}{63} %
\newcommand{\DemoTThreeRowAAK}{64} %
\newcommand{\DemoTThreeRowAARate}{0.984375} %
\newcommand{\DemoTThreeRowAACpNineFiveLower}{0.9159896736} %
\newcommand{\DemoTThreeRowAACpNineFiveUpper}{0.9996044875} %
\newcommand{\DemoTThreeRowABEffectReports}{58} %
\newcommand{\DemoTThreeRowABK}{64} %
\newcommand{\DemoTThreeRowABRate}{0.90625} %
\newcommand{\DemoTThreeRowABCpNineFiveLower}{0.8070308956} %
\newcommand{\DemoTThreeRowABCpNineFiveUpper}{0.9648126671} %
\newcommand{\DemoTThreeRowACEffectReports}{64} %
\newcommand{\DemoTThreeRowACK}{64} %
\newcommand{\DemoTThreeRowACRate}{1} %
\newcommand{\DemoTThreeRowACCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowACCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowADEffectReports}{64} %
\newcommand{\DemoTThreeRowADK}{64} %
\newcommand{\DemoTThreeRowADRate}{1} %
\newcommand{\DemoTThreeRowADCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowADCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowAEEffectReports}{58} %
\newcommand{\DemoTThreeRowAEK}{64} %
\newcommand{\DemoTThreeRowAERate}{0.90625} %
\newcommand{\DemoTThreeRowAECpNineFiveLower}{0.8070308956} %
\newcommand{\DemoTThreeRowAECpNineFiveUpper}{0.9648126671} %
\newcommand{\DemoTThreeRowAFEffectReports}{60} %
\newcommand{\DemoTThreeRowAFK}{64} %
\newcommand{\DemoTThreeRowAFRate}{0.9375} %
\newcommand{\DemoTThreeRowAFCpNineFiveLower}{0.8476365266} %
\newcommand{\DemoTThreeRowAFCpNineFiveUpper}{0.9827099726} %
\newcommand{\DemoTThreeRowAGEffectReports}{64} %
\newcommand{\DemoTThreeRowAGK}{64} %
\newcommand{\DemoTThreeRowAGRate}{1} %
\newcommand{\DemoTThreeRowAGCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowAGCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowAHEffectReports}{60} %
\newcommand{\DemoTThreeRowAHK}{64} %
\newcommand{\DemoTThreeRowAHRate}{0.9375} %
\newcommand{\DemoTThreeRowAHCpNineFiveLower}{0.8476365266} %
\newcommand{\DemoTThreeRowAHCpNineFiveUpper}{0.9827099726} %
\newcommand{\DemoTThreeRowAIEffectReports}{64} %
\newcommand{\DemoTThreeRowAIK}{64} %
\newcommand{\DemoTThreeRowAIRate}{1} %
\newcommand{\DemoTThreeRowAICpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowAICpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowAJEffectReports}{64} %
\newcommand{\DemoTThreeRowAJK}{64} %
\newcommand{\DemoTThreeRowAJRate}{1} %
\newcommand{\DemoTThreeRowAJCpNineFiveLower}{0.9439909106} %
\newcommand{\DemoTThreeRowAJCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowAKEffectReports}{1} %
\newcommand{\DemoTThreeRowAKK}{32} %
\newcommand{\DemoTThreeRowAKRate}{0.03125} %
\newcommand{\DemoTThreeRowAKCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowAKCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowALEffectReports}{1} %
\newcommand{\DemoTThreeRowALK}{32} %
\newcommand{\DemoTThreeRowALRate}{0.03125} %
\newcommand{\DemoTThreeRowALCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowALCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowAMEffectReports}{5} %
\newcommand{\DemoTThreeRowAMK}{32} %
\newcommand{\DemoTThreeRowAMRate}{0.15625} %
\newcommand{\DemoTThreeRowAMCpNineFiveLower}{0.0527505644} %
\newcommand{\DemoTThreeRowAMCpNineFiveUpper}{0.3278787657} %
\newcommand{\DemoTThreeRowANEffectReports}{0} %
\newcommand{\DemoTThreeRowANK}{32} %
\newcommand{\DemoTThreeRowANRate}{0} %
\newcommand{\DemoTThreeRowANCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowANCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowAOEffectReports}{7} %
\newcommand{\DemoTThreeRowAOK}{32} %
\newcommand{\DemoTThreeRowAORate}{0.21875} %
\newcommand{\DemoTThreeRowAOCpNineFiveLower}{0.09277153228} %
\newcommand{\DemoTThreeRowAOCpNineFiveUpper}{0.3997282637} %
\newcommand{\DemoTThreeRowAPEffectReports}{3} %
\newcommand{\DemoTThreeRowAPK}{32} %
\newcommand{\DemoTThreeRowAPRate}{0.09375} %
\newcommand{\DemoTThreeRowAPCpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowAPCpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowAQEffectReports}{0} %
\newcommand{\DemoTThreeRowAQK}{32} %
\newcommand{\DemoTThreeRowAQRate}{0} %
\newcommand{\DemoTThreeRowAQCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowAQCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowAREffectReports}{0} %
\newcommand{\DemoTThreeRowARK}{32} %
\newcommand{\DemoTThreeRowARRate}{0} %
\newcommand{\DemoTThreeRowARCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowARCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowASEffectReports}{2} %
\newcommand{\DemoTThreeRowASK}{32} %
\newcommand{\DemoTThreeRowASRate}{0.0625} %
\newcommand{\DemoTThreeRowASCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowASCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowATEffectReports}{0} %
\newcommand{\DemoTThreeRowATK}{32} %
\newcommand{\DemoTThreeRowATRate}{0} %
\newcommand{\DemoTThreeRowATCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowATCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowAUEffectReports}{32} %
\newcommand{\DemoTThreeRowAUK}{32} %
\newcommand{\DemoTThreeRowAURate}{1} %
\newcommand{\DemoTThreeRowAUCpNineFiveLower}{0.8911188393} %
\newcommand{\DemoTThreeRowAUCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowAVEffectReports}{1} %
\newcommand{\DemoTThreeRowAVK}{32} %
\newcommand{\DemoTThreeRowAVRate}{0.03125} %
\newcommand{\DemoTThreeRowAVCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowAVCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowAWEffectReports}{0} %
\newcommand{\DemoTThreeRowAWK}{32} %
\newcommand{\DemoTThreeRowAWRate}{0} %
\newcommand{\DemoTThreeRowAWCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowAWCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowAXEffectReports}{0} %
\newcommand{\DemoTThreeRowAXK}{32} %
\newcommand{\DemoTThreeRowAXRate}{0} %
\newcommand{\DemoTThreeRowAXCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowAXCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowAYEffectReports}{3} %
\newcommand{\DemoTThreeRowAYK}{32} %
\newcommand{\DemoTThreeRowAYRate}{0.09375} %
\newcommand{\DemoTThreeRowAYCpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowAYCpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowAZEffectReports}{0} %
\newcommand{\DemoTThreeRowAZK}{32} %
\newcommand{\DemoTThreeRowAZRate}{0} %
\newcommand{\DemoTThreeRowAZCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowAZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBAEffectReports}{32} %
\newcommand{\DemoTThreeRowBAK}{32} %
\newcommand{\DemoTThreeRowBARate}{1} %
\newcommand{\DemoTThreeRowBACpNineFiveLower}{0.8911188393} %
\newcommand{\DemoTThreeRowBACpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowBBEffectReports}{0} %
\newcommand{\DemoTThreeRowBBK}{32} %
\newcommand{\DemoTThreeRowBBRate}{0} %
\newcommand{\DemoTThreeRowBBCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBCEffectReports}{0} %
\newcommand{\DemoTThreeRowBCK}{32} %
\newcommand{\DemoTThreeRowBCRate}{0} %
\newcommand{\DemoTThreeRowBCCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBCCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBDEffectReports}{0} %
\newcommand{\DemoTThreeRowBDK}{32} %
\newcommand{\DemoTThreeRowBDRate}{0} %
\newcommand{\DemoTThreeRowBDCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBEEffectReports}{1} %
\newcommand{\DemoTThreeRowBEK}{32} %
\newcommand{\DemoTThreeRowBERate}{0.03125} %
\newcommand{\DemoTThreeRowBECpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowBECpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowBFEffectReports}{0} %
\newcommand{\DemoTThreeRowBFK}{32} %
\newcommand{\DemoTThreeRowBFRate}{0} %
\newcommand{\DemoTThreeRowBFCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBFCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBGEffectReports}{11} %
\newcommand{\DemoTThreeRowBGK}{32} %
\newcommand{\DemoTThreeRowBGRate}{0.34375} %
\newcommand{\DemoTThreeRowBGCpNineFiveLower}{0.1857190917} %
\newcommand{\DemoTThreeRowBGCpNineFiveUpper}{0.5319310363} %
\newcommand{\DemoTThreeRowBHEffectReports}{7} %
\newcommand{\DemoTThreeRowBHK}{32} %
\newcommand{\DemoTThreeRowBHRate}{0.21875} %
\newcommand{\DemoTThreeRowBHCpNineFiveLower}{0.09277153228} %
\newcommand{\DemoTThreeRowBHCpNineFiveUpper}{0.3997282637} %
\newcommand{\DemoTThreeRowBIEffectReports}{0} %
\newcommand{\DemoTThreeRowBIK}{32} %
\newcommand{\DemoTThreeRowBIRate}{0} %
\newcommand{\DemoTThreeRowBICpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBICpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBJEffectReports}{0} %
\newcommand{\DemoTThreeRowBJK}{32} %
\newcommand{\DemoTThreeRowBJRate}{0} %
\newcommand{\DemoTThreeRowBJCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBKEffectReports}{4} %
\newcommand{\DemoTThreeRowBKK}{32} %
\newcommand{\DemoTThreeRowBKRate}{0.125} %
\newcommand{\DemoTThreeRowBKCpNineFiveLower}{0.0351306531} %
\newcommand{\DemoTThreeRowBKCpNineFiveUpper}{0.2899484202} %
\newcommand{\DemoTThreeRowBLEffectReports}{0} %
\newcommand{\DemoTThreeRowBLK}{32} %
\newcommand{\DemoTThreeRowBLRate}{0} %
\newcommand{\DemoTThreeRowBLCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBLCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBMEffectReports}{5} %
\newcommand{\DemoTThreeRowBMK}{32} %
\newcommand{\DemoTThreeRowBMRate}{0.15625} %
\newcommand{\DemoTThreeRowBMCpNineFiveLower}{0.0527505644} %
\newcommand{\DemoTThreeRowBMCpNineFiveUpper}{0.3278787657} %
\newcommand{\DemoTThreeRowBNEffectReports}{2} %
\newcommand{\DemoTThreeRowBNK}{32} %
\newcommand{\DemoTThreeRowBNRate}{0.0625} %
\newcommand{\DemoTThreeRowBNCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowBNCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowBOEffectReports}{2} %
\newcommand{\DemoTThreeRowBOK}{32} %
\newcommand{\DemoTThreeRowBORate}{0.0625} %
\newcommand{\DemoTThreeRowBOCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowBOCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowBPEffectReports}{2} %
\newcommand{\DemoTThreeRowBPK}{32} %
\newcommand{\DemoTThreeRowBPRate}{0.0625} %
\newcommand{\DemoTThreeRowBPCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowBPCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowBQEffectReports}{4} %
\newcommand{\DemoTThreeRowBQK}{32} %
\newcommand{\DemoTThreeRowBQRate}{0.125} %
\newcommand{\DemoTThreeRowBQCpNineFiveLower}{0.0351306531} %
\newcommand{\DemoTThreeRowBQCpNineFiveUpper}{0.2899484202} %
\newcommand{\DemoTThreeRowBREffectReports}{0} %
\newcommand{\DemoTThreeRowBRK}{32} %
\newcommand{\DemoTThreeRowBRRate}{0} %
\newcommand{\DemoTThreeRowBRCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBRCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBSEffectReports}{31} %
\newcommand{\DemoTThreeRowBSK}{32} %
\newcommand{\DemoTThreeRowBSRate}{0.96875} %
\newcommand{\DemoTThreeRowBSCpNineFiveLower}{0.8378290058} %
\newcommand{\DemoTThreeRowBSCpNineFiveUpper}{0.9992091314} %
\newcommand{\DemoTThreeRowBTEffectReports}{5} %
\newcommand{\DemoTThreeRowBTK}{32} %
\newcommand{\DemoTThreeRowBTRate}{0.15625} %
\newcommand{\DemoTThreeRowBTCpNineFiveLower}{0.0527505644} %
\newcommand{\DemoTThreeRowBTCpNineFiveUpper}{0.3278787657} %
\newcommand{\DemoTThreeRowBUEffectReports}{0} %
\newcommand{\DemoTThreeRowBUK}{32} %
\newcommand{\DemoTThreeRowBURate}{0} %
\newcommand{\DemoTThreeRowBUCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBUCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBVEffectReports}{0} %
\newcommand{\DemoTThreeRowBVK}{32} %
\newcommand{\DemoTThreeRowBVRate}{0} %
\newcommand{\DemoTThreeRowBVCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowBVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowBWEffectReports}{2} %
\newcommand{\DemoTThreeRowBWK}{32} %
\newcommand{\DemoTThreeRowBWRate}{0.0625} %
\newcommand{\DemoTThreeRowBWCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowBWCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowBXEffectReports}{3} %
\newcommand{\DemoTThreeRowBXK}{32} %
\newcommand{\DemoTThreeRowBXRate}{0.09375} %
\newcommand{\DemoTThreeRowBXCpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowBXCpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowBYEffectReports}{12} %
\newcommand{\DemoTThreeRowBYK}{32} %
\newcommand{\DemoTThreeRowBYRate}{0.375} %
\newcommand{\DemoTThreeRowBYCpNineFiveLower}{0.2110003164} %
\newcommand{\DemoTThreeRowBYCpNineFiveUpper}{0.5630775449} %
\newcommand{\DemoTThreeRowBZEffectReports}{2} %
\newcommand{\DemoTThreeRowBZK}{32} %
\newcommand{\DemoTThreeRowBZRate}{0.0625} %
\newcommand{\DemoTThreeRowBZCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowBZCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowCAEffectReports}{0} %
\newcommand{\DemoTThreeRowCAK}{32} %
\newcommand{\DemoTThreeRowCARate}{0} %
\newcommand{\DemoTThreeRowCACpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCACpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCBEffectReports}{0} %
\newcommand{\DemoTThreeRowCBK}{32} %
\newcommand{\DemoTThreeRowCBRate}{0} %
\newcommand{\DemoTThreeRowCBCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCBCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCCEffectReports}{1} %
\newcommand{\DemoTThreeRowCCK}{32} %
\newcommand{\DemoTThreeRowCCRate}{0.03125} %
\newcommand{\DemoTThreeRowCCCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowCCCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowCDEffectReports}{0} %
\newcommand{\DemoTThreeRowCDK}{32} %
\newcommand{\DemoTThreeRowCDRate}{0} %
\newcommand{\DemoTThreeRowCDCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCDCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCEEffectReports}{6} %
\newcommand{\DemoTThreeRowCEK}{32} %
\newcommand{\DemoTThreeRowCERate}{0.1875} %
\newcommand{\DemoTThreeRowCECpNineFiveLower}{0.07207616546} %
\newcommand{\DemoTThreeRowCECpNineFiveUpper}{0.3643923099} %
\newcommand{\DemoTThreeRowCFEffectReports}{3} %
\newcommand{\DemoTThreeRowCFK}{32} %
\newcommand{\DemoTThreeRowCFRate}{0.09375} %
\newcommand{\DemoTThreeRowCFCpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowCFCpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowCGEffectReports}{0} %
\newcommand{\DemoTThreeRowCGK}{32} %
\newcommand{\DemoTThreeRowCGRate}{0} %
\newcommand{\DemoTThreeRowCGCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCGCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCHEffectReports}{0} %
\newcommand{\DemoTThreeRowCHK}{32} %
\newcommand{\DemoTThreeRowCHRate}{0} %
\newcommand{\DemoTThreeRowCHCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCHCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCIEffectReports}{4} %
\newcommand{\DemoTThreeRowCIK}{32} %
\newcommand{\DemoTThreeRowCIRate}{0.125} %
\newcommand{\DemoTThreeRowCICpNineFiveLower}{0.0351306531} %
\newcommand{\DemoTThreeRowCICpNineFiveUpper}{0.2899484202} %
\newcommand{\DemoTThreeRowCJEffectReports}{0} %
\newcommand{\DemoTThreeRowCJK}{32} %
\newcommand{\DemoTThreeRowCJRate}{0} %
\newcommand{\DemoTThreeRowCJCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCJCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCKEffectReports}{32} %
\newcommand{\DemoTThreeRowCKK}{32} %
\newcommand{\DemoTThreeRowCKRate}{1} %
\newcommand{\DemoTThreeRowCKCpNineFiveLower}{0.8911188393} %
\newcommand{\DemoTThreeRowCKCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowCLEffectReports}{4} %
\newcommand{\DemoTThreeRowCLK}{32} %
\newcommand{\DemoTThreeRowCLRate}{0.125} %
\newcommand{\DemoTThreeRowCLCpNineFiveLower}{0.0351306531} %
\newcommand{\DemoTThreeRowCLCpNineFiveUpper}{0.2899484202} %
\newcommand{\DemoTThreeRowCMEffectReports}{1} %
\newcommand{\DemoTThreeRowCMK}{32} %
\newcommand{\DemoTThreeRowCMRate}{0.03125} %
\newcommand{\DemoTThreeRowCMCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowCMCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowCNEffectReports}{1} %
\newcommand{\DemoTThreeRowCNK}{32} %
\newcommand{\DemoTThreeRowCNRate}{0.03125} %
\newcommand{\DemoTThreeRowCNCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowCNCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowCOEffectReports}{5} %
\newcommand{\DemoTThreeRowCOK}{32} %
\newcommand{\DemoTThreeRowCORate}{0.15625} %
\newcommand{\DemoTThreeRowCOCpNineFiveLower}{0.0527505644} %
\newcommand{\DemoTThreeRowCOCpNineFiveUpper}{0.3278787657} %
\newcommand{\DemoTThreeRowCPEffectReports}{0} %
\newcommand{\DemoTThreeRowCPK}{32} %
\newcommand{\DemoTThreeRowCPRate}{0} %
\newcommand{\DemoTThreeRowCPCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCPCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCQEffectReports}{31} %
\newcommand{\DemoTThreeRowCQK}{32} %
\newcommand{\DemoTThreeRowCQRate}{0.96875} %
\newcommand{\DemoTThreeRowCQCpNineFiveLower}{0.8378290058} %
\newcommand{\DemoTThreeRowCQCpNineFiveUpper}{0.9992091314} %
\newcommand{\DemoTThreeRowCREffectReports}{3} %
\newcommand{\DemoTThreeRowCRK}{32} %
\newcommand{\DemoTThreeRowCRRate}{0.09375} %
\newcommand{\DemoTThreeRowCRCpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowCRCpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowCSEffectReports}{0} %
\newcommand{\DemoTThreeRowCSK}{32} %
\newcommand{\DemoTThreeRowCSRate}{0} %
\newcommand{\DemoTThreeRowCSCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCSCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCTEffectReports}{0} %
\newcommand{\DemoTThreeRowCTK}{32} %
\newcommand{\DemoTThreeRowCTRate}{0} %
\newcommand{\DemoTThreeRowCTCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCTCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCUEffectReports}{1} %
\newcommand{\DemoTThreeRowCUK}{32} %
\newcommand{\DemoTThreeRowCURate}{0.03125} %
\newcommand{\DemoTThreeRowCUCpNineFiveLower}{0.000790868598} %
\newcommand{\DemoTThreeRowCUCpNineFiveUpper}{0.1621709942} %
\newcommand{\DemoTThreeRowCVEffectReports}{0} %
\newcommand{\DemoTThreeRowCVK}{32} %
\newcommand{\DemoTThreeRowCVRate}{0} %
\newcommand{\DemoTThreeRowCVCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCVCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCWEffectReports}{7} %
\newcommand{\DemoTThreeRowCWK}{32} %
\newcommand{\DemoTThreeRowCWRate}{0.21875} %
\newcommand{\DemoTThreeRowCWCpNineFiveLower}{0.09277153228} %
\newcommand{\DemoTThreeRowCWCpNineFiveUpper}{0.3997282637} %
\newcommand{\DemoTThreeRowCXEffectReports}{2} %
\newcommand{\DemoTThreeRowCXK}{32} %
\newcommand{\DemoTThreeRowCXRate}{0.0625} %
\newcommand{\DemoTThreeRowCXCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowCXCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTThreeRowCYEffectReports}{0} %
\newcommand{\DemoTThreeRowCYK}{32} %
\newcommand{\DemoTThreeRowCYRate}{0} %
\newcommand{\DemoTThreeRowCYCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCYCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowCZEffectReports}{0} %
\newcommand{\DemoTThreeRowCZK}{32} %
\newcommand{\DemoTThreeRowCZRate}{0} %
\newcommand{\DemoTThreeRowCZCpNineFiveLower}{0} %
\newcommand{\DemoTThreeRowCZCpNineFiveUpper}{0.1088811607} %
\newcommand{\DemoTThreeRowDAEffectReports}{3} %
\newcommand{\DemoTThreeRowDAK}{32} %
\newcommand{\DemoTThreeRowDARate}{0.09375} %
\newcommand{\DemoTThreeRowDACpNineFiveLower}{0.01976718017} %
\newcommand{\DemoTThreeRowDACpNineFiveUpper}{0.2502269507} %
\newcommand{\DemoTThreeRowDBEffectReports}{10} %
\newcommand{\DemoTThreeRowDBK}{32} %
\newcommand{\DemoTThreeRowDBRate}{0.3125} %
\newcommand{\DemoTThreeRowDBCpNineFiveLower}{0.1611847241} %
\newcommand{\DemoTThreeRowDBCpNineFiveUpper}{0.5000775816} %
\newcommand{\DemoTThreeRowDCEffectReports}{32} %
\newcommand{\DemoTThreeRowDCK}{32} %
\newcommand{\DemoTThreeRowDCRate}{1} %
\newcommand{\DemoTThreeRowDCCpNineFiveLower}{0.8911188393} %
\newcommand{\DemoTThreeRowDCCpNineFiveUpper}{1} %
\newcommand{\DemoTThreeRowDDEffectReports}{2} %
\newcommand{\DemoTThreeRowDDK}{32} %
\newcommand{\DemoTThreeRowDDRate}{0.0625} %
\newcommand{\DemoTThreeRowDDCpNineFiveLower}{0.007660736346} %
\newcommand{\DemoTThreeRowDDCpNineFiveUpper}{0.2080694299} %
\newcommand{\DemoTFourRowARhoHat}{0} %
\newcommand{\DemoTFourRowALambda}{1} %
\newcommand{\DemoTFourRowALambdaC}{0.06929353246} %
\newcommand{\DemoTFourRowADeffKish}{1} %
\newcommand{\DemoTFourRowADeffContrast}{14.43136126} %
\newcommand{\DemoTFourRowBRhoHat}{0} %
\newcommand{\DemoTFourRowBLambda}{1} %
\newcommand{\DemoTFourRowBLambdaC}{0.108714213} %
\newcommand{\DemoTFourRowBDeffKish}{1} %
\newcommand{\DemoTFourRowBDeffContrast}{9.198429278} %
\newcommand{\DemoTFourRowCRhoHat}{0.0004086758129} %
\newcommand{\DemoTFourRowCLambda}{0.905622923} %
\newcommand{\DemoTFourRowCLambdaC}{1} %
\newcommand{\DemoTFourRowCDeffKish}{1.104212332} %
\newcommand{\DemoTFourRowCDeffContrast}{1} %
\newcommand{\DemoTFourRowDRhoHat}{0} %
\newcommand{\DemoTFourRowDLambda}{1} %
\newcommand{\DemoTFourRowDLambdaC}{0.06330480217} %
\newcommand{\DemoTFourRowDDeffKish}{1} %
\newcommand{\DemoTFourRowDDeffContrast}{15.79658992} %
\newcommand{\DemoTFourRowERhoHat}{0} %
\newcommand{\DemoTFourRowELambda}{1} %
\newcommand{\DemoTFourRowELambdaC}{0.08052933957} %
\newcommand{\DemoTFourRowEDeffKish}{1} %
\newcommand{\DemoTFourRowEDeffContrast}{12.41783436} %
\newcommand{\DemoTFourRowFRhoHat}{0} %
\newcommand{\DemoTFourRowFLambda}{1} %
\newcommand{\DemoTFourRowFLambdaC}{1} %
\newcommand{\DemoTFourRowFDeffKish}{1} %
\newcommand{\DemoTFourRowFDeffContrast}{1} %
\newcommand{\DemoTFourRowGRhoHat}{0} %
\newcommand{\DemoTFourRowGLambda}{1} %
\newcommand{\DemoTFourRowGLambdaC}{0.07177434782} %
\newcommand{\DemoTFourRowGDeffKish}{1} %
\newcommand{\DemoTFourRowGDeffContrast}{13.93255432} %
\newcommand{\DemoTFourRowHRhoHat}{0} %
\newcommand{\DemoTFourRowHLambda}{1} %
\newcommand{\DemoTFourRowHLambdaC}{0.07979779351} %
\newcommand{\DemoTFourRowHDeffKish}{1} %
\newcommand{\DemoTFourRowHDeffContrast}{12.53167482} %
\newcommand{\DemoTFourRowIRhoHat}{0} %
\newcommand{\DemoTFourRowILambda}{1} %
\newcommand{\DemoTFourRowILambdaC}{1} %
\newcommand{\DemoTFourRowIDeffKish}{1} %
\newcommand{\DemoTFourRowIDeffContrast}{1} %
\newcommand{\DemoTFourRowJRhoHat}{0} %
\newcommand{\DemoTFourRowJLambda}{1} %
\newcommand{\DemoTFourRowJLambdaC}{0.06294164159} %
\newcommand{\DemoTFourRowJDeffKish}{1} %
\newcommand{\DemoTFourRowJDeffContrast}{15.88773306} %
\newcommand{\DemoTFourRowKRhoHat}{0} %
\newcommand{\DemoTFourRowKLambda}{1} %
\newcommand{\DemoTFourRowKLambdaC}{0.1007229388} %
\newcommand{\DemoTFourRowKDeffKish}{1} %
\newcommand{\DemoTFourRowKDeffContrast}{9.928225007} %
\newcommand{\DemoTFourRowLRhoHat}{0.004029192953} %
\newcommand{\DemoTFourRowLLambda}{0.4932318229} %
\newcommand{\DemoTFourRowLLambdaC}{1} %
\newcommand{\DemoTFourRowLDeffKish}{2.027444203} %
\newcommand{\DemoTFourRowLDeffContrast}{1} %
\newcommand{\DemoTFourRowMRhoHat}{0} %
\newcommand{\DemoTFourRowMLambda}{1} %
\newcommand{\DemoTFourRowMLambdaC}{0.07213554155} %
\newcommand{\DemoTFourRowMDeffKish}{1} %
\newcommand{\DemoTFourRowMDeffContrast}{13.86279189} %
\newcommand{\DemoTFourRowNRhoHat}{0} %
\newcommand{\DemoTFourRowNLambda}{1} %
\newcommand{\DemoTFourRowNLambdaC}{0.08414528205} %
\newcommand{\DemoTFourRowNDeffKish}{1} %
\newcommand{\DemoTFourRowNDeffContrast}{11.8842076} %
\newcommand{\DemoTFourRowORhoHat}{0.003922747284} %
\newcommand{\DemoTFourRowOLambda}{0.4999248719} %
\newcommand{\DemoTFourRowOLambdaC}{1} %
\newcommand{\DemoTFourRowODeffKish}{2.000300557} %
\newcommand{\DemoTFourRowODeffContrast}{1} %
\newcommand{\DemoTFourRowPRhoHat}{0} %
\newcommand{\DemoTFourRowPLambda}{1} %
\newcommand{\DemoTFourRowPLambdaC}{0.07290539437} %
\newcommand{\DemoTFourRowPDeffKish}{1} %
\newcommand{\DemoTFourRowPDeffContrast}{13.71640615} %
\newcommand{\DemoTFourRowQRhoHat}{0} %
\newcommand{\DemoTFourRowQLambda}{1} %
\newcommand{\DemoTFourRowQLambdaC}{0.07704156083} %
\newcommand{\DemoTFourRowQDeffKish}{1} %
\newcommand{\DemoTFourRowQDeffContrast}{12.98000701} %
\newcommand{\DemoTFourRowRRhoHat}{0.003629325398} %
\newcommand{\DemoTFourRowRLambda}{0.5193515647} %
\newcommand{\DemoTFourRowRLambdaC}{1} %
\newcommand{\DemoTFourRowRDeffKish}{1.925477977} %
\newcommand{\DemoTFourRowRDeffContrast}{1} %
\newcommand{\DemoTFourRowSRhoHat}{0} %
\newcommand{\DemoTFourRowSLambda}{1} %
\newcommand{\DemoTFourRowSLambdaC}{0.4028536875} %
\newcommand{\DemoTFourRowSDeffKish}{1} %
\newcommand{\DemoTFourRowSDeffContrast}{2.482290794} %
\newcommand{\DemoTFourRowTRhoHat}{0} %
\newcommand{\DemoTFourRowTLambda}{1} %
\newcommand{\DemoTFourRowTLambdaC}{0.68840976} %
\newcommand{\DemoTFourRowTDeffKish}{1} %
\newcommand{\DemoTFourRowTDeffContrast}{1.452623217} %
\newcommand{\DemoTFourRowURhoHat}{0} %
\newcommand{\DemoTFourRowULambda}{1} %
\newcommand{\DemoTFourRowULambdaC}{1} %
\newcommand{\DemoTFourRowUDeffKish}{1} %
\newcommand{\DemoTFourRowUDeffContrast}{1} %
\newcommand{\DemoTFourRowVRhoHat}{0.1745549653} %
\newcommand{\DemoTFourRowVLambda}{0.08335443023} %
\newcommand{\DemoTFourRowVLambdaC}{0.1411223666} %
\newcommand{\DemoTFourRowVDeffKish}{11.99696282} %
\newcommand{\DemoTFourRowVDeffContrast}{7.086048967} %
\newcommand{\DemoTFourRowWRhoHat}{0.1760152431} %
\newcommand{\DemoTFourRowWLambda}{0.0827200995} %
\newcommand{\DemoTFourRowWLambdaC}{0.3525721441} %
\newcommand{\DemoTFourRowWDeffKish}{12.08896031} %
\newcommand{\DemoTFourRowWDeffContrast}{2.836298944} %
\newcommand{\DemoTFourRowXRhoHat}{0.2077564705} %
\newcommand{\DemoTFourRowXLambda}{0.07097908299} %
\newcommand{\DemoTFourRowXLambdaC}{1} %
\newcommand{\DemoTFourRowXDeffKish}{14.08865764} %
\newcommand{\DemoTFourRowXDeffContrast}{1} %
\newcommand{\DemoTFourRowYRhoHat}{0} %
\newcommand{\DemoTFourRowYLambda}{1} %
\newcommand{\DemoTFourRowYLambdaC}{0.5085419469} %
\newcommand{\DemoTFourRowYDeffKish}{1} %
\newcommand{\DemoTFourRowYDeffContrast}{1.966406126} %
\newcommand{\DemoTFourRowZRhoHat}{0} %
\newcommand{\DemoTFourRowZLambda}{1} %
\newcommand{\DemoTFourRowZLambdaC}{0.7013469406} %
\newcommand{\DemoTFourRowZDeffKish}{1} %
\newcommand{\DemoTFourRowZDeffContrast}{1.425827849} %
\newcommand{\DemoTFourRowAARhoHat}{0.004949996495} %
\newcommand{\DemoTFourRowAALambda}{0.7622824014} %
\newcommand{\DemoTFourRowAALambdaC}{1} %
\newcommand{\DemoTFourRowAADeffKish}{1.311849779} %
\newcommand{\DemoTFourRowAADeffContrast}{1} %
\newcommand{\DemoTFourRowABRhoHat}{0} %
\newcommand{\DemoTFourRowABLambda}{1} %
\newcommand{\DemoTFourRowABLambdaC}{0.3523578345} %
\newcommand{\DemoTFourRowABDeffKish}{1} %
\newcommand{\DemoTFourRowABDeffContrast}{2.838024026} %
\newcommand{\DemoTFourRowACRhoHat}{0} %
\newcommand{\DemoTFourRowACLambda}{1} %
\newcommand{\DemoTFourRowACLambdaC}{0.4096762634} %
\newcommand{\DemoTFourRowACDeffKish}{1} %
\newcommand{\DemoTFourRowACDeffContrast}{2.440951769} %
\newcommand{\DemoTFourRowADRhoHat}{0} %
\newcommand{\DemoTFourRowADLambda}{1} %
\newcommand{\DemoTFourRowADLambdaC}{1} %
\newcommand{\DemoTFourRowADDeffKish}{1} %
\newcommand{\DemoTFourRowADDeffContrast}{1} %
\newcommand{\DemoTFourRowAERhoHat}{0.170270686} %
\newcommand{\DemoTFourRowAELambda}{0.08527291394} %
\newcommand{\DemoTFourRowAELambdaC}{0.1883116085} %
\newcommand{\DemoTFourRowAEDeffKish}{11.72705322} %
\newcommand{\DemoTFourRowAEDeffContrast}{5.310347077} %
\newcommand{\DemoTFourRowAFRhoHat}{0.1665368869} %
\newcommand{\DemoTFourRowAFLambda}{0.08701838896} %
\newcommand{\DemoTFourRowAFLambdaC}{0.3490404656} %
\newcommand{\DemoTFourRowAFDeffKish}{11.49182388} %
\newcommand{\DemoTFourRowAFDeffContrast}{2.864997324} %
\newcommand{\DemoTFourRowAGRhoHat}{0.1958965287} %
\newcommand{\DemoTFourRowAGLambda}{0.07495419563} %
\newcommand{\DemoTFourRowAGLambdaC}{1} %
\newcommand{\DemoTFourRowAGDeffKish}{13.34148131} %
\newcommand{\DemoTFourRowAGDeffContrast}{1} %
\newcommand{\DemoTFourRowAHRhoHat}{0} %
\newcommand{\DemoTFourRowAHLambda}{1} %
\newcommand{\DemoTFourRowAHLambdaC}{0.3577268451} %
\newcommand{\DemoTFourRowAHDeffKish}{1} %
\newcommand{\DemoTFourRowAHDeffContrast}{2.795429009} %
\newcommand{\DemoTFourRowAIRhoHat}{0} %
\newcommand{\DemoTFourRowAILambda}{1} %
\newcommand{\DemoTFourRowAILambdaC}{0.3904495344} %
\newcommand{\DemoTFourRowAIDeffKish}{1} %
\newcommand{\DemoTFourRowAIDeffContrast}{2.561150448} %
\newcommand{\DemoTFourRowAJRhoHat}{0.004524168237} %
\newcommand{\DemoTFourRowAJLambda}{0.7781964308} %
\newcommand{\DemoTFourRowAJLambdaC}{1} %
\newcommand{\DemoTFourRowAJDeffKish}{1.285022599} %
\newcommand{\DemoTFourRowAJDeffContrast}{1} %
\newcommand{\DemoTFourRowAKRhoHat}{0} %
\newcommand{\DemoTFourRowAKLambda}{1} %
\newcommand{\DemoTFourRowAKLambdaC}{0.2872620812} %
\newcommand{\DemoTFourRowAKDeffKish}{1} %
\newcommand{\DemoTFourRowAKDeffContrast}{3.481141667} %
\newcommand{\DemoTFourRowALRhoHat}{0} %
\newcommand{\DemoTFourRowALLambda}{1} %
\newcommand{\DemoTFourRowALLambdaC}{0.3102614267} %
\newcommand{\DemoTFourRowALDeffKish}{1} %
\newcommand{\DemoTFourRowALDeffContrast}{3.223088383} %
\newcommand{\DemoTFourRowAMRhoHat}{0} %
\newcommand{\DemoTFourRowAMLambda}{1} %
\newcommand{\DemoTFourRowAMLambdaC}{1} %
\newcommand{\DemoTFourRowAMDeffKish}{1} %
\newcommand{\DemoTFourRowAMDeffContrast}{1} %
\newcommand{\DemoTFourRowANRhoHat}{0.1593146391} %
\newcommand{\DemoTFourRowANLambda}{0.09060578996} %
\newcommand{\DemoTFourRowANLambdaC}{0.2825602897} %
\newcommand{\DemoTFourRowANDeffKish}{11.03682226} %
\newcommand{\DemoTFourRowANDeffContrast}{3.539067719} %
\newcommand{\DemoTFourRowAORhoHat}{0.1595051632} %
\newcommand{\DemoTFourRowAOLambda}{0.09050735932} %
\newcommand{\DemoTFourRowAOLambdaC}{0.3352820182} %
\newcommand{\DemoTFourRowAODeffKish}{11.04882528} %
\newcommand{\DemoTFourRowAODeffContrast}{2.98256377} %
\newcommand{\DemoTFourRowAPRhoHat}{0.1920346336} %
\newcommand{\DemoTFourRowAPLambda}{0.07634647359} %
\newcommand{\DemoTFourRowAPLambdaC}{1} %
\newcommand{\DemoTFourRowAPDeffKish}{13.09818192} %
\newcommand{\DemoTFourRowAPDeffContrast}{1} %
\newcommand{\DemoTFourRowAQRhoHat}{0} %
\newcommand{\DemoTFourRowAQLambda}{1} %
\newcommand{\DemoTFourRowAQLambdaC}{0.3000282731} %
\newcommand{\DemoTFourRowAQDeffKish}{1} %
\newcommand{\DemoTFourRowAQDeffContrast}{3.333019217} %
\newcommand{\DemoTFourRowARRhoHat}{0} %
\newcommand{\DemoTFourRowARLambda}{1} %
\newcommand{\DemoTFourRowARLambdaC}{0.2967037922} %
\newcommand{\DemoTFourRowARDeffKish}{1} %
\newcommand{\DemoTFourRowARDeffContrast}{3.370364742} %
\newcommand{\DemoTFourRowASRhoHat}{0.001700723908} %
\newcommand{\DemoTFourRowASLambda}{0.9032235637} %
\newcommand{\DemoTFourRowASLambdaC}{1} %
\newcommand{\DemoTFourRowASDeffKish}{1.107145606} %
\newcommand{\DemoTFourRowASDeffContrast}{1} %
\newcommand{\DemoTFourRowATRhoHat}{0} %
\newcommand{\DemoTFourRowATLambda}{1} %
\newcommand{\DemoTFourRowATLambdaC}{0.1540100215} %
\newcommand{\DemoTFourRowATDeffKish}{1} %
\newcommand{\DemoTFourRowATDeffContrast}{6.493083956} %
\newcommand{\DemoTFourRowAURhoHat}{0} %
\newcommand{\DemoTFourRowAULambda}{1} %
\newcommand{\DemoTFourRowAULambdaC}{0.4497697998} %
\newcommand{\DemoTFourRowAUDeffKish}{1} %
\newcommand{\DemoTFourRowAUDeffContrast}{2.223359595} %
\newcommand{\DemoTFourRowAVRhoHat}{0.0001147471279} %
\newcommand{\DemoTFourRowAVLambda}{0.9715713203} %
\newcommand{\DemoTFourRowAVLambdaC}{1} %
\newcommand{\DemoTFourRowAVDeffKish}{1.029260518} %
\newcommand{\DemoTFourRowAVDeffContrast}{1} %
\newcommand{\DemoTFourRowAWRhoHat}{0.1751782773} %
\newcommand{\DemoTFourRowAWLambda}{0.02189599107} %
\newcommand{\DemoTFourRowAWLambdaC}{0.03797585919} %
\newcommand{\DemoTFourRowAWDeffKish}{45.67046071} %
\newcommand{\DemoTFourRowAWDeffContrast}{26.33251811} %
\newcommand{\DemoTFourRowAXRhoHat}{0.1773628606} %
\newcommand{\DemoTFourRowAXLambda}{0.02163213159} %
\newcommand{\DemoTFourRowAXLambdaC}{0.1321733286} %
\newcommand{\DemoTFourRowAXDeffKish}{46.22752945} %
\newcommand{\DemoTFourRowAXDeffContrast}{7.565822926} %
\newcommand{\DemoTFourRowAYRhoHat}{0.2020125176} %
\newcommand{\DemoTFourRowAYLambda}{0.01904283404} %
\newcommand{\DemoTFourRowAYLambdaC}{1} %
\newcommand{\DemoTFourRowAYDeffKish}{52.513192} %
\newcommand{\DemoTFourRowAYDeffContrast}{1} %
\newcommand{\DemoTFourRowAZRhoHat}{0.0002296967472} %
\newcommand{\DemoTFourRowAZLambda}{0.9446682574} %
\newcommand{\DemoTFourRowAZLambdaC}{0.1674630688} %
\newcommand{\DemoTFourRowAZDeffKish}{1.058572671} %
\newcommand{\DemoTFourRowAZDeffContrast}{5.971465869} %
\newcommand{\DemoTFourRowBARhoHat}{0} %
\newcommand{\DemoTFourRowBALambda}{1} %
\newcommand{\DemoTFourRowBALambdaC}{0.3960198929} %
\newcommand{\DemoTFourRowBADeffKish}{1} %
\newcommand{\DemoTFourRowBADeffContrast}{2.525125676} %
\newcommand{\DemoTFourRowBBRhoHat}{0.003878546998} %
\newcommand{\DemoTFourRowBBLambda}{0.5027577559} %
\newcommand{\DemoTFourRowBBLambdaC}{1} %
\newcommand{\DemoTFourRowBBDeffKish}{1.989029484} %
\newcommand{\DemoTFourRowBBDeffContrast}{1} %
\newcommand{\DemoTFourRowBCRhoHat}{0} %
\newcommand{\DemoTFourRowBCLambda}{1} %
\newcommand{\DemoTFourRowBCLambdaC}{0.1156469937} %
\newcommand{\DemoTFourRowBCDeffKish}{1} %
\newcommand{\DemoTFourRowBCDeffContrast}{8.647003851} %
\newcommand{\DemoTFourRowBDRhoHat}{0} %
\newcommand{\DemoTFourRowBDLambda}{1} %
\newcommand{\DemoTFourRowBDLambdaC}{0.1271119333} %
\newcommand{\DemoTFourRowBDDeffKish}{1} %
\newcommand{\DemoTFourRowBDDeffContrast}{7.867081982} %
\newcommand{\DemoTFourRowBERhoHat}{0.0003317517951} %
\newcommand{\DemoTFourRowBELambda}{0.9220016923} %
\newcommand{\DemoTFourRowBELambdaC}{0.9726503409} %
\newcommand{\DemoTFourRowBEDeffKish}{1.084596708} %
\newcommand{\DemoTFourRowBEDeffContrast}{1.028118696} %
\newcommand{\DemoTFourRowBFRhoHat}{0.1820510883} %
\newcommand{\DemoTFourRowBFLambda}{0.02108680218} %
\newcommand{\DemoTFourRowBFLambdaC}{0.04995398989} %
\newcommand{\DemoTFourRowBFDeffKish}{47.42302752} %
\newcommand{\DemoTFourRowBFDeffContrast}{20.01842099} %
\newcommand{\DemoTFourRowBGRhoHat}{0.180828344} %
\newcommand{\DemoTFourRowBGLambda}{0.02122636256} %
\newcommand{\DemoTFourRowBGLambdaC}{0.09472280471} %
\newcommand{\DemoTFourRowBGDeffKish}{47.11122772} %
\newcommand{\DemoTFourRowBGDeffContrast}{10.55711983} %
\newcommand{\DemoTFourRowBHRhoHat}{0.2080672564} %
\newcommand{\DemoTFourRowBHLambda}{0.01849894034} %
\newcommand{\DemoTFourRowBHLambdaC}{1} %
\newcommand{\DemoTFourRowBHDeffKish}{54.05715038} %
\newcommand{\DemoTFourRowBHDeffContrast}{1} %
\newcommand{\DemoTFourRowBIRhoHat}{0} %
\newcommand{\DemoTFourRowBILambda}{1} %
\newcommand{\DemoTFourRowBILambdaC}{0.1121914611} %
\newcommand{\DemoTFourRowBIDeffKish}{1} %
\newcommand{\DemoTFourRowBIDeffContrast}{8.913334315} %
\newcommand{\DemoTFourRowBJRhoHat}{0} %
\newcommand{\DemoTFourRowBJLambda}{1} %
\newcommand{\DemoTFourRowBJLambdaC}{0.1252313402} %
\newcommand{\DemoTFourRowBJDeffKish}{1} %
\newcommand{\DemoTFourRowBJDeffContrast}{7.985221579} %
\newcommand{\DemoTFourRowBKRhoHat}{0.002855441209} %
\newcommand{\DemoTFourRowBKLambda}{0.5786576561} %
\newcommand{\DemoTFourRowBKLambdaC}{1} %
\newcommand{\DemoTFourRowBKDeffKish}{1.728137508} %
\newcommand{\DemoTFourRowBKDeffContrast}{1} %
\newcommand{\DemoTFourRowBLRhoHat}{0} %
\newcommand{\DemoTFourRowBLLambda}{1} %
\newcommand{\DemoTFourRowBLLambdaC}{0.0934670397} %
\newcommand{\DemoTFourRowBLDeffKish}{1} %
\newcommand{\DemoTFourRowBLDeffContrast}{10.69895873} %
\newcommand{\DemoTFourRowBMRhoHat}{0} %
\newcommand{\DemoTFourRowBMLambda}{1} %
\newcommand{\DemoTFourRowBMLambdaC}{0.09223475437} %
\newcommand{\DemoTFourRowBMDeffKish}{1} %
\newcommand{\DemoTFourRowBMDeffContrast}{10.84190018} %
\newcommand{\DemoTFourRowBNRhoHat}{0.0002606616387} %
\newcommand{\DemoTFourRowBNLambda}{0.9376740107} %
\newcommand{\DemoTFourRowBNLambdaC}{0.9959998699} %
\newcommand{\DemoTFourRowBNDeffKish}{1.066468718} %
\newcommand{\DemoTFourRowBNDeffContrast}{1.004016195} %
\newcommand{\DemoTFourRowBORhoHat}{0.1660069835} %
\newcommand{\DemoTFourRowBOLambda}{0.0230777499} %
\newcommand{\DemoTFourRowBOLambdaC}{0.08275915499} %
\newcommand{\DemoTFourRowBODeffKish}{43.33178079} %
\newcommand{\DemoTFourRowBODeffContrast}{12.08325532} %
\newcommand{\DemoTFourRowBPRhoHat}{0.1644252574} %
\newcommand{\DemoTFourRowBPLambda}{0.02329458012} %
\newcommand{\DemoTFourRowBPLambdaC}{0.09558202643} %
\newcommand{\DemoTFourRowBPDeffKish}{42.92844064} %
\newcommand{\DemoTFourRowBPDeffContrast}{10.46221803} %
\newcommand{\DemoTFourRowBQRhoHat}{0.2044618572} %
\newcommand{\DemoTFourRowBQLambda}{0.0188190045} %
\newcommand{\DemoTFourRowBQLambdaC}{1} %
\newcommand{\DemoTFourRowBQDeffKish}{53.13777358} %
\newcommand{\DemoTFourRowBQDeffContrast}{1} %
\newcommand{\DemoTFourRowBRRhoHat}{0} %
\newcommand{\DemoTFourRowBRLambda}{1} %
\newcommand{\DemoTFourRowBRLambdaC}{0.09907683221} %
\newcommand{\DemoTFourRowBRDeffKish}{1} %
\newcommand{\DemoTFourRowBRDeffContrast}{10.09317696} %
\newcommand{\DemoTFourRowBSRhoHat}{0} %
\newcommand{\DemoTFourRowBSLambda}{1} %
\newcommand{\DemoTFourRowBSLambdaC}{0.09171396071} %
\newcommand{\DemoTFourRowBSDeffKish}{1} %
\newcommand{\DemoTFourRowBSDeffContrast}{10.90346543} %
\newcommand{\DemoTFourRowBTRhoHat}{0.004173600666} %
\newcommand{\DemoTFourRowBTLambda}{0.484433183} %
\newcommand{\DemoTFourRowBTLambdaC}{0.7154107597} %
\newcommand{\DemoTFourRowBTDeffKish}{2.06426817} %
\newcommand{\DemoTFourRowBTDeffContrast}{1.397798379} %
\newcommand{\DemoTFourRowBURhoHat}{0} %
\newcommand{\DemoTFourRowBULambda}{1} %
\newcommand{\DemoTFourRowBULambdaC}{0.05715555073} %
\newcommand{\DemoTFourRowBUDeffKish}{1} %
\newcommand{\DemoTFourRowBUDeffContrast}{17.49611345} %
\newcommand{\DemoTFourRowBVRhoHat}{0} %
\newcommand{\DemoTFourRowBVLambda}{1} %
\newcommand{\DemoTFourRowBVLambdaC}{0.1765187745} %
\newcommand{\DemoTFourRowBVDeffKish}{1} %
\newcommand{\DemoTFourRowBVDeffContrast}{5.665119775} %
\newcommand{\DemoTFourRowBWRhoHat}{0} %
\newcommand{\DemoTFourRowBWLambda}{1} %
\newcommand{\DemoTFourRowBWLambdaC}{1} %
\newcommand{\DemoTFourRowBWDeffKish}{1} %
\newcommand{\DemoTFourRowBWDeffContrast}{1} %
\newcommand{\DemoTFourRowBXRhoHat}{0.1788660277} %
\newcommand{\DemoTFourRowBXLambda}{0.005435374997} %
\newcommand{\DemoTFourRowBXLambdaC}{0.007121208953} %
\newcommand{\DemoTFourRowBXDeffKish}{183.9799463} %
\newcommand{\DemoTFourRowBXDeffContrast}{140.4255944} %
\newcommand{\DemoTFourRowBYRhoHat}{0.1793987115} %
\newcommand{\DemoTFourRowBYLambda}{0.005419323346} %
\newcommand{\DemoTFourRowBYLambdaC}{0.02254369696} %
\newcommand{\DemoTFourRowBYDeffKish}{184.5248818} %
\newcommand{\DemoTFourRowBYDeffContrast}{44.35829676} %
\newcommand{\DemoTFourRowBZRhoHat}{0.203381587} %
\newcommand{\DemoTFourRowBZLambda}{0.004783330358} %
\newcommand{\DemoTFourRowBZLambdaC}{1} %
\newcommand{\DemoTFourRowBZDeffKish}{209.0593635} %
\newcommand{\DemoTFourRowBZDeffContrast}{1} %
\newcommand{\DemoTFourRowCARhoHat}{0} %
\newcommand{\DemoTFourRowCALambda}{1} %
\newcommand{\DemoTFourRowCALambdaC}{0.04047161839} %
\newcommand{\DemoTFourRowCADeffKish}{1} %
\newcommand{\DemoTFourRowCADeffContrast}{24.70867338} %
\newcommand{\DemoTFourRowCBRhoHat}{0} %
\newcommand{\DemoTFourRowCBLambda}{1} %
\newcommand{\DemoTFourRowCBLambdaC}{0.2278519956} %
\newcommand{\DemoTFourRowCBDeffKish}{1} %
\newcommand{\DemoTFourRowCBDeffContrast}{4.388813877} %
\newcommand{\DemoTFourRowCCRhoHat}{0.003861822924} %
\newcommand{\DemoTFourRowCCLambda}{0.2019938877} %
\newcommand{\DemoTFourRowCCLambdaC}{1} %
\newcommand{\DemoTFourRowCCDeffKish}{4.950644851} %
\newcommand{\DemoTFourRowCCDeffContrast}{1} %
\newcommand{\DemoTFourRowCDRhoHat}{0} %
\newcommand{\DemoTFourRowCDLambda}{1} %
\newcommand{\DemoTFourRowCDLambdaC}{0.02657081164} %
\newcommand{\DemoTFourRowCDDeffKish}{1} %
\newcommand{\DemoTFourRowCDDeffContrast}{37.63528242} %
\newcommand{\DemoTFourRowCERhoHat}{0} %
\newcommand{\DemoTFourRowCELambda}{1} %
\newcommand{\DemoTFourRowCELambdaC}{0.03295699369} %
\newcommand{\DemoTFourRowCEDeffKish}{1} %
\newcommand{\DemoTFourRowCEDeffContrast}{30.3425734} %
\newcommand{\DemoTFourRowCFRhoHat}{7.865711048e-06} %
\newcommand{\DemoTFourRowCFLambda}{0.9920176089} %
\newcommand{\DemoTFourRowCFLambdaC}{0.9455709317} %
\newcommand{\DemoTFourRowCFDeffKish}{1.008046622} %
\newcommand{\DemoTFourRowCFDeffContrast}{1.057562121} %
\newcommand{\DemoTFourRowCGRhoHat}{0.170630628} %
\newcommand{\DemoTFourRowCGLambda}{0.005696216259} %
\newcommand{\DemoTFourRowCGLambdaC}{0.01011826174} %
\newcommand{\DemoTFourRowCGDeffKish}{175.5551325} %
\newcommand{\DemoTFourRowCGDeffContrast}{98.83120493} %
\newcommand{\DemoTFourRowCHRhoHat}{0.1654851534} %
\newcommand{\DemoTFourRowCHLambda}{0.005872290188} %
\newcommand{\DemoTFourRowCHLambdaC}{0.02564419434} %
\newcommand{\DemoTFourRowCHDeffKish}{170.2913119} %
\newcommand{\DemoTFourRowCHDeffContrast}{38.995181} %
\newcommand{\DemoTFourRowCIRhoHat}{0.2003536853} %
\newcommand{\DemoTFourRowCILambda}{0.004855268804} %
\newcommand{\DemoTFourRowCILambdaC}{1} %
\newcommand{\DemoTFourRowCIDeffKish}{205.9618201} %
\newcommand{\DemoTFourRowCIDeffContrast}{1} %
\newcommand{\DemoTFourRowCJRhoHat}{0.0005043317596} %
\newcommand{\DemoTFourRowCJLambda}{0.6596604613} %
\newcommand{\DemoTFourRowCJLambdaC}{0.02827010767} %
\newcommand{\DemoTFourRowCJDeffKish}{1.51593139} %
\newcommand{\DemoTFourRowCJDeffContrast}{35.3730524} %
\newcommand{\DemoTFourRowCKRhoHat}{0} %
\newcommand{\DemoTFourRowCKLambda}{1} %
\newcommand{\DemoTFourRowCKLambdaC}{0.03805401718} %
\newcommand{\DemoTFourRowCKDeffKish}{1} %
\newcommand{\DemoTFourRowCKDeffContrast}{26.27843456} %
\newcommand{\DemoTFourRowCLRhoHat}{0.003742217339} %
\newcommand{\DemoTFourRowCLLambda}{0.2071127344} %
\newcommand{\DemoTFourRowCLLambdaC}{0.9409184647} %
\newcommand{\DemoTFourRowCLDeffKish}{4.828288338} %
\newcommand{\DemoTFourRowCLDeffContrast}{1.062791344} %
\newcommand{\DemoTFourRowCMRhoHat}{0} %
\newcommand{\DemoTFourRowCMLambda}{1} %
\newcommand{\DemoTFourRowCMLambdaC}{0.02627853876} %
\newcommand{\DemoTFourRowCMDeffKish}{1} %
\newcommand{\DemoTFourRowCMDeffContrast}{38.05386628} %
\newcommand{\DemoTFourRowCNRhoHat}{0} %
\newcommand{\DemoTFourRowCNLambda}{1} %
\newcommand{\DemoTFourRowCNLambdaC}{0.02452408956} %
\newcommand{\DemoTFourRowCNDeffKish}{1} %
\newcommand{\DemoTFourRowCNDeffContrast}{40.77623341} %
\newcommand{\DemoTFourRowCORhoHat}{2.420713697e-05} %
\newcommand{\DemoTFourRowCOLambda}{0.9758345302} %
\newcommand{\DemoTFourRowCOLambdaC}{0.9847520506} %
\newcommand{\DemoTFourRowCODeffKish}{1.024763901} %
\newcommand{\DemoTFourRowCODeffContrast}{1.015484049} %
\newcommand{\DemoTFourRowCPRhoHat}{0.1733468846} %
\newcommand{\DemoTFourRowCPLambda}{0.005607459984} %
\newcommand{\DemoTFourRowCPLambdaC}{0.02046214586} %
\newcommand{\DemoTFourRowCPDeffKish}{178.3338629} %
\newcommand{\DemoTFourRowCPDeffContrast}{48.87072974} %
\newcommand{\DemoTFourRowCQRhoHat}{0.1746349869} %
\newcommand{\DemoTFourRowCQLambda}{0.005566329756} %
\newcommand{\DemoTFourRowCQLambdaC}{0.02566385977} %
\newcommand{\DemoTFourRowCQDeffKish}{179.6515916} %
\newcommand{\DemoTFourRowCQDeffContrast}{38.9653002} %
\newcommand{\DemoTFourRowCRRhoHat}{0.2092629265} %
\newcommand{\DemoTFourRowCRLambda}{0.004649519806} %
\newcommand{\DemoTFourRowCRLambdaC}{1} %
\newcommand{\DemoTFourRowCRDeffKish}{215.0759738} %
\newcommand{\DemoTFourRowCRDeffContrast}{1} %
\newcommand{\DemoTFourRowCSRhoHat}{0} %
\newcommand{\DemoTFourRowCSLambda}{1} %
\newcommand{\DemoTFourRowCSLambdaC}{0.02462437576} %
\newcommand{\DemoTFourRowCSDeffKish}{1} %
\newcommand{\DemoTFourRowCSDeffContrast}{40.61016651} %
\newcommand{\DemoTFourRowCTRhoHat}{0} %
\newcommand{\DemoTFourRowCTLambda}{1} %
\newcommand{\DemoTFourRowCTLambdaC}{0.0232637683} %
\newcommand{\DemoTFourRowCTDeffKish}{1} %
\newcommand{\DemoTFourRowCTDeffContrast}{42.98529745} %
\newcommand{\DemoTFourRowCURhoHat}{0.003798978278} %
\newcommand{\DemoTFourRowCULambda}{0.2046515338} %
\newcommand{\DemoTFourRowCULambdaC}{0.3461760263} %
\newcommand{\DemoTFourRowCUDeffKish}{4.886354778} %
\newcommand{\DemoTFourRowCUDeffContrast}{2.888703792} %
\newcommand{\DemoTFourRowCVRhoHat}{0} %
\newcommand{\DemoTFourRowCVLambda}{1} %
\newcommand{\DemoTFourRowCVLambdaC}{0.0159884742} %
\newcommand{\DemoTFourRowCVDeffKish}{1} %
\newcommand{\DemoTFourRowCVDeffContrast}{62.54505512} %
\newcommand{\DemoTFourRowCWRhoHat}{0} %
\newcommand{\DemoTFourRowCWLambda}{1} %
\newcommand{\DemoTFourRowCWLambdaC}{0.07489571447} %
\newcommand{\DemoTFourRowCWDeffKish}{1} %
\newcommand{\DemoTFourRowCWDeffContrast}{13.3518988} %
\newcommand{\DemoTFourRowCXRhoHat}{0} %
\newcommand{\DemoTFourRowCXLambda}{1} %
\newcommand{\DemoTFourRowCXLambdaC}{1} %
\newcommand{\DemoTFourRowCXDeffKish}{1} %
\newcommand{\DemoTFourRowCXDeffContrast}{1} %
\newcommand{\DemoTFourRowCYRhoHat}{0.1757760221} %
\newcommand{\DemoTFourRowCYLambda}{0.001387341982} %
\newcommand{\DemoTFourRowCYLambdaC}{0.002217260987} %
\newcommand{\DemoTFourRowCYDeffKish}{720.8028106} %
\newcommand{\DemoTFourRowCYDeffContrast}{451.0068981} %
\newcommand{\DemoTFourRowCZRhoHat}{0.1727724081} %
\newcommand{\DemoTFourRowCZLambda}{0.001411426605} %
\newcommand{\DemoTFourRowCZLambdaC}{0.008239012706} %
\newcommand{\DemoTFourRowCZDeffKish}{708.5030112} %
\newcommand{\DemoTFourRowCZDeffContrast}{121.373766} %
\newcommand{\DemoTFourRowDARhoHat}{0.1985164003} %
\newcommand{\DemoTFourRowDALambda}{0.001228614945} %
\newcommand{\DemoTFourRowDALambdaC}{1} %
\newcommand{\DemoTFourRowDADeffKish}{813.9246591} %
\newcommand{\DemoTFourRowDADeffContrast}{1} %
\newcommand{\DemoTFourRowDBRhoHat}{0.0006285293272} %
\newcommand{\DemoTFourRowDBLambda}{0.2798120428} %
\newcommand{\DemoTFourRowDBLambdaC}{0.01086480663} %
\newcommand{\DemoTFourRowDBDeffKish}{3.573827595} %
\newcommand{\DemoTFourRowDBDeffContrast}{92.04029436} %
\newcommand{\DemoTFourRowDCRhoHat}{0} %
\newcommand{\DemoTFourRowDCLambda}{1} %
\newcommand{\DemoTFourRowDCLambdaC}{0.03965206601} %
\newcommand{\DemoTFourRowDCDeffKish}{1} %
\newcommand{\DemoTFourRowDCDeffContrast}{25.21936687} %
\newcommand{\DemoTFourRowDDRhoHat}{0.003825693932} %
\newcommand{\DemoTFourRowDDLambda}{0.0600016201} %
\newcommand{\DemoTFourRowDDLambdaC}{1} %
\newcommand{\DemoTFourRowDDDeffKish}{16.66621665} %
\newcommand{\DemoTFourRowDDDeffContrast}{1} %
\newcommand{\DemoTFourRowDERhoHat}{0} %
\newcommand{\DemoTFourRowDELambda}{1} %
\newcommand{\DemoTFourRowDELambdaC}{0.00812542692} %
\newcommand{\DemoTFourRowDEDeffKish}{1} %
\newcommand{\DemoTFourRowDEDeffContrast}{123.0704565} %
\newcommand{\DemoTFourRowDFRhoHat}{0} %
\newcommand{\DemoTFourRowDFLambda}{1} %
\newcommand{\DemoTFourRowDFLambdaC}{0.008999140309} %
\newcommand{\DemoTFourRowDFDeffKish}{1} %
\newcommand{\DemoTFourRowDFDeffContrast}{111.1217256} %
\newcommand{\DemoTFourRowDGRhoHat}{7.217183882e-07} %
\newcommand{\DemoTFourRowDGLambda}{0.9970532721} %
\newcommand{\DemoTFourRowDGLambdaC}{0.9701379511} %
\newcommand{\DemoTFourRowDGDeffKish}{1.002955437} %
\newcommand{\DemoTFourRowDGDeffContrast}{1.03078124} %
\newcommand{\DemoTFourRowDHRhoHat}{0.171979419} %
\newcommand{\DemoTFourRowDHLambda}{0.0014179254} %
\newcommand{\DemoTFourRowDHLambdaC}{0.002472254914} %
\newcommand{\DemoTFourRowDHDeffKish}{705.2557208} %
\newcommand{\DemoTFourRowDHDeffContrast}{404.4890332} %
\newcommand{\DemoTFourRowDIRhoHat}{0.1705741153} %
\newcommand{\DemoTFourRowDILambda}{0.001429590518} %
\newcommand{\DemoTFourRowDILambdaC}{0.006499453757} %
\newcommand{\DemoTFourRowDIDeffKish}{699.5010022} %
\newcommand{\DemoTFourRowDIDeffContrast}{153.8590838} %
\newcommand{\DemoTFourRowDJRhoHat}{0.1981697138} %
\newcommand{\DemoTFourRowDJLambda}{0.00123076169} %
\newcommand{\DemoTFourRowDJLambdaC}{1} %
\newcommand{\DemoTFourRowDJDeffKish}{812.5049779} %
\newcommand{\DemoTFourRowDJDeffContrast}{1} %
\newcommand{\DemoTFourRowDKRhoHat}{0.0002615712312} %
\newcommand{\DemoTFourRowDKLambda}{0.4828272373} %
\newcommand{\DemoTFourRowDKLambdaC}{0.009071567815} %
\newcommand{\DemoTFourRowDKDeffKish}{2.071134192} %
\newcommand{\DemoTFourRowDKDeffContrast}{110.2345284} %
\newcommand{\DemoTFourRowDLRhoHat}{0} %
\newcommand{\DemoTFourRowDLLambda}{1} %
\newcommand{\DemoTFourRowDLLambdaC}{0.01018253121} %
\newcommand{\DemoTFourRowDLDeffKish}{1} %
\newcommand{\DemoTFourRowDLDeffContrast}{98.20740825} %
\newcommand{\DemoTFourRowDMRhoHat}{0.003828928712} %
\newcommand{\DemoTFourRowDMLambda}{0.05995396828} %
\newcommand{\DemoTFourRowDMLambdaC}{0.6168483027} %
\newcommand{\DemoTFourRowDMDeffKish}{16.67946307} %
\newcommand{\DemoTFourRowDMDeffContrast}{1.621144122} %
\newcommand{\DemoTFourRowDNRhoHat}{0} %
\newcommand{\DemoTFourRowDNLambda}{1} %
\newcommand{\DemoTFourRowDNLambdaC}{0.007071970794} %
\newcommand{\DemoTFourRowDNDeffKish}{1} %
\newcommand{\DemoTFourRowDNDeffContrast}{141.4032989} %
\newcommand{\DemoTFourRowDORhoHat}{0} %
\newcommand{\DemoTFourRowDOLambda}{1} %
\newcommand{\DemoTFourRowDOLambdaC}{0.006383813391} %
\newcommand{\DemoTFourRowDODeffKish}{1} %
\newcommand{\DemoTFourRowDODeffContrast}{156.6461829} %
\newcommand{\DemoTFourRowDPRhoHat}{1.34787462e-05} %
\newcommand{\DemoTFourRowDPLambda}{0.9476917145} %
\newcommand{\DemoTFourRowDPLambdaC}{0.9709514055} %
\newcommand{\DemoTFourRowDPDeffKish}{1.055195466} %
\newcommand{\DemoTFourRowDPDeffContrast}{1.029917661} %
\newcommand{\DemoTFourRowDQRhoHat}{0.1746317802} %
\newcommand{\DemoTFourRowDQLambda}{0.001396419586} %
\newcommand{\DemoTFourRowDQLambdaC}{0.005144104981} %
\newcommand{\DemoTFourRowDQDeffKish}{716.11714} %
\newcommand{\DemoTFourRowDQDeffContrast}{194.3972768} %
\newcommand{\DemoTFourRowDRRhoHat}{0.1739338373} %
\newcommand{\DemoTFourRowDRLambda}{0.001402015131} %
\newcommand{\DemoTFourRowDRLambdaC}{0.00617099269} %
\newcommand{\DemoTFourRowDRDeffKish}{713.2590637} %
\newcommand{\DemoTFourRowDRDeffContrast}{162.0484823} %
\newcommand{\DemoTFourRowDSRhoHat}{0.2108622324} %
\newcommand{\DemoTFourRowDSLambda}{0.001156763634} %
\newcommand{\DemoTFourRowDSLambdaC}{1} %
\newcommand{\DemoTFourRowDSDeffKish}{864.4808418} %
\newcommand{\DemoTFourRowDSDeffContrast}{1} %
\newcommand{\DemoTFourRowDTRhoHat}{0} %
\newcommand{\DemoTFourRowDTLambda}{1} %
\newcommand{\DemoTFourRowDTLambdaC}{0.007318266306} %
\newcommand{\DemoTFourRowDTDeffKish}{1} %
\newcommand{\DemoTFourRowDTDeffContrast}{136.6443852} %
\newcommand{\DemoTFourRowDURhoHat}{0} %
\newcommand{\DemoTFourRowDULambda}{1} %
\newcommand{\DemoTFourRowDULambdaC}{0.006314474574} %
\newcommand{\DemoTFourRowDUDeffKish}{1} %
\newcommand{\DemoTFourRowDUDeffContrast}{158.366304} %
\newcommand{\DemoTFourRowDVRhoHat}{0.003869455454} %
\newcommand{\DemoTFourRowDVLambda}{0.05936331626} %
\newcommand{\DemoTFourRowDVLambdaC}{0.1019225198} %
\newcommand{\DemoTFourRowDVDeffKish}{16.84542008} %
\newcommand{\DemoTFourRowDVDeffContrast}{9.811374387} %

